The Caporaso-Harris-Ran degeneration principle: proof and applications

Severi varieties are the parameter spaces for curves with prescribed homology class and genus on a smooth surface. We describe their limits along degenerations of surfaces, with a view towards the enumeration of curves. This includes a complete proof of the Caporaso-Harris recursive formula, with all the necessary background on deformations of curves and singularities.

==> 01.ciro/seminar.tex <==
\chaptitle{Limits of nodal curves: generalities and examples}
\chapauthor{Ciro Ciliberto and Thomas Dedieu}

\startchap
\label{01.ciro}



\newcounter{caseno}
\def\caseitem#1{%
  \smallskip
  \refstepcounter{caseno}
  \subparagraph*{Case~\thecaseno: #1}%
  \par%\smallskip
}
\newenvironment{catalogo}{\setcounter{caseno}{0}}{}

\newcommand{\cru}[1]{#1^{\mathrm{cr}}}
\newcommand{\reg}[1]{#1^{\mathrm{reg}}}
\newcommand{\loc}[1]{#1^{\mathrm{loc}}}
\newcommand{\tetra}[1]{#1_{\mathrm{tetra}}}
\newcommand{\kum}[1]{#1_{\mathrm{Kum}}}
\newcommand{\seqN}{\underline{\N}}
\newcommand{\utau}%{\underbar{\hphantom{t}}\hspace{-.45em}\tau}
                   {\underline{\tau}}
\newcommand{\ubtau}{\underline{\boldsymbol{\tau}}}
\newcommand{\bdelta}{\boldsymbol{\delta}}


\let\mathbb\mathbf


% \begin{abstract} This is the expanded text of the first of a series of lectures given by various authors at the seminar of algebraic geometry at the University of Roma ``Tor Vergata'' in the years 2015--2017, devoted to the study of enumerative (and not only) problems concerning singular curves on surfaces (and not only on them) attacked via degeneration techniques. This lecture is an introduction to some of the problems, the techniques, the examples and the objectives which will be met in the forthcoming lectures. 
% \end{abstract}


\startcontents[ciro]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[ciro]{}{1}[2]{}

% {\small
% \setlength{\cftaftertoctitleskip}{0.2cm}
% \renewcommand{\cfttoctitlefont}{\normalfont\large\bfseries}
% \setlength{\cftbeforesecskip}{0.05cm}
% \setcounter{tocdepth}{1}
% \tableofcontents
% }

\def\H{\mathcal{H}}

\section{The basic question}\label{sec:bquest}

The objective of this lecture  is to introduce to the subject of interest in this series of seminars.
This exposition is mainly based on \cite {CD}. In this text we will work over the complex field.

Let $f:S\to \D$ be a flat, projective family of surfaces of degree $d$ in $\P^r$ (with $r\geqslant 3$), with $S$ a smooth threefold, and $\D$ the complex unit disc, usually called a \emph{degeneration} of the \emph{general  fibre} $S_t:=f^{-1}(t)$, for $t\in \D^ *:=\D-\{0\}$, which we assume is a smooth irreducible surface, 
to the \emph{central fibre} $S_0$,
 which may be  singular and even reducible. This is also called a \emph{smooth deformation} of $S_0$. One has $S\subset \D\times \P^ r$, so that $S$ is endowed with the line bundle $\L=p^ *(\O_{\P^ r}(1))$, where $p: S\to \P^ r$ is the projection to the second factor: this is called the \emph{polarizing (hyperplane) bundle} on $S$. 

\begin{question}
\label{quest}
What are the limits of tangent, or in general of multitangent, hyperplanes 
to $S_t$, for $t\neq 0$,  as $t$ tends to $0$?
\end{question}

The same question makes sense, more generally, for varieties of any dimension. In the case of degeneration of (plane) curves we refer to \cite[pp. 134--135]{harris-morrison} for a glimpse on this subject. In dimension higher than 2 the problem is quite complicated and few results are known (however, B. Segre's paper \cite {bsegre} is an interesting classical source of basic information on the subject).  

One of  the main interests in Question \ref {quest} arises form enumerative geometry, since, by degenerating a  surface to a reducible one, whose components are much simpler than the original surface (e.g., a degeneration into a union of planes), we may  hope that the configuration of limits of pluritangent hyperplanes is easier to understand and their number (if finite), or in general the degree of the variety parameterising them, may be  computed.  This is indeed the subject of the  foundational
work by L. Caporaso and J. Harris
\cite{caporaso-harris,caporaso-harris2}, 
and independently by Z. Ran \cite{Ran1,Ran2,Ran3},
which were both aimed to the study, with degeneration techniques, of the so--called
\emph{Severi varieties}, i.e., the families of irreducible 
nodal plane curves of a given degree.

Section \ref{sec:salmon} contains classical enumerative formulae for
surfaces.
Sections \ref{s:setting}--\ref{s:Severi-1} present general facts about
Question \ref{quest}, following the presentation given in \cite{CD}.
Finally, Sections \ref{ssec:1nodal}--\ref{S:planes} present several
examples in detail in order to illustrate the general theory.



\section{Classical results}\label{sec:salmon}


Enumerative results  on  the number of (pluri)tangent planes to a
\emph{general} surface $S$ of degree $d>1$ in $\P^ 3$ are quite
classical, and probably the first of them go back to G. Salmon, see
\cite{Salmon1,Salmon2}.




The set $\check S\subset \check \P^ 3$ of tangent planes to $S$ is the \emph{dual} of $S$, which is birational to $S$. One has 
\[
\deg(\check S)=d(d-1)^ 2.
\]

As soon as $d>2$, $\check S$ is singular. How do the singularities of $\check S$ look like if $S$ is general enough? There is a \emph{nodal curve} $D_b$, whose general points  correspond to \emph{bitangent planes} to $S$. Salmon computes
\[
\deg(D_b)=\frac 12 d(d-1)(d-2)(d^ 3-d^ 2+d-12).
\]

There is also a \emph{cuspidal curve} $D_s$, whose points  correspond to \emph{stationary tangent planes} to $S$, i.e., tangent planes to $S$ in \emph{parabolic points}, namely points $x\in  S$ such that the tangent plane to $S$ at $x$ cuts $S$ in a curve with a cusp at $x$. Salmon computes
\[
\deg(D_s)=4d(d-1)(d-2),
\]
whereas the curve $\Gamma_p$ of parabolic points on $S$ is the complete intersection of $S$ with its \emph{Hessian surface}, hence
\[
\deg(\Gamma_p)=4d(d-2).
\]

Finally, there are finitely many triple points of $\check S$, which are triple points of $D_b$ too. Salmon computes their number
\begin{equation}\label{eq:salmon}
t=\frac 16 d(d-2)(d^ 7-4d^ 6+7d^ 5-45d^ 4+114d^ 3-111d^ 2+548 d-960).
\end{equation}
For all these classical formulae, the reader is invited to consult
\cite{13.th-classic,16.th+l-redres}.


All these numbers have been computed in recent times by I. Vainsencher
\cite {vainsencher, vainsencher2} and by S. Kleiman and R. Piene \cite
{KP1, KP2}, via Chern class computations,
see \cite{14.th-vainsencher}.
However several questions are still open, like:

\begin{question}\label{quest:2} What are the singularities of $D_b$ and of $D_s$? Are these curves irreducible? How do they intersect? Is $\Gamma_p$ smooth? What is the monodromy of the covering
$T\to U$, given by the triple points of $\check S$, when $S$ moves in the open subset $U\subset |\O_{\P^ 3}(d)|$ 
of smooth surfaces?
\end{question}

Partial answers to some of these question have been given for $d=4$ in \cite {CD}.

\section{Semistable degenerations}

\label{s:setting}

A degeneration $f: S\to \D$ as in \S \ref {sec:bquest} is said to be \emph{semistable} if the central fibre $S_0$  is reduced and with \emph{local normal crossing} singularities. We will often assume that all irreducible components of $S_0$ are smooth, so the singularities of $S_0$ are: \emph{double curves}, along which only two irreducible components of $S_0$ intersect transversally and \emph{triple points}, where only three irreducible components of $S_0$ intersect transversally.



As in \S  \ref {sec:bquest}, we will assume there is a \emph{polarising line bundle}  $\L$ on $S$ (although, in principle, it could be neither ample nor relatively ample). Denote by $L_t$ the restriction of $\L$ to $S_t$ for all $t\in \D$. Then we will say that $(S_0,L_0)$ is \emph{a limit} of $(S_t,L_t)$ (with $t\in \D^ *$), when $t\to 0$ (or that $(S_t,L_t)$ with $t\in \D^ *$ is a deformation of $(S_0,L_0)$).

The limit $(S_0,L_0)$ \emph{is not unique} if $S_0$ is reducible. Indeed, if $W$ is an effective divisor supported
on the central fibre $S_0$, consider the line bundle $\L(-W)$,
which is said to be obtained from $\L$ by \emph{twisting} by $W$. 
For $t\in \D^ *$, its restriction to $S_t$ is the same as $L_t$,
but in general this is not the case for $S_0$;
any such line bundle $\left. \L(-W) \right |_{S_0}$ is called a
\emph{limit line bundle} of $\L_t$ for $t\in \D^ *$.  If $Q$ is an irreducible component of $S_0$, 
the restriction $\L_{W,Q}:=\L(-W)_{|Q}$ is called the \emph{aspect} of $\L(-W)$ on $Q$.  
 
 \begin{remark}
\label{r:twist}
Since $\Pic(\D)$ is trivial,   the
divisor $S_0 \subset S$ is linearly equivalent to $0$.
So if  $W$ is a divisor supported on $S_0$, one has
$\L(-W) \cong  \L(mS_0-W)$ for all integers $m$. 
In particular if $W+W'=S_0$ then $\L(-W)\cong \L(W')$.
\end{remark}


Another family of surfaces $f': S'\to \D$ as above is said to be
a \emph{model of} $f: S\to \D$ if there is a commutative diagram
\[\xymatrix@C=25pt@R=20pt{
S' \ar[d]_{f'} \ar@{}[dr]|{\Box}
& \bar S' \ar[d] \ar[l] \ar@{-->}[r]^p
& \bar S \ar[r] \ar[d] & S \ar[d]^f \ar@{}[dl]|{\Box} \\
\D & \D \ar[l]^{t^{d'} \mapsfrom t} \ar@{=}[r]
& \D \ar[r]_{t\mapsto t^d} & \D
}\]
where the two squares marked with a $\Box$ are Cartesian, and $p$ is
a birational map, which is an isomorphism over $\D^*$.
The family $f': S'\to \D$, if semistable, is a \emph{semistable
model of} $f: S\to \D$ if in addition $d'=1$
and $p$ is a morphism.
The \emph{semistable reduction theorem} of \cite {Kempf} asserts
that any family  $f:S\to \D$ as in \S \ref {sec:bquest} has a semistable model.

\begin{example} [Families of surfaces in $\P^3$] \label{ex:pi3}
Consider a \emph{linear pencil} of degree $d$ surfaces in $\P^3$, 
generated by a \emph{general} surface $S_{\infty}$ and a \emph{special} one $S_0$.
We will usually consider the case in which $S_0$ has local normal crossing singularities, and $S_\infty$ intersects transversally the double curve of $S_0$ at smooth points of it. This pencil gives rise to a flat, proper family $\varphi: \cal S\to$ $\P^1$, with $\cal S$ a hypersurface of type $(d,1)$
in $\P^3\times \P^1$, isomorphic to the blow--up of $\P^3$ along the
\emph{base locus scheme} $S_0\cap S_\infty$ of the pencil,
 and it has $S_0,S_\infty$ as fibres over $0,\infty\in \P^1$, respectively.



We will study the family  obtained by
restricting $\cal S$ to a  disk ${\D} \subset \P^1$  centered at $0$, that by abuse of notation we will still denote by $f: \cal S \to \D$,
such that $S_t$ is smooth for all $t\in {\D}^ *$, and
we will consider a semistable model  
of  $f: S \to \D$. To do so, we resolve the singularities
of $S$ which occur only in the central fibre of $f$, at the points mapped by 
$\mathcal{S}_0 \to S_0 \subset \P^3$
to the intersection
points of $S_{\infty}$ with the double curves of $S_0$ (they are the
singular points of the curve $S_0\cap S_\infty$).
These are \emph{ordinary double points} of $S$, 
i.e., singularities analytically equivalent to the one at the origin of the hypersurface
$xy=zt$ in $\A^4$. 
Such a singularity is resolved by a single blow--up, which produces an
exceptional divisor  $E\cong \P^1\times\P^1$, and then it is possible to contract $E$ in the direction of either one of its rulings 
without introducing any singularity: the result is called a \emph{small resolution} of the ordinary double point.


Let $\tilde f: \tilde S\to \D$ be a semistable model thus obtained. One has $\tilde S_t\cong S_t$ for $t\in \D^ *$. 
If  $S_0$ has irreducible components $Q_1,\ldots,Q_r$, 
then $\tilde S_0$ consists of irreducible components $\tilde Q_1,\ldots,\tilde Q_r$
which are suitable blow--ups of $Q_1,\ldots,Q_r$, respectively. 
If $q$ is the number of ordinary double points of the original total space $S$,
we will denote by $E_1,\ldots,E_{q}$ the exceptional curves on $\tilde Q_1,\ldots,\tilde Q_r$ arising from 
the small resolution process. 

The simplest example of this situation is when $S_0$ is the union of a general surface $S'$ of degree $h$ with a general surface $S''$ of degree $d-h$ (and $1\leqslant h\leqslant \left \lfloor \frac d2 \right \rfloor$), intersecting along a smooth curve $R$ of degree $h(d-h)$. In this case $\tilde S_0$ consists of two components $Q_1,Q_2$, and we may assume that $Q_2=S''$, whereas $Q_1=\tilde S'$ is the blow--up of $S'$ at the $q=dh(d-h)$ intersection points of $R$ with $S_\infty$. Then $Q_1$ and $Q_2$ intersect along a curve which can be identified with $R$ and the exceptional curves $E_1,\ldots,E_{q}$ all lie on $Q_1$.   

The case $h=1$ in which $S'=P$ is a general plane, is particularly interesting since it shows the geometric significance of twisting the polarising line bundle $\L=p^*(\O_{\P^ 3}(1))$ on $\tilde S$. The polarising line bundle $L_0$ maps $\tilde S_0$ to the reducible surface $S''\cup P$. If we twist by $Q_1=\tilde P$ and consider $\L'=\L(-\tilde P)$, then its aspects are:\\
\begin{inparaenum}
\item [$\bullet$] the trivial bundle on $Q_2=S''$;\\
\item [$\bullet$]  $\vert  \O_{\tilde P}(dH-\sum_{i=1}^ {d(d-1)}E_i)\vert $ on
$Q_1=\tilde P$.\\
\end{inparaenum}
Hence $L'_0$ contracts $S''$ to a point $x$. Moreover $\dim(| \O_{\tilde P}(dH-\sum_{i=1}^ {d(d-1)}E_i|)=3$ and  this linear system maps 
$\tilde P$ to a \emph{monoid} $\Sigma$, i.e., to a rational surface of degree $d$ with a point of multiplicity $d-1$ at $x$ (see Remark \ref {rem:mon} for the case $d=4$). 

In conclusion, by twisting, we see that the degeneration of $(S_t, \O_{S_t}(1))$ to $(S''\cup \tilde P, L_0)$ is also a semistable model of the degeneration of $(S_t, \O_{S_t}(1))$ to a general monoid $(\Sigma, \O_\Sigma(1))$. 
\end{example}

\begin{example} [Families of  polarised K3 surfaces] \label{ex:K3} A special case of the previous example is the one of a general quartic surface in $\P^ 3$ degenerating to the general union of two quadrics. This is also a special case of degenerations of polarised K3 surfaces to a union of two scrolls (see \cite {clm}), which are type II degenerations according to the Kulikov-Persson-Pinkham classification  of semistable degenerations of $K3$ surfaces (see \cite{K, PP}).  


Let $\mathcal K_p$  be the moduli space of primitively polarized $K3$ surfaces $(S,L)$ of genus $p\geqslant 3$, i.e., the dualising sheaf $\omega_S$ of $S$ is trivial, $h^ 1(S,\O_S)=0$, and $L$ is big, nef and indivisible in ${\rm Pic}(S)$, with $L^ 2=2p-2$. Write  $p=2l+\varepsilon$, with $\varepsilon=0,1$ and $l \in \mathbb N$. If $E' \subset \P^{p}$ is an elliptic normal curve of degree $p+1$,  set $L_{E'}=\O_{E'}(1)$. 
Consider two {\it general} line bundles $L_1, L_2 \in \Pic^2(E') $ with $L_1\neq L_2$.
Denote by $\Sigma'_i$ the rational normal scroll of degree $p-1$ in
$\P^p$ described by the secant lines to $E'$ spanned by the divisors in $|L_i|$, for $1\leqslant i\leqslant 2$. One has 
\[ \Sigma'_i \cong  
\begin{cases} 
\P^1 \times \P^1 &  \; \mbox{if $p=2l+1$ is odd, } \\ 
 \mathbb{F}_1 &  \; \mbox{if $p=2l$ is even}.
\end{cases} 
\] 

The surfaces $\Sigma'_1$ and $\Sigma'_2$ are $\P^ 1$--bundles on $\P^ 1$. 
Denote by $\sigma_i$ and $f_i$ a minimal section and a fiber of the ruling of $\Sigma_i'$, respectively, so that $\sigma_i^ 2=\varepsilon -1$, $f_i^ 2=0$, and   \begin{equation}
  \label{eq:A}
L_{\Sigma'_i}:=\O_{\Sigma'_i}(1) \simeq \O_{\Sigma'_i}(\sigma_i + lf_i), \;\;\; \text{for}\;\;\;  1 \leqslant i \leqslant 2.
\end{equation}

By \cite[Thm.\;1]{clm}, $\Sigma'_1$ and $\Sigma'_2$  intersect transversally along $E'$, which is anticanonical on $\Sigma'_i$, i.e.
 \begin{equation}
  \label{eq:B1}
E'\sim -K_{\Sigma'_i} \sim 2\sigma_i+(3-\epsilon)f_i \;\;\; \text{for}\;\;\;  1 \leqslant i \leqslant 2,
\end{equation}
where $\sim$ is the linear equivalence. Hence $\Sigma'=\Sigma'_1\cup \Sigma'_2$ has normal crossings and its dualising sheaf $\omega_{\Sigma'}$ is trivial.  Set $L_{\Sigma'}:=\O_{\Sigma'}(1)$. 
The first cotangent sheaf $T^1_{\Sigma'}$ (cf. \cite[\S\;1]{Frie})  is the degree $16$ line bundle on $E'$
 \begin{equation}
  \label{eq:B}
T^1_{\Sigma'}\cong \N_{E'/\Sigma'_1}\otimes \N_{E'/\Sigma'_2}\cong L_{E'}^ {\otimes 4}\otimes (L_1\otimes L_2)^ {\otimes (3-2l-\epsilon)},
\end{equation}
where $\N_{E'/\Sigma'_i}$ is the normal sheaf of $E'$ in $\Sigma'_i$, for $i=1,2$,  and the last isomorphism comes from \eqref {eq:A} and \eqref {eq:B1}.


The surface $\Sigma'$ is a flat limit of smooth $K3$ surfaces in $\P^p$. Namely, if $\H_p$ is the component of the Hilbert scheme of surfaces in $\P^ p$ containing $K3$ surfaces $S$ such that $(S, \O_S(1))\in \mathcal K_p$, then $\Sigma'$ sits in $\H_p$ and, for general choices of $E', L_1, L_2$, the Hilbert scheme is smooth at $\Sigma'$ (see   \cite {clm}).  The fact that $T^1_{\Sigma'}$ is non-trivial implies that $\Sigma'$ is not a semi--stable limit of $K3$ surfaces: indeed, the total space $\mathfrak S'$ of every flat deformation of $\Sigma'$ to $K3$ surfaces in $\H_p$ is singular along a divisor $T\in |T^1_{\Sigma'}|$ (cf. \cite[Prop. 1.11 and \S\;2]{Frie}).  More precisely (see again \cite{clm} for details), if  
\begin{equation}\label{eq:defo}
\xymatrix{
\Sigma'\ar[d]\,\, \ar@{^{(}->}[r]& \mathfrak S'\ar[d]^ {\pi'} \ar@{^{(}->}[r] \ar[dr]^ {{\rm pr_2}} &\mathbb D\times \P^ p\ar[d] \\\
0\,\, \ar@{^{(}->}[r]& \mathbb D&\P^ p
 }
\end{equation}
is a deformation of 
$\Sigma'$ in $\mathbb P^p$ whose general member is a smooth $K3$ surface, then  $\mathfrak S'$ has  double points at the support of a divisor $T\in \vert T^1_{\Sigma'}\vert$ 
associated to the tangent direction to $\H_p$ at $\Sigma'$ determined by the  deformation \eqref {eq:defo}, via the  map
\begin{equation}\label{standard}
T_{\H_p, \Sigma'}\cong H^ 0(\Sigma', \N_{\Sigma'/\P^ p})\to H^ 0(T^ 1_{\Sigma'})
\end{equation}
induced  by the surjective sheaf map
\[
\N_{\Sigma'/\P^ p}\to T^ 1_{\Sigma'}.
\]
If $T$ is reduced (this is the case if \eqref {eq:defo} is general enough), then  the tangent cone to $\mathfrak S$ at each of the 16 points of $T$ has rank 4. If 
 $\Pi: \mathfrak S \to \mathfrak S'$ is a small resolution of singularities, one gets a
semistable degeneration $\pi:=\pi'\circ \Pi: \mathfrak S {\longrightarrow}\mathbb D$ of $K3$ surfaces, with central fiber $\Sigma := \Sigma_1\cup \Sigma_2$, where  $\Sigma_i=\Pi^{-1}(\Sigma'_i)$, for $i=1,2$, and still $\omega_\Sigma\cong \O_\Sigma$.  The polarising line bundle
on $\mathfrak S$ is  $\L:=\Pi^ *({\rm pr}_2^ *(\O_{\P^ p}(1)))$. 

Set  $E = \Sigma_1 \cap \Sigma_2$; then $E\cong E'$ and  
\begin{equation}\label{eq:t1}
T^1_{\Sigma}\simeq \O_E.
\end{equation}
\end{example}\medskip

Equation \eqref {eq:t1} is a particular case of the following general fact (see \cite {CCFM, Frie} for a more general formulation). 
%Suppose one has a semistable degeneration as above and that $S_0$ has smooth, irreducible components $Q_1,\ldots,Q_r$, intersecting transversally along the double curves $R_1,\ldots,R_s$. One has:


\begin{lemma}[Triple Point Formula]
\label{l:triple-point}
%{\normalfont (Triple Point Formula)}
Assume  $f: S \to \D$ is semistable. Let $Q,Q'$ be smooth irreducible components of $S_0$ intersecting along 
the \emph{double curve} $R$. Then
\begin{equation*}
\deg ({\bf N}_{R/ Q} )+\deg({\bf N}_{R/Q'})
+\mathrm{Card}\left\lbrace \begin{array}{c}
\text{triple points of $S_0$} \\
\text{along}\ R
\end{array} \right\rbrace=0,
\end{equation*}
where a \emph{triple point} is the intersection $R\cap Q''$ with a component $Q''$  of $S_0$ different from $Q,Q'$. 
\end{lemma}

%%%
\begin{comment}
\begin{remark} [See \cite {CCFM, Frie}]  \label {rem:TPF} There is a version of the  Triple Point Formula for the case in which the central fibre 
is not reduced, but its support 
has local normal crossings. Then, if the multiplicities of $Q,Q'$ are $m,m'$ respectively, 
one has
\begin{equation*}
m'\deg (N_{R\vert Q} )+m\deg(N_{R\vert Q'})
+\mathrm{Card}\left\lbrace \begin{array}{c}
\text{triple points of $S_0$} \\
\text{along}\ R_s
\end{array} \right\rbrace=0,
\end{equation*}
where each triple point $R\cap Q''$  has to be counted with
the multiplicity $m''$ of $Q''$ in $S_0$.  
\end{remark} 
\end{comment}

\section{Limit linear systems}
\label{s:resolving}

Consider a semistable degeneration $f: \cal S\to \D$ as in \S
\ref {s:setting}.
Suppose there is a polarising, ample, fixed components free line bundle $\L$ on the total
space $\cal S$, such that $h^ 0(S_t,L_t)$ is
constant for $t\in \D$.

Consider the subscheme ${\rm Hilb}(\L)$ of the \emph{relative Hilbert
  scheme} of curves 
of $\cal S$ over $\D$, which is the Zariski closure of the set of all curves $C\in \vert L_t\vert$, for $t\in \D^ *$.  
Assume  that ${\rm Hilb}(\L)$ is a component of the relative
Hilbert scheme, a condition  satisfied if $\Pic (S_t)$ has no
torsion for $t\in \D^ *$. 
One has a natural projection morphism $\varphi: {\rm Hilb}(\L)\to
\D$, which is a projective bundle over $\D^ *$, because ${\rm
  Hilb}(\L)$ is isomorphic to $\fP:=\P(f_*(\L))$ over $\D^ *$.  
We call the fibre of $\varphi$ over $0$ the \emph{limit linear system}
of $\vert L_t\vert$ as $t\in \D^*$ tends to $0$,
and we will denote it by  $\fL$.  

 \begin{remark}
\label{r:twist2} In general,
\emph{the limit linear system is not a linear system}.
One would be tempted to say that $\fL$ coincides with $\vert
L_0\vert$. This is the case if $S_0$ is irreducible, but it is 
in general no longer true when $S_0$ is reducible. Indeed in this case,
there may be non--zero sections of $L_0$ whose zero--locus
contains some irreducible component of $S_0$, and accordingly points
of $\vert L_0\vert$ which do not correspond to points in  the Hilbert
scheme of curves. This is related to the non--uniqueness of the limit line bundle
 and to the twisting procedure mentioned in \S~\ref {s:setting}
(see, e.g., Example \ref{ex:gh} below). We will come back to this in a while. 
\end{remark} 

The variety ${\rm Hilb}(\L)$ is birational to
$\fP$, and $\fL$ is a suitable degeneration of the projective
space  $\vert L_t\vert$, $t\in \Delta^ *$.  

%%%
\begin{comment}
\begin{lemma}
\label{l:lim-lin}
Let $\fP'\to \D$ be a flat and proper morphism, 
isomorphic to $\fP$ over $\D^*$,
and such that $\fP'$ is a Zariski closed subset of $\Hilb(\L)$. 
Then $\fP'=\Hilb(\L)$.
\end{lemma}

\begin{proof}
Note that $\fP'$ is open in  $\Hilb(\L)$, which is 
irreducible.
\end{proof}
\end{comment}
%%%

As the following example shows, in passing from $\fP$ to ${\rm Hilb}(\L)$,
one has to perform a series of blow--ups along
smooth centres contained in the central fibre, which correspond to
spaces of non--trivial sections of some (twisted)  line  bundles which
vanish on divisors contained in the central fibre. 
The exceptional divisors
one gets in this way give rise to components of $\fL$, and may be
identified with birational modifications of sublinear systems of
twisted linear systems restricted to $S_0$. 


\begin{example} [See \cite{gh-degen}] 
\label {ex:gh}
Consider a family of degree $d$ surfaces $f: \cal S\to \D$ arising,
as in Example \ref{ex:pi3}, from a linear pencil
  generated by a general surface $S_\infty$ and by $S_0=S''\cup P$,
  where $P$ is a plane and $S''$ a general surface of degree $d-1$. 
One has a semistable model 
$\tilde f: \tilde S\to \D$
as described in  Example \ref {ex:pi3}, from which we keep the notation.  

Let $\L$ be the polarising hyperplane bundle. 
The component $\Hilb(\L)$ of the Hilbert scheme is gotten from the
projective bundle $\P(\L)$, by blowing up  
the point of the central fibre $\vert \O_{S_0}(1)\vert $ corresponding to the 1--dimensional space of non--zero sections vanishing on the plane $P$.  
The limit linear system $\fL$ is  the union of $\fL_1$, the blown--up
$\vert \O_{S_0}(1)\vert $, and of the exceptional divisor $\fL_2\cong
\P^ 3$, 
identified as the twisted linear system $\vert \O_{\tilde S_0}(1)\otimes
\O_{\tilde S}(-\tilde P)\vert$, whose aspects have been described in Example \ref{ex:pi3}.

The components $\fL_1$ and $\fL_2$ of $\fL$  meet along the
exceptional divisor $\mathfrak{E}\cong \P^ 2$ of the morphism 
$\fL_1\to |\O_{S_0}(1)|$. 
The elements of 
$\mathfrak{E}\subset \fL_1$ 
identify as the points of $\vert \O_R(1)\vert\cong \vert \O_P(1)\vert$, 
whereas the plane $\mathfrak{E}\subset \fL_2$ is the set of elements  
$C\in \vert \O_{\tilde P}(d)\otimes \O_{\tilde P}(-\sum_{i=1}^
{d(d-1)}E_i)\vert$ containing the proper transform $\hat R \cong R$ of
$R$ on $\tilde P$. The corresponding element of $\vert \O_R(1)\vert$
is cut out on $\hat R$ by the further component of $C$, which
is the pull--back to $\tilde P$ of a line in $P$. 

All this will be made  explicit in the case $d=4$ in \S\ref {ssec:another}.  \end{example} 


\section{Severi varieties and their limits}
\label{s:Severi-1}

Let $f: \cal S\to \D$ be a (not necessarily semistable) family as in \S \ref {s:setting}, polarised by a line bundle $\L$ on $\cal S$.  
Fix  a non--negative integer $\delta$, and consider 
the locally closed subset  $\mathring{V}_{\delta}(\cS,\L)$ of  $\Hilb(\L)$
formed by all curves $D\in \vert L_t\vert$, for $t\in \D^ *$,
such that $D$ is  irreducible, nodal, and has exactly $\delta$ nodes.
Define ${V}_{\delta}(\cS,\L)$ (resp. $\cru{V}_{\delta}(\cS,\L)$) as
the Zariski closure of 
$\mathring{V}_{\delta}(\cS,\L)$ in $\Hilb(\L)$ (resp. in $\fP=\P(f_*(\mathcal
L))$). This is the \emph{relative Severi variety} (resp. the
\emph{crude relative Severi variety}).
Sometimes we may write  $\mathring{V}_{\delta}$,
${V}_{\delta}$,  and $\cru V_\delta$, rather than $\mathring{V}_{\delta}(\cS,\L)$,  
 ${V}_{\delta}(\cS,\L)$ and $\cru{V}_{\delta}(\cS,\L)$, respectively.
  
There is a natural map $f_{\delta}: {V}_{\delta}\to \D$. If $t\in
\D^* $, the fibre $V_{\delta,t}$
of $f_{\delta}$ over $t$ is the  \emph{Severi variety}
${V}_{\delta}(S_t,L_t)$ of $\delta$--nodal curves in the linear
system $\vert L_t\vert$ on $S_t$. The degree of  $V_{\delta,t}$ as a subvariety of $|L_t|$ is independent on $t\in \D^ *$,  and will be denoted by $d_\delta(\L)$ (or simply by $d_\delta$).  
Let ${\fV}_{\delta}(\cS,\L)$ (or simply $\fV_\delta$) be
the central fibre of $f_{\delta}: {V}_{\delta}\to \D$;
it is the \emph{limit Severi variety} of ${V}_{\delta}(S_t,\L_t)$ as
$t\in \D^*$ tends to $0$.  This is a subscheme of  the
limit linear system $\fL$, which has been studied by
various authors (in the present setting by Z. Ran \cite {Ran1, Ran2, Ran3}, then by
L. Caporaso, J. Harris \cite {caporaso-harris, caporaso-harris2}, more
recently by C. Galati  and C. Galati and A. Knutsen \cite{concettina1, concettina2} following Z. Ran; this theme is however quite classical
as B. Segre's paper \cite {bsegre} shows, and it appears in disguise
in work of other authors, like S. Kleiman \cite {KL}).  

In a similar way, one defines the \emph{crude limit Severi variety}
$\cru{\fV}_{\delta}(\cal S,\L)$ (or $\cru\fV_\delta$),
sitting in $\vert L_0 \vert$. 

\begin{remark}\label{rem:exp} For $t\in \D^ *$, the \emph{expected dimension} of the Severi variety ${V}_{\delta}(S_t,\L_t)$ is
$\dim (\vert L_t\vert)-\delta$ (see \cite[Thm. 6.3]{ser2}). We will always assume that the dimensions of (all components of) ${V}_{\delta}(S_t,L_t)$  equal the expected dimension for all 
$t\in \D^ *$. This is a strong assumption, implying that $\mathring{V}_{\delta}$ is smooth; it will be satisfied
in our applications. 
\end{remark}

%%%
\begin{comment}
\begin{notation}
Let  $f: S\to \D$ be a family of degree $d$ surfaces in $\P^ 3$ as
in Example \ref {ex:pi3}, and let $\tilde f: \tilde S\to \D$ be a
semistable model of $f: S\to \D$.
Consider the line bundle $\O_S(1)$, defined as the pull--back of
$\O_{\P^3}(1)$ via the  map $S\to \P^3$, and let 
$\O_{\tilde S}(1)$ be its pull--back  on $\tilde S$.
Denote by $\fV_{n,\delta}(\tilde S)$
(resp. $\fV_{n,\delta}(S)$), or simply $\fV_{n,\delta}$,
the limit Severi variety $\fV_{\delta}(\tilde S,\O_{\tilde S}(n))$
(resp. $\fV_{\delta}(S,\O_{S}(n))$).
Similar notation $\cru \fV_{n,\delta}(\tilde S)$
(resp. $\cru \fV_{n,\delta}(S)$), or $\cru \fV_{n,\delta}$, will be used for
the crude limit. 
\end{notation}
\end{comment}
%%%


Let us come now to the description of the limit Severi variety, under
the assumption that the family $f: \cal S\to \D$ is semistable. We will freely use the notation introduced above and follow the approach in  \cite{concettina1,concettina2}.
We will suppose  that the central fibre $S_0$  has smooth irreducible components $Q_1,\ldots,Q_r$, with double curves
$R_1,\ldots,R_s$.  We will assume, in addition, that there are $q$ exceptional curves $E_1,\ldots, E_q$ on $S_0$, arising from a small resolution of an original family with singular total space, as discussed in \S \ref {s:setting}. 

\begin{notation}
Let $\seqN$ be the set of sequences $\utau=(\tau_m)_{m\geqslant 2}$ of
non--negative integers 
 with only finitely many non--vanishing terms. Define two maps $\nu,\ \mu: \seqN \to \N$ as follows
\begin{equation*}
\nu\left( \utau \right) =
\sum\nolimits_{m \geqslant 2} \tau_m \cdot (m-1),
\quad \text{and} \quad
\mu\left( \utau \right) =
\prod\nolimits_{m \geqslant 2} m^{\tau_m}.
\end{equation*}
Given a $p$-tuple
$\ubtau=(\utau_1,\ldots,\utau_p) \in  \seqN^p$,
set 
\begin{equation*}
\nu(\ubtau) = \nu(\utau_1)+\cdots + \nu(\utau_p),
\quad \text{and} \quad
\mu(\ubtau) = \mu(\utau_1) \cdots \mu(\utau_p),
\end{equation*}
 defining two maps $\nu,\ \mu: \seqN^p \to \N$.
Given $\bdelta=(\delta_1,\ldots,\delta_r) \in \N^r$, set
\begin{equation*}
|\bdelta| := \delta_1 + \cdots + \delta_r.
\end{equation*}
Given a subset $I \subset \{1,\ldots,q\}$, $|I|$
will denote its cardinality.
\end{notation}

\begin{definition}
\label{d:zrr}
Consider a divisor
$W$ on $\cal S$, supported on the central fibre $S_0$, such that the twist $\L(-W)$ is \emph{centrally effective}, i.e., all the aspects of $\L(-W)$ on the components $Q_1,\ldots, Q_r$ of $S_0$ are effective. Fix 
\[\bdelta \in \N^r, \quad \ubtau\in
\seqN^p\quad \text{ and}\quad I\subseteq \{1,\ldots,r\}.
\]
Let $\mathring{V}(W,\bdelta,I,\ubtau)$
be the Zariski locally closed subset in
$|\L(-W)\otimes \O_{S_0}|$ parametrizing curves $D$ such that:\\
\begin{inparaenum}[\normalfont (i)]
\item
\label{no-double-curve}
  $D$ contains no double curve $R_l$, with $l\in \{1,\ldots, s\}$, 
and no triple point of $S_0$;\\
\item $D$ contains $E_i$, with multiplicity 1,
  if and only if $i\in I$, and has a node on it;\\
\item off the singular locus of $S_0$ the curve $D-\sum_{i\in I} E_i$ has only nodes as singularities, and their number is  $\delta_s$ on $Q_s$, for $s\in \{1,\ldots, r\}$;\\
\item 
\label{c:tacnodes}
for every $l\in \{1,\ldots, s\}$ and $m \geqslant 2$, there are exactly
$\tau_{l,m}$ points on $R_l$, off the intersections with $\sum_{i\in I} E_i$ and off the triple points of $S_0$ along $R_l$, 
at which $D$ has an \emph{$m$-tacnode} (see below for the definition),
%with local branches given by $D_{l'}$ and $D_{l''}$,
with reduced tangent cone equal to the tangent line of $R_l$ there.
\end{inparaenum}

We let ${V}(W,\bdelta,I, \ubtau)$ be the Zariski closure of
$\mathring{V}(W,\bdelta,I, \ubtau)$ in
$|\L(-W)\otimes \O_{S_0}|$.
\end{definition}


Recall that an \emph{$m$-tacnode} is an $A_{2m-1}$-double point,
\ie a plane
curve singularity locally analytically isomorphic 
to the curve of $\C^2$ defined by the equation 
$y^2=x^{2m}$ at the origin.
Condition \eqref{c:tacnodes} in Definition \ref {d:zrr} requires that $D$ is a Cartier divisor on $S_0$, having $\tau_{l,m}$ 
$m$--th order tangency points with the curve $R_l$, at 
points of $R_l$ which are neither points on $\sum_{i\in I} E_i$ nor triple points of $S_0$.


\begin{notation}\label{not:1}
Rather than using the notation ${V}(W,\bdelta,I, \ubtau)$,
we may sometimes use a more expressive one like, e.g., 
$V(W,\delta_{Q_1}=2,E_1,\tau_{R_1,2}=1)$ for the variety
parametrizing curves in $|\L(-W)\otimes \O_{S_0}|$, with two nodes on $Q_1$, one
simple tacnode along $R_1$, and containing the exceptional curve
$E_1$. Similarly  $V(\delta_{Q_1}=1)$  is the variety
parametrizing curves in $|\L\otimes \O_{S_0}|$, with only one node on $Q_1$, etc.
\end{notation}



\begin{proposition} [\cite{concettina1, concettina2},
  see \cite{04b.concettina}]
\label{p:zrr}
Let $W,\bdelta, I, \ubtau$ be as above,
and set 
\[
\delta=|\bdelta|+\vert I\vert+\nu(\ubtau).
\]
Let $V$ be an irreducible component of $V(W,\bdelta,I,\ubtau)$.
If \\
\begin{inparaenum}[(i)]
\item
\label{c:hilb}
the linear system $|\L(-W)\otimes \O_{S_0}|$
has the same dimension
as $|\L_t|$ for $t\in \D^*$, and\\
\item
\label{c:versal}
$V$ has (the expected) codimension $\delta$ in 
$|\L(-W)\otimes \O_{S_0}|$,
\end{inparaenum}\\
then $V$ is an irreducible component of multiplicity $\mu(V):=\mu(\ubtau)$
of the limit Severi variety $\mathfrak V_\delta(S,\L)$.
\end{proposition}



%%%%
\begin{comment}
As we said already, we will usually assume that the surfaces $X_t$, with $t\in \Delta^*$, are \emph{regular}, i.e.
$h^1(X_t,\O_{X_t})=0$, condition \eqref{c:hilb} ensures that the
component ${\cal H}^n_{X/\Delta}$ of the relative Hilbert scheme is
smooth at the general point of $|\O_{X}(n\H-W)\otimes \O_{X_0}|$.
On the other hand, condition \eqref{c:versal} ensures the smoothness
of a suitable map in the product of the \'etale versal deformation
spaces of the singularities of a general member of $V$.
\end{comment}
%%%%%%

\begin{remark}
\label{r:smoothness}
Same assumptions as in Proposition \ref{p:zrr}. If  there is
at most one tac\-node (i.e. all $\tau_{l,m}$ but 
possibly one vanish, and this is equal to $1$), 
the relative Severi variety $V_\delta$ is smooth at the general
point of $V$ (see \cite {concettina1, concettina2}),
and thus $V$ belongs to only one
 irreducible component of $V_\delta$.
There are other cases in which such a smoothness property holds (see
\cite{caporaso-harris} or, in this volume,
\cite{04.concettina}).


If $V_\delta$  is smooth at the
general point  $D\in V$, the multiplicity of $V$ in the limit Severi
variety $\mathfrak V_\delta$  is the minimal integer $m$
such that there are local analytic \emph{$m$--multisections} of
$V_\delta \to \D$, i.e. analytic smooth curves in 
$V_\delta$, passing through $D$ and intersecting the general
fibre $V_{\delta, t}$, $t\in \D^ *$, at $m$ distinct points.
\end{remark}



Proposition \ref{p:zrr}  does not provide a complete picture of 
the limit Severi variety.
For instance, curves passing
through a  triple point of $S_0$ could  (and in fact do; see \cite {CD}, and \S \ref {ssec:bad} below) play a role in this limit.
It would be desirable to know that one can always  obtain a semistable model of the original family,
where  \emph{every} irreducible component of the limit Severi variety
is realized 
as a family of curves of the kind stated in Definition \ref{d:zrr}. 

\begin{definition}
\label{def:reg-comps}
Let $f: \cal S\to \D$ be a semistable family as in \S \ref {s:setting}, with a polarising line bundle
$\L$,
and $\delta$ a positive integer.
The \emph {regular part of the limit Severi variety}
$\fV_\delta(\cal S,\L)$ is the cycle in the limit linear system $\fL
\subset \Hilb(\L)$ defined as
\begin{equation}
\label{reg-Severi}
%\tag{$\dagger$}
\reg \fV_\delta(\cS,\L):=
\sum_W \sum_{|\bdelta|+|I|+\nu(\ubtau)=\delta} \mu(\ubtau) \cdot
\Biggl( \sum_{V \in \mathrm{Irr}^\delta\left( V(W,\bdelta,I,\ubtau)
    \right)}  V \Biggr),
\end{equation}
(sometimes simply denoted by $\reg \fV_\delta$) where:\\
\begin{inparaenum}[(i)]
\item \label{def:2} $W$ varies among all effective divisors on $S$
supported on the central fibre $S_0$, such that  $\L(-W)$ is {centrally effective} and
$h^0(\L_0(-W))=h^0(L_t)$ for $t\in \D^*$;\\
\item ${\rm Irr}^\delta(Z)$ denotes the set of all codimension
  $\delta$ irreducible components of a scheme $Z$. 
\end{inparaenum}
\end{definition}

Proposition \ref{p:zrr} asserts that the cycle
$Z(\fV_\delta)-\reg \fV_\delta$ is effective
%, with support disjoint in codimension $1$ from that of $\reg \fV_\delta$
where $Z(\fV_\delta)$ is the cycle associated to $\fV_\delta$.
We call the irreducible components of the support of $\reg \fV_\delta$
the \emph {regular components} of the limit Severi variety.

Let  now $\tilde f: {\tilde \cS} \to \D$ be a semistable model of a (not necessarily semistable) degeneration
$f: \cS\to \D$, and $\tilde \L$ the pull--back on $\tilde \cS$ of a polarising line bundle
$\L$ on $\cS$.
There is a natural map $\Hilb(\tilde\L)\to \Hilb(\L)$, which induces a
morphism $\phi: \tilde\fL\to |L_0|$.

\begin{definition}
\label{def:good-model}
The semistable model $\tilde f: {\tilde \cS} \to \D$ is a 
$\delta$--\emph{good model} of $f: \cS\to \D$
(or simply a \emph{good model}, if it is clear which $\delta$ we are
considering), if the following equality of cycles holds
\[
\phi_* \bigl( \reg\fV_\delta(\tilde \cS, \tilde \L) \bigr)=
\cru\fV_\delta(\cS,\L).
\]
\end{definition}

Note that the cycle $\cru\fV_\delta(\cS,\L)-
\phi_* \bigl( \reg\fV_\delta(\tilde \cS, \tilde \L) \bigr)$
is effective.
The family $f:\cS\to \D$ is said to be $\delta$--\emph{well behaved}
(or simply \emph{well behaved} if $\delta$ is understood) if it has a $\delta$-good model.

%A semistable model $\tilde f: \tilde S\to \D$ of $f: S\to \D$ as above
%is said to be  $\delta$--\emph{absolutely good} if $\fV_\delta(\tilde S, \tilde \L)=
%\reg \fV_\delta(\tilde S, \tilde \L)$ as cycles in the relative Hilbert scheme.
%It is then a $\delta$--good model both of itself and of $f: S\to \D$.


\begin{remark}
\label{r:other-lim}
Suppose that $f: \cS\to \D$ is $\delta$--well behaved, with
$\delta$--good model $\tilde f:{\tilde \cS} \to \D$. 
It is possible that some components in
$\reg\fV_\delta(\tilde \cS,\tilde \L)$ are
contracted by $\phi$ to varieties of
smaller dimension, and therefore  their push--forwards to $\cru\fV_\delta(\cS,\L)$ are zero.
Hence these components of $\fV_\delta(\tilde \cS, \tilde \L)$ are 
\emph{not visible} in $\cru\fV_\delta(\cS,\L)$.
They are however usually visible in the crude limit Severi variety of
some other model $f': \cS'\to \D$, obtained from $\tilde \cS$ via an
appropriate twist of $\L$.
The central fibre $S'_0$ is then a flat limit of $S_t$, as
$t\in\D^*$ tends to $0$, different from $S_0$ (a situation met in  Example \ref {ex:pi3}).
\end{remark}

\begin{conjecture}[See \cite {CD}] \label{conj:goodness}
Let $f:\cS\to \D$ be a degeneration of surfaces, endowed with a
line bundle $\L$ as above, and $\delta$ a positive integer. Then  $f: \cS\to \D$ is $\delta$--well behaved.
\end{conjecture}

The local computations in \cite{concettina1,concettina2} provide a criterion for being 
well behaved:

\begin{proposition}\label{prop:criterion}
Assume there is a semistable model $\tilde f:{\tilde \cS} \to \D$ of
$f:\cS \to \D$, 
with a limit linear system $\tilde \fL$ which does not contain, in codimension $\delta+1$,
curves of the following types: \\
\begin{inparaenum}[(i)]
\item
\label{cat:first} curves containing 
double curves  of $\tilde S_0$;\\
\item \label {cat:trip} curves passing through a triple point of
  $\tilde S_0$;\\
 \item
\label{cat:last}
non--reduced  curves.\\
\end{inparaenum}
If in addition, for $W,\bdelta,I,\ubtau$ as in Definition \ref{d:zrr},
every irreducible component of ${V}(W,\bdelta,I, \ubtau)$ has the
expected codimension in $|L_0(-W)|$,
then $\tilde f:{\tilde \cS} \to \D$ is  $\delta$--well behaved.
\end{proposition}


\begin{remark} While there are good reasons to believe that Conjecture \ref {conj:goodness} has an affirmative answer, one cannot expect that, in the algebraic category,  there is a good model of a given  family, which  \emph{universally} works for all polarising line bundles $\L$. 
This in fact could require infinitely many birational modifications of the total space. 
\end{remark}



On the other hand, it is hopeless to ask for a semistable model on
which all irreducible components of the limit Severi variety would
parametrize nodal curves
(\ie such that there are no tacnodes as in Item (iv) of Definition
\ref{d:zrr}):
we explain this in \cite{15.tacnodo}, together with C.~Galati.


The three final sections are 
devoted to examples which will hopefully clarify the considerations and  results in Section~\ref {s:Severi-1}.


\section{Example: Limits of 1--nodal plane sections for surfaces in
  $\P^ 3$}\label{ssec:1nodal}
Consider a degeneration of a general degree $d$ surface $S$ in $\P^ 3$
to a reducible surface $S'\cup S''$, as in Example \ref {ex:pi3}, from
which we keep the notation.  Here $S_0=S'\cup S''$, and $R=S'\cap S''$
is a smooth curve of degree $h(d-h)$. Then in the semistable model
$\tilde f: \tilde \cS\to \D$ constructed in Example \ref {ex:pi3},
$\tilde S_0=Q_1\cup Q_2$, and
$Q_1$ and $Q_2$ intersect transversally along a curve  which may be identified with $R$.

\paragraph{}
Assume $h\geqslant 2$. Then  the only twist which is centrally effective is the trivial one and $\fV_1^ {\rm reg}$ consists of $3+q$ components (remember that $q=hd(d-h)$), precisely:\\
\begin{inparaenum}
\item [(1)] $V(\delta_{Q_i}=1)$, with $i=1,2$, with multiplicity 1;\\
\item [(2)] $V(\tau_{R,2}=1)$, with multiplicity 2;\\
\item [(3)] $V(E_i)$, for $i=1,\ldots, q$, with  multiplicity 1.
\end{inparaenum}

This tells us that in the above degeneration, the limit of the dual
variety $\check S$,
which sits in $\L_0=\check \P^3$ and coincides with the crude limit of the Severi variety $\fV_1^ {\rm cr}$, contains: \\
\begin{inparaenum}
\item [(i)] the dual varieties $\check S'$ and $\check S''$ with multiplicity 1 (corresponding to (1));\\
\item [(ii)] the dual variety $\check R$ with multiplicity 2 (corresponding to (2));\\
\item [(iii)] the $q$ planes $x_i^ \perp\subset \check \P^3$, orthogonal to the points $x_i$, for $i=1,\ldots, q$, with multiplicitiy 1 (corresponding to (3)).
\end{inparaenum}

One computes:\\
\begin{inparaenum}
\item [(a)] $\deg (\check S')=h(h-1)^ 2$ and $\deg(\check S'')=(d-h)(d-h-1)^ 2$;\\
\item [(b)] $\deg(\check R)=h(d-h)(d-2)$.
\end{inparaenum}\\
So adding up, we see that the sum of the degrees of the components in (i)--(iii) above, counted with the appropriate multiplicities, is $d(d-1)^ 2$, hence the components in (1)--(3) exhaust the limit Severi variety
$\fV_1$, i.e., the above degeneration is 1--well behaved. 

\paragraph{}
If $h=1$, one needs to change the analysis, due to the presence of the non--trivial twist by  $Q_1$ which is centrally effective. In this case  $\fV_1^ {\rm reg}$ consists of the following components:\\
\begin{inparaenum}
\item [($\alpha$)] $V(\delta_{Q_2}=1)$, with multiplicity 1 (note that $V(\delta_{Q_1}=1)$ is zero);\\
\item [($\beta$)] $V(Q_1,\delta_{Q_1}=1)$, with multiplicity 1;\\
\item [($\gamma$)] $V(\tau_{R,2}=1)$, with multiplicity 2;\\
\item [$(\delta$)] $V(E_i)$, for $i=1,\ldots, q$, with  multiplicity 1.
\end{inparaenum}\\
However, only the components in $(\alpha), (\gamma)$ and  $(\delta)$ contribute to the crude limit of the Severi variety $\fV_1^ {\rm cr}$, and exhaust it (same computation as above), because the component in $(\beta)$ is not visible in the crude limit, since it is contracted to a point (see Remark \ref {r:other-lim}). In conclusion also this degeneration is 1--well behaved and the limit of $\check S$ is the union of $\check S'$ 
plus $d(d-1)$ planes plus the dual of the plane curve $R$ counted with multiplicity 2. 


\section{Example: Limits of 3--nodal plane sections for quartic surfaces in
  $\P^ 3$}
\label{ssec:3nodal}

The number of 3--nodal plane sections of a general quartic surface $S$ in $\P^ 3$ (or of triple points of the dual $\check S$) given by Salmon's formula \eqref {eq:salmon} is 3200. 

\subsection{Degeneration to two quadrics}
\label{ssec:3nodal:1st}

Let us recover this first by considering a degeneration to two
quadrics: thus we will look 
at the case $h=d-h=2$ in Example \ref {ex:pi3} (from which we keep the notation; this is the same as the degeneration in Example \ref {ex:K3} for $p=3$).

In this case $R$ is an elliptic quartic curve, the semistable degeneration has central fibre
$Q_1\cup Q_2$, with $R=Q_1\cap Q_2$, $Q_1$ is a quadric, and $Q_2$ a quadric blown up at the complete intersection points $x_1,\ldots, x_{16}$ of $R$ with a general quartic surface $S$  (see Figure \ref{fig:quadrics}).

\begin{figure}
\begin{center}
\includegraphics[height=5cm]{quadrics.eps}
\end{center}
\caption{Degeneration into two quadrics}
\label{fig:quadrics}
\end{figure}

For the computation, one has to consider 
the various cases for ${V}(W,\bdelta,I, \ubtau)$ as in Definition \ref {d:zrr}. No non--trivial twist is centrally effective, so $W=0$. If $|\bdelta|=3$, then ${V}(W,\bdelta,I, \ubtau)$ is empty,  
because one cannot have two (or more) singular points on a plane section of a smooth quadric. Hence:\\
\begin{inparaenum}
\item [$\bullet$] $0\leqslant |\bdelta| \leqslant 2$, and if $|\bdelta|=2$ then $\delta_1=\delta_2=1$;\\
\item  [$\bullet$]  ${\bf \tau}=(\tau_2,\tau_3,\tau_4)$ and $|I|+2\tau_2+3\tau_3+4\tau_4\leqslant 4$;\\
\item  [$\bullet$]  $|\bdelta|+|I|+\tau_2+2\tau_3+3\tau_4=3$.\\
\end{inparaenum}
Therefore the cases to be discussed are the following.

\begin{catalogo}

\caseitem{$\delta_1=\delta_2=1$, $|I|=1$}

For each $i=1,\ldots,16$, a plane tangent to both $S'$ and $S''$, and
passing through $x_i$ in $\P^3$ is entirely determined by the choice
of a line passing through $x_i$ in both $Q_1$ and $Q_2$. 
There are exactly $2 \times 2 = 4$ such choices (two rulings on each
quadric). We get $16 \times 4 = 64$ curves.


\caseitem{$\delta_1=\delta_2=1$, $\tau_2=1$}
\label{case:uso-polare}

The intersection $\check{S'} \cap \check{S''} \cap \check{R}$
consists of $2 \times 2 \times 8 = 32$ points. 
From this, we want to remove the points corresponding to planes
tangent to one quadric at some point lying on $R$. Each of them has 
multiplicity $2$ in the intersection $\check{S'}\cap \check{S''}\cap \check{R}$ by  the:

\begin{lemma} [Lemma 3.5, \cite {CD}]
\label{l:tangency}
Let $R$ be a smooth, irreducible curve contained in a smooth
surface $S$ in $\P^3$.
Let $\check{R}_S$ be the irreducible curve in $\check \P^3$
parametrizing planes tangent to $S$ along $R$.
Then the dual varieties $\check{S}$ and $\check{R}$ both contain
$\check{R}_S$, and do not intersect transversally at its general point. 
\end{lemma}

\begin{proof}
Clearly  $\check{R}_S$ is contained in  $\check{S}\cap \check{R}$.
If either  $\check{S}$ or $\check{R}$ are singular at the general
point of $\check{R}_S$, there is nothing to prove. Assume that
$\check{S}$ and $\check{R}$ are both smooth at the general point of
$\check{R}_S$. 
One has to show that they are tangent there. Let $x\in R$ be
general. Let $H$ be the tangent plane to $S$ at $x$. Then $H\in
\check{R}_S$ is the general point. The biduality theorem (see ,
e.g., \cite [Example 16.20]{harris2}) says that the tangent planes to
$\check{S}$ and $\check{R}$ at $H$ both coincide with the set of
planes in $\P^ 3$ containing $x$, hence the assertion.
\end{proof} 

The curve parametrizing planes tangent to $S'$ at some point of $R$
has degree $4$ (to see this, intersect $R$ with a general polar plane
of $S'$, \cf \cite[Appendix~\tref{S:polarity}]{13.th-classic}).
Hence
this curve intersects $\check{S''}$ at $8$ distinct points (without
multiplicities). Eventually, we have to remove $2\times 2\times 8$ points
from $\check{S'}\cap \check{S''} \cap \check{R}$, and there does not
remain anything.


\caseitem{$\delta_i=1$ for an $i=1,2$,  $|I|=2$}


For each $i=1,2$ and each set $\{r,s\}\subset I$, $r\not= s$, we count points
of intersection of $\check{Q}_i$ with the line of $\check{\P}^3$ orthogonal to the line $\langle x_r, x_s\rangle$. There are
$ 2 \times \binom{16}{2} \times 2 = 480$
such points.

\caseitem{$\delta_i=1$ for an $i=1,2$,  $|I|=1$, $\tau_2=1$}

For each $i=1,2$ and $r=1,\ldots, 16$, there are two lines on $Q_i$ through the point
$x_r$. They determine two pencils of planes tangent to $Q_i$ and
passing through $x_r$. 

The planes of each of these pencils cut out a $g^1_2$ on $R$: the intersection of such a
plane with $R$ consists of $4$ points, two of which are
fixed (the two intersection points of the chosen line
through $x_r$ with $R$).

Since a $g^1_2$ on an elliptic curve has $4$ double points, we get $2
\times 4$ planes satisfying our conditions for each $i$ and $r$. 
These give a contribution of  $2 \times 16
\times 2 \times 8 = 512$ to our computation.


\caseitem{$\delta_i=1$ for an $i=1,2$,  $\tau_2=2$}

Planes satisfying these conditions are spanned by two lines
belonging respectively to the two rulings of $Q_i$, both tangent to
$R$.  By genericity, two such lines do not meet on $R$.

Each ruling of $Q_i$ cuts out a $g^1_2$ on $R$, and thus contains
exactly $4$ tangent lines to $R$ (since a $g^1_2$ on $R$ has $4$
ramification points). 
We thus get $16$ planes satisfying our conditions for each $i$.
This contributes $2 \times 4\times 16 = 128$ to our computation.

\caseitem{$\delta_i=1$ for an $i=1,2$,  $\tau_3=1$}

This requires planes spanned by two lines on $Q_i$,
one of which is tangent to $R$, and meets the other line on $R$ at
this tangency point. Such a plane is  tangent to $Q_i$ at a point
lying on $R$, and therefore cuts a curve with worse singularity than required.
Hence they do not contribute to our computation.

\caseitem{$\tau_4=1$}

Since $R$ is a smooth degree $4$ elliptic curve in $\P^3$, the set of
its hyperplane sections is  
$$\{ (a,b,c,d) \in \mathrm{Sym}^4 (R) \ | \ a+b+c+d=0 \in (R,+)
\}.$$ 
Hence, the planes we are looking for are in 1-1 correspondence
with 4-torsion points of $R$ and so there are 16 of them, each to be counted
with multiplicity $4$, so we get a
contribution of  64.

\caseitem{$|I|=1$, $\tau_3=1$}


Fix $r=1,\ldots, 16$, and consider the projection $\pi$ from $x_r$. It maps $R$ to
a smooth cubic plane curve. Since this has 9 flexes, this gives us 9 planes through
$x_r$ satisfying the required condition. Each of them has to be counted with multiplicity 3,
and this gives a contribution of $16 \times 3 \times 9 = 432$ to our computation. 

\caseitem{$|I|=2$, $\tau_2=1$}


For given $r,s$ distinct in $\{1,\ldots,16\}$, the pencil of planes through $x_r$ and $x_s$
cuts out (off of $x_r+x_s$) a $g^1_2$ on $R$. It has $4$ double points, hence the pencil
contains $4$ tangent planes to $R$. By genericity, the tangency points
are distinct from $x_r$ and $x_s$. This gives a contribution of 
$\binom{16}{2} \times 2 \times 4 = 960$  to the computation.

\caseitem{$|I|=3$}
% last case so far

For each choice of three different indices $r$, $s$ and $l$ in $\{1,\ldots,16\}$, there is one plane through $x_r$, $x_s$ and $x_l$. So we  get a
contribution of $\binom{16}{3}=560$.\medskip

\end{catalogo}

Adding up all the non--trivial contributions as in the following table, we get exactly 3200, which is the number predicted by Salmon's formula.  
This shows that this degeneration is  
3--good.

\begin{center}
\begin{tabular}{|l|r|}
\hline
$\text{Cases} $ & \text{Contribution} \\
\hline
$\text{Case 1}$ & 64 \\
\hline
$\text{Case 3}$ & 480 \\
\hline
$\text{Case 4}$ & 512 \\
\hline
$\text{Case 5}$ & 128 \\
\hline
$\text{Case 7}$ & 64 \\
\hline
$\text{Case 8}$ & 432 \\
\hline
$\text{Case 9}$ & 960 \\
\hline
$\text{Case 10}$ & 560 \\
\hline \hline
\textbf{Total} & $\mathbf{3200}$ \\
\hline
\end{tabular}
\end{center}


\subsection{Degeneration to a cubic and a plane}
\label {ssec:another}


We will now do the same enumeration as in Section \ref{ssec:3nodal:1st},
this time by considering a degeneration to a cubic and a plane.
Thus, we want to count 3--nodal plane sections of a general quartic
surface $S$ in $\P^ 3$, and we will look
at the degeneration in Example \ref {ex:pi3}, with $d=4$ and $h=1$. This will be instructive, because it will require to make one of the first non--trivial cases of  computation of the degree of a Severi variety of plane curves with nodes.

We simplify a bit the notation of Example \ref {ex:pi3}. We denote by $T+P_0$ the reducible surface $S_0$ in  Example \ref {ex:pi3} (so $T$ is a general cubic, $P_0$ a general plane, with $P_0\cap T=R$ a general plane cubic), and we denote by $T+P$ the central fibre of the semistable degeneration, where $P$ is the plane $P_0$ blown--up at $12$ points  $x_1,\ldots, x_{12}$ forming a general divisor in $|\O_R(4)|$ (see Figure \ref {fig:cubic}). 


\begin{figure}
\begin{center}
\includegraphics[height=5cm]{cubic.eps}
\end{center}
\caption{Degeneration into a cubic plus a plane}
\label{fig:cubic}
\end{figure}

Now we explain in some detail in this case what we stated in Example \ref {ex:pi3} about the limit linear system $\mathfrak L$ of the plane sections of $S_t$.


\begin{proposition}
\label{prop:limitT+P}
Let $\tilde{\mathcal{H}}_{\P^3}$ be the blow up of
$|\O_{\P^3}(1)|=\check{\P}^3$ at the point corresponding to the plane
$P_0\subset \P^3$. Let $D_{P_0}\cong \P^ 2$ be the exceptional divisor of this blow up.

Set $\mathcal{H}_{P}=|\O_{P}(4H-\sum_{i=1}^{12}E_i)| \cong\P^3$ and denote by $D_R\subset \mathcal{H}_{P}$ the plane 
parametrizing strict transforms of plane quartic curves that contain
$R$ ($H$ denotes the pull back to $P$ of a general line of
$P_0$). 

Then the limit of the limit linear system $\mathfrak L$ of $|\O_{S_t}(1)|$ as $t$ tends to
$0$ is obtained by glueing $\tilde{\mathcal{H}}_{\P^3}$ and
$\mathcal{H}_{P}$ along  $D_{P_0}$ and $D_R$.
\end{proposition}

\begin{figure}
\begin{center}
\includegraphics[height=3cm]{hilbT+P.eps}
\end{center}
\caption{Limit hyperplane linear system for a degeneration into a
  cubic and plane}
\label{fig:hilbT+P}
\end{figure}


\begin{proof}
One has $\dim (|4H-\sum_{i=1}^{12}E_i|)=3$ (see Example \ref {ex:pi3} and Remark \ref {rem:mon} below). 

There is only one non--trivial  twist of the polarising hyperplane bundle $\L$, i.e., the twist by $P$, which is centrally effective.  As we saw in Example \ref {ex:pi3}, the twist $\L(-P)$ is trivial on $T$, whereas on $P$ it restricts to $\O_P(H+R)=\O_P(4H-\sum_{i=1}^{12}E_i)$. 

Up to a multiplicative constant, there is only one non--zero section of $\L_{|T+P}$ vanishing on
$P$, hence it gives no element in $\mathfrak L$. To see the corresponding curves in $\mathfrak L$ we have to blow up  $|\L_{|T+P}|=|\O_{\P^ 3}(1)|$ at $P_0$.
One has
$$T_{\check{\P}^3,[P_0]} = H^0(\P^ 3, \O_{\P^3}(1))/H^0(\P^ 3, \O_{\P^3})
\cong H^0(\P^ 3,\O_{P_0}(1)).$$
This says that $D_{P_0} \cong \P(T_{\check{\P}^3,[P_0]})$ identifies
with the 2-dimensional linear system $|\O_{P_0}(1)|$. To give a geometric interpretation of this, let us look at the limits of the curves cut out on $T+P_0$ by a plane  $\Pi$ of $\P^3$
tending to $P_0$. The limit curve $\Pi\cap T$ tends to $R$, while
the limit curve of $\Pi \cap P_0$ is a line moving freely in
$|\O_{P_0}(1)|$. 


On the other hand, the plane $D_R$ is 
$$|4H-R| \cong |\O_P(H)| \subset |4H -
\textstyle{\sum_{i=1}^{12}}E_i|.$$ 
There is therefore a natural identification between $D_{P_0}$ and
$D_R$, with the glueing as in the statement.\end{proof}


\begin{remark}\label{rem:mon} As mentioned in Example \ref {ex:pi3}, 
the surface $P$ is mapped to a quartic with a triple point in $\P^3$
by the linear system $|4H-\sum_{i=1}^{12}E_i|$.
This mapping is an isomorphism outside $R$, and contracts $R$
to the triple point. 

Indeed, one has an exact sequence
\[
0\to \O_{P}(H)\to \O_{P}(4H-\sum_{i=1}^{12}E_i)\to \O_R\to 0.
\]
Since $h^ 1(P,\O_{P}(H))=h^1(\P^ 2, \O_{\P^2}(1))=0$, the sequence is exact on global sections, which implies  $h^ 0(P, \O_{P}(4H-\sum_{i=1}^{12}E_i))=4$.

 The linear system $|4H-\sum_{i=1}^{12}E_i|$ has no base points and the morphism determined by it is birational onto its image (we leave this to the reader to check).
The image of $P$ via this map has degree 4, since
$(4H-\sum_{i=1}^{12}E_i)^2=4$. The map contracts $R\equiv 3H-\sum_{i=1}^{12}E_i$ because
$(4H-\sum_{i=1}^{12}E_i)\cdot (3H-\sum_{i=1}^{12}E_i)=0$, and its
image is a triple point because $R^2=(3H-\sum_{i=1}^{12}E_i)^2=-3$.
\end{remark}

\subsubsection{Curves in the hyperplane bundle}
According to the structure of the limit linear system $\mathfrak L$,  one has to compute the limit of trinodal curves appearing in both 
$\tilde{\mathcal{H}}_{\P^3}$ and in $\mathcal H_P$. First we perform the computation for $\tilde{\mathcal{H}}_{\P^3}$. 

Here one has to consider 
the various cases for ${V}(0,\bdelta,I, \ubtau)$ as in Definition \ref {d:zrr}, with $I\subset \{1,\ldots, 12\}$. Since there cannot be any node on $P$ in this linear system, one has $|\bdelta|=\delta$, the number of nodes on $T$. Then:\\
\begin{inparaenum}
\item [$\bullet$] $0\leqslant \delta \leqslant 3$ and ${\bf \tau}=(\tau_2,\tau_3)$;\\
\item [$\bullet$] $|I|+2\tau_2+3\tau_3\leqslant 3$;\\
\item [$\bullet$] $\delta+|I|+\tau_2+2\tau_3=3$.\end{inparaenum}

Hence the cases to be discussed are the following.

\begin{catalogo}

\caseitem{$\delta=3$}

Tritangent planes to the general cubic surface $T$ correspond to the triangles
contained in $T$. These are 45: the reader may apply Salmon's formula  \eqref {eq:salmon} or, better, directly compute this number as an exercise.

\caseitem{$\delta=2$, $|I|=1$}

Binodal hyperplane sections of $T$ must contain a line. Since $T$ contains 27 lines, there
are 27 pencils of such curves. In each of these pencils, and for
every $r\in \{1,\ldots,12\}$, there is exactly one curve passing in addition through the
point $x_r$. This gives a contribution of $27 \times 12
= 324$ to the computation. 

\caseitem{$\delta=2$, $\tau_2=1$}

Each
of the 27 pencils of bitangent planes to $T$
 cuts out a $g^1_2$ on $R$, off the fixed intersection of the line with $R$.

A $g^1_2$ on an elliptic curve possesses 4 ramification points. Each of this contributes to the computation, with multiplicity 2, hence the total contribution is  $27\times 4
\times 2= 216$.  

\caseitem{$\delta=1$, $|I|=2$}

For any pair of distinct indices $r$ and $s$ in $\{1,\ldots,12\}$, the pencil of
planes passing through $x_r$ and $x_s$ contains $12 = \deg (\check{T})$
tangent planes to $T$. The contribution is then $\binom{12}{2} \times 12 = 792$. 

\caseitem{$\delta=1$, $|I|=1$, $\tau_2=1$}

For each $r=1,\ldots,12$,  consider the projection $\pi_r$ from the
point $x_r$. It gives a double cover $\tilde{T} \to \P^2$ branched
along a plane quartic curve $B$, where $\tilde{T}$ is the blow up of
$T$ at $x_r$
(the curve $B$ is the projection from $x_r$ of the curve
$T \cap \mathrm D ^{x_r} T$, which has degree $6$ and multiplicity $2$
at $x_r$, see \cite[Section \tref{s:double-curves}]{13.th-classic};
by $\mathrm D ^{x_r} T$ we denote the first polar of
$T$ with respect to the point $x_r$).
Being contained in the plane $P_0$, which passes through $x_r$, $R$ is mapped 2-1
to a line $\ell_R \subset \P^2$, which  is
nowhere tangent to $B$.

Tangent planes to $T$ containing $x_r$ in $\P^3$ map via $\pi_r$ to
tangent lines to $B$. 
Tangent planes to $R$ containing $x_r$
map to lines passing through one of the 4 points of $\ell_R
\cap B$.

Let $p$ be a point in $\ell_R \cap B$. The pencil of lines through
$p$ in $\P^2$ contains $12 = \deg (\check{B})$ tangent lines to $B$. 
Among them there is the tangent line to $B$ at $q$, with multiplicity 2 (this can be seen as 
in  Lemma \ref{l:tangency}), which corresponds to a plane tangent to
$T$ at a point lying on $R$ in $\P^3$. Such a plane gives a section of
$T+P$ with a singularity worse than a tacnode, so it has to be
discarded from computation. 

Finally, the contribution in this case is $12 \times 4
\times 2\times 10 = 960$.

\caseitem{$\delta=1$, $\tau_3=1$}

The plane cubic $R$ possesses 9 flexes. For each of them, there is the 
pencil of planes containing the
tangent line to $R$ at that flex.
Such a pencil is  a line in $\check{\P}^3$, meeting
$\check{T}$ at 12 points. One needs to remove from these 12 points the
one corresponding to the tangent plane to $T$ at the flex of $R$. It
is of multiplicity 3 (the proof of this fact is similar to the one of Lemma \ref{l:tangency} and we leave it to the reader).

Planes satisfying the given conditions have to be counted with
multiplicity 3. So we get a contribution of $3 \times 9 \times 9 =
243$.

\end{catalogo}

The table below shows the result of the total summation. 


\begin{center}
\begin{tabular}{|l|r|}
\hline
$\text{Cases}$ & \text{Contribution} \\
\hline
$\text{Case 1}$ & 45 \\
\hline
$\text{Case 2}$ & 324 \\
\hline
$\text{Case 3}$ & 216 \\
\hline
$\text{Case 4}$ & 792 \\
\hline
$\text{Case 5}$ & 960 \\
\hline
$\text{Case 6}$ & 243 \\
\hline \hline
\textbf{Total} & $\mathbf{2580}$ \\
\hline
\end{tabular}
\end{center}

\subsubsection{Curves in the twisted hyperplane bundle: plane quartics} 
\label{s:ciro-3nodal-4ics}
% Now we compute
% the limit of trinodal curves appearing in 
% $\mathcal H_P$.
Since Salmon's formula \eqref {eq:salmon} gives a total of 3200 tritangent planes to a general quartic, we are missing a total of $3200-2580=620$ limit trinodal curves. These have to be seen in $\mathcal H_P= |4H-\sum_{i=1}^{12}E_i|$. This system however contains the 2--dimensional system $D_R$ of trinodal curves, which is the plane along which $\mathcal H_P$ and $\tilde{\mathcal{H}}_{\P^3}$ glue. So these curves do not contribute to the computation. Hence, we have to compute the number of trinodal curves in $|4H-\sum_{i=1}^{12}E_i|$ off $D_R$.
All such curves will be irreducible, since, by the genericity assumptions, the only reducible curves in  $|4H-\sum_{i=1}^{12}E_i|$ are the ones in $D_R$ (the reader is invited to prove this).

The linear system $|4H-\sum_{i=1}^{12}E_i|$
is mapped to the plane $P_0$ to $|\O_{\P^2}(4)\otimes \mathcal{I}_D|$, where  $D=\{x_1,\ldots,x_{12}\}$ and $x_1+\cdots+x_{12}\in |\O_R(4)|$ is a general divisor. 
The varieties of $\delta$-nodal curves not containing $R$ 
in this linear system are
logarithmic Severi varieties of the pair $(\P^2,R)$:
on logarithmic Severi varieties, see \cite{03.th-acz}, and in
particular \cite[Section \tref{s:logK3}]{03.th-acz} about the
particular kind we are considering right now.

Since $\dim(|\O_{\P^2}(4)|)=14$, $D$ imposes only 11 conditions to $|\O_{\P^2}(4)|$. Since passing through a point imposes at most one condition, there is a set $Y$ of 11 points in $D$ that  imposes the 11 conditions (in fact, by genericity
of $x_1+\cdots+x_{12}\in |\O_R(4)|$, any subset of 11 points does). Hence 
\[
|\O_{\P^2}(4)\otimes \mathcal{I}_D|=|\O_{\P^2}(4)\otimes \mathcal{I}_{Y}|.
\]
Finally, $Y$ can be seen as the limit of $|\O_{\P^2}(4)\otimes \mathcal{I}_{Z}|$, where $Z$ is a general set of $11$ points in the plane.

We will compute the number of trinodal curves in 
$|\O_{\P^2}(4)\otimes \mathcal{I}_{Z}|$. Their limits, when $Z$ tends to $Y$, will be trinodal curves in $|\O_{\P^2}(4)\otimes \mathcal{I}_{Y}|=|\O_{\P^2}(4)\otimes \mathcal{I}_D|$, and this  gives the required information on the number we want to compute.

Finally what we have to compute is the number of trinodal quartics passing through 11 general points in the plane, which is the degree of the codimension 3 family of trinodal curves in $|\O_{\P^2}(4)|\cong \P^ {14}$, i.e., this is the degree of the appropriate Severi variety. This has been done, in general, by Caporaso and Harris in \cite {caporaso-harris, caporaso-harris2}. Their result in this case reads as follows:

\begin{proposition}\label{prop:ch} If $Z$ is a general set of 11 points in $\P^ 2$, then the $3$--dimensional linear system $|\O_{\P^2}(4)\otimes \mathcal{I}_{Z}|$ contains 675 trinodal curves:\\
\begin{inparaenum}
\item [(i)] 620 of them are irreducible;\\
\item [(ii)] $55={{11}\choose 2}$ are reducible in a line joining 2 of the points of $Z$ and the cubic through the remaining 9 points of $Z$.
\end{inparaenum}
\end{proposition}

When $Z$ tends to $Y$ as above, the 55 reducible quartics as in (ii)
of Proposition \ref {prop:ch} tend to curves in $D_R$, which ought to
be discarded. The limit of the 620 curve in (i) is  the missing contribution we need. 

It would be however unsatisfactory at this point to rely on (the quite difficult) general Caporaso--Harris' result to finish the computation. And in fact we can perform it \emph{our way}, by using a new degeneration. 
%It would be desirable to have another proof of Caporaso--Harris' theorem along the lines of the computation we am going to sketch now.

The degeneration we want to use is the following. Consider the blow up $\cS$ of 
$\mathbb D\times \P^ 2$ along a general line $E$ of $\P^ 2$ in the \emph{central fibre} over $0\in \mathbb D$. Then there is a morphism $f: \cS\to \mathbb D$ which is a semistable degeneration of $S_t=\P^ 2$ for $t\neq 0$ to $S_0=P\cup  F$, with $P\cong \P ^ 2$ the proper transform of the original central fibre and $F$ the exceptional divisor of the blow up  (see Figure \ref {fig:1x}). 

\begin{figure}[ht]
\centering
\includegraphics[scale=.85]{degen-plane.eps}
\caption{the degeneration of the plane}\label{fig:1x}
\end{figure}

Note that $F\cong \mathbf F_1$, i.e., the plane blown up at a point $p$, and $P\cap F=E$, with $E^ 2=-1$ on $F$ (i.e., the exceptional divisor corresponding to $p$), according to the Triple Point Formula in Lemma \ref {l:triple-point}. 

There is  an obvious polarizing bundle $\L$ on $\cS$, which restrict to $\O_{\P^ 2}(1)$ on the general fibre and to $L_0$ on the central fibre, with the aspects
\[
\L_{P}=\O_{\P^ 2}(1),\quad \L_{F}=\O_{F}(f),
\]
where $f$ is a fibre of the morphism $\pi: F\cong \mathbf F_1\to \P^ 1$.

Now pick a set $A=\{\alpha_1,\ldots, \alpha_6\}$ of six general points  on $P$ and 
a set $B=\{\beta_1,\ldots, \beta_5\}$ of five general points on $F$. Then  $Z_0:=A\cup B$ is the limit of a set $Z_t$ of 11 general points on the general fibre $S_t$. Denote by $\cZ$ the curve $\{Z_t\}_{t\in \mathbb D}$ in $\cS$. Consider $\L^{\otimes 4}\otimes {\mathcal I}_{\cZ|\cS}$, which restricts to $\O_{\P^2}(4)\otimes \mathcal{I}_{Z_t}$ on the general fibre $S_t$.  In order to have information about trinodal curves in $|\O_{\P^2}(4)\otimes \mathcal{I}_{Z_t}|$, we have to look at their limits in the limit linear system $\mathfrak L$ of $\L^{\otimes 4}\otimes {\mathcal I}_{\cZ|\cS}$. 


\begin{lemma}\label{lem:twist}
There is only one twist of $\L^{\otimes 4}\otimes {\mathcal I}_{\cZ|\cS}$ which is centrally effective, namely $\L^{\otimes 4}\otimes \O_S(-F)\otimes {\mathcal I}_{\cZ|\cS}$.
\end{lemma}
\begin{proof} Any twist is of the form
$\L^{\otimes 4}\otimes \O_S(-aF)\otimes {\mathcal I}_{\cZ|\cS}$ and on $S_0$ this resticts to:\\
\begin{inparaenum}
\item [(i)] $\O_{\P^ 2}(4-a)\otimes \mathcal{I}_{A}$ on $P\cong \P^ 2$;\\
\item [(ii)] $\O_{\mathbf F_1}(4f+aE)\otimes \mathcal{I}_{B}$ on $F\cong \mathbf F_1$.
As $\mathbf F_1$ is the blow up of $\P^ 2$ at $p$, then (with a slight abuse of notation) one has $|\O_{\mathbf F_1}(4f+aE)\otimes \mathcal{I}_{B}|\cong |\O_{\P^ 2}(4)\otimes \mathcal{I}_{B}\otimes \mathcal{I}_{p}^ {\otimes 4-a}|$.
\end{inparaenum}

Since $B$ is a general set of 5 points on $F$, for the effectivity on $F$ one needs $a\geqslant 1$, because $\dim(|\O_{\mathbf F_1}(4f)|)=4$. Similarly, for the effectivity on $P$ we need $a\leqslant 1$, because  $|\O_{\P^ 2}(h)\otimes \mathcal{I}_{A}|$ is empty for $h\leqslant 2$. This proves the assertion.\end{proof}

In conclusion, we have to look at limits of trinodal curves only in  
$|\L^{\otimes 4}\otimes \O_\cS(-F)\otimes {\mathcal I}_{\cZ|\cS}\otimes \O_{S_0}|$, which is:\\
\begin{inparaenum}
\item [(i)] $\L_P:=|\O_{\P^ 2}(3)\otimes \mathcal{I}_{A}|$, the aspect on $P$, of dimension $3$;\\
\item [(ii)] $\L_F:=|\O_{\mathbf F_1}(4f+E)\otimes \mathcal{I}_{B}|$, the aspect on $F$, which is the same as
$|\O_{\P^ 2}(4)\otimes \mathcal{I}_{p}^ {\otimes 3}\otimes
\mathcal{I}_{B}|$ in the identification of $F$ with the blow-up of
$\P^2$ at a point $p$, also of dimension 3;\\
\item [(iii)] the two curves on $P$ and $F$ in the two aspects have to 
\emph{match} along $E$, i.e., they have to cut out on $E$ the same divisor. This \emph{matching condition} implies dimension 3 for 
$|\L^{\otimes 4}\otimes \O_\cS(-F)\otimes {\mathcal I}_{\cZ|\cS}\otimes \O_{S_0}|$: indeed, given a curve in $|\O_{\P^ 2}(3)\otimes \mathcal{I}_{A}|$, which depends on 3 parameters, this fixes the degree 3 divisor it cuts on $E$ and there is only one curve in 
$|\O_{\mathbf F_1}(4f-E)\otimes \mathcal{I}_{B}|$ matching it. 
\end{inparaenum}

Next we introduce the self-explanatory notation $\bdelta=(\delta_P,\delta_F)$ and ${\bf \tau}=(\tau_2,\tau_3)$ (in this case there is no $I$ to be considered) and 
$$|\bdelta|+\tau_2+2\tau_3=3.$$ 

It is useful to notice that a curve in $|\O_{\mathbf F_1}(4f+E)|\otimes \mathcal{I}_{B}$ with a node at a point $x\in F$, splits in the unique element $f_x$ of $|f|$ through $x$, and in a curve of $|\O_{\mathbf F_1}(3f+E)\otimes \mathcal{I}_{B}|$ (which is the same as
$|\O_{\P^ 2}(3)\otimes \mathcal{I}_{B}\otimes \mathcal{I}_{p}^ {\otimes 2}|$) passing through $x$. 

Now the cases to be analyzed are the following. We will be sketchy, leaving the details to the reader. 
The corresponding analysis for the simpler enumeration of $2$-nodal
plane quartics is carried out in \cite[Section
\tref{S:ourway}]{08.th-exem}. 
\begin{catalogo}
\caseitem{$\delta_F=3$}

A trinodal curve on $F$ contains three curves in $|f|$
with residual in 
$|\O_{\mathbf F_1}(f+E)|$, which is the same as
$|\O_{\P^ 2}(1)|$ (with the curves in $|f|$ mapping to lines through $p$). This implies that  the three splitting curves in $|f|$ have to contain three points of $B$, and the residual in $|\O_{\mathbf F_1}(f+E)|$ contains the remaining 2. This fixes the curve on $F$ and accordingly also the curve on $P$. This shows that the contribution in this case is ${{5}\choose 2}=10$.

\caseitem{$\delta_F=2, \delta_P=1$}

Two curves in $|f|$ split from the curve on $F$ and either only one or exactly two points of $B$ lie on splitting elements of  $|f|$. If two points $\beta_1,\beta_2$ of $B$ lie on splitting elements of  $|f|$, these curves cut $E$ each in one point $b_1,b_2$. Then the matching curves on $P$ lie in the pencil of cubics $|\O_{\P^ 2}(3)\otimes \mathcal I_{A\cup \{b_1,b_2\}}|$ which, as well known, contains exactly 12 nodal curves (the reader may be asked to verify this as an exercise). Each such curve cuts a divisor on $E$ (which contains $b_1+b_2$), and the matching uniquely determines the remaining component of the curve on $F$, which lies in the  pencil 
$|\O_{\mathbf F_1}(2f+E)\otimes \mathcal{I}_{B-\{\beta_1,\beta_2\}}|=
|\O_{\P^ 2}(2)\otimes \mathcal{I}_{B-\{\beta_1,\beta_2\}\cup \{p\}}|$. This gives a contribution of ${{5}\choose 2}\times 12=120$ to our computation.

The reader may check, with similar arguments, that if only one point of $B$ lies on a splitting element of  $|f|$ (and there are 5 possibilities for this), then one also has a well determined pencil of curves on $P$ with 12 nodal curves, hence we have $5\times 12=60$ more limit trinodal curves of this type, for a total of $180$.

\caseitem{$\delta_F=2, |{\bf \tau}|\neq 0$}

Since, as above, two curves in $|f|$ split from the curve on $F$, it is not possible to have a tangency to $E$, so this case gives no contribution to the computation.

\caseitem{$\delta_F=1, \delta_P=2$} 

Only one curve in $|f|$ splits from the curve on $F$, and there are two possible cases:\\
\begin {inparaenum}
\item [(a)] this curve does not contain any point of $B$;\\
\item [(b)] this curve contains one point of $B$ (this depends on 5 choices).
\end{inparaenum}

Also the curve on $P$ is reducible in a conic and a line, and there are two possible cases:\\
\begin {inparaenum}
\item [(a')] 5 of the points in $A$ lie on the conic, and one lies on the line (this depends of 6 choices);\\
\item [(b')] 4 of the points in $A$ lie on the conic, and two lie on the line (this depends of 15 choices).
\end{inparaenum} 

One has that:\\
\begin{inparaenum}
\item [Case (a,a')]  contributes with 12 curves,\\
\item [Case (a,b')]  contributes with 30 curves,\\
\item [Case (b,a')]  contributes with 30 curves,\\
\item [Case (b,b')]  contributes with 75 curves,
\end{inparaenum}
for a total contribution of $147$.\\
Let us check case (b,b'), and leave the others to the reader.
Each of the $15$ choices of $2$ points in $A$ determines a unique line,
and then the residual conic through the $4$ remaining points moves
in a pencil.
Each choice of one point in $B$ determines a unique curve in $|f|$,
and then the residual curve in $|3f+E|$ through the $4$ remaining
points moves in a $2$-dimensional linear system.
Finally, the residual conic on $P$ 
is determined by its matching with the fixed curve in $|f|$ on $F$,
and then the residual curve in $|3f+E|$ on $F$ is fixed with its
matching with the conic on $P$ at its remaining point of intersection with
$E$ and with the fixed line on $P$.
Hence the contribution is of $5\times 15=75$.


\caseitem{$\delta_F=1, \delta_P=1, \tau_2=1$} 

Again one has the two alternatives (a) and (b) as  in Case 4. Case (a) contributes with 40 curves, case (b) with 160. Let us check case (b), and leave case (a) to the reader.

Once the splitting curve of $|f|$ has been fixed (which depends on 5
choices, i.e., the choice of the point in $B$), it intersects $E$ at a
point $q$. The matching condition on $P$ gives the net of cubics
through $A$ and $q$. This net maps $P$ to $\P^ 2$ as a double cover,
branched along a quartic $D$ which, by genericity, is smooth. The
curve $E$ is mapped to a conic $C$. We have to count the number of
lines tangent to both, $D$ and $C$, which is the intersection number
24 of $\check C$ (a conic) and $\check D$ (a curve of degree 12),
minus the number of points where $D$ and $C$ are tangent to each other
(which is 4, the number of branch points of the double cover $E\to
C$), counted with multiplicity 2 (this is similar to Lemma \ref
{l:tangency}). Since each of these curves contributes with
multiplicity 2  to the total,  we have a total of $2\times 5\times
16=160$. 


\caseitem{$\delta_P=1, \tau_3=1$} 

%This is the most complicated number to be checked in this computation. 

Each of the curves in question counts with multiplicity 3. 
The linear system  $\L_P$ maps $P$ to a smooth cubic surface $\Phi$ in $\P^ 3$, and $E$ is mapped to a rational normal cubic $\Gamma\subset \Phi$. Consider the duals:\\
\begin{inparaenum}
\item [$\bullet$] $\check \Phi$, which is a surface of degree 12;\\
\item  [$\bullet$] $\check \Gamma$, which is a scroll of degree 4, with a cuspidal curve $\Gamma^ *$ of degree 3, which  is the rational normal cubic of $\check \P^ 3$ described by all osculating planes to $\Gamma$ in $\P^ 3$
(see \cite{13.th-classic}).
\end{inparaenum}


The surface $\check \Gamma$ is the projection of a smooth rational normal scroll $\Sigma$ of degree 4 in $\P^ 5$, and we denote by $H$ the hyperplane class in this embedding and $|\mathfrak f|$ the pencil of lines on $\Sigma$. One has $H^2=4, \mathfrak f^2=0, H\cdot \mathfrak f=1$. \footnote{One has that $\Sigma\cong \mathbb F_0$ embedded in $\P^ 5$ via the morphism determined by the linear system $|H|$ of curves of type $(2,1)$. Indeed it cannot be 
$\Sigma\cong \mathbb F_2$ because otherwise there would be a pencil of tangent planes to $\Gamma$ along moving points, which is not possible.}

The strict transform of   
$\Gamma^ *$ on $\Sigma$ is clearly unisecant with the curves in $|\mathfrak f|$ and therefore  $\Gamma^ *\equiv H-\mathfrak f$. 


The curve $\Gamma'$ described by the tangent planes to $\Phi$ at the points of $\Gamma$ sits in $\check \Phi\cap \check \Gamma$. It is a rational curve of degree 6 (to see this, intersect $\Gamma$ with a general polar quadric of $S'$), 
meeting the curves of $|\mathfrak f|$ in 1 point. Hence on $\Sigma$ one has $\Gamma'\equiv H+2\mathfrak f$, and therefore $\Gamma'\cdot \Gamma^ *=5$. 

We have to compute the intersection number of $\check \Phi$ and $\Gamma^ *$, which is 36, and subtract the number of osculating planes to $\Gamma$ tangent to $\Phi$ at a point of $\Gamma$, which is  $\Gamma'\cdot \Gamma^ *=5$, counted with multiplicity 3 (to see this, imitate the proof of Lemma \ref {l:tangency}). In conclusion we get a contribution of $3\times 21=63$. 

\caseitem{$\delta_P=2, \tau_2=1$}

Each of the curves in question counts with multiplicity 2. 
The curve on $P$ splits, and we have the two alternatives (a') and (b') as in Case 4. However, case (a') gives no contribution to the computation, because in a pencil of lines there is no line tangent to $E$. Each of the situations in  case (b') (which depend on 15 choices, i.e., the pairs of points of the splitting line $\ell$ on $P$) gives rise to 2 curves, corresponding to the conics of  the residual pencil  to $\ell$ tangent to $E$. In conclusion, one has a contribution of $2\times 15\times 2=60$.

\caseitem{$\delta_P=3$}

The curve on $P$ splits in 3 lines, which have to contain the points in $A$. The reader will readily check that their number  is 15.
\end{catalogo}

\smallskip\noindent
The following table shows the result of the total summation of non--trivial contributions. 
\begin{center}
\begin{tabular}{|l|r|}
\hline
$\text{Cases}$ & \text{Contribution} \\
\hline
$\text{Case 1}$ & 10 \\
\hline
$\text{Case 2}$ & 180 \\
\hline
$\text{Case 4}$ & 147 \\
\hline
$\text{Case 5}$ & 200 \\
\hline
$\text{Case 6}$ & 63 \\
\hline
$\text{Case 7}$ & 60 \\
\hline
$\text{Case 8}$ & 15 \\
\hline \hline
\textbf{Total} & $\mathbf{675}$ \\
\hline
\end{tabular}
\end{center}

From this total we have to subtract the limit of reducible quartic
curves passing through 11 general points of the plane. Their number is
$55={{11}\choose 2}$, since they are the ones appearing in (ii) of
Proposition \ref {prop:ch}. We leave it to the reader to check that the limits of these 55 curves are the ones in Case 1 and Case 4 (b,a') and (a,b').

\begin{remark}
In conclusion, also the degeneration to a cubic plus a plane is $1$--good. However the reader will have noticed that, both in this case and in the previous one, we do not have an a priori proof of this (as in the intentions of Conjecture \ref {conj:goodness}), but the proof relies on Salmon's formula \eqref {eq:salmon}, rather than proving it. 
\end{remark}


\section{A non-good case}
\label{S:planes}

\subsection{Degeneration of cubics to three planes}\label{ssec:bad}

Consider a degeneration as in Example \ref {ex:pi3}, where $d=3$, with
$S_0$ consisting of the union of three distinct planes $P_0,P_1,
P_2$. Let us denote by $\ell_{i}$ the intersection line of $P_i$ and
$P_{i+1}$ (for $i=0,1,2$; the indices will now be considered to vary
in $\mathbb Z/3\mathbb Z$),
and by $p$ the intersection point of $P_0,P_1, P_2$.
The central fibre of the corresponding semistable degeneration
constructed in Example \ref{ex:pi3}
is $\tilde S_0=Q_0\cup Q_1\cup Q_2$ as in Figure \ref {fig:1y}, and we may assume that each of the surfaces $Q_i$ is the blow up of $P_i$ at three points along $\ell_{i}$. 

\begin{figure}[ht]
\setlength{\unitlength}{0.5mm}
\centering
\begin{picture}(20,64)(0,22)
\put(15,80){\line(1,-1){40}}
\put(15,60){\line(1,0){5}}
\put(15,58){\line(1,0){5}}
\put(15,56){\line(1,0){5}}
\put(-5,60){\line(1,0){5}}
\put(-7,58){\line(1,0){5}}
\put(-9,56){\line(1,0){5}}
\put(30,60){\line(1,0){5}}
\put(32,58){\line(1,0){5}}
\put(34,56){\line(1,0){5}}
\put(15,80){\line(0,-1){50}}
\put(15,80){\line(-1,-1){40}}
\multiput(-20,40)(20,0){4}{\line(1,0){10}}

\put(15,20){$\ell_1$}
\put(60,35){$\ell_2$}
\put(-32,35){$\ell_0$}

\put(14,85){$p$}

\put(15,50){$\,\,\,\,\,Q_2$}
\put(30,30){$\,\,\,\,\,Q_1$}
\put(-15,30){$Q_0$}
\end{picture}
\caption{the degeneration of a cubic to the union of three planes}\label{fig:1y}
\end{figure}


If we look at limits of nodal curves in the polarising hyperplane
bundle, according to Proposition \ref {p:zrr} we have to consider only
planes passing by one  of the aforementioned blown up points. This
gives a contribution of 9 to the degree of the dual of a general cubic
surface in $\P^ 3$, whereas we know that this degree is 12. So we are
missing something of degree 3, which shows that this degeneration is
not  1--good. In what follows we will construct a 1--good model, which
will show that the degeneration under consideration is $1$--well behaved. 

\begin{remark}  This degeneration is however 3--good. To see this, notice that the limit of the 27 lines on a general cubic can be seen here as the lines different from the $\ell_{i}$'s joining pairs of blown up points. Hence we see all triangles formed by these lines, which are 45, so we see also the limit of all 3--nodal planes sections of a general cubic surface.

For the same reason this degeneration is also 2--good. \end{remark}

The obvious guess is that the limit of the dual of the general cubic
consists of the 9 aforementioned planes in $\check \P^ 3$ plus the
plane $p^ \perp$ counted with multiplicity 3, i.e., \emph{there is
  something of degree 3 hidden at $p$}. This is indeed the case and to
see it, one has to look at another model of the degeneration. This is
explained in detail in \cite {CD} in the more complicated situation of
a general quartic degenerating to a tetrahedron
(\ie the union of four linearly independent planes in $\P^3$).
Let us now see how this 1--good model is gotten in the present case.


\paragraph{Construction of a good model}
\label{p:construction}
Let 
$\bar{f}:\bar{S} \to \D$
be the family obtained from $\tilde{f}:\tilde{S} \to \D$
(notation as in Example \ref{ex:pi3})
by the
base change $t\in\D \mapsto t^3\in\D$. The  central fibre
$\bar S_0$ is isomorphic to $\tilde S_0$, so we will keep the above
notation for it.

Analytically locally around $p$,
the total space $\bar{S}$ is
isomorphic to the hypersurface of $\mathbf C^ 4$ defined by the
equation $ xyz = t^3$ at the origin.
Blow-up $\bar{S}$ at $p$. The blown--up total space locally sits in
$\bf C^ 4\times \P ^ 3$. 
Let $[\xi:\eta:\zeta:\vartheta]$ be the homogeneous coordinates in
$\bf P^ 3$. Then the new total space is locally defined in $\bf C^
4\times \P ^ 3$ by the equations
\begin{equation}
\label{eq1-3piani}
\rk
\begin{pmatrix}
  x & y & z & t \\
  \xi & \eta & \zeta & \vartheta
\end{pmatrix}
\leq 1
\Et
\xi\eta\zeta=\vartheta^3.
\end{equation}
Denote the exceptional divisor by $T$;
it is isomorphic
to the cubic surface with equation $\xi\eta\zeta=\vartheta^3$ 
in the $\P^3$ with coordinates $[\xi:\eta:\zeta:\vartheta]$.
This cubic contains three lines, along which it intersects the proper
transforms $\tilde{Q}_0,\tilde{Q}_1,\tilde{Q}_2$ of $Q_0,Q_1,Q_2$
respectively; 
thus, each line on $T$ identifies with the exceptional $(-1)$-curve
on one of $\tilde{Q}_0,\tilde{Q}_1,\tilde{Q}_2$. 
% We will denote these exceptional $(-1)$-curve by $E_0,E_1,E_2$
% respectively.
The cubic $T$ has three $A_2$ double points, located at
the intersections of $T$ with the proper transforms
$\tilde\ell_0,\tilde\ell_1,\tilde\ell_2$ of
$\ell_0,\ell_1,\ell_2$ respectively.
See Remark \ref{rk:cubicT} below for more about this cubic.
The new central fibre is shown in Figure \ref {fig:1z}.

\begin{figure}[ht]
\centering
\setlength{\unitlength}{0.5mm}
\begin{picture}(30,75)(00,18)

\put(30,80){\line(1,-1){40}}
\put(15,65){\line(0,-1){50}}
\put(0,80){\line(-1,-1){40}}
\multiput(0,80)(9,0){4}{\line(1,0){3}}
\put(0,80){\line(1,-1){15}}
\put(15,65){\line(1,1){15}}

% \put(15,65){\line(0,1){30}} %p_1 p'
% \put(30,80){\line(-1,1){15}} %p' p_2
% \put(0,80){\line(1,1){15}} % p_0 p'
\put(15,80){\oval(30,30)[t]}
\multiput(-30,40)(20,0){5}{\line(1,0){10}}

%\put(15,100){$p'$}
\put(-15,25){$\tilde Q_0$}
\put(35,25){$\tilde Q_1$}
\put(25,55){$\tilde Q_2$}

% \put(-15,90){$\,\,\,\,\, A_0$}
%put(-05,90){$T$}
\put(13,85){$T$}
% \put(20,90){$\,\,\,\,\,A_1$}
% \put(10,82){$\,\,\,\,\,A_3$}

% \put(-23,78){$\,\,\,\,\, p_0$}
% \put(10,60){$\,\,\,\,\,p_1$}
% \put(30,78){$\,\,\,\,\,p_2$}


\put(18,15){$\tilde\ell_1$}
\put(70,35){$\tilde\ell_2$}
\put(-45,35){$\tilde\ell_0$}

\end{picture}
\caption{the central fibre after base change and blow--up of the
  vertex $p$}\label{fig:1z}
\end{figure}

The model we have arrived at at this point is good enough to see all
limits of 
$1$-nodal curves, but it is not yet a good model because it is not
semistable. Indeed, the total space is singular along the proper
transforms $\tilde\ell_0,\tilde\ell_1,\tilde\ell_2$ of
$\ell_0,\ell_1,\ell_2$: analytically locally around the general point
of one of these curves, it is isomorphic to a neighbourhood of the
origin in the hypersurface defined by $xy = t^3$ in $\C^4$;
thus, the total space is locally the product of an $A_2$ surface
singularity with a smooth curve.

To resolve these singularities, we blow up along the three (disjoint)
curves $\tilde\ell_0,\tilde\ell_1,\tilde\ell_2$. This has the effect
of replacing each of these curves by a chain of two ruled surfaces;
correspondingly, all three $A_2$ double points of $T$ are resolved,
each being replaced by a chain of two $(-2)$-curves. Thus, $T$ is
replaced by its minimal resolution, which we will denote by
$\tilde T$. The three surfaces $\tilde{Q}_0,\tilde{Q}_1,\tilde{Q}_2$,
on the other hand, remain unchanged, and we will denote their proper
transforms by the same symbols.

The new central fibre is shown in Figure \ref {fig:2z}.
We leave to the reader the verification of the self-intersections of
the double curves of the central fibre indicated on the figure, as an
exercise in the triple point formula. With our choice of distribution
of the $(-1)$-curves in the small resolution at the beginning, the
chains of rational ruled surfaces are made of an $\F_1$ and an $\F_2$
surface, as indicated on the figure.

\begin{figure}
\centering
\includegraphics{3piani.eps}
\caption{the central fibre of the good model (seen from above)}
\label{fig:2z}
\end{figure}



\begin{remark}
\label{rk:cubicT}
\def\ell{L}
The cubic surface $T$ is the image of the plane 
via the linear system $\mathcal C$ of cubic curves with two base
points $x_1,x_2$,
and infinitely near base points such that the cubics $C\in \mathcal C$ 
have two common flexes along lines $\ell_1$ and $\ell_2$.
One has to blow up
the plane at $x_1$ and $x_2$ three consecutive times to make the
proper transform $\tilde {\mathcal C}$ of ${\mathcal C}$ base point
free. This is shown in Figure \ref {fig:1s}, where we denote by
$\tilde C$ the proper transform of the general curve $C\in \mathcal
C$, by $\tilde \ell_i$ the proper transforms of the lines $\ell_i$,
for $i=1,2$, and by $E_{ij}$, for $i=1,2$, $j=1,2,3$, the exceptional
curves of the blow--ups, and one has $E_{i3}^2=-1$ for $i=1,2$ and
$E_{ij}^2=-2$, for $i,j=1,2$. \footnote{In \cite {CD} we gave a different plane linear system of cubics representing  the same surface $T$. It is the linear system of cubics that pass through three independent points $y_1,y_2,y_3$ in the plane and are tangent there to the lines $\langle y_i,y_{i+1}\rangle$, with $i=\in \Z/3\Z$. To pass from ${\mathcal C}$ to this linear system, just make a quadratic transformation based at  $x_1$ and $x_2$ and at the point infinitely near to $x_1$ along $\ell_1$.} 


\begin{figure}[ht]
\centering
\setlength{\unitlength}{0.8mm}
\begin{picture}(30,64)(0,15)

\put(15,80){\line(1,-1){40}}
\put(15,80){\line(-1,-1){40}}

\put(-15,50){\line(1,0){15}}
\put(-6,53){\line(0,-1){15}}
\put(-7,40){\line(1,0){12}}

\put(45,50){\line(-1,0){15}}
\put(36,53){\line(0,-1){15}}
\put(37,40){\line(-1,0){12}}

\put(15,53){\oval(50,80)[b]}

\put(15,42){\oval(30,30)[b]}
\put(15,30){$\ell_3$}

% \put(100,50){\line(-1,0){15}}
% \put(36,53){\line(0,-1){15}}
% \put(37,40){\line(-1,0){12}}
% \put(15,53){\oval(50,80)[b]}

\put(60,35){$\ell_2$}
\put(-32,35){$\ell_1$}
\put(15,15){$\tilde C$}
\put(6,37){\footnotesize $E_{11}$}
\put(20,37){\footnotesize $E_{21}$}
\put(2,50){\footnotesize $E_{13}$}
\put(23,50){\footnotesize $E_{23}$}
\put(-8,35){\footnotesize $E_{12}$}
\put(33,35){\footnotesize $E_{22}$}
\end{picture}
\caption{the linear system of curves $\tilde C$}\label{fig:1s}
\end{figure}

The cubic  $T$ has
three $A_2$--double points, at the vertices of the triangle $\vartheta=0$,
$\xi\eta\zeta=0$. They are the images of $\tilde \ell_1+\tilde \ell_2$
and of $E_{i1}+E_{i2}$, for $i=1,2$. The three lines pairwise   joining the $A_2$--double points, lie on $T$ and are easily seen to be the only lines on $T$. They correspond to  the two exceptional divisors 
$E_{13}$ and $E_{23}$ and to the line $\ell_3$ joining $x_1$ and $x_2$. 

The cubic $T$
is \emph{self--dual}, i.e., $\check T$ is projectively equivalent to $T$, hence it has degree 3. This   (heuristically) explains the contribution by 3 to the degree of the dual hidden at $p$. 
\end{remark}


\paragraph{Goodness of the new model}
The degeneration we have just constructed is 1--good. Indeed now there
is a new centrally effective twist,
which corresponds to a degeneration of the cubics $S_t$, $t\in \D
\setminus \0$, to the cubic $T \subset \P^3$.
It provides the missing contribution by 3, as we will now briefly
explain.

Let $\cL$ be the pull-back to the new degeneration of the polarising
hyperplane bundle on the initial degeneration. On the central fibre,
it restricts to the pull-back $H$ of the line class on the surfaces
$\tilde Q_0, \tilde Q_1, \tilde Q_2$, to the trivial class on $\tilde
T$, and to the class of the ruling on the chains of ruled surfaces.
The new relevant twist is $\cL(-\tilde T)$: it restricts to the class
$H-E_i$ on $\tilde Q_i$ for all $i=0,1,2$ (recall the notation from 
\ref{p:construction}), to the pull-back of the hyperplane class of
$T\subset \P^3$ on $\tilde T$, and it is trivial on the chains of
ruled surface; thus, it maps $\tilde T$ to $T$, contracts $\tilde Q_i$
to the line $E_i$ on $T$ for all $i=0,1,2$, and contracts the three
chains of ruled surfaces to the three $A_2$ double points of $T$.

Now, let us fix a general pencil of planes in the $\P^3$ spanned by
$S_0$, and let us count the ``tangent planes to $S_0$'' in this
pencil.
Nine of them are the planes in the pencil passing through each of the special
points on the lines $\ell_i$, $0\leq i\leq 2$. As for the remaining
three, consider the plane in the pencil passing through the triple
point; it cuts out three coplanar lines meeting at the point $p$, the
triple point of $S_0$.
Thus its proper transform determines three points on $T$, one on each line
of $T$, and these three points are collinear.
The planes in the $\P^3$ spanned by $T$ which contain these three
points form a pencil, and in this pencil there are
three planes which are tangent to $T$ in simple points.
This provides us with the remaining three ``tangent
planes to $S_0$''. For further details, see \cite {CD}.


\subsection{Degeneration of quartics to four planes}
\label{ssec:quartiche}

We conclude this text by a brief discussion of degenerations,
as in Example \ref {ex:pi3} and Section \ref{ssec:bad} above,
of smooth
quartics $S_t$ to the union $S_0$ of four planes
$P_0,P_1,P_2,P_3$ in linear general
position, which we call a \emph{tetrahedron}.
This is one of the main topics in \cite{CD}, and many
examples in this volume are inspired by this situation.
An interesting feature is that this is a degeneration of $K3$ surfaces.

There are four different kinds of alternative degenerations of the
$S_t$'s to be considered in order to reveal all limits of $\delta$-nodal
hyperplane sections, $1 \leq \delta \leq 3$. Each corresponds to a
kind of twist in some suitable good model of the initial degeneration.
\begin{compactitem}[---]
\item The contributions of the \emph{faces} of the tetrahedron
  (\ie the planes $P_i$ themselves) are visible in degenerations to
  monoid quartic surfaces, similarly to what we have seen for the
  degeneration to a cubic and a plane in Section \ref{ssec:another}.
\item The contributions of the sections by a hyperplane containing a
  \emph{vertex} (\ie a triple point $P_i\cap P_j \cap P_k$) are
  visible in degenerations to the union of a cubic $T \subset \P^3$ as
  in the previous Section \ref{ssec:bad}
  and the plane spanned by the three lines of $T$; the
  plane corresponds to the face of the tetrahedron opposite to the
  vertex in consideration.
\item The contributions of the sections by a hyperplane containing an
  \emph{edge} (\ie a double line $P_i\cap P_j$) are
  visible in degenerations to a rational quartic surface with a double
  line and two triple points on the latter; the double
  line is the image of the opposite edge, and the two triple points are
  the respective images of the two faces adjacent to the edge.
\end{compactitem}
More can be found on the rational surfaces appearing in these
degenerations in \cite[Section \tref{s:degenK3}]{11.th-toric-trop}.

The construction of a good model follows the same lines as in Section
\ref{ssec:bad}; it is rather complicated in practice, but can be
organized so as to be manageable, see \cite{CD}. Starting from the
degeneration to $S_0=P_0+P_1+P_2+P_3$ as in Example \ref {ex:pi3}, one
performs the base change $t\mapsto t^6$ and then resolve the
singularities. Morally, a degree $3$ base change is needed to unravel
the contributions involving the vertices, as in Section
\ref{ssec:bad}, and a degree $2$ base change is needed for those
involving the edges. The central fibre of this good model is
represented in Figure \ref{fig:granchio}; the reader may also see
\cite[p.~143]{CD} for another picture, with a different design. The
dotted curve represents (in a tropical fashion,
see \cite[Section \tref{s:trop-design}]{11.th-toric-trop})
the pull-back of a hyperplane section of the
initial tetrahedron.

\begin{figure}
\centering
\includegraphics[width=\textwidth]{tetraedro.eps}
\caption{Central fibre of a good model of the degeneration of quartic
  surfaces to a tetrahedron}
\label{fig:granchio}
\end{figure}




\begin{references}


\begin{thebibliography}[Chapters in this Volume]{XIV}

\bibitem[\tref{03.th-acz}]{03.th-acz}
Th.~Dedieu,
\emph{Geometry of logarithmic Severi varieties at a general point}.

\bibitem[\tref{04.concettina}]{04.concettina}
Th.~Dedieu {\normalfont \smfandname} C.~Galati,
\emph{Degenerations and deformations of generalized Severi varieties}.

\bibitem[\tref{08.th-exem}]{08.th-exem}
Th.~Dedieu,
\emph{The Caporaso--Harris recursion within a degeneration of the
  plane}.

\bibitem[\tref{04b.concettina}]{04b.concettina}
C.~Galati,
\emph{Proving the existence of curves  on smooth surfaces
  by smoothing tacnodes on reducible surfaces}.

\bibitem[\tref{11.th-toric-trop}]{11.th-toric-trop}
  Th.~Dedieu,
  \emph{Enumeration of curves in toric surfaces, tropical geometry,
    and floor diagrams}.

\bibitem[\tref{15.tacnodo}]{15.tacnodo}
  C~Ciliberto, Th.~Dedieu, {\normalfont \smfandname} C.~Galati,
  \emph{Flag semi-stable reduction of tacnodal curves at the limit
  of nodal curves}.

\bibitem[\tref{13.th-classic}]{13.th-classic}
Th.~Dedieu,
\emph{Some classical formul{\ae} for curves and surfaces}.

\bibitem[\tref{14.th-vainsencher}]{14.th-vainsencher}
Th.~Dedieu,
\emph{Node polynomials for curves on surfaces}.

\bibitem[\tref{16.th+l-redres}]{16.th+l-redres}
L.~Busé {\normalfont \smfandname} Th.~Dedieu,
\emph{Generalized weight properties of resultants and discriminants,
and applications to projective enumerative geometry}.

\end{thebibliography}


\begin{thebibliography}[External References]{99}

\bibitem {CCFM}
A. Calabri, C. Ciliberto, F. Flamini, R. Miranda:
\emph{On the $K^2$ of degenerations of surfaces
and the multiple point formula}, 
Ann. of Math., {\bf 165} (2007), 335--395.

\bibitem{caporaso-harris}
L. Caporaso, J. Harris:
{\it Counting plane curves of any genus}, 
Invent. Math. {\bf 131} (1998), no.2, 345--392.

\bibitem{caporaso-harris2}
L. Caporaso, J. Harris:
{\it Parameter spaces for curves on surfaces and enumeration of
  rational curves},
Compositio Math. {\bf 113} (1998), no.2, 155--208.

\bibitem {CD} 
C. Ciliberto, Th. Dedieu:
{\it Limits of pluri--tangent planes to quartic surfaces}, in ``Algebraic and Complex Geometry'', Springer Proceedings in Math. \& Statistics, {\bf 71}, 2014, pp. 123--200. 

\bibitem {clm} C.~Ciliberto, A.~F.~Lopez, R.~Miranda: {\it Projective degenerations of $K3$ surfaces, Gaussian maps and Fano threefolds}, Invent. Math. {\bf 114} (1993), 641--667.

\bibitem {Frie} R. Friedman: 
{\it Global smoothings of varieties with normal
crossings}, Ann. of Math. {\bf 118} (1983), 75--114.

\bibitem{concettina1}
C. Galati:
{\it Degenerating curves and surfaces: first results},
Rend. Circ. Mat. Palermo {\bf 58} (2009), no. 2, 211--243.

\bibitem{concettina2} C. Galati, A.L. Knutsen: {\it On the existence of curves with $A_k$--singularities on $K3$ surfaces}, Mathematical Research Letters {\bf 21},  (2014), 1069--1109.

\bibitem{gh-degen}
P. Griffiths, J. Harris:
{\it On the Noether-Lefschetz theorem and some remarks on
  codimension-two cycles},
Math. Ann. {\bf 271} (1985), 31--51.

\bibitem{harris2}
J. Harris:
{\it Algebraic Geometry, A First Course},  Graduate Texts in Math. 133, Springer--Verlag, 
1992. 

\bibitem{harris-morrison}
J. Harris, I. Morrison:
{\it Moduli of Curves}, Graduate Texts in Mathematics 187, 
Springer-Verlag, 1998.

\bibitem {Kempf}
G. Kempf, F. F. Knudsen, D. Mumford,  B. Saint--Donat:
{\it Toroidal embeddings I}, Lecture Notes in Mathematics 339,
Springer--Verlag, Berlin-New York, 1973.

\bibitem {KL} S. Kleiman:
{\it About the conormal scheme}, in  Complete intersections, Springer Berlin Heidelberg, 1984. 161--197.

\bibitem {KP1} S. Kleiman, R. Piene:
{\it  Enumerating singular curves on surfaces}, in: Algebraic Geometry -- Hirzebruch 70, Cont.
Math. {\bf  241} (1999) 209--238 (corrections and revision in math.AG/9903192).

\bibitem {KP2} S. Kleiman, R. Piene:
{\it Node polynomials for families: methods and applications}, Math. Nachr. 271 (2004), 69 -- 90.

\bibitem {K} V. Kulikov:
{\it Degenerations of K3 surfaces and Enriques surfaces}, 
Math. USSR Izvestiya {\bf 11} (1977), 957--989.

\bibitem {PP} U. Persson, H. Pinkham: {\it  Degenerations of surfaces with trivial canonical bundle}, Ann. of Math. {\bf 113} (1981), 45--66.

\bibitem{Ran1}
Z. Ran:
{\it On nodal plane curves},
Invent. Math. {\bf 86} (1986), no. 3, 529--534.

\bibitem{Ran2}
Z. Ran:
{\it Families of plane curves and their limits: Enriques' conjecture
  and beyond},
Ann. of Math. {\bf 130} (1989), no. 2, 121--157.

\bibitem{Ran3}
Z.~Ran:
{\it Enumerative geometry of singular plane curves},
Invent. Math. {\bf 97} (1989), no. 3, 447--465.

\bibitem{Salmon1} G. Salmon:
{\it On the degree of a surface reciprocal to a given one}, Camb. and
Dubl. Math. J. {\bf 2} (1847), 65--73.

\bibitem{Salmon2} G. Salmon:
{\it On the degree of the surface reciprocal to a given one}, Trans. Royal Irish Acad., {\bf 23}
(1859), 461--488.

\bibitem {bsegre} B. Segre: 
{\it On limits of algebraic varieties, in particular of their intersections and tangential forms}, Proc. London Math. Soc., (2), {\bf 47} (1942), 351--403. 

\bibitem{ser2} E.~Sernesi, {\it A smoothing criterion for families of curves}, 
\url{http://www.mat.uniroma3.it/users/sernesi/papers.html}
  
\bibitem{vainsencher}
I. Vainsencher:
{\it Counting divisors with prescribed singularities},
Trans. Amer. Math. Soc. {\bf 267} (1981), no. 2, 399--422. 

\bibitem{vainsencher2}
I. Vainsencher, Israel: 
{\it Enumeration of $n$--fold tangent hyperplanes to a surface}, Journal of Algebraic Geometry {\bf 4} (1995), 503--526.

\end{thebibliography}

\end{references}


% \small
% \vskip .2cm \noindent
% \textsc{%
% Dipartimento di Matematica, 
% Universit\`a degli Studi di Roma Tor Vergata,
% Via della Ricerca Scientifica,
%  00133 Roma, Italy} \\
% \texttt{cilibert@mat.uniroma2.it}

%\end{closing}


\stopcontents[ciro]





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End:


==> 02.edoardo/TorVergata.tex <==
% \input{enumTV}

% \begin{document}

\chaptitle{Deformations of curves on surfaces}
\chapauthor{Thomas Dedieu and Edoardo Sernesi}

\startchap
\label{02.edoardo}
\begingroup

\def\bP{\mathbb{P}}
\def\cO{\mathcal{O}}
 \def\bC{\mathbb{C}}
 \def\bQ{\mathbb{Q}}
\def\bN{\mathbb{N}}
 \def\cC{\mathcal{C}}
 \def\cA{\mathcal{A}}
 \def\cB{\mathcal{B}}
 \def\c{\mathcal}
 \def\rm{\mathrm}

\def\rk{\mathrm{rk}}
\def\k{\mathbb{C}}
\def\fr{\mathfrak}
\def\wh{\widehat}
\def\wt{\widetilde}
\def\ol{\overline}
\def\Spec{\mathrm{Spec}}



\startcontents[02.edoardo]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[02.edoardo]{}{1}[2]{}

\providecommand\O{\mathcal{O}}
\providecommand{\sHom}{\mathcal {H}\kern -.08em om} % sheaf Hom
\providecommand{\sExt}{{\mathcal {E}}\kern -.1em xt} % sheaf Ext
\providecommand{\sAnn}{\mathcal{A}nn} % sheaf Ann
\providecommand{\ie}{i.e.,\ }


\bigskip
This text surveys some foundational material from the deformation
theory of singular curves on surfaces, of ubiquitous use and necessity
in this whole collection.
The included topics are best described by the above table of contents.



\section{Algebroid plane curves}\label{S:algebroid}



A \emph{curve singularity} is a scheme of the form $\Spec(B)$, where $(B,\mathfrak m)$ is the local ring at a singular point of a reduced algebraic curve. If the curve is contained  in a nonsingular algebraic  surface then we speak of a
 \emph{planar curve singularity}. We will be mostly interested in this second case  and in  some of our  considerations it will be convenient to replace such a $B$ by its  $\mathfrak m$-adic completion.  In this section we will focus on this case and therefore we will   consider  local rings of the form
\[
B=\k[[X,Y]]/(f)
\]
for some power series $f$ without constant term and without multiple factors. The scheme $C:=\Spec(B)$ for such a ring is called an \emph{algebroid plane curve}.  If $f$ is irreducible then $C$ is called an \emph{analytic branch}.

Assume that $f$ is irreducible.  Then the normalization $\wt B$ of $B$ is a complete DVR and therefore it is isomorphic to a formal power series ring in one variable. Thus there exists $t\in K(B)$, the field of fractions  of $B$, such that  $\wt B =\k[[t]]$ and $K(B)=\k((t))$, the fraction field of $\k[[t]]$, which coincides with the field of formal Laurent power series in $t$.
  


We can write:
\[
f(X,Y) = f_n(X,Y)+f_{n+1}(X,Y)+ \cdots
\]
for some $n \ge 1$, where $f_i$ is a homogeneous polynomial of degree $i$. The integer $n$ is the \emph{multiplicity} of $f$ (or of $C$) at $0=[\mathfrak m]$. The polynomial $f_n(X,Y)$ is called the \emph{initial form} of $f$.  

 
 \medskip
 
 

We have two ideals associated to the algebroid plane curve $C$:
\[
\left(\frac{\partial f}{\partial X},\frac{\partial f}{\partial Y}\right) = (f_X,f_Y)
\]
is called the \emph{Milnor ideal} or \emph{gradient ideal} of $f$.  The corresponding algebra:
\[
M_f := \k[[X,Y]]/\left(f_X,f_Y\right)
\]
is the \emph{Milnor algebra} of $f$.

The ideal
\[
\left(f,f_X,f_Y\right)
\]
is called the \emph{Tjurina ideal} of $f$ and 
\[
T_f := \k[[X,Y]]/\left(f,f_X,f_Y\right)
\]
is the \emph{Tjurina algebra} of $f$.   
It will be convenient to describe the Tjurina algebra as follows:
\[
T_f = B/J
\]
where $J= (f,f_X,f_Y)/(f)\subset B$ is the so-called \emph{jacobian ideal}.  Viewed as a $B$-module $T_f$ is also called the \emph{first cotangent module} of $B$, and denoted by   $T^1_B$.
Since $C$ is either nonsingular or has an isolated singularity at $[\mathfrak m]$, the Tjurina ideal is either $(1)$ or  supported at	$[\mathfrak m]$,   and therefore    $T_f$ is a finite dimensional  $\k$-vector space. Then 
  \[
  \tau(f):= \dim(T_f) < \infty
  \]
  is   called  the \emph{Tjurina number} of $f$ (or of $B$).  On the other hand it is also true    that $M_f$ is   finite dimensional because of the following:
	
	\begin{lemma}[Risler \cite{jR71}]\label{L:risler}
	If $f \in (X,Y)^2\subset \k[[X,Y]]$ has no multiple factors then $f_X,f_Y$ form a regular sequence.
	\end{lemma}
	
	\proof It suffices to prove that $f_X$ and $f_Y$ have no common factors because they are contained in $(X,Y)$. Assume that they have a non-constant irreducible factor $p$ and consider the algebra $A=\k[[X,Y]]/(p)$. Let $\ol f\in A$ be the image of $f$.  Then $\ol f$ is annihilated by every $\k$-derivation $D: K(A) \to K(A)$. Let $t\in K(A)$ be such that $K(A)=\k((t))$ and consider the derivation $D=\frac{d}{dt}$. Then $\rm{ker}(D) = \k$.  Therefore $\ol f\in \k$ and therefore $\ol f=0$, which means that $f=pq$ for some $q\in (X,Y)$. Therefore, since
	$f_X=p_Xq+pq_X$ is divisible by $p$ but $p_X$ is not, it follows that $q$ is divisible by $p$, and therefore $f$ is divisible by $p^2$, a contradiction. \qed
	
	
	\medskip
	
For a proof of  Lemma \ref{L:risler} in the case of convergent power series see \cite{GLS07}, Lemma 2.3 p. 113.	
The   dimension
  \[
  \mu(f)= \dim(M_f)
  \]
  is called the \emph{Milnor number} of $f$ (or of $B$).
By construction we have:
\[
\tau(f) \le \mu(f)
\]
and equality holds if and only if  $f \in \left(f_X,f_Y\right)$.  Notice also that 
\[
\mu(f) = i(f_X,f_Y)
\]
where $i(-,-)$ denotes intersection multiplicity.


\begin{definition}\label{D:quasihom}
A polynomial $P(X,Y) = \sum_\alpha a_\alpha X^{\alpha_1}Y^{\alpha_2}$ is called \emph{quasi-homogeneous} (qh) of weights $w=(w_1,w_2)\in \bN^2$ and   degree $d$ if
\[
\alpha_1w_1+\alpha_2w_2 = d
\]
for all $\alpha$ such that $a_\alpha \ne 0$.
An algebroid plane curve $\Spec\left(\k[[X,Y]]/(f))\right)$ is quasi homogeneous if there is a q.h. polynomial $P$ such that $\k[[X,Y]]/(f)\cong \k[[X,Y]]/(P)$.    
\end{definition}

 If $P(X,Y)$ is qh then we have the generalized \emph{Euler relation} in $\k[X,Y]$:
\[
d P = w_1XP_X+w_2YP_Y
\]
and therefore
$P\in (P_X,P_Y)$.  Therefore an algebroid qh plane curve  satisfies $\mu(f)=\tau(f)$.  The converse is true, by the following:

\begin{theorem}[Saito \cite{kS71}]
The algebroid plane curve $\Spec\left(\k[[X,Y]]/(f)\right)$ 
is qh if and only if $\mu(f)=\tau(f)$.
\end{theorem}

 
\begin{example}[{\cite[p.~111]{GLS07}}]\label{ex:nonqh}
The polynomial $P(X,Y)= X^5+Y^5+ X^2Y^2$ is not qh. One can compute that a $\k$-basis of $T_f$ is defined by the monomials $1,X,\dots, X^4,XY,Y,\dots,Y^4$ and a $\k$-basis of $M_f$ has the additional monomial $Y^5$.  Thus $\tau(P)=10 <\mu(P)=11$.
\end{example}

\begin{example}\label{ex:ordsing}
The polynomial $f= X^a\pm Y^b$  is qh of weights $(b,a)$ and degree $ab$.  Therefore:
\[
\tau(f) = \mu(f) = (a-1)(b-1)
\]
\end{example}

\begin{example}\label{ex:simple}
The \emph{simple singularities} (also called \emph{ADE singularities}) are qh. They have the following equations:
 \begin{compactitem}
    \item $A_k$: $x^{k+1}+y^2=0$, \quad $k \ge 1$.
    \item $D_k$: $x(y^2+x^{k-2})=0$, \quad $k \ge 4$.
    \item $E_6$: $x^3+y^4=0$.
    \item $E_7$: $x(x^2+y^3)=0$.
    \item $E_8$: $x^3+y^5=0$.
 \end{compactitem}
 We have:
 \[
   \mu(A_k)=\mu(D_k)=\mu(E_k)=k.
 \]
\end{example}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{The conductor}
\label{E:S:cond}

Let $B$ be a ring and let $\ol B \subset \rm{Frac}(B)$ be a subring of the total ring of fractions containing $B$. The homomorphism 
\[
\rm{Hom}_B(\ol B,B) \to B, \quad \varphi \mapsto \varphi(1)
\]
induces an isomorphism
\[
\rm{Hom}_B(\ol B,B) \cong \rm{Ann}_B(\ol B/B).
\]
Then $\rm{Ann}_B(\ol B/B)$ is an ideal both in $B$ and in $\ol B$. It is called  the \emph{conductor} of $\ol B$ in $B$. We define the \emph{$\delta$-invariant} of $B \subset \ol B$ as
\[
 \delta(\ol B/B):=\dim_\k(\ol B/B).
 \]
If $\ol B$ is the integral closure of $B$ in $\rm{Frac}(B)$ then $\rm{Ann}_B(\ol B/B)$ is simply called the \emph{conductor of $B$} and denoted by $\c A(B)$;  $ \delta(\ol B/B)$ is   denoted by $\delta(B)$ and called \emph{$\delta$-invariant of $B$}.


 In case $C=\Spec(B)$ is either  a curve singularity or  an algebroid plane curve, $\delta(B)$
 is denoted by $\delta(C)$ or $\delta(f)$ in case $B=\k[[X,Y]]/(f)$. It is called the \emph{$\delta$-invariant}  of $B$ (of $C$). 

   Notice   that if $C=\Spec(B)$ is any curve singularity then  $\delta(B)= \delta(\wh B)$, by the flatness of $\wh B$ over $B$.
 
   


 

\begin{definition}
    \label{D:conductor}\index{conductor}\index{$\delta$-invariant}
Let $\varphi: \wt C \longrightarrow C$ be a birational morphism of
reduced  curves. The \emph{conductor of} $\varphi$ is the sheaf
of $\cO_C$-ideals:
\[
\c A(\varphi) := \sAnn(\varphi_*\cO_{\wt C}/\cO_C)
\]
or, equivalently:
\[
\c A(\varphi)= \sHom(\varphi_*\cO_{\wt C},\cO_C).
\]
For each $x \in C$, the finite nonnegative
integer
\[
\delta(\varphi,x) := \delta \bigl((\varphi_*\cO_{\wt C})_x/\cO_{C,x}\bigr)=
\dim_{\k}\left((\varphi_*\cO_{\wt C})_x/\cO_{C,x}\right)
\]
is called the (local) \emph{$\delta$-invariant of $\varphi$ at
$x$,} and
\[
\delta(\varphi) := h^0(\varphi_*\cO_{\wt C}/\cO_C)=\sum_{x\in
C}\delta(\varphi,x)
\]
is the (global) \emph{$\delta$-invariant of} $\varphi$. In case $\varphi$ is the normalization of $C$ (\ie $\wt C$ is nonsingular) we write $\c A(\varphi)=\c A(C)$ and 
$\delta(\varphi)=\delta(C)$ and call them the \emph{conductor of $C$} and the \emph{$\delta$-invariant of $C$} respectively.
\end{definition}


The exact sequence
\[
\xymatrix{
0\ar[r] & \cO_C \ar[r] & \nu_*\cO_{\wt C}  \ar[r] & \nu_*\cO_{\wt C}/\cO_C \ar[r]&0}
\]
gives
\[
\chi(\cO_{\wt C}) = \chi(\nu_*\cO_{\wt C})= \chi(\cO_C)+ \delta(\varphi),
\]
which can be rephrased as:
 \begin{equation}\label{E:cogenus}
  \delta(\varphi) =   p_a(C)- p_a(\wt C)
\end{equation}
where as usual $p_a(-)$ denotes \emph{arithmetic genus}  of $-$. In case $\varphi$ is the normalization of $C$,   the above identity takes the form:
\begin{equation}\label{E:cogenus2}
  \delta(C) =   p_a(C)- p_g(C)
\end{equation}
which shows that the $\delta$-invariant of $C$ measures the difference between the arithmetic genus and the geometric genus of the curve. 

  
For the next lemma,
observe that $\c A(\varphi)$ is naturally a sheaf of $\varphi_*\cO_{\wt C}$-modules. Therefore, since $\varphi$ is affine, we have $\wt C=\mathrm{Spec}(\varphi_*\cO_{\wt C})$ and  $\c A(\varphi)$ corresponds to a sheaf of $\cO_{\wt C}$-modules which we denote by
$\wt {\c A}(\varphi)$.
%see \cite[II, Ex.~5.17e, p.~128]{rH77}.


\begin{lemma}\label{L:adj1}
Let $\varphi:\wt C \to C$ be a birational morphism of reduced projective curves. Then there is a canonical isomorphism:
\begin{equation}\label{E:cond1}
\varphi_*\omega_{\wt C} \cong \sHom_{\cO_C}(\varphi_*\cO_{\wt C},\omega_C)
\end{equation}
If moreover $C$ is Gorenstein, then 
\begin{equation}\label{E:cond2}
  \varphi_*\omega_{\wt C} \cong \c A(\varphi)
  \otimes_{\O_C} \omega_C
\end{equation}
and 
\begin{equation}\label{E:cond3}
\omega_{\wt C} = \wt {\c A}(\varphi)\otimes_{\cO_{\wt C}}\varphi^*\omega_C.
\end{equation}
\end{lemma}

\begin{proof} The proof of (\ref{E:cond1}) follows from standard facts
and is valid for finite morphisms of   projective schemes.
Recall the two following facts from
\cite[III, Ex. 6.10, p.~239]{rH77}.  
For each quasi-coherent sheaf $\mathcal{G}$
on $C$, the module $\sHom_{\cO_C}(\varphi_*\cO_{\wt C},\mathcal{G})$ has a
natural structure of quasi-coherent sheaf on $\wt C$, and as such it
is denoted by $\varphi^!\mathcal{G}$.  For each quasi-coherent
sheaf $\mathcal{F}$ on $\wt C$, there is a natural isomorphism:
\[
\varphi_*\sHom_{\cO_{\wt C}}(\mathcal{F},\varphi^!\mathcal{G}) \cong
\sHom_{\cO_C}(\varphi_*\mathcal{F},\mathcal{G}).
\]
Taking $\mathcal{G}=\omega_C$ and $\c F=\cO_{\wt C}$ gives
\[
\varphi_*(\varphi^!\omega_C) \cong
Hom_{\cO_C}(\varphi_*\cO_{\wt C},\omega_C).
\]
Therefore it suffices to prove that $\varphi^!\omega_C=\omega_{\wt C}$
(which is \cite[III, Ex.~7.2(a)]{rH77}.
For all coherent $\mathcal{F}$ on $\wt C$ we have:
\[
H^1(\wt C,\mathcal{F})^\vee=H^1(C,\varphi_*\mathcal{F})^\vee=
\rm{Hom}_{\cO_C}(\varphi_*\mathcal{F},\omega_C) \cong
\rm{Hom}_{\cO_{\wt C}}(\mathcal{F},\varphi^!\omega_C),
\]
and this isomorphism is functorial in $\mathcal F$.
 This implies
that $\varphi^!\omega_C$ is a dualizing sheaf for $\wt C$
in the sense of \cite[Definition p.~241]{rH77} (see \cite[Exercise 29.1.A]{rVxx}) , and thus
\eqref{E:cond1} is proved.

If $\omega_C$ is invertible, then we
have:
\[
\varphi_*\omega_{\wt C}
= \sHom_{\cO_C}(\varphi_*\cO_{\wt C},\omega_C)
\cong
\sHom_{\cO_C}(\varphi_*\cO_{\wt C},\O_C) \otimes \omega_C
= \c A(\varphi)
\otimes\omega_C,
\]
which is \eqref{E:cond2}.
Then, by the Projection Formula we have
\[
\varphi_* \bigl(
\wt{\c A}(\varphi) \otimes
\varphi^* \omega_C
\bigr)
= \varphi_* \wt {\c A} (\varphi)
\otimes \omega_C
= \c A(\varphi) \otimes \omega_C,
\]
where the equality $\varphi_* \wt {\c A} (\varphi) =
\c A(\varphi)$
follows from \cite[II, Ex.~5.17e]{rH77}.
Thus
\[
\varphi_*\omega_{\wt C}=
\varphi_* \bigl(
\wt{\c A}(\varphi) \otimes
\varphi^* \omega_C
\bigr),
\]
hence
$\omega_{\wt C}=
\wt{\c A}(\varphi) \otimes
\varphi^* \omega_C$,
again by \cite[II, Ex.~5.17e]{rH77}.
\end{proof}


We refer the reader to
\cite[\S 29.3--4]{rVxx}
for versions of the formula
$\varphi^!\omega_C=\omega_{\wt C}$
valid in a more general framework.



\begin{corollary}\label{C:cond1}\begin{enumerate}[(a)]
\item
Let $C = \Spec(B)$ be a Gorenstein reduced curve singularity. Then:
\[
\delta(B)= \dim_\k(B/\c A(B)).
\]
\item
Let $C$ be a Gorenstein reduced projective curve and $\varphi:\wt C \to  C$ a birational morphism. Then 
\[
\delta(\varphi) = h^0(\cO_C/\c A(\varphi)).
\]
\end{enumerate}
\end{corollary}

\begin{proof} It suffices to prove (b).
Let $\c A=\c A(\varphi)$. By definition we have an exact sequence:
\[
\xymatrix{
0\ar[r] & \sHom_{\cO_C}(\varphi_*\cO_{\wt C},\cO_C) \ar[r]& \cO_C \ar[r] & \cO_C/\c A \ar[r] & 0}.
\]
Tensoring by $\omega_C$, using the fact that $C$ is Gorenstein and recalling \eqref{E:cond1}, we obtain:
\[
\xymatrix{
0\ar[r] & \varphi_*\omega_{\wt C} \ar[r] & \omega_C \ar[r] & [ \cO_C/\c A]\otimes\omega_C \ar[r] & 0}.
\]
From this exact sequence we deduce:
\begin{align}
h^0(\cO_C/\c A)  &=\chi( [ \cO_C/\c A]\otimes\omega_C)  \notag \\
& =\chi(\omega_C) - \chi( \varphi_*\omega_{\wt C}) \notag \\
&  = \chi(\omega_C) - \chi(\omega_{\wt C}) \notag \\
& = p_a(C) - p_a(\wt C) \notag \\
& = \delta(\varphi) \notag
\end{align}
and comparing with \eqref{E:cogenus} we conclude.
\end{proof}



\begin{corollary}\label{C:adj1}
Let $\varphi:\wt C \to C$ be a birational morphism of   projective reduced curves and assume that $C \subset Y$, a projective nonsingular surface. Then 
\[
\c A(\varphi)\otimes \cO_C(C) = \varphi_*\omega_{\wt C}\otimes \omega_Y^{-1}
\]
and
\[
  \wt{\c A}(\varphi)\otimes \varphi^* \cO_C(C)
  = \omega_{\wt C}\otimes \varphi^* \omega_Y^{-1}.
\]
\end{corollary}
\begin{proof} The assumptions imply that $C$ is Gorenstein. Then the corollary  is an easy consequence of Lemma~\ref{L:adj1}.  \end{proof}





\begin{lemma}\label{L:adj2}
Let $C$ be a reduced curve contained in a nonsingular algebraic surface $Y$. Let $p\in C$ be a point of multiplicity $m$ and $b: Z \to Y$ the blow-up of $Y$ at $p$.  Then, letting $\ol C \subset Z$ be the proper transform of $C$ and $E\subset Z$ the exceptional curve we have:
\[
b_*\omega_{\ol C} = \omega_C\otimes b_*\cO_Z\bigl(-(m-1)E\bigr).
\]
\end{lemma}

\proof Left to the reader.  \qed

\medskip

The Milnor number and the $\delta$-invariant are related as follows:

\begin{proposition}[Milnor formula]\label{P:milnorform}
Let   $f=f_1\cdots f_r \in \k[[X,Y]]$, where $f_1, \dots, f_r$  are pairwise distinct analytic branches.  Then:
\[
\delta(f) =  \frac{1}{2}\,\bigl[\mu(f)+r-1\bigr].
\]
\end{proposition}

\begin{proof}
  See \cite[Prop.~3.35, p.~208]{GLS07}.
\end{proof}



\begin{remark}
Let $\varphi: \wt C \longrightarrow C$ be a birational morphism of
reduced  curves, and denote by $\Delta \subset C$ and
$\wt\Delta \subset \wt C$ the two subschemes defined by
$\c A(\varphi)$ and $\wt {\c A}(\varphi)$ respectively.
% If $C$ has property $S_2$ then so has the conductor ideal
% (see, e.g., \cite[Lemma 7.4]{GT80}), and thus both $\Delta$ and
% $\wt\Delta$ are of pure codimension $1$ and without embedded point.
If both $C$ and $\wt C$ are Gorenstein, then it follows from
\eqref{E:cond3} that $\wt\Delta$ is Cartier.
However it is not true in general that $\Delta$ is a Cartier
divisor
(for instance, at a node $xy=0$ the conductor is the ideal generated
by $x$ and $y$).
\end{remark}

\begin{remark}
In general the two sheaves of $\O_{\wt C}$-modules $\wt{\c A} (\varphi)$ and
$\varphi^* {\c A} (\varphi)$ are different, even though,
in the words of \cite[(1.6), p.~350]{YPG}, ``many writers who should
know better write $\varphi^* {\c A} (\varphi)$ for the ideal
$\c A (\varphi) \cdot \O_{\wt C}$'' (the latter being $\wt {\c A} (\varphi)$ in our
situation). 

For the remainder of this remark, we write $\c A$ and $\wt {\c A}$ for
$\c A (\varphi)$ and $\wt {\c A} (\varphi)$
respectively.
By definition, $\varphi^* {\c A}
= \varphi^{-1} \c A \otimes_{\varphi^{-1} \O_C} \O_{\wt C}$,
and then the multiplication map induces an exact sequence
of $\O_{\wt C}$-modules
\[
  0
  \longrightarrow \c K
  \longrightarrow \varphi^* {\c A}
  \longrightarrow \wt {\c A}
  \longrightarrow 0.
\]
We shall see in the two following examples that in general $\c K$ is
non-trivial and $\varphi^* {\c A}$ has a non-trivial torsion part,
which is a manifestation of the fact that $\varphi$ is not flat.
The conclusion is that the object we want to consider is indeed
$\wt {\c A}$ and not $\varphi^* {\c A}$.

Our first example is the normalization of the node $xy=0$.
The adjoint ideal is $(x,y)$.
Locally on the branch $y=0$ in the normalization, the multiplication
map
$\varphi^{-1} \c A \otimes_{\varphi^{-1} \O_C} \O_{\wt C} \to
\O_{\wt C}$ corresponds to the multiplication map
\[
  (x,y) \otimes_{\k[x,y]/(xy)} \k[x]
  \longrightarrow \k[x],
\]
which has non-trivial kernel, generated by $y\otimes 1$ and thus
killed by multiplication by $x$.
The upshot is that the torsion part of $\varphi^* {\c A}$ is
$\O_{\wt \Delta}$, where $\wt \Delta$ consists of the two points in
the preimage of the node.

Our second example is the normalization of the cusp $y^2-x^3=0$,
which we see as $t \mapsto (t^2,t^3)$.
The adjoint ideal is again $(x,y)$, equivalently $(t^2,t^3)$.
The multiplication map
$\varphi^{-1} \c A \otimes_{\varphi^{-1} \O_C} \O_{\wt C} \to
\O_{\wt C}$ corresponds to the multiplication map
\[
  (t^2,t^3) \otimes _{\k[t^2,t^3]} \k[t]
  \longrightarrow \k[t],
\]
which has non-trivial kernel generated by
$t^2\otimes t - t^3\otimes 1$ and thus killed by multiplication by
$t^2$. Again the torsion part of $\varphi^* {\c A}$ is
$\O_{\wt \Delta}$, where this time $\wt \Delta$ is defined by the
ideal $(t^2)$ of $\k[t]$.
\end{remark}



\section{Equivalence of singularities}

   We say that two algebroid plane curves:
\[
C = \Spec(\k[[X,Y]]/(f), \quad D = \Spec(\k[[X,Y]]/(g)
\]
are \emph{isomorphic} or \emph{analytically equivalent} if there is an  isomorphism of $\k$-algebras
\[
\k[[X,Y]]/(f) \cong \k[[X,Y]]/(g)
\]
Because of the following result it is not restrictive to assume that $f$ is a polynomial when studying isomorphism classes of algebroid plane curves.


\begin{theorem}[Samuel \cite{pS56}]\label{T:samuel}
Given a reduced non-constant $f\in \k[[X,Y]]$  there is   a polynomial $g$ such that $\k[[X,Y]]/(f) \cong \k[[X,Y]]/(g)$.
\end{theorem}


A weaker equivalence relation has been introduced by Zariski as follows.  Consider and analytic branch
$C = \Spec(\k[[X,Y]]/(f)$ and let $n=e(C)$ be its multiplicity (at $0$).  The blowing up of $\Spec(\k[[X,Y]])$ at $0$ is defined by the substitution 
\[
X=X', \quad Y = X'Y'
\]
Then 
\[
f(X,Y) = f(X',X'Y') = X'^n f'(X',Y')
\]
and $f'$ is the \emph{proper transform} of $f$. One easily shows (see \cite{oZ86}, p. 3) that $f'$ is irreducible, \ie defines an analytic branch $C'$. Let $e(C')$ its multiplicity.  Then $e(C') \le e(C)$.  The theorem of resolution of singularities guarantees that after a finite number of iterations of this operation  we obtain a nonsingular branch $\ol C$, \ie such that $e(\ol C)=1$.  Let 
\[
C,C', \dots, C^{(i)}, \dots
\]
be the successive proper transforms of $C$ and $e_i = e(C^{(i)})$.   Let $N \ge 1$ be such that $e_N=1$ but $e_{N-1} \ne 1$ and let
\[
e^*(C) = \{e_0, e_1, \dots ,e_{N-1}\}
\]
The sequence $e^*(C)$ is uniquely determined by $C$.  

\begin{definition}\label{D:equis} Two analytic branches $C, D$ are said to be  \emph{equivalent} or  \emph{equisingular}, if 
\[
e^*(C) = e^*(D)
\]
\end{definition}

It is possible to show that two simple singularities are   equisingular if and only if they are analytically equivalent.  
The   simplest examples for which the two notions differ are ordinary $n$-fold points, with $n \ge 4$. For example, any two ordinary $4$-fold points are equisingular, but they are isomorphic if and only if their respective 4-tuples of principal tangent lines  have equivalent cross ratios.    
For more details about equisingularity we refer to  \cite{oZ86}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Generalities on deformations}\label{S:gendefs}

 Deformation theory studies local deformations of a given algebro-geometric object $X$ (a projective scheme, a singularity, etc.). Under good hypotheses it produces a family   containing all sufficiently small deformations of $X$, up to isomorphism,  and having certain functorial properties. Here we are interested  in deformations of planar curve singularities, a case where the theory simplifies consistently. Before adventuring into the details we need a general preamble about what we mean by  (local) deformations.  %In deformation theory the term ``local'' is intended in a restrictive sense \ie it means that one is considering deformations parametrized by the spectrum of either an artinian local $\k$-algebra or  a complete local $\k$-algebra. 
 
  Consider the category $\mathfrak{Loc}$ of local $\k$-algebras with residue field $\k$.  A \emph{deformation} of $X$ parametrized by $\Spec(R)$, where $R\in \rm{Ob}(\mathfrak{Loc})$ is a pullback diagram:
  \[
  \zeta:\xymatrix{
  X \ar[d]\ar@{^(->}[r]& \c X \ar[d]^-\pi\\
  \rm{Spec}(\k)\ar[r]&\Spec(R)}
  \]
 where $\pi$ is flat.  Given another deformation of $X$ parametrized by $\Spec(R)$:
 \[
 \eta: \xymatrix{
  X \ar[d]\ar@{^(->}[r]& \c Y \ar[d]^-\rho\\
  \rm{Spec}(\k)\ar[r]&\Spec(R)}
  \]
we say that $\zeta$ and $\eta$ are  \emph{isomorphic} if there is an isomorphism of $R$-schemes
\[
\xymatrix{
\c X \ar[rr]^-\cong\ar[dr]_-\pi&&\c Y\ar[dl]^-\rho \\
&\Spec(R)}
\]
 compatible with the identifications of $X$ with the fibres over $\Spec(\k)$.
 
 %The following general definitions are given with the purpose of clarifying this statement and introducing the standard terminology. 

Deformation theory    associates to $X$ a covariant functor $M_X: \fr{Loc} \to \fr{Sets}$       taking values in the category of sets. It is defined by: 
\[
M_X(R) = \left\{\text{isom. classes of def.s of $X$ parametrized by $\Spec(R)$}\right\}
\]
for all $  R \in \rm{Ob}(\fr{Loc})$, and $M_X(f:R\to S)$ is defined by pullback. 
This functor can   be extended to the category of pointed $\k$-schemes in an obvious way.  Since   deformation theory   is   unable to give a satisfactory information on either of these functors what can be done is to restrict $M_X$ to more amenable subcategories of $\fr{Loc}$.  Two full subcategories   are relevant in deformation theory. The first one is $\wh{\fr{Loc}}$, the category of complete local $\k$-algebras with residue field $\k$. The second one is $\fr{Art}$, whose objects are the local artinian $\k$-algebras with residue field $\k$. 

Covariant functors $F: \fr{Art} \to \fr{Sets}$ are called \emph{functors of Artin rings}. The restriction of $M_X$ to $\fr{Art}$ is such  a functor. 
If $A \in \rm{Ob}(\fr{Art})$ then the elements of $M_X(A)$ are called \emph{infinitesimal deformations} of $X$ parametrized by $A$. 

A \emph{formal deformation} of $X$ is a pair $(R,\wh\xi)$ where $(R,\fr{m})$ is a complete local $\k$-algebra, \ie $R \in \rm{Ob}(\wh{\fr{Loc}})$, and $\wh\xi =\{\xi_n \in M_X(R/\fr{m}^{n+1})\}_{n\ge 1}$  is a sequence of infinitesimal deformations which are compatible, \ie such that $\xi_n \mapsto \xi_{n-1}$ under the map
\[
  M_X(R/\fr{m}^{n+1}) \to M_X(R/\fr{m}^n)
	\]
	for each $n \ge 1$. Associating to every $R \in \rm{Ob}(\wh{\fr{Loc}})$ the set of formal deformations $(R,\wh\xi)$ we define a new functor 
\[
\wh M_X: \wh{\fr{Loc}} \to \fr{Sets}.
\]
A formal deformation $(R,\wh\xi)$ is called \emph{effective} if there is a deformation  $\xi\in M_X(R)$ such that $\xi \mapsto \xi_n$ under the map:
	\[
	M_X(\pi_n): M_X(R) \to M_X(R/\fr{m}^{n+1})
	\]
	 induced by the projection $\pi_n: R \to  R/\fr{m}^{n+1}$, for each $n \ge 1$.  
	 
	 \medskip

	 \emph{Important point:} Not every formal deformation is effective, \ie the functor $\wh M_X$  is not isomorphic to the restriction of $M_X$ to $\wh{\fr{Loc}}$. Namely in general $\wh M_X(R) \ne M_X(R)$. 
	 
	 \medskip

A formal deformation $(R,\wh\xi)$ is called \emph{algebraizable} if there is    a deformation $\zeta$ of $X$ parametrized by a pointed algebraic scheme $(S,s_0)$ and an isomorphism $u:R \cong \wh{\cO_{S,s_0}}$ and such that the sequence of deformations 
\[
\wh\zeta=\{\zeta_n\in M_X(\cO_{S,s_0}/\fr{m}^{n+1})\}
\]
 obtained by pulling back $\zeta$ is mapped to $\wh\xi$ under  $u$.  Every algebraizable formal deformation is effective because $\zeta$ can be pulled back to $\wh{\cO_{S,s_0}}$, but the converse is not true. 
	
\medskip

To every $R \in \rm{Ob}(\wh{\fr{Loc}})$ one can associate the functor of Artin rings:
\[
h_R: \fr{Art} \to \fr{Sets}, \quad A \mapsto \rm{Hom}(R,A).
\]
Functors of this form are called \emph{prorepresentable}. 
Consider a formal deformation $\wh\xi\in \wh M_X(R)$, for some $R \in
\rm{Ob}(\wh{\fr{Loc}})$. Let $A \in \rm{Ob}(\fr{Art})$ and  $f\in
h_R(A)=\rm{Hom}(R,A)$. Since $A$ is artinian there is an $n \gg 0$ such that $f$ factors as
\[
\xymatrix{
R \ar[r]\ar[dr]_-f& R/\fr{m}^{n+1}\ar[d]^-{f_n} \\
&A}
\]
One can then associate to $f$ the element  $M_X(f_n)(\xi_n)\in M_X(A)$. Since this is independent of $n$ we have 
 defined a morphism of functors of Artin rings that we denote with the same symbol:
\[
\wh\xi: h_R \to M_X.
\]

\begin{definition}\label{prorepr}
If a formal deformation $\wh\xi\in \wh M_X(R)$ is such that $\wh\xi$ is an isomorphism of functors then we say that the pair $(R,\wh\xi)$  \emph{prorepresents}  $M_X$. In this case $M_X$ is prorepresentable.
\end{definition}

In practice if a pair $(R,\wh\xi)$ prorepresents $M_X$ it means that for every $A \in \rm{Ob}(\fr{Art})$  every $\xi\in M_X(A)$  is induced as above by a unique $f:R \to A$. 

The prorepresentability of $M_X$ is a strong property which is often
not satisfied even by very simple objects $X$.  For example, if $X$ is
the singularity $XY=0$ then $M_X$ is not prorepresentable (see
\cite[Example 2.6.8, p.~95]{eS06}). The condition can be weakened in two ways as follows.


\begin{definition}\label{D:versal}
A formal deformation $\wh\xi\in \wh M_X(R)$ is called \emph{versal} if for every $A \in \rm{Ob}(\fr{Art})$ the induced map
\[
\wh\xi: h_R(A) \to M_X(A)
\]
is surjective.

A formal deformation $\wh\xi\in \wh M_X(R)$ is called \emph{miniversal} (or \emph{semiuniversal}) if it is versal and in addition 
\[
\wh\xi(\k[\epsilon]): h_R( \k[\epsilon]) \to M_X( \k[\epsilon])
\]
is bijective.
\end{definition}


The map $\wh \xi(\k[\epsilon])$ is called the \emph{differential} of $\wh\xi$.  Versality and miniversality are satisfied in most natural geometrical situations. Finally we give the following:

\begin{definition}\label{D:formversal}
An algebraic deformation $\zeta$ of $X$ parametrized by a pointed algebraic scheme $(S,s_0)$ is called \emph{formally versal} (resp. \emph{formally semiuniversal}) if the associated algebraizable formal deformation 
$(\wh\cO_{S,s_0},\wh\zeta)$ is versal (resp. semiuniversal). 
\end{definition}

For more details on the  contents of this section we refer to \cite{eS06} and \cite{rH10}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{The semiuniversal deformation of an isolated singularity}\label{S:semiuniv}

 
The case we will consider is $X=\rm{Spec}(B)$ where $(B,\fr m)$ is a noetherian local $\k$-algebra  with residue field $B/\fr m =\k$.  Assume that $B$ is either essentially of finite type (eft), \ie a localization of a $\k$-algebra of finite type, or complete, and that $\Spec(B)$ has an isolated singularity at $[\fr m]$.  Under these conditions deformation theory ensures the existence of a formal semiuniversal family of deformations of $B$, or of $\Spec(B)$  (see \cite{eS06}).  In the cases of interest for us such a deformation can be easily constructed explicitly. Note firstly the following:



\begin{proposition}\label{P:formal1}
If $B$ and $B'$ are local $\k$-algebras as above such that  $\wh B = \wh B'$, then their deformation functors are isomorphic.
\end{proposition}

\proof \cite[ex.~18.6, p.~127]{rH10}.  \qed


\medskip

This  means that it is not restrictive to   study deformations of a complete local $\k$-algebra.  Since we are interested in planar curve singularities, \ie in the local ring $B$ of a reduced curve $C$ contained in a nonsingular surface $Y$ at a point $p\in C$, we can replace $B$ by its completion and therefore we may assume that $=\k[[X,Y]]/(f)$, \ie that $C$ is an algebroid plane curve.

 Consider indeterminates $t_1, \dots, t_N$ where $N =\tau(f)$ and let 
 \[
 p_1(X,Y), \dots , p_N(X,Y)\in \k[[X,Y]]
 \]
  be polynomials inducing a basis of the Tjurina algebra $T_f$. Consider  the following family:
 %\[
 %\xymatrix{
 %\cB:=\k[[t_1,\dots,t_N,X,Y]]/f(Y,Y)+\sum_1^N t_ip_i(X,Y))\ar[r] & B \\
 %\k[[t_1,\dots,t_N]] \ar[u]\ar[r] & \k \ar[u]}
% \]
 %or, geometrically:
 \begin{equation}\label{E:semiuniv}
 \xymatrix{
 C \ar[d]\ar@{^(->}[r]&\Spec(\cB)=:\cC \ar[d]^-\pi\\ 
 \Spec(\k) \ar[r] &\Spec(\k[[t_1,\dots,t_N]]) =:M(B)}
 \end{equation}
 where  
 \[
 \c B:=\k[[t_1,\dots,t_N,X,Y]]/(f(Y,Y)+\sum_1^N t_ip_i(X,Y)).
 \]

\begin{proposition}\label{P:miniv1}
The family \eqref{E:semiuniv}
is a formally semiuniversal deformation of $C$. 

Replacing $\k[[t_1,\dots,t_N]]$  by $\k[t_1,\dots,t_N]$ we obtain an algebraic formally semiuniversal family of deformations of $C$:
\begin{equation}\label{E:semiuniv1}
\xymatrix{
 C \ar[d]\ar@{^(->}[r]&\Spec\left(\k[t_1,\dots,t_N][[X,Y]])/ (f(Y,Y)+\sum_1^N t_ip_i(X,Y))\right) \ar[d]^-{\pi_a}\\ 
 \Spec(\k) \ar[r] &\Spec(\k[t_1,\dots,t_N])}
 \end{equation}
 Therefore, letting 
 \[
 S_n:=\Spec(\k[[t_1,\dots,t_N]]/(t_1,\dots,t_N)^{n+1}),  \quad n \ge 1,
 \]
  the restrictions of \eqref{E:semiuniv} (or, what is the same,  of \eqref{E:semiuniv1}) to $S_n$  define a  sequence of (infinitesimal) deformations of $C$:
 \[
 \xymatrix{
 C \ar[d]\ar@{^(->}[r]& \cC_n \ar[d]^-{\pi_n}\\ 
 \Spec(\k) \ar[r] &S_n}
 \]
which is an algebraizable formal semiuniversal deformation $\wh\pi = \{\pi_n\}$ of $C$.
\end{proposition}

\proof See \cite{rH10}, \S 14, for a detailed explicit proof.   \qed 

\medskip


 The support of $\cC$ is different from the support of $\pi_n$, which is $C$, and a priori there is no information on how to recover $\cC$ starting from $\wh\pi$. Nevertheless from general properties of formal schemes   it follows that $\pi$ is uniquely determined by $\wh\pi :=\{\pi_n\}$ (see e.g. \cite{eS06}, Theorem 2.5.11, p. 81). 
This fact implies that Proposition \ref{P:miniv1} can be strengthened as follows.

\begin{corollary}
  a) For every %infinitesimal 
 deformation  
 \[
 \xymatrix{
 C \ar[d]\ar@{^(->}[r]& \c D \ar[d]\\ 
 \Spec(\k) \ar[r] &\Spec(R)}
 \]
of $C$ where $R \in \rm{Ob}(\wh{\fr{Loc}})$, there is a morphism $\varphi:\Spec(R) \to M(B)$ (not unique, but whose differential is unique) inducing an isomorphism
\[
\c D \cong \Spec(R)\times_{M(B)}\cC
\]
compatible with the isomorphisms of the closed fibres with $C$. 

 \medskip
 
 
 
 b) Given a family of deformations of $C$:
 \[
 \xymatrix{
 C \ar[d]\ar@{^(->}[r]& \c X \ar[d] \\
 \Spec(\k) \ar[r]^-{s_0} & S}
 \]
 parametrized by an \emph{algebraic} scheme $S$ (or by the spectrum of an eft local $\k$-algebra) there is      a morphism (not unique, but whose differential is unique)
 \[
 \Spec(\wh\cO_{S,s_0}) \to \Spec(\k[[t_1,\dots,t_N]])=M(B)
 \]
 which  induces an isomorphism of deformations over $\Spec(\wh\cO_{S,s_0})$:
 \[
 \Spec(\wh\cO_{S,s_0})\times_S\c X \cong \Spec(\wh\cO_{S,s_0})\times_{M(B)}\cC.
 \]
  \end{corollary}


 For another discussion of this property see \cite{rH10}, Prop. 15.2, p. 108.
 
 \begin{remarks}\label{rm:formal}
 (1)  If $C$ is nonsingular then $T^1_B=0$ and the semiuniversal deformation is:
 \[
 \xymatrix{
 C \ar[d]\ar@{=}[r] & C \ar[d] \\
 \Spec(\k) \ar@{=}[r] & \Spec(\k)}
 \]
 (see \S \ref{S:algebroid}
 for the definition of $T^1_B)$.
 
 
 (2) If $C: f=0$ is singular then it is immediate to verify that $f+\epsilon=0$ is nonsingular for small values of $\epsilon$.  This implies that $C$   has nonsingular deformations, \ie that it is \emph{smoothable}. The same proof shows that any germ of hypersurface in $\k^n$ with an isolated singularity at the origin is smoothable.  An obvious modification of the argument shows that a germ of complete intersection isolated singularity is smoothable.
 
 
 (3) Versality is an open property, but not semiuniversality.  In other words, the semiuniversal family
 \eqref{E:semiuniv} is versal in a neighborhood of $0$. Obviously it is not semiuniversal, e.g. where the fibres are smooth, because there the fibres are rigid and their semiuniversal deformation just consists of the fibre itself (see Remark (1) above).  The standard reference for  openness of versality  is \cite{hF81}.

 \end{remarks}
 
 \begin{example}\label{ex:defAk}
 (i) The semiuniversal deformation of  $A_1:X^2-Y^2=0$ is $X^2-Y^2+t=0$.
 The only singular fibre is for $t=0$.
 
 (ii) Consider $A_2: X^2-Y^3=0$.  Then the semiuniversal deformation is 
 \[
 F(t,u,X,Y) = X^2-Y^3+tY+u=0
 \]
 The singular fibres are determined by the conditions $F=F_X=F_Y=0$ which are equivalent to $t=3Y^2, \ u=-2Y^3$.  We obtain the locus $\Delta:27u^2-4t^3=0$ inside $M(B)$. The fibres are the cusp at $(0,0)$ and one node  over the other points of $\Delta$. The fibres over $M(B)\setminus \Delta$ are nonsingular.
 \end{example}  
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 \section{Equigenericity and equisingularity}
 
 It is possible to define two interesting loci inside $M(B)$, the equigeneric locus
 and the equisingular locus.
 
 \medskip
 
 The \emph{equigeneric locus}  $EG\subset M(B)$ is supported on the points of $M(B)$ whose fibre is a singularity imposing the same number of conditions to adjoints as $C$ does, \ie on the points having the same $\delta$-invariant as $C$.  
 The locus $EG\subset M(B)$ is only defined set-theoretically, it does not have a functorial definition. As a locally closed subset of $M(B)$ it is analytically irreducible near $0\in M(B)$ and   its tangent cone is a vector subspace of $T_f$. Identifying  $T_f= B/J$ the tangent cone to $EG$ at $0$ is identified with $A/J$.  In particular $A$ contains $J$ and $EG$ has codimension $\delta(C)$ in $M(B)$.
In Example \ref{ex:defAk}(ii)  we have $EG=\Delta$.

 
\medskip

The \emph{equisingular locus}  $ES\subset M(B)$ is roughly the locus where the topological type of the singularity is the same as that of $C$.  
In particular $ES \subset EG$.  In example \ref{ex:defAk}(ii) we have $ES=\{0\}$.

The locus $ES$ has a scheme structure because it has a (complicated) functorial definition that we do not need to recall here. $ES$ is nonsingular and its tangent space at $0\in M(B)$ is the vector space $I/J\subset B/J =T_f$  where $I\subset A \subset B$ is an ideal called the \emph{equisingular ideal}.

\begin{lemma}\label{L:equis1}%
\begin{enumerate}[(i)]
\item  $I=A$ if and only if  $B$ is an $A_1$-singularity (a node).

\item All the simple singularities satisfy $I=J$, \ie they have no nontrivial equisingular  deformations.  Equivalently $ES=\{0\}$.

\item  The simplest example such that $\dim(ES)> 0$, \ie $J \ne I$,  is an ordinary 4-ple point.
\end{enumerate}
\end{lemma}

For detailed information on equisingularity and many examples we refer to \cite{GLS07}.
The following results due to Teissier are important in this context. 

\begin{theorem}[Teissier \cite{bT80}]\label{T:teis1}
Let $\c C \to S$ be an equigeneric family of reduced curves, $S$ reduced.  Then there is a Zariski dense open set $U\subset S$ such that  $\c C\times_SU \to U$ is equisingular.
\end{theorem}

\begin{theorem}[Teissier \cite{bT80}]\label{T:teis2}
Let $p:\c C \to S$ be a flat family of reduced curves with $\c C, S$ reduced of finite type. If $S$ is normal then the following are equivalent:
\begin{itemize}
\item[(a)] $p:\c C \to S$ is equigeneric.
\item[(b)] The composition 
\[
\xymatrix{
\c C' \ar[r]^-\nu & \c C \ar[r]^-p & S}
\]
where $\nu$ is the normalization, is smooth and for all $s \in S$ the induced morphism on the fibres $\nu_s:\c C'_s \to \c C_s$ is the normalization.
\end{itemize} 
\end{theorem}

\noindent
{\bf Note:} if $S$ is not assumed to be normal the theorem is false: see \cite{DH88}, Ex. (2.6).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 

\section{Families of curves on surfaces}

We now fix a projective nonsingular algebraic surface $Y$, a class $\xi \in \rm{NS}(Y)$ and the scheme of curves of class $\xi$ in $Y$, denoted $\rm{Curves}^\xi_Y$.  We have a universal family:
\[
\xymatrix{
\c C\ar[d]\ar@{^(->}[r]  & \rm{Curves}^\xi_Y \times Y \\
\rm{Curves}^\xi_Y}
\]
whose fibres have arithmetic genus $p_a(\xi)$ depending only of $\xi$.  If $[C]\in \rm{Curves}^\xi_Y$ then
\[
p_a(\xi) = \frac{(C+ K_Y) \cdot C}{2}+1.
\]
 For a given $0 \le g \le p_a(\xi)$ one can consider the (possibly empty) locally closed locus $V^\xi_g\subset \rm{Curves}^\xi_Y$ parametrizing reduced curves having geometric genus $g$.  Inside $V^\xi_g$ one has the locus $V^{\xi,\delta}$ parametrizing reduced curves having $\delta=p_a(\xi)-g$ nodes and no other singularities.  We want to compare these two loci, exploring the conditions under which we have $\overline{V^{\xi,\delta}} = \overline{V^\xi_g}$.
 
 Let $C\subset Y$ be a reduced curve parametrized by a point of  $V^\xi_g$.  Dualizing the conormal sequence we obtain an exact sequence of sheaves on $C$:
 \[
 \xymatrix{
 0\ar[r]& T_C \ar[r] & T_{Y|C} \ar[r] & \cO_C(C) \ar[r] & T^1_C \ar[r] & 0}
 \]
 where $T^1_C$ is the first cotangent sheaf of $C$, which has been described locally in \S \ref{S:algebroid}. Note that in \S \ref{S:algebroid} we considered the case of algebroid plane curves. The module $T^1_B$ has an analogous definition for eft local rings  and, being a torsion module 
 in our case (isolated singularities), it is    invariant under completion.
 
 Locally at the point $v\in V^\xi_g$ parametrizing $C$ the restricted universal family
 \[
 p: \c C_g \to V^\xi_g 
 \]
 induces a family of deformations of the singular points of $C$.  The semiuniversal families induce a morphism from $\Spec(\wh\cO_{V^\xi_g,v})$  to the product of the bases of the semiuniversal families of deformations of the singularities of  $C$.  The differential of this morphism turns out to be precisely the map:
 \[
 H^0(C,\cO_C(C)) \to H^0(T^1_C)
 \]
 appearing in the above exact sequence.  Let's denote, as before, by
 $\c J\subset \c I\subset \c A\subset \cO_C$  respectively the
 jacobian, equisingular, and conductor ideal sheaves. Then this observation implies the following:
 
 \begin{proposition}\label{P:diff1}
 If we identify $T_v(\rm{Curves}^\xi_Y) = H^0(C,\cO_C(C))$ then:
 \begin{itemize}
 \item[(i)] $H^0(C,\c J\otimes \cO_C(C))$ is the tangent space to the subscheme of formally locally trivial deformations of $C$ in $Y$.
 
 \item[(ii)] $H^0(C,\c I\otimes \cO_C(C))$ is the tangent space to the subscheme of equisingular deformations of $C$ in $Y$.

\item[(iii)] $H^0(C,\c A\otimes \cO_C(C))$ contains  the reduced tangent cone to the subscheme of equigeneric deformations of $C$ in $Y$.

\end{itemize}

 \end{proposition}
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 \section{Deformations of morphisms}
 
 Given $C \subset Y$ as in the previous section we may consider a partial normalization morphism:
 \[
 \varphi: \wt C \to C\subset Y
 \]
where we assume that $\wt C$ has at worst local complete intersection
singularities. There is a well defined deformation theory for such a morphism, which produces a semiuniversal deformation of $\varphi$:
 \[
 \xymatrix{
 \wt{\c C} \ar[d] \ar[r]^-\Phi &M(\varphi)\times Y \\
 M(\varphi) }
 \]
 where $M(\varphi)=\Spec(R)$ for some complete local $\k$-algebra. 
 Semiuniversality here means a property analogous to the one considered in  \S \ref{S:semiuniv} for   deformations of local rings; in particular $\varphi$ is the fibre of $\Phi$ over the the closed point $0:=[\fr m_R]\in M(\varphi)$.
  The  properties of $M(\varphi)$ are determined by the deformation functor $\mathrm{Def}_\varphi$ of $\varphi$. For the infinitesimal study  of $M(\varphi)$ one considers the complex:
  $$
  \Omega^\bullet_\varphi := [\varphi^*\Omega^1_Y\to \Omega^1_{\wt C}].
  $$
The hyperext spaces $\mathrm{Ext}^1_{\cO_{\wt
    C}}(\Omega^\bullet_\varphi,\cO_{\wt C})$ and
$\mathrm{Ext}^2_{\cO_{\wt C}}(\Omega^\bullet_\varphi,\cO_{\wt C})$ are
respectively the tangent space and the obstruction space of $\mathrm{Def}_\varphi$. Then deformation theory implies the following:
  \begin{proposition}
     There is a canonical identification
     $$
     T_0M(\varphi) = \mathrm{Ext}^1_{\cO_{\wt C}}(\Omega^\bullet_\varphi,\cO_{\wt C})
     $$
     and   inequalities:
     $$
     \mathrm{ext}^1_{\cO_{\wt C}}(\Omega^\bullet_\varphi,\cO_{\wt C})- \mathrm{ext}^2_{\cO_{\wt C}}(\Omega^\bullet_\varphi,\cO_{\wt C})\le \dim (M(\varphi)) \le \mathrm{ext}^1_{\cO_{\wt C}}(\Omega^\bullet_\varphi,\cO_{\wt C}).
     $$
  \end{proposition}


   
          For details we refer to \cite[Sec.~3.2]{sDxx}.  Our assumptions  imply that $\varphi$ is unramified at the general point of every component of $\wt C$. Therefore a simple computation (see 
\cite[Lemma 11]{BHT11}) implies that there is a sheaf $N_\varphi$ which fits into an exact sequence:
  \begin{equation}\label{E:normalsheaf}
      0\to \sHom(\Omega^1_{\wt C}, \cO_{\wt C})\to \sHom(f^*\Omega^1_Y,\cO_{\wt C})\to N_\varphi \to \sExt^1(\Omega^1_{\wt C},\cO_{\wt C})\to 0
  \end{equation}
  and such that
  $$
  H^0(C,N_\varphi)=\mathrm{Ext}^1_{\cO_{\wt C}}(\Omega^\bullet_\varphi,\cO_{\wt C}), \quad H^1(C,N_\varphi)=\mathrm{Ext}^2_{\cO_{\wt C}}(\Omega^\bullet_\varphi,\cO_{\wt C}).
  $$
  The sheaf $N_\varphi$ is called \emph{normal sheaf} of $\varphi$.


  We will be interested in two special cases:
  \begin{itemize}
      \item[(a)] $\wt C$ is nonsingular, \ie $\varphi$ is the normalization map.
      \item[(b)]  $\varphi$ is unramified.
  \end{itemize}
  
  In case (a) the sheaf $\Omega^1_{\wt C}$ is locally free and therefore the sequence \eqref{E:normalsheaf} becomes:
  \begin{equation}\label{E:maps1}
      0 \longrightarrow T_{\wt C} \longrightarrow \varphi^*T_Y
      \longrightarrow N_\varphi
      \longrightarrow 0.
  \end{equation}
The sheaf $N_\varphi$ has torsion in general. More precisely we have an exact sequence:
\begin{equation}\label{E:maps2}
0\longrightarrow \c H_\varphi \longrightarrow N_\varphi
\longrightarrow \overline{N}_\varphi \longrightarrow 0
 \end{equation}
 where $\c H_\varphi = \cO_Z$ for some effective divisor $Z$ supported
 on the locus where the differential $d\varphi$ degenerates. Therefore $\varphi(Z)\subset C$ is the set of points where $C$ has a non-linear branch.
 The exact sequences \eqref{E:maps1} and \eqref{E:maps2} imply that:
 \[
 c_1(N_\varphi) = \omega_{\wt C}\otimes\varphi^*\omega_Y^{-1}
 \]
 and 
 \[
 \overline{N}_\varphi \cong \omega_{\wt C}\otimes\varphi^*\omega_Y^{-1}(-Z).
 \]
 We have the following useful:
 
 \begin{lemma}[Arbarello-Cornalba \cite{AC81}]
 \label{lem:Arbarello-Cornalba}
 If $\theta\in H^0(\c H_\varphi)$ then the corresponding infinitesimal (first order) deformation of $\varphi$ leaves the image fixed.
 \end{lemma}
 
 In case (b) we have an exact sequence
  \begin{equation}\label{E:Emaps3}
      0\to \c K \longrightarrow \varphi^* \Omega^1_Y \longrightarrow \Omega^1_{\wt C}  \to 0
  \end{equation}
  where $\c K$ is invertible because  $\Omega^1_{\wt C}$ has
  homological dimension 1 since $\wt C$ has l.c.i.\ singularities
  (which implies that $\Omega^1_{\wt C}$ is resolved by the conormal exact sequence of a local embedding). Then in the sequence \eqref{E:normalsheaf} we have an identification $N_\varphi =\c K^\vee$.

\begin{lemma}\label{L:Emaps3}
    In case (b) we have
    $$
    N_\varphi \cong  \omega_{\wt C}\otimes \varphi^*\omega_Y^{-1}.
    $$
\end{lemma}

\begin{proof}
    Since $\wt C$ is a local complete intersection, we have 
    $$
    \omega_{\wt C} =\det(\Omega^1_{\wt C})
    $$
    by \cite[Thm.~III.7.11]{rH77}.
    On the other hand the exact sequence  \eqref{E:Emaps3} yields
    $$
   \det(\Omega^1_{\wt C})=\det(\varphi^*\Omega^1_Y)\otimes \c K^{-1}=\varphi^*\omega_Y\otimes N_\varphi.
   $$
   The result follows since $\varphi^*\omega_Y$ is invertible.
\end{proof}

\begin{corollary}\label{C:Emaps1}
  In case (b) we have, in the notation of
  Section~\ref{E:S:cond} for the conductor:
    $$
    N_\varphi \cong \varphi^*N_{C/Y}\otimes \wt {\mathcal A}(\varphi)
    $$
    and
    $$
    \varphi_*N_\varphi \cong N_{C/Y}\otimes \mathcal{A}(\varphi).
    $$
\end{corollary}

\begin{proof}
  It is a direct consequence of the previous lemma and
  Corollary~\ref{C:adj1}.
  %Lemma \ref{L:adj1}.
\end{proof}
   
  
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 \section{A criterion for the density of nodal curves}
 
 
 We keep the same notations of the previous section.
 
 \begin{theorem}\label{T:density}
 Let $V \subset V^\xi_g$ be an irreducible component and let $[C]\in V$ be a general point with normalization $\varphi: \wt C \to Y$.  Consider the following conditions:
 \begin{itemize}
 \item[(a)] $\omega_{\wt C}\otimes\varphi^*\omega_Y^{-1}$ is globally generated.
 \item[(b)]  $\dim(V) \ge h^0(\wt C,\omega_{\wt C}\otimes\varphi^*\omega_Y^{-1})$.
 \item[(c)] $h^0(\omega_{\wt C}\otimes\varphi^*\omega_Y^{-1}(-\fr a))=
 h^0(\omega_{\wt C}\otimes\varphi^*\omega_Y^{-1})-3$ for every effective divisor $\fr a$ of degree 3 on $\wt C$.
  \end{itemize}
  If (a) and (b) are satisfied then $C$ is immersed, \ie all its local branches are linear. If also (c) is satisfied then $C$ is nodal.
\end{theorem}
 
 For the proof we refer to \cite{DS15}. Let's see an application.
 
 \begin{corollary}[Arbarello-Cornalba \cite{AC80}, Zariski \cite{oZ82}]\label{C:ACZ}
The general element of any component of the Severi variety $V_{d,g}$ of integral plane curve of degree $d$ and genus $g$ is a nodal curve.
 \end{corollary}
 
 \begin{proof}[Proof (outline)]
 Let $[C]\in V_{d,g}$ be a general element of a component. We have
 \[
 \deg(\omega_{\wt C}\otimes\varphi^*\omega_{\bP^2}^{-1}) = 2g-2+3d
 \]
Since $d \ge 3$ (otherwise there is nothing to prove) conditions (a)
and (c)  of the Theorem are clearly satisfied.  One can   construct a
family of curves in $V_{d,g}$ as the image of the semiuniversal
deformation of $\varphi$.  Using  \eqref{E:maps2} one can easily
deduce that this family satisfies (b)     as well. 
\end{proof}


 
 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{references}

\begin{thebibliography}{9999}


\bibitem{AC80}
Arbarello E., Cornalba M., \emph{Su una propriet\`a
  notevole dei morfismi di una curva a moduli generali in uno spazio
  proiettivo}, Rend. Sem. Mat. Univ. Politec. Torino \textbf{38} (1980), no.~2,
  87--99 (1981).
  
  \bibitem{AC81}
\bysame , \emph{Su una congettura di {P}etri}, Comment. Math. Helv. \textbf{56}
  (1981), no.~1, 1--38.

\bibitem{BHT11}
  Bogomolov F., Hassett B., Tschinkel Y.,
  \emph{Constructing rational curves on K3 surfaces},
  {Duke Math. J.} {\bf 157} (2011), 535- 550.


\bibitem{DS15}
  Dedieu Th., Sernesi E.,
  \emph{Equigeneric and equisingular families of curves on surfaces},
  Pub. Mat. \textbf{62} (2017),
  175--212.

\bibitem{DH88}
Diaz S.,  Harris J.,
{\em Ideals associated to deformations of singular plane curves},
{Trans. AMS} {\bf 309} (1988), no. 2, 433--468.


\bibitem{sDxx}
  Druel S.,
  \emph{Courbes sur les variétés et leurs espaces de modules --
    Quelques applications},
  lecture notes available at
  \url{http://druel.perso.math.cnrs.fr/textes/ecole2010.pdf}.


\bibitem{hF81}
  Flenner H.,
  \emph{Ein Kriterium f\"ur die Offenheit der Versalit\"at},
  {Math. Z.} {\bf 178} (1981), 449-473.

% \bibitem{GT80}
% Greco S., Traverso C.;
% \emph{On seminormal schemes},
% {Compositio Mathematica} {\bf 40}, n~3 (1980), p.~325--365.

\bibitem{GLS07}
  Greuel M., Lossen C., Shustin E.,
  \emph{Introduction to
Singularities and Deformations,} Springer Monographs in
Mathematics (2007).

\bibitem{rH77}
Hartshorne R., {\it Algebraic Geometry}, Springer  GTM n.~52  (1977).

\bibitem{rH10}
\bysame, \emph{Deformation Theory}, Springer GTM n.~257
(2010).

\bibitem{YPG}
  Reid M.:
  \emph{Young Person's Guide to Canonical Singularities},
  in 
  Algebraic geometry, Proc. Summer Res. Inst., Brunswick/Maine 1985, part 1, Proc. Symp. Pure Math. 46, 345--414 (1987). 

\bibitem{jR71}
  Risler J.J., \emph{Sur l'id\'eal jacobien d'une courbe plane},
  {Bull. Soc. Math. de France} {\bf 99} (1971), 305-311.

\bibitem{kS71}
Saito K., \emph{Quasihomogene isolierte Singularit\"aten von
  Hyperfl\"achen},
{Inventiones Math.} {\bf 14} (1971), 123-142.

\bibitem{pS56}
  Samuel P.,
  \emph{Algebraicité de certains points singuliers algébroides},
  {J. de Mathématiques Pures et  Appliquées} {\bf 35} (1956), p. 1-6.


\bibitem{eS06}
  Sernesi E., {\it Deformations of Algebraic Schemes},
  Springer  Grundlehren b.~334 (2006).


\bibitem{bT77}
Teissier B., \emph{The hunting of invariants in the geometry of discriminants},
  in \emph{Real and complex singularities ({P}roc. {N}inth {N}ordic {S}ummer
  {S}chool/{NAVF} {S}ympos. {M}ath., {O}slo, 1976)}, Sijthoff and Noordhoff,
  Alphen aan den Rijn, 1977, 565--678.

\bibitem{bT80}
\bysame , \emph{{R\'esolution simultan\'ee I, II}}, in \emph{S\'eminaire sur
  les singularit\'es des surfaces, Cent. Math. \'Ec. Polytech., Palaiseau
  1976--77}, Lecture Notes in Mathematics, vol.~777, Springer-Verlag, Berlin,
  1980, 71--146.

\bibitem{rVxx}
  Vakil R.,
  \emph{The rising sea --- Foundations of Algebraic Geometry},
  February 21, 2024 version,
  available at
  \url{http://math.stanford.edu/~vakil/216blog/FOAGfeb2124public.pdf}.

  \bibitem{oZ82}
Zariski O., \emph{Dimension-theoretic characterization of maximal irreducible
  algebraic systems of plane nodal curves of a given order {$n$} and with a
  given number {$d$} of nodes}, Amer. J. Math. \textbf{104} (1982), no.~1,
  209--226.
  
  \bibitem{oZ86}
  \bysame, \emph{Le problème des modules pour les branches planes}, Hermann (Paris), 1986.



\end{thebibliography}

\end{references}

\stopcontents[02.edoardo]
\endgroup


% \end{document}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End: 
 	


==> 03.th-acz/thomasCH.tex <==
\chaptitle{Geometry of logarithmic Severi varieties at a general
  point}
\chapauthor{Thomas Dedieu}

\startchap
\label{03.th-acz}


\renewcommand{\curve}{\operatorname{Curve}}
\newcommand{\Nseq}{\underline{\N}}
\newcommand{\Def}{\operatorname{Def}}
\newcommand{\Mgbir}{M_g ^{\xi, \text{bir}}}
\newcommand{\Img}{\operatorname{Im}}
\newcommand{\out}{\mathrm{out}}
\newcommand{\nir}{\mathrm{ni}}
\newcommand{\irr}{\mathrm{irr}}

\newcounter{memoire}


\startcontents[severi]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[severi]{}{1}[2]{}


\bigskip
This lecture is devoted to the study of logarithmic Severi varieties
of a pair $(S,R)$, where $S$ is a surface and $R$ is a curve on $S$:
these are the families of curves on $S$ with prescribed homology
class and geometric genus, and prescribed contact pattern with $R$,
meaning that contact orders with $R$ are prescribed both
at fixed assigned points and at unassigned, a priori mobile, points.
Logarithmic Severi varieties are often referred to as relative Severi
varieties.

Logarithmic Severi varieties naturally appear as irreducible
components of limit Severi varieties in degenerations of smooth
surfaces, see \cite{01.ciro}.
The emblematic example is that of logarithmic Severi varieties of the
pair $(\P^2, \text{line})$ appearing in degenerations of Severi
varieties of plane curves of a given degree and genus, see
\cite{04.concettina}
and \cite{08.th-exem} in this collection.
On the other hand, in degenerations of $K3$ surfaces we will rather
encounter logarithmic Severi varieties of pairs $(S,R)$ such that
$K_S+R=0$, see Section \ref{s:logK3}.

The central result of this text is Theorem~\ref{T}.
On the one hand it gives the
expected dimension of logarithmic Severi varieties, together with a
condition ensuring that this is indeed the actual dimension. On
the other hand it gives various regularity properties of the general
members of logarithmic Severi varieties, under suitable assumptions on
the positivity of $-K_S$ with respect to the prescribed homology class
and contact conditions with $R$.

Another important result is Proposition~\ref{pr:charact}, which
characterizes logarithmic Severi varieties as essentially the families
of curves of maximal dimension with respect to the homology class, the
genus, and the number of moving contact points with $R$, under a
positivity assumption on the logarithmic canonical divisor
$-(K_S+R)$.
It will be used in subsequent lectures to prove
(in specific situations)
that the irreducible components of a degeneration of logarithmic
Severi varieties are again logarithmic Severi varieties
(or rather, irreducible components thereof).

The main source for this lecture is
Caporaso and Harris' \cite[\S 2]{ch};
slightly earlier important works are \cite{zariski} and
\cite{AC81}. I have adapted the presentation
given in \cite{ch},
which is restricted to the pair consisting of the projective
plane and a line, in order to make it fit to the more general
situation studied here, and needed further in this volume.
My treatment is very much inspired by \cite{DS15}, which I worked out
together with Edoardo Sernesi, see also \cite{02.edoardo} earlier in
this volume.
I have included many examples throughout, with the two purposes of
clarifying the subtleties of the various definitions and statements,
and of putting these results in perspective.

The organization of the text is as follows.
Section~\ref{S:results} is devoted to the definition of logarithmic
Severi varieties and the statement of the main theorem \ref{T}, and
Section~\ref{S:deformation} contains the material in
deformation theory necessary for the proof of the main theorem, which
is given in Section~\ref{S:proofT}.
Section~\ref{S:dim-charact} is devoted to the aforementioned
Proposition~\ref{pr:charact} characterizing logarithmic Severi
varieties by the maximality of their dimensions, and its proof.
Finally, Section~\ref{S:examples} is devoted to expanded examples,
featuring many examples of superabundant logarithmic Severi varieties,
and highlighting some specificities of the case when the logarithmic
canonical divisor $K_S+R$ is trivial;
we also point out some interesting applications of logarithmic Severi
varieties (\eg to the tropical vertex group, and to $\A^1$-curves on
open surfaces obtained as the complement of an anticanonical curve).


\section{Definitions and main results}
\label{S:results}

\paragraph{}
Let $S$ be a nonsingular, projective, connected, algebraic surface over
the field $\C$ of complex numbers, and let $R \subset S$ be a reduced
curve.

By a curve on $S$, we always mean a closed subscheme of $S$ of
pure dimension $1$.
The \emph{geometric genus} of a reduced curve $C$ is the 
(arithmetic) genus of its
normalization $\bar C$, namely 
\[
1 - \chi (\O _{\bar C}) = \sum _{i=1 } ^n g_i -n +1
\]
where $g_1,\ldots,g_n$ are the respective genera of the connected
components $\bar C_1,\ldots,\bar C_n$ of $\bar C$.
Note that with this definition, denoting by $g$ the geometric genus of
$C$, the canonical bundle of the normalization $\bar C$ has degree
$2g-2$, and one has the usual Riemann--Roch Formula on $\bar C$, \ie
\[
  \chi(L) = 1 - g + \deg(L)
\]
for all line bundles on $\bar C$.

For every $\xi \in \NS (S)$ (thus,
$\xi$ is a homology class on $S$ that can be represented by a divisor)
and integer $g$, we consider the space $M _g ^{\xi, \text{bir}}(S)$
parametrizing morphisms
\[
\phi: C \to S
\]
from a smooth genus $g$ curve $C$ (projective, but possibly
disconnected) that are birational on their image, and such that
$\phi_* [C] = \xi$.
The space $M _g ^{\xi, \text{bir}}(S)$ is defined more precisely and
studied in Subsection~\ref{s:M}. 

\par We also consider the locally closed subscheme $V_g ^\xi (S)$ of
$\curve (S)$, consisting of those 
points $[C]$ such that $C$ is a reduced curve having geometric genus
$g$ and homology class $\xi$; 
by $\curve (S)$, we denote the Hilbert scheme of curves on $S$.


\paragraph{}
We denote by $\Nseq$ the set of sequences $\alpha =
[\alpha_1,\alpha_2,\ldots]$ of non-negative integers with all but
finitely many $\alpha_i$ non-zero. 
In practice, we may omit the infinite sequence of zeros at the end.
We may also drop the brackets if only $\alpha_1$ is non-zero.

For all $\alpha \in \Nseq$, we let
\begin{align*}
% \sharp \alpha &= \sharp \{ i : \alpha_i \neq 0\} \,;\\
|\alpha| &= \alpha_1 + \alpha_2 + \cdots \,;\\
I\alpha &= \alpha_1 + 2\alpha_2 + \cdots + n\alpha_n + \cdots.% \,; \\
% I ^\alpha &= 1^{\alpha _1} 2^{\alpha _2} \cdots n^{\alpha _n} \cdots
% \,; \\ % \lcm (\alpha) &= \lcm \{ i: \alpha_i \neq 0 \}
\end{align*}
For all $\alpha,\alpha' \in \Nseq$, we say that $\alpha
\geq \alpha'$ if $\alpha_i \geq \alpha'_i$ for all $i \geq 1$.

By a set $\Omega$ of cardinality $\alpha \in \Nseq$, we mean a
sequence of sets $\Omega = (\Omega_1,\Omega_2,\ldots)$ such that each
$\Omega_i$ has cardinality $\alpha_i$.

\begin{definition}
\label{d:log-severi}
Let $g \in \Z$, $\xi \in \NS (S)$, and $\alpha,\beta \in \Nseq$
be such that
\[
I\alpha + I\beta = \xi \cdot R,
\]
and consider a
set $\Omega = \bigl( \{p _{i,j}\} _{1 \leq j \leq \alpha_i}
\bigr) _{i \geq 1}$ of $\alpha$ points on $R$.\footnote
{If $R$ is reducible one should consider more precise data, specifying
  the distribution of the contact points with $R$ on its various
  components: let $R_1,\ldots,R_n$ be the irreducible components of
  $R$; one should consider $\alpha_1,\ldots,\alpha_n \in \Nseq$
  and  $\beta_1,\ldots,\beta_n \in \Nseq$ such that
  $I\alpha_i + I\beta_i = \xi \cdot R_i$ for all $i=1,\ldots,n$,
  and $\Omega_1,\ldots,\Omega_n$ sets of points on $R_1,\ldots,R_n$
  respectively, with cardinalities $\alpha_1,\ldots,\alpha_n$.
For the purposes of this chapter we can safely ignore this, and we
will do so for obvious reasons of simplicity.
(There will be, however, some examples with reducible $R$, in
Section~\ref{S:examples} most notably, and then of course we will 
consider data with the necessary precision).
}

We define $M_g^\xi (\alpha,\beta)(\Omega)$ as the locally closed
subset of $M_g^{\xi,\text{bir}}(S)$ consisting of those $[\phi: C \to
S]$ such that the intersection
$\phi(C) \cap R$ is proper and contained in the smooth locus of $R$,
and there exist $\alpha$ points $q _{i,j} \in C$, $1 \leq j
\leq \alpha_i$, and $\beta$ points $r _{i,j} \in C$, $1 \leq j \leq
\beta_i$, such that
\begin{gather}
\label{C1-def}
\forall\, 1 \leq j \leq \alpha_i:
\quad \phi (q_{i,j}) = p_{i,j} 
%\end{equation}
\qquad and \\
%\begin{equation}
\label{C2-def}
\phi^* R = \sum _{1 \leq j \leq \alpha_i} i \, q_{i,j}
+ \sum _{1 \leq j \leq \beta_i} i\, r_{i,j}.
\end{gather}
\end{definition}

Note that this definition is functorial. In other
words, $M_g^\xi (\alpha,\beta)(\Omega)$ represents a certain functor,
see \ref{p:deform-tg}.

\begin{remark}
We emphasize that we do not assume the points in $\Omega$ to be
general, and neither do we in the Main Theorem~\ref{T} below.
It will be important for some applications to have this flexibility. 
\end{remark}


\begin{definition}
\label{d:log-severi:curve}
Continuing with the situation of Definition~\ref{d:log-severi},
we let ${V}_g ^\xi (\alpha,\beta)(\Omega)$
be the locally closed subscheme of $V_g^\xi(S)$ consisting of those
points $[C]$ such that the normalization $\nu: \bar C \to C \subset S$
belongs to $M_g^\xi (\alpha,\beta)(\Omega)$. 
We call it a \emph{logarithmic\footnote
{in \cite{ch} it is a called a \emph{generalized} Severi variety; the
  terminology \emph{relative} Severi variety is nowadays quite
  popular; I prefer the term \emph{logarithmic} which refers to the
  fact that we consider pairs instead of ``absolute'' surfaces, whereas
  \emph{relative} often refers to the consideration of a map (or a
  family) instead of a surface.}
Severi variety} of the pair
$(S,R)$.
\end{definition}


\paragraph{Notation, examples, and comments}
\label{sp:notation}
In practice we will try to find a balance between rigorous and
decipherable notation. For instance we will frequently drop the
$\Omega$, and replace $\xi$ with an adequate shorthand.


\begingroup
\def\p{\mathrm{p}}
Let us consider the emblematic case when $S=\P^2$ and $R$ is a line.
Let $\xi=d [H]$ with $[H]$ the hyperplane class; we shall simply
denote $\xi$ by $d$.
For example, for all $g$, we may write $V_g^d\bigl( [0,1], d-2\bigr)$
for the family of plane $d$-ics
of genus $g$,
tangent to the line $R$ at some prescribed general point $p\in R$
(in this case, $\Omega=\{p\}$).

Let $\p(d)$ be the arithmetic genus of plane curves of degree
$d$.
The logarithmic Severi variety
$V_{\p(d)}^d\bigl( [0,1], d-2\bigr)$
parametrizes smooth $d$-ics tangent to $R$ at $p$; it has codimension
$2$ in the linear system $|dH|$.
The logarithmic Severi variety $V_{\p(d)-1}^d\bigl( [0,1], d-2\bigr)$
parametrizes plane $d$-ics of cogenus $1$, tangent to $R$ at $p$; it
has codimension $3$ in the linear system $|dH|$
(hence $V_{\p(d)-1}^d\bigl( [0,1], d-2\bigr)$ is a divisor in 
$V_{\p(d)}^d\bigl( [0,1], d-2\bigr)$), and its general
member is a curve with one node at a general point of $\P^2$, as we
will see.

We emphasize that
% On the other hand, the family $W$ of plane $d$-ics with a
% node at the point 
% $p$ has codimension $3$ in $|dH|$ as well, and is a
% divisor in the logarithmic Severi variety $V_{\p(d)}^d\bigl( [0,1],
% d-2\bigr)$. However $W$ is not part of 
% $V_{\p(d)-1}^d\bigl( [0,1], d-2\bigr)$,
% as 
Definition~\ref{d:log-severi} requires that curves in 
$V_{\p(d)-1}^d\bigl( [0,1], d-2\bigr)$ have one local branch
with the prescribed order two of contact with $R$ at $p$; we
illustrate this below. 
%Figure~\ref{fig:illus-def}.

\begin{center}
\begin{minipage}{\textwidth}
\ \hfill \begin{minipage}[b]{40mm}
\centering
\includegraphics[height=20mm]{illus1}\\
not in $V_{p(d)-1}^d\bigl( [0,1]\bigr)$
\end{minipage}
\hfill
\begin{minipage}[b]{40mm}
\centering
\includegraphics[height=20mm]{illus2}\\
in $V_{p(d)-1}^d\bigl( [0,1]\bigr)$
\end{minipage}
\hfill
\begin{minipage}[b]{40mm}
\centering
\includegraphics[height=11mm]{illus3}\\[2mm]
in $V_{p(d)-1}^d\bigl( [0,1]\bigr)$
\end{minipage}
\ \hfill
%\captionof{figure}{Member of}
\end{minipage}
\end{center}

Another subtlety of Definition~\ref{d:log-severi} worth noting is the
following. Consider the logarithmic Severi variety
$V = V_{\p(d)}^d\bigl( 1, [d-3,1]\bigr)$:
loosely speaking, it parametrizes curves passing through an assigned
point on $R$, call it $p$, and tangent to $R$. However, looking
closely at the definition, one sees that a curve that is simply
tangent to $R$ at $p$ and otherwise intersects it transversely does
not belong $V$; a curve having an order $3$ contact at $p$ and
otherwise transverse does belong to $V$, on the other hand.

\endgroup
% local \def\p

\medskip

\noindent
The following is the main result of this chapter.
It is a vast generalization of the result proved independently by
Arbarello and Cornalba \cite{AC80}
and Zariski \cite{zariski} for plane curves of fixed degree and genus.

\begin{theorem}
\label{T}
\pointlessenum
% from package paralist
% no point after enumi
Let $g \in \Z$, $\xi \in \NS (S)$, $\alpha,\beta \in \Nseq$,
and $\Omega = \{p _{i,j}\} _{1 \leq j \leq \alpha_i} \subset R$ be as in
Definition~\ref{d:log-severi}, and consider an irreducible component $V$ of
${V}_g ^\xi (\alpha,\beta)(\Omega)$.
Let $[C]$ be a general member of $V$, $\phi: \bar C \to C
\subset S$ its normalization, $q_{i,j}$ ($1 \leq j \leq \alpha_i$),
$r_{i,j}$ ($1 \leq j \leq \beta_i$) points on $\bar C$ such that
\eqref{C1-def} and \eqref{C2-def} hold.
Set
\begin{equation*}
D= \sum _{1 \leq j \leq \alpha_i} i \, q_{i,j}
+ \sum _{1 \leq j \leq \beta_i} (i-1)\, r_{i,j}.
\end{equation*}

{\renewcommand{\thesubparagraph}{(\thesection.\arabic{paragraph}.00)}
\smallskip\subparagraph{} \label{P00}
One has
\begin{equation*}
\dim V \geq -(K_S+R) \cdot \xi +g-1 +|\beta|.
\end{equation*}
}%

\setcounter{subparagraph}{-1}
\smallskip\subparagraph{} \label{P0}
If
$-K_S \cdot C_i - \deg \left. \phi_* D\right|_{C_i} \geq 1$
for every irreducible component $C_i$ of $C$,
then the inequality in \ref{P00} above is an equality.

\smallskip\subparagraph{} \label{P1}
If
$-K_S \cdot C_i - \deg \left. \phi_* D\right|_{C_i} \geq 2
\ \text{for every irreducible component $C_i$ of $C$},$
then:
\begin{compactenum}
\renewcommand{\theenumi}{\normalfont (\alph{enumi})}
{\renewcommand{\theenumi}
      {{\normalfont ($\rm\alph{enumi}^{\flat\kern -.3ex \flat}$)}}
\item \label{t:a--} 
\newcounter{Ta} \setcounter{Ta}{\value{enumi}}
the normalization map $\phi$ is an immersion, except
possibly at the points $r_{i,j}$;
}
\item \label{t:b}
the points $q_{i,j}$ and $r_{i,j}$ of $\bar C$ are pairwise
  distinct;
{\renewcommand{\theenumi}{{\normalfont ($\rm\alph{enumi}^\flat$)}}
\item \label{t:c-}
\newcounter{Tc} \setcounter{Tc}{\value{enumi}}
none of the points $s_{i,j} := \phi (r_{i,j})$ belongs to
$\Omega$;
}
\item \label{t:e}
for every curve $G \subset S$ and finite set $\Gamma \subset S$
  such that $(G\cup \Gamma) \cap \Omega = \emptyset$, if $[C]$ is
  general with respect to $G$ and $\Gamma$, then $C$ intersects
  $G$ transversely and does not intersect $\Gamma$.
\setcounter{memoire}{\value{enumi}}
\end{compactenum}

\smallskip\subparagraph{} \label{P2}
If
$-K_S \cdot C_i - \deg \left. \phi_* D\right|_{C_i} \geq 3
\ \text{for every irreducible component $C_i$ of $C$},$
then:
\begin{compactenum}
\renewcommand{\theenumi}{\normalfont (\alph{enumi})}
\setcounter{enumi}{\value{Ta}-1}
{\renewcommand{\theenumi}{\normalfont ($\rm\alph{enumi}^\flat$)}
\item \label{t:a-}
the normalization map $\phi$ is an immersion;
}
\setcounter{enumi}{\value{Tc}-1}
\item \label{t:c}
the points $p_{i,j}$ and $s_{i,j}=\phi(r_{i,j})$ on $C$ are
  pairwise distinct;
\setcounter{enumi}{\value{memoire}}
\item \label{t:d}
the curve $C$ is smooth at its intersection points with $R$.
\end{compactenum}

\smallskip\subparagraph{} \label{P3}
If
$-K_S \cdot C_i - \deg \left. \phi_* D\right|_{C_i} \geq 4
\ \text{for every irreducible component $C_i$ of $C$},$
then
\begin{compactenum}
\renewcommand{\theenumi}{\normalfont (\alph{enumi})}
\setcounter{enumi}{\value{Ta}-1}
\item \label{t:a}
the curve $C$ is nodal.
\end{compactenum}
\end{theorem}


The tangent space of $V_g^\xi(\alpha,\beta)(\Omega)$ at the
general point $[C]$ of $V$ is described in Remark
\ref{rk:tg-logSeveri} under the assumptions of \ref{P2},
and in Paragraph \ref{rk:tg-logSeveri0} under the weaker assumptions
of \ref{P0}.

We emphasize once again that it is not required in the above statement
that the set $\Omega$ be general. The only requirement is that the
points in $\Omega$ be smooth points of $R$, which in turn is imposed
by the requirement, in 
Definitions \ref{d:log-severi}
and \ref{d:log-severi:curve},
that the intersection with $R$ be proper and contained in the smooth
locus of $R$.

% It is most likely possible to adapt these definitions to authorize
% intersection with $R$ at singular points, but then one probably wants
% to introduce some condition in order to avoid, say, that a
% prescribed order two
% contact with $R$ be accounted for by intersecting $R$ at one of its
% double points. We won't need this in this volume, so I don't dwell on
% this. 

We will see examples in Section~\ref{S:examples} of the effect that
imposing the passing through a set $\Omega$ of non-general points may
have. 
We will also see examples of components of
Severi varieties parametrizing reducible curves, for which the
assumption of \ref{P0} fails for one irreducible component $C_i$,
and having dimension strictly larger than expected
(\ie the inequality in \ref{P00} is strict).


\section{Background from deformation theory}
\label{S:deformation}

Throughout this section, we consider a 
nonsingular, connected, projective surface $S$, defined over $\C$.


% \etocsetnexttocdepth{3}
% \etocsettocstyle{\bfseries\large Local contents \vspace{1mm}}{}
% \cftsubsecindent 0pt
% \localtableofcontents

\subsection{Deformations of maps with fixed target}
\label{s:M}

\paragraph{}
\label{p:deform-funct}
Let $\phi : C \to S$ be a non-constant morphism from a smooth
projective curve $C$. A \emph{deformation of $\phi$ with fixed target}
over a pointed base $(B,0)$ is the data of a deformation 
\smash{${\cal C} \xrightarrow {\pi} B$} of
$C$ over $(B,0)$ together with a morphism $\Phi : {\cal C} \to S
\times B$ of $B$-schemes, such that the restriction of $\Phi$ over $0$
equals $\phi$.

This defines the \emph{deformation functor} $\Def _{\phi/S}$ of $\phi$
with fixed target $S$. It is prorepresented by a complete local
$\C$-algebra $R_\phi$, see \cite[Thm.~3.4.8]{eS06}.

\paragraph{}
\label{p:Nbar}
The deformations of $\phi$ with fixed target $S$ are controlled by the
\emph{normal sheaf of $\phi$}, \ie the sheaf $N_\phi$ of
$\O_{C}$-modules defined by the exact sequence on $C$
\begin{equation}\label{normal-phi} 0 \to T_{C} \xrightarrow{d\phi}
\phi^*T_S \to N_\phi \to 0\ :
\end{equation}
the spaces $H^0(C,N_\phi)$ and $H^1 (C, N_\phi)$ are
respectively the Zariski tangent space and an obstruction space for
the deformations of $\phi$ with fixed target $S$.
In particular, we have
\begin{equation}
\label{dim-Rphi}
\chi(N_\phi) \leq \dim  R_\phi %\dim _{[\phi]} M_ {g(C)} ^{\phi_* [C]} (S)
\leq h^0(N_\phi).
\end{equation}

\paragraph{}
The rank $1$ sheaf $N _\phi$ may have torsion. We denote by ${\cal H} _\phi$
its torsion part and by $\bar N _\phi$ its maximal torsion-free
quotient; they fit in an exact sequence
\begin{equation}
0 \to {\cal H}_\phi \to N_\phi \to
\bar{N}_\phi \to 0.
\end{equation}
The torsion sheaf ${\cal H}_\phi$ is supported on the divisor $Z$ of
zeroes of the differential $d\phi$, and it is zero if and only if
$Z=0$,
\ie if and only if the differential $d\phi$ is everywhere
non-vanishing; in this case, we say that $\phi$ is an immersion.
Moreover,
there is an exact sequence of locally free sheaves on $C$
\begin{equation}
\label{red-normal}
0 \to
T _{C} (Z) \to \phi ^* T_S \to
{\bar N} _\phi
\to 0,
\end{equation}
which readily implies the identification of line bundles on $C$
\begin{equation}
\label{Nbar}
\bar N _\phi \cong \omega_C \otimes \phi^* \omega_S ^{-1} (-Z).
\end{equation}


\paragraph{The scheme of morphisms}
\label{p:constr-Hom}
We will pretend in this text that the global deformation functor of
maps from smooth genus $g$ curves to the surface $S$ is represented by
a scheme, which we will denote by $M_g(S)$.
This comports the existence of a family
${\cal U} \to M_g(S)$ of smooth genus $g$ curves defined over
$M_g(S)$, and of a universal morphism
$\Phi: {\cal U} \to S \times M_g(S)$.

It is not strictly true that the global deformation functor of genus
$g$ maps to $S$ is representable in the category of schemes, but it
will be harmless for our purposes to pretend it is: one possible way
to make things rigorously work out is to use Hartshorne's modular
families \cite[Def. p.171]{hartshorne-def}, as in
\cite[Subsec.~2.1]{DS15}.
A modular family of curves of genus $g$ is a surrogate of a universal
family of curves of genus $g$. Let us consider such a modular family
$\mathcal{C}_g / \mathcal{M}_g$, with the abuse of notation of
denoting its base $\mathcal{M}_g$ although it is not the moduli space
of genus $g$ curves.
Then we may work with the scheme
$\Hom _{\mathcal{M}_g} \bigl( \mathcal{C}_g,\, S \times
\mathcal{M}_g)$ as a surrogate for $M_g(S)$,
with $\Hom$ defined as in \cite[Thm.~I.1.10]{jK96}.
We will not enter in these technicalities here, and refer the reader
to \cite[Subsec.~2.1]{DS15} for the complete details.

In this text, we will be mostly interested in the following subspace
of $M_g(S)$.
For all $\xi \in \NS (S)$,
we consider $M _g ^{\xi, \text{bir}}(S)$ the subspace of $M_g(S)$
parametrizing morphisms $\phi$
that are birational on their image, and such that
$\phi_* [C] = \xi$.



\subsection{Comparison of the spaces of maps and curves}

Let $\xi \in \NS (S)$, and $g$ be a non-negative integer.

\paragraph{From maps to curves}
\label{p:maps-curves}
Consider the universal morphism
$\Phi: {\cal U}_M \to S \times M_g ^{\xi, \text{bir}}$
defined over $\Mgbir$.
Let $\bar M$ be the semi-normalization of
the reduced scheme underlying $\Mgbir$, 
% $\bar {\cal U}_M$ the
% normalization of ${\cal U}_M \times _{\Mgbir} \bar M$, 
$\bar {\cal U}_M := {\cal U}_M \times _{\Mgbir} \bar M$
the base change of the universal family ${\cal U}_M$, 
and
$\bar \Phi : \bar {\cal U}_M \to S \times \bar M$ the induced morphism
of $\bar M$-schemes.
I claim that the scheme-theoretic image $\bar \Phi (\bar
{\cal U}_M)$ is flat over $\bar M$.

Indeed, the morphism $\varpi:=\mathrm{pr}_2: \bar \Phi (\bar {\cal
U}_M) \to \bar M$ is a well-defined family of codimension $1$
algebraic cycles of $S$ in the sense of \cite[I.3.11]{jK96}.  Since
$\bar M$ is normal, the claim follows from \cite[I.3.23.2]{jK96}.

It follows that there is a morphism from $\bar M$ to the Hilbert
scheme of curves on $S$. It factorizes through $V_g
^\xi(S)$, and actually through the normalization
$\bar V_g ^\xi \to V_g ^\xi$ by
the universal property of the normalization.  Since by definition the
semi-normalization morphism $\bar M \to \Mgbir$ is $1:1$, two points
$[\phi:C\to S], [\phi':C'\to S] \in \bar M$ are mapped
to the same point $[\Gamma] \in V_g^\xi$ if and only if there exists
an isomorphism $\iota:C \cong C'$ such that $\phi = \phi' \circ \iota$.

% Phrase suivante expurgée car trop cryptique~:
%
% To draw a precise conclusion about the morphism $\bar M \to V_g ^\xi$
% from this, it is necessary to specify precisely who is $\Mgbir$; we
% will need and state less, see Prop.~\ref{pr:comparison}.


\paragraph{From curves to maps}
\label{p:curves-maps}
On the other hand, consider the universal family ${\cal U}_V \to
V_g^\xi$ of curves gotten from the universal family over the Hilbert
scheme of curves on $S$. Let $\bar V$ be the normalization of
$V_g^\xi$, and $\bar {\cal U}_V$ the normalization of ${\cal U}_V
\times _{V_g ^\xi} \bar V$. Teissier's Résolution Simultanée Theorem
\cite{bT80} asserts that $\bar {\cal U}_V \to \bar V$ is a family of
smooth genus $g$ curves; it comes with a morphism of $\bar V$-schemes
\[
\bar {\cal U}_V \to 
{\cal U}_V \times _{V_g ^\xi} \bar V
\subset S \times \bar V.
\]
It follows that there is a morphism from $\bar V$ to the space
$\Mgbir$. It is generically injective, because the universal family of
curves over $V_g^\xi$ is nowhere isotrivial.

\bigskip % \vparskip
From the considerations in \ref{p:maps-curves} and
\ref{p:curves-maps} above, one deduces the following.
\begin{proposition}
\label{pr:comparison}
Let $[\phi:C \to S] \in \Mgbir (S)$ be  a general  point 
(i.e., a general point of any irreducible component of $\Mgbir (S)$).
Let $\Gamma:= \phi(C)$, $\xi \in \NS (S)$ the homology class of
$\Gamma$, and $g$ its geometric genus.
Then
$[\Gamma]$ belongs to a unique irreducible component of $V^\xi_g$ and  
\[
\dim_{[\Gamma]} V^\xi_g
= \dim R_{\phi}.
\]
\end{proposition}

\noindent
(Recall that $R_{\phi_0}$ is the complete local $\C$-algebra that
prorepresents $\Def_{{\phi}/S}$).

% \begin{proposition}
% \label{pr:comparison}
% Let $g \in \Z$, $\xi \in \NS (S)$.
% The respective normalizations $\bar M_g ^{\xi, \text{bir}}$ and $\bar
% V_g ^\xi$ of $M_g ^{\xi, \text{bir}} (S)$ (i.e., that of its
% underlying reduced scheme) and $V_g ^\xi (S)$ are isomorphic.
% \end{proposition}

% \subparagraph{Warning}
% \label{w:comparison} The above statement is presumably a little too
% bold, since we need the existence of a universal family over $M_g
% ^{\xi, \text{bir}} (S)$ (compare \ref{p:constr-Hom}) to prove it. As
% already said, we shall not discuss this here; it is in any event true
% that there exist Zariski dense open subsets of $M_g ^{\xi, \text{bir}}
% (S)$ and $V_g ^\xi (S)$ the normalizations of which are isomorphic,
% which is already much more than we need.

\medskip
The next result provides a sharper upper bound on the
dimension of the Severi varieties than that given by the inequality
$\dim R_\phi \leq h^0(N_\phi)$ in \eqref{dim-Rphi}.

Let $\phi : C \to S$ be a morphism from a smooth projective curve $C$,
birational onto its image $\Gamma$.  Let $\xi \in \NS (S)$ be the
homology class of $\Gamma$, and $g$ its geometric genus.  We consider
$\Phi : {\cal C} \to S \times B$ a deformation of $\phi$ over a
pointed normal connected scheme $(B,0)$. Then $\Phi (\mathcal{C})
\subset S \times B$ is a deformation of $\Gamma$ over $(B,0)$, see
\ref{p:maps-curves}. There are thus two classifying morphisms $\kappa$ and
$\gamma$ from $(B,0)$ to $\Mgbir (S)$ (or $R_\phi$) and $\curve (S)$
respectively, with differentials
\[ d\kappa : T_{B,0} \to H^0 (C, N _{\phi})
\quad \text{and} \quad
d\gamma : T
_{B,0} \to H^0 (\Gamma, N _{\Gamma /X}).
\]
\begin{lemma}
\label{l:ac} %AC = entrambi Arbarello--Cornalba e assai curioso 
The inverse image by $d\kappa$ of the torsion $H^0 (C, \mathcal{H}_{\phi})
\subset H^0 (C, N _{\phi})$ is contained in the kernel of $d\gamma$.
\end{lemma}

\begin{proof} Given a non-zero section $\sigma \in H^0(C,N_{\phi})$,
the first order deformation of ${\phi}$ defined by $\sigma$ can be
described in the following way: consider an affine open cover
$\{U_i\}_{i\in I}$ of $C$, and for each $i \in I$ consider a lifting
$\theta_i\in C(U_i,{\phi^*}T_X)$ of the restriction
$\sigma_{|U_i}$. Each $\theta_i$ defines a morphism
\[ \tilde \phi _i: U_i\times \mathrm{Spec}(\C[\epsilon])\to S
\] extending ${\phi}_{|U_i}: U_i\to X$.  The morphisms $\tilde \phi
_i$ are then made compatible after gluing the trivial deformations
$U_i\times \mathrm{Spec}(\C[\epsilon])$ into the first order
deformation of $C$ defined by the coboundary $\partial(\sigma) \in
H^1(C,T_{C})$ of the exact sequence \eqref{normal-phi}. In case
$\sigma \in \H^0(C,{\cal H}_{\phi})$, everyone of the maps $\tilde
\phi _i$ is the trivial deformation of $\sigma_{|U_i}$ over an open
subset. This implies that the corresponding first order deformation of
${\phi}$ leaves the image fixed, hence the vanishing of $dq_0
(\sigma)$.
\end{proof}

\vspace{-2ex}
\begin{corollary}
\label{c:ac} Let $g\in \Z$, $\xi \in \NS (S)$.  Let $[C]$ be a general
point of $V_g^\xi$, and $\phi: \bar C \to C \subset S$ its
normalization. Then
\[ \dim V_g ^\xi \leq h^0(\bar C, \bar N _\phi).
\] 
% Let $[\phi:C \to S] \in \Mgbir (S)$ be a general point.  
% Then $\dim R_\phi \leq h^0(C, \bar N _\phi)$.
\end{corollary}

\begin{proof} By generality we may assume that $[C]$ is a smooth point
of $V_g^\xi$. Then $\dim V_g ^\xi = \dim T _{[C]} V_g^\xi$, and by
\ref{p:curves-maps} there is a map
\[ d\kappa _{[\phi]}: T _{[C]} V_g^\xi \to H^0(\bar C, N _\phi).
\] It is injective because to every tangent vector $\theta \in T
_{[C]} V$ corresponds a non-trivial deformation of $C$.  On the other
hand, it follows from Lemma~\ref{l:ac} that $\operatorname{Im}
d\kappa_{[\phi]} \subset H^0 (\bar C, \bar N _{\phi})$.
\end{proof}

Lemma~\ref{l:ac} 
(see also \cite[Lemma \tref{lem:Arbarello-Cornalba}]{02.edoardo})
is a crucial observation (and indeed one of the cornerstones
of the proof of Theorem~\ref{T}) that was made by Arbarello and Cornalba
\cite[p. 26]{AC81}, who deemed it a \emph{fenomeno assai
curioso}. They write: <<~nel caso in cui $\phi$ sia una birazionalità
tra $C$ e $\Gamma$, la presenza di ``cuspidi'' su $\Gamma$, comporta
l'esistenza, dal punto di vista infinitesimo, di più di un modello
liscio della curva $\Gamma$, se così ci possiamo
esprimere.~>>\footnote {a very curious phenomenon; in the case when
$\phi$ is birational between $C$ and $\Gamma$, the presence of
``cusps'' on $\Gamma$ comports the existence, at the infinitesimal
level, of more than one smooth model of the curve $\Gamma$, if we may
say so.}
\par Next, paraphrasing them, in order to use this phenomenon
constructively they establish \cite[Cor.~6.11]{AC81}: in the above
notation, if $B$ is the
complex unit disk and if the family of curves is \emph{equisingular},
then $d\kappa(\partial / \partial t)$ belongs to $H^0 (C,
\mathcal{H}_{\phi})$ if and only if it is zero. Later, Caporaso and
Harris (together with J. de Jong, they write) state and prove
\cite[Lem.~2.3]{ch}. They add the remark that this is linked to the
notion of equisingularity, even though they make absolutely no use of
that notion, neither in their statement nor in its proof.

\par The treatment I give above is that of Sernesi and myself in
\cite{DS15}. Although essentially equivalent to that of \cite{ch}, it
slightly differs in its formulation. This formulation, I hope,
sheds some light on what is actually going on, and in particular
shows that it is not necessary to invoke equisingularity
in order to prove Corollary~\ref{c:ac}.

The standard application of Corollary~\ref{c:ac} is to the proof that
curves in a given family are immersed, \ie they have no cusps:
we will use it in Paragraph \ref{p:P1}
below to prove assertion \ref{t:a--} of Theorem \ref{T}.

\subsection{Tangency conditions with respect to a fixed curve}

We consider $R$ a fixed reduced curve on $S$.
In this subsection we study deformations of curves on $S$ satisfying
some tangency conditions with $R$; it follows from our
Definition~\ref{d:log-severi} that it suffices to treat the case when
$R$ is smooth.


\paragraph{}
\label{p:deform-tg}
Let $m$ be a non-negative integer.
Let $\phi : C \to S$ be a non-constant morphism from a smooth
projective curve $C$. A deformation of $\phi$ with fixed target
\emph{preserving a tangency of order $m$ with $R$} over
a pointed base $(B,0)$ is a deformation $\Phi : {\cal C} \to S \times
B$ of $\phi$ with fixed target as in \ref{p:deform-funct}, such that
there exists a section $Q$
of ${\cal C} \to B$ such that
the pulled-back divisor $\Phi^* R$
contains $Q$ with multiplicity $m$ (\ie
$\Phi^* R - m Q \geq 0$).
\[\xymatrix@=15pt{
{\cal C} \ar[d] _\pi \ar[r] ^(.35)\Phi & S \times B \ar[dl] ^{\pr_2}
\\
\ar@/^1pc/[u] ^{Q}
B
}\]

The tangency is said to be respectively at a 
\emph{fixed point} $p \in R$ if
$\Phi(Q)= \{p\} \times B$, and at a 
\emph{variable point} if
$\pr_1 \circ \Phi (Q)$ is a curve.

We say that a family of maps $\Phi: {\cal C} \to S \times B$ preserves
a tangency of order $m$ with $R$ if for all $b\in B$ it is locally
around $b$ a
deformation of maps preserving a tangency of order $m$.

% % ci-dessous version précédente
% % avec des contorsions pour définir une espèce de foncteur des
% % déformations à partir d'une définition locale
% % (contorsions peut-être inutiles, d'ailleurs)
% \paragraph{}
% \label{p:deform-tg}
% Let $\phi : C \to S$ be a non-constant morphism from a smooth
% projective curve $C$. A deformation of $\phi$ with fixed target
% \emph{preserving a tangency of order $m$ with $R$} over
% a pointed base $(B,0)$ is a deformation $\Phi : {\cal C} \to S \times
% B$ of $\phi$ with fixed target as in \ref{p:deform-funct} such that
% there exists an open neighbourhood $B^\circ$ of $0$ and a section $Q^\circ$
% of ${\cal C}^\circ := {\cal C} \times_B B^\circ \to B^\circ$ such that
% the pull-back divisor $(\Phi^* R) ^\circ := \Phi^* R \cap {\cal
%   C}^\circ$ contains $Q^\circ$ with multiplicity $m$ (i.e.\ 
% $(\Phi^* R) ^\circ - m Q^\circ \geq 0$).
% \[\xymatrix@=15pt{
% {\cal C}^\circ \ar[d]  \ar@{}[r]|{\subset}
% & {\cal C} \ar[d] _\pi \ar[r] ^(.35)\Phi & S \times B \ar[dl] ^{\pr_2}\\
% B^\circ \ar@{}[r]|{\subset} \ar@/^1pc/[u] ^{Q^\circ} & B
% }\]

% The tangency is said to be respectively at a fixed point $p \in R$ if
% $\Phi(Q^\circ)= \{p\} \times B^\circ$ and at a variable point if
% $\pr_1 \circ \Phi (Q^\circ)$ is a curve.

% \smallskip
% \subparagraph{Remark.} It is too strong a condition to impose that
% there be a section $Q$ of ${\cal C} \to B$ over the whole $B$
% satisfying the above requirement, as
% there may be monodromy. This is not relevant if one only considers
% local deformations. 


\bigskip % \vparskip
The following result displays the additional conditions the class of a
deformation of maps has to meet for this deformation to preserve a
tangency with $R$. It is \cite[Lem.~2.6]{ch}.
%\par 
Let $B$ be a {reduced} scheme,
and $\Phi : {\cal C} \to S \times B$ be a family of maps preserving a
tangency with $R$ of order exactly $m$.
Let $b \in B$ be a general point, and $\phi: C \to S$ be the
corresponding map.
This comes with a classifying
map $\kappa$, with differential $d\kappa: T_0B \to H^0(C,N_\phi)$;
we call $\bar d\kappa$ its composition with the projection
$H^0(C,N_\phi) \to H^0(C,\bar N_\phi)$.
\par Let $q:=Q \cap C$, and $l-1$ be the order of vanishing of the
differential $d\phi$ at $q$ (\ie $l$ is the multiplicity of the point
$p:=\phi(q)$ in the local branch of $\phi(C)$ corresponding to $q$).
Note that necessarily $l\leq m$.

\begin{lemma}
\label{l:log-tg}
Let $\sigma \in \Img (\bar d \kappa)
\subset H^0(C, \bar N_\phi)$ be a non-zero section, and
denote by $v_q(\sigma)$ its order of vanishing at $q=Q \cap C$.\\
\renewcommand{\thesubparagraph}
{(\arabic{section}.\arabic{paragraph}.\alph{subparagraph})}
\refstepcounter{subparagraph}\label{l:log-tg-gnl}%
{\normalfont (\alph{subparagraph})}
One has $v_q(\sigma) \in \{m-l\} \cup \dlbrack m, +\infty
\dlbrack$.\footnote
{I use the notation
$\dlbrack a,b \drbrack = [a,b] \cap \Z$ for $a,b \in \R \cup \{ \pm
\infty \}$;
albeit being standard probably only in France, it is convenient.} 

\refstepcounter{subparagraph}\label{l:log-tg-fix}
\noindent
{\normalfont (\alph{subparagraph})}
If the tangency is at a fixed point of $R$, then actually 
$v_q(\sigma) \in \dlbrack m, +\infty
\dlbrack$.
\end{lemma}

\begin{proof}
This is a local computation.
Let $(x,y)$ be (analytic) local coordinates on $S$ at $p=\phi(q)$,
such that $R$ is defined by the equation $y=0$. 
Then the vector fields $\partial/\partial x$ and $\partial/\partial y$
generate $T_S$ near $p$, and their pull-backs generate 
$\phi^* T_S$ near $q$; by abuse of notation we shall denote them by 
$\partial/\partial x$ and $\partial/\partial y$ as well.

We may assume that $B$ is a curve. Let $\epsilon$ be a local
coordinate on $B$ centered at $b$, and $t$ be a local equation of the
section $Q$ near $q$. Thus $(t, \epsilon)$ are local coordinates on
${\cal C}$ at $q$. We may assume that $t$ gives a local coordinate on
$C$ at $q$, in such a way that $\phi$ is given locally
by 
\begin{equation*}
\phi(t) = 
\begin{cases}
\bigl(
t^l + a_{l+1} t^{l+1} + \cdots, 
t^m
\bigr),
& \text {if}\ l<m \\
\bigl(
t^n + a_{n+1} t^{n+1} + \cdots, 
t^m
\bigr)
\ \text{for some}\ n\geq m,
& \text{if}\ l=m.
\end{cases}
\end{equation*}
From now on we assume $l<m$ and leave the other, similar, case to the
reader. 
Then the differential of $\phi$ at $q$ is
\begin{align*}
\textstyle
\frac \partial {\partial t} \longmapsto
&
\textstyle
( lt^{l-1} + (l+1)a_{l+1} t^l + \cdots )
\cdot \frac \partial {\partial x}
+ mt^{m-1} \cdot \frac \partial {\partial y}
\\
&
\textstyle
 = t^{l-1} \bigl(
( l + (l+1)a_{l+1} t + \cdots )
\cdot \frac \partial {\partial x}
+ mt^{m-l} \cdot \frac \partial {\partial y}
\bigr).
\end{align*}
We see that around $q$ on $C$, the torsion part ${\cal H}_\phi$ of
$N_\phi$ is a skycraper sheaf of length $l-1$ concentrated at $q$, 
generated by the image in $N_\phi$ of the local section
\[
\textstyle
\tau: t \mapsto 
\bigl( l + (l+1)a_{l+1} t + \cdots \bigr)
\cdot \frac \partial {\partial x}
+ mt^{m-l} \cdot \frac \partial {\partial y}
\]
of $\phi^*T_S$;
thus the torsion-free quotient $\bar N_\phi$ is
generated by the class of $\partial/\partial y$ modulo $\tau$.
Observe that modulo $\tau$, $\partial/\partial x$ equals
$t^{m-l}\cdot \partial/\partial y$ times an invertible, hence the
image of $\partial/\partial x$ in $\bar N_\phi$ vanishes to the order
exactly $m-l$ at $q$.

In turn the family $\Phi$ may be written locally as
\begin{equation*}
\Phi(t, \epsilon) = 
\bigl(
(t^l + a_{l+1} t^{l+1} + \cdots)
+ \epsilon (u_0+u_1t+\cdots) + O(\epsilon^2), 
t^m,
\epsilon
\bigr),
\qquad
\end{equation*}
since $\Phi^*R$ contains $Q$ with multiplicity $m$.
By definition, the corresponding section 
$\bar d \kappa(\partial/\partial \epsilon)$
of $\bar N_\phi$ is 
\[
\textstyle
\bar d \kappa(\frac \partial {\partial \epsilon}) =
(u_0+u_1t+\cdots) \cdot \frac \partial {\partial x} \mod \tau.
\]
Since $\partial / \partial x$ itself vanishes modulo $\tau$ to the
order $m-l$ as we 
have seen, one has
$v_q\bigl(\bar d \kappa(\partial/\partial \epsilon)\bigr) \geq m-l$
in any event.

Moreover, by generality of $b\in B$ we may assume that all
$\Phi(\cdot,\epsilon)$ have their differential vanishing to the order
$l$ at $Q \cap {\cal C}_\epsilon$, which translates into the fact that
$u_1=\cdots=u_{l-1}=0$.
Then $\bar d \kappa(\partial/\partial \epsilon)$
vanishes either to the order $m-l$, if $u_0 \neq 0$, or to some order
larger than $m$, if $u_0=0$.
When the tangency is maintained at a fixed point we are necessarily in
the latter case. The lemma is proved.
\end{proof}

\bigskip % \vparskip
Let ${\cal C} \subset S \times B$ be a family of a reduced curves over
a reduced base $B$. It is said to preserve a tangency of order $m$
with $R$ if the corresponding family of normalization maps over
the normalization $\bar B$ of $B$ (see \ref{p:curves-maps}) does.

\begin{corollary}
\label{c:log-tg}
Let $V \subset \curve (S)$ be a family of curves of genus $g$ having a
tangency of order $m$ with the divisor $R$. Let $[C]$ be a general
member of $V$, $\phi: \bar C \to C \subset S$ be the normalization of
$C$, $q \in \bar C$ the tangency point, and $l-1$ the order of
vanishing of the differential $d\phi$ at $q$. Then
\[
  \dim V \leqslant
  h^0 \bigl( \bar C, \bar N _\phi (-(m-l)_+ \cdot q) \bigr),
\]
where $(m-l)_+$ denotes $\max(m-l,0)$.
If the tangency is at a fixed prescribed point on $R$, then
actually
\[
  \dim V \leqslant
  h^0 \bigl( \bar C, \bar N _\phi (-m \cdot q) \bigr).
\]
\end{corollary}

\begin{proof}
As in the proof of Corollary~\ref{c:ac}, we have $\dim V = \dim T _{[C]} V$
by generality of $[C]$, and there is an injective map $T _{[C]} V \to
H^0(\bar C, \bar N _\phi)$. By Lemma~\ref{l:log-tg} the image of this
map is contained in $H^0 \bigl( \bar C, \bar N _\phi (-a \cdot q)
\bigr)$ with $a=(m-l)_+$ if the tangency is mobile, and $a=m$ if the
tangency is fixed. This ends the proof.
\end{proof}


\section{Proof of the Main Theorem}
\label{S:proofT}

In this section we prove Theorem~\ref{T}. The proof itself is in
Subsection~\ref{s:proof-main}, after we give some lemmas in
Subsection~\ref{s:RR}. 
% fix $g\in\Z$ and $\xi \in \NS(S)$. We consider an
% irreducible component $V$ of $V_g ^\xi$, and its counterpart $M$ in
% $\Mgbir (S)$. Or rather, we assume that $V$ is normal, which enables
% us to view it as the parameter space of a family of morphisms.


\subsection{Applications of the Riemann--Roch formula}
\label{s:RR}

Lemma~\ref{l:RR0} below is standard, but we will also use the more
clever Lemma~\ref{fucking-obs},
which amounts to \cite[Observation 2.5]{ch}.

\begin{lemma}
\label{l:RR0}
Let $X$ be a smooth (possibly disconnected) projective curve,
and $L$ a line bundle on $X$.
Let $k \in \N^*$.
If $\deg\bigl(\restr {L\otimes \omega_X^{-1}} {X_i} \bigr)>k$
for all irreducible component $X_i$ of $X$, then the linear system
$|L|$ separates any $k$ points on $X$.
\end{lemma}

\begin{proof}
Let $Z$ be a subscheme of $X$ of length $k$,
and let $Z'$ be another subscheme of $X$ such that $Z' \subsetneq Z$.
The assumption on the degree of $L$ ensures that both $L(-Z)$ and
$L(-Z')$ are non-special, hence 
$h^0\bigl( L(-Z) \bigr) < h^0 \bigl(L(-Z')\bigr)$
by the Riemann--Roch formula.
\end{proof}

\begin{lemma} \label{fucking-obs}
Let $X$ be a smooth (possibly disconnected) projective curve of genus
$g=1-\chi(\O_X)$, and $L,M$ two line bundles on $X$ such that
\begin{equation*}
\forall\, X_i\ \text{irreducible component of}\ X:
\quad
\deg ( \restr M {X_i}) \leq 
\deg( \restr L {X_i}).
 \end{equation*}
%On note $d$ le degré de $L$.\\
\begin{mycpctenum}
\renewcommand{\theenumi}{\normalfont (\alph{enumi})}
\item \label{fake-nonspec}
If $\deg \left.L \otimes \omega _X^{-1} \right|_{X_i} >0$
for every component $X_i$ of $X$, then
\begin{equation} \label{eq:fake-nonspec}
h^0 (X,M) \leq h^0(X,L) = \deg (L) -g+1.
\end{equation}

\item \label{fake-bpf}
If $\deg \left.L \otimes \omega _X^{-1} \right|_{X_i} >1$
for every component $X_i$ of $X$, then
equality holds in \eqref{eq:fake-nonspec} if and only if $\deg M
= \deg L$.
\end{mycpctenum}
\end{lemma}

\begin{proof}
Assumption \ref{fake-nonspec} ensures that $L$ is non-special, hence
the right-hand-side equality in \eqref{eq:fake-nonspec}, by the
Riemann--Roch formula.
If $M$ is non-special as well, then $h^0(L)-h^0(M)=\deg(L)-\deg(M)$
again by the Riemann--Roch formula, which gives the result in both
cases \ref{fake-nonspec} and \ref{fake-bpf}.

We thus assume from now on that $M$ is special. Then,
\[
h^0(X,M) \leq h^0(X,\omega_X) = g+n-1.
\]
Under Assumption~\ref{fake-nonspec}, 
\[
\deg(L)
= \sum_{i=1}^n \deg (\restr L {X_i})
\geq \sum_{i=1}^n (2g_i-1) = 2g-2+n,
\]
where $n$ is the number of components of $X$ and $g_i$ is the genus of
$X_i$ for all $i=1,\ldots,n$;
recall that $g=\sum g_i -n+1$.
By the Riemann--Roch formula, one has
\[
h^0(X,L)
= \deg (L) -g+1
\geq g-1+n
\]
hence $h^0(X,L) \geq h^0(X,M)$.

Under Assumption~\ref{fake-bpf} one has in the same fashion 
$\deg(L)\geq 2g-2+2n$, hence
\[
h^0(X,L)\geq g +2n-1
> h^0(X,M).
\]
This ends the proof, as the specialty of $M$ implies $\deg(M)<\deg(L)$
under the assumption of \ref{fake-nonspec}, and a fortiori under the
assumption of \ref{fake-bpf}.
\end{proof}

\subsection{Proof of the main theorem}
\label{s:proof-main}

This section is dedicated to the proof of Theorem~\ref{T}.
We consider an irreducible component $V$ of
$V^\xi_g(\alpha,\beta)(\Omega)$
and a general point $[C]$ of $V$, as in the theorem. 
We use freely the notation introduced in the statement.

\paragraph{} \label{p:expdim}
{\itshape
We start by proving that $V$ has expected dimension
\begin{equation} \label{expdim-logsev}
\expdim {V}_g ^\xi (\alpha,\beta)(\Omega)
= -(K_S+R) \cdot \xi +g-1 +|\beta|.
\end{equation}
}

By \eqref{dim-Rphi} the expected dimension of $V_g ^\xi$ is
$\chi(N_\phi)$, which by the Riemann--Roch formula and the exact
sequence \eqref{normal-phi} equals
\begin{equation} \label{expdim-sev}
\expdim V_g ^\xi
 = \deg \omega_{\bar C} - \deg \phi^* \omega_S + 1 - g
= -K_S \cdot C + g-1.
\end{equation}
Now requiring that a curve $C$ have tangency of order $m$ with $R$ at
a specified point $p$ is $m$ linear conditions on the coefficients of
the equation of $C$, and if we let the point $p$ vary along $R$ the
expected codimension of the corresponding locus of curves $C$ is one
less, i.e.\ $m-1$. We thus end up with
\begin{align*}
\expdim \bigl( {V}_g ^\xi (\alpha,\beta)(\Omega) \bigr)
& = \expdim \bigl( V_g ^\xi \bigr) - \sum_i \sum _{1 \leq j \leq \alpha_i} i 
- \sum_i \sum _{1 \leq
 j \leq \beta_i} (i-1) \\
& = \expdim \bigl( V_g ^\xi \bigr) - I\alpha - (I\beta-|\beta|),
\end{align*}
which together with \eqref{expdim-sev} gives 
\eqref{expdim-logsev} after one remarks that $I\alpha + I\beta = R
\cdot \xi$.
\par Note that this proves that, in any event,
\begin{equation} \label{expdim-upbnd}
\dim (V) \geq -(K_S+R) \cdot \xi +g-1 +|\beta|,
\end{equation}
which is assertion \ref{P00}.
\qed

\paragraph{} \label{p:dim-logsev}
{\itshape
We now turn to the proof that the dimension of $V$ equals its expected
dimension under assumption~\ref{P0}.
}

\medskip
Note that the points $q _{i,j}$ are necessarily pairwise distinct
because they have distinct images $p _{i,j} \in R$.
Let us first assume in addition that the points $q _{i,j}$ and $r
_{i,j}$ are all together pairwise distinct; the case when this does
not hold will be dealt with in \ref{p:not-pwise-disjt}.

We set
\begin{equation}
\label{div-tg-cond}
D:= \sum _{1 \leq j \leq \alpha_i} i \, q_{i,j}
+ \sum _{1 \leq j \leq \beta_i} (i-1)\, r_{i,j},
\end{equation}
the divisor on $\bar C$ of ``infinitesimal tangency conditions with
$R$''
(compare \ref{p:expdim}),
and 
\begin{equation}
\label{ramif-var}
D_0 := \sum _{1 \leq j \leq \beta_i} (l_{i,j}-1)\, r_{i,j},
\end{equation}
where $l_{i,j}:= v_{r_{i,j}} (d\phi)$ is
the order of vanishing of the differential $d\phi$ at the point
$r_{i,j}$, \ie $D_0$ is
the ``ramification divisor of $\phi$ in the points $r_{i,j}$''. We
then decompose the difference of these two divisors as
\begin{equation}
D-D_0 = D_1 - D_1'
\end{equation}
where $D_1$ and $D_1'$ are non-negative divisors on $\bar C$ with disjoint
supports; note that $D_1'$ may be nonzero only at the points
$r_{i,j}$, and that it is so if and only if $l_{i,j}>i$.
\par It follows from Corollary~\ref{c:log-tg} that
\begin{equation}
\label{dim-upperbnd}
\dim (V) \leq h^0\bigl(\bar C, \bar N _\phi(-D_1) \bigr).
\end{equation}
Let $Z_0$ be the non-negative divisor on $\bar C$ such that the
ramification divisor of $\phi$ is $D_0+Z_0$. Then by \eqref{Nbar} we
have $\bar N _\phi \cong \omega_{\bar C} \otimes \phi^* \omega_S ^{-1}
(-D_0-Z_0)$, and therefore \eqref{dim-upperbnd} above reads
\begin{align}
\dim (V) & \leq 
h^0\bigl(\bar C, \omega_{\bar C} \otimes \phi^* \omega_S ^{-1}
(-D_0-Z_0-D_1) \bigr) \\
& = h^0\bigl(\bar C, \omega_{\bar C} \otimes \phi^* \omega_S ^{-1}
(-D-D_1'-Z_0) \bigr) \\
 & \leq \label{upbnd-dim}
h^0\bigl(\bar C, \omega_{\bar C} \otimes \phi^* \omega_S ^{-1}
(-D) \bigr).
\end{align}
Now by assumption~\ref{P0}
the line bundle $\omega_{\bar C} \otimes \phi^*
\omega_S ^{-1} (-D)$ is non-special, hence
\begin{align}
h^0\bigl(\bar C, \omega_{\bar C} \otimes \phi^* \omega_S ^{-1}
(-D) \bigr)
& = h^0\bigl(\bar C, \omega_{\bar C} \otimes \phi^* \omega_S(R) ^{-1} 
(\phi^*R -D) \bigr) \\
&= 2g-2 -(K_S+R)\cdot \xi + |\beta| +1-g \\
& =\, \expdim  V_g ^\xi(\alpha,\beta)(\Omega).
\end{align}
We thus have $\dim V \leq \expdim V_g ^\xi(\alpha,\beta)(\Omega)$
which, together with \eqref{expdim-upbnd} implies that $V$ has the expected
dimension, if indeed the points  $q _{i,j}$ and $r
_{i,j}$ are all together pairwise distinct.

\paragraph{} \label{p:not-pwise-disjt}
Now if it is not true that the points $q _{i,j}$ and $r
_{i,j}$ are all together pairwise distinct, then $V$ is actually a
component of some Severi variety $V_g ^\xi(\alpha',\beta')(\Omega')$
with $|\beta'| < |\beta|$ for which the corresponding points $q'
_{i,j}$ and $r' _{i,j}$ are indeed pairwise disjoint 
(as sets $\Omega=\Omega'$, \ie $\bigcup_i \Omega_i = \bigcup_i
\Omega_i'$, and $\Omega_i \subseteq \bigcup_{k\geq i} \Omega'_k$).
% in this case,
% $\Omega'$ is merely obtained from $\Omega$ by some relabeling).
\par Then, setting correspondingly $D'$ as in \eqref{div-tg-cond}, one
gets
$\dim V \leq h^0(\bar C, \omega_{\bar C} \otimes \phi^* \omega_S ^{-1}
(-D'))$ exactly as in \ref{p:dim-logsev}. Now $\deg D' > \deg D$
because $|\beta'| < |\beta|$, and it therefore follows from
Lemma~\ref{fucking-obs}, part~\ref{fake-nonspec} that
\begin{equation} \label{estdim-not-pwise}
h^0\bigl(\bar C, \omega_{\bar C} \otimes \phi^* \omega_S ^{-1}
(-D') \bigr)
\leq h^0\bigl(\bar C, \omega_{\bar C} \otimes \phi^* \omega_S ^{-1}
(-D) \bigr),
\end{equation}
so that it still holds that $\dim V \leq \expdim V_g
^\xi(\alpha,\beta)(\Omega)$, hence $V$ has the expected dimension.
%\phantom{p} 
\qed

\paragraph{}
\label{rk:tg-logSeveri0}
{\itshape
Note that the above proof gives the additional fact that,
under the assumption of \ref{P0},
the tangent space of $V_g^\xi(\alpha,\beta)(\Omega)$ at the general
point $[C]$ of $V$ identifies with
}\[
H^0 \bigl(\bar C, \omega_{\bar C} \otimes \phi^* \omega_S ^{-1}
(-D) \bigr)
\cong H^0 \bigl( \bar C, \bar N _\phi (-D_1) \bigr)
\cong H^0 \bigl( \bar C, \bar N _\phi (D_0-D) \bigr)
\subset H^0 \bigl( \bar C, \bar N _\phi \bigr).
\]


\paragraph{} \label{p:P1}
{\itshape
We now prove that under Assumption~\ref{P1}
the assertions \ref{t:a--}, {\ref{t:b}}, \ref{t:c-},
and {\ref{t:e}} hold.}

\medskip
\par Suppose by contradiction that \ref{t:b} doesn't hold. Then we
argue as in \ref{p:not-pwise-disjt}. In this case, part~\ref{fake-bpf}
of Lemma~\ref{fucking-obs} applies thanks to Assumption~\ref{P1}, and
we get that the inequality \eqref{estdim-not-pwise} is strict, which is
in contradiction with \eqref{expdim-upbnd}.

\par The same argument shows that none of the points $\phi(r_{i,j})$
can be fixed on $R$. This implies in particular that \ref{t:c-} holds.

The proof of \ref{t:e} is similar: if $C$ were tangent to $G$, then it
would belong to an irreducible component $W$ of some Severi variety of
the pair $(S,R+G)$. Assumption~\ref{P1} implies that $W$ is liable for
part \ref{P0} of Theorem~\ref{T}, hence $\dim(W) < \dim(V)$, in
contradiction with the fact that $[C]$ is a general member of $V$.
The same argument shows that $C$ avoids $\Gamma$ (pick some random
curve on $S$ containing $\Gamma$).

\par Finally, we note that equality holds in \eqref{upbnd-dim} if
and only if $D_1'=Z_0=0$ since the line bundle $\omega_{\bar C}
\otimes \phi^* \omega_S ^{-1} (-D)$ is globally generated by
assumption~\ref{P1}. Now it is indeed the case that equality holds in
\eqref{upbnd-dim} since we have proved that $\dim (V) = \expdim \bigl(V_g
^\xi(\alpha, \beta)\bigr)$. We conclude that $D_1'=Z_0=0$, which means that
(i) $\phi$ is an immersion outside of the points $r _{i,j}$ (this is
assertion~\ref{t:a--}) and (ii) $l _{i,j} \leq i$ for $1 \leq j \leq
\beta_i$.
\qed

\bigskip
\subparagraph*{Remark} It is not enough to assume that $\omega_{\bar
  C} \otimes \phi^* \omega_S ^{-1} (-D)$ is non-special and globally
generated because of the argument we made to assume that the points
$q_{i,j}$ and $r_{i,j}$ are pairwise distinct.
We actually need to know something about every possible $\omega_{\bar
  C} \otimes \phi^* \omega_S ^{-1} (-D')$, where $D'=\sum i q'_{i,j} +
\sum (i-1)r'_{i,j}$ in the notation used for this argument.


\paragraph{} 
\label{p:imm-at-prescr}
{\itshape
We now prove that, under the assumption~\ref{P2}, $\phi$
is an immersion also at the points $r_{i,j}$, i.e.\ that $l_{i,j}=1$
for $1 \leq j \leq \beta_i$,
thus completing the proof of assertion~\smash{\ref{t:a-}}.}
% of Thm.~\ref{T}).}

\medskip
Let $i \geq 1$ and $1 \leq j \leq \beta_i$. It follows from the
assumption that the linear series $\bigl| \omega_{\bar C} \otimes
\phi^* \omega_S ^{-1} (-D) \bigr|$ separates any two points, so there
exists a section $\sigma \in H^0 \bigl(\bar C, \omega_{\bar C} \otimes
\phi^* \omega_S ^{-1} (-D) \bigr)$ with vanishing order $v_{r_{i,j}}
(\sigma) = 1$ at the point $r _{i,j}$.  Seen as a section $\tilde \sigma \in
H^0 (\bar C, \bar N_\phi)$, it vanishes at $r_{i,j}$ with order
$v_{r_{i,j}} (\tilde \sigma) = 1 + (i-l_{i,j})$
(see \eqref{Nbar}).
By Lemma~\ref{l:log-tg} this implies 
\[
1 + i-l_{i,j} \in \{ i-l_{i,j} \} \cup \dlbrack i, +\infty \dlbrack
\]
and therefore $l _{i,j} =1$ as required.
\qed


\begin{remark}
\label{rk:tg-logSeveri}
Under the conditions of \ref{P2} the map $\phi$ is an immersion,
hence
$N_\phi = \bar N _\phi \cong
\omega_C \otimes \phi^* \omega_S^{-1}$, see Paragraph \ref{p:Nbar}.
Therefore, the tangent space of $V_g^\xi(\alpha,\beta)(\Omega)$ at the
general point $[C]$ of $V$ identifies with
\[
  H^0 \bigl( \bar C, N _\phi (-D) \bigr)
  \cong
  H^0 \bigl(\bar C, \omega_{\bar C} \otimes \phi^* \omega_S ^{-1}
  (-D) \bigr)
\]
(the definition of $D$ is in \eqref{div-tg-cond} above).
\end{remark}


\paragraph{} 
{\itshape
Let us prove that Assumption~\ref{P2} implies Assertion~{\ref{t:c}},
\ie the points $p_{i,j}$ and $s_{i,j}=\phi(r_{i,j})$ are pairwise
distinct.}

\medskip
By \ref{p:P1}, we already know that \ref{t:c-} holds,
\ie none of the $s_{i,j}=\phi(r_{i,j})$ belongs to $\Omega = \{
p_{i,j} \}$. We thus only need to show that no two of the points
$s_{i,j}$ coincide.
\par Suppose there exist $(i,j)$ and $(i',j')$ distinct such that
$\phi (r_{i,j}) = \phi (r_{i',j'})$. Assumption~\ref{P2} implies
that the series $|\omega_{\bar C} \otimes \phi^* \omega_S ^{-1} (-D)|
= |T_{[C]} V|$ separates any two points.
Therefore there exists a section
$\sigma \in T_{[C]} V \cong H^0(\bar N_\phi(-D))$ such that
\[
v _{r_{i,j}} (\sigma) = 1
\quad \text{and} \quad
v _{r_{i',j'}} (\sigma) = 0.
\]
This implies the existence of a deformation of $C$ in which the points
$\phi (r_{i,j})$ and $\phi (r_{i',j'})$ no longer coincide, a
contradiction to the generality of $[C]$ in $V$. 
\qed

\paragraph{}
{\itshape
Let us prove that Assumption~\ref{P2} implies Assertion~{\ref{t:d}},
\ie $C$ is smooth at its intersection points with $R$.}

\medskip
At this point we know that \ref{t:a-} and \ref{t:c} hold under
Assumption~\ref{P2}, \ie the curve $C$ is immersed and the points
$p_{i,j}$ and $s_{i,j}$ are pairwise distinct.
Because the intersection $C \cap R$ is set-theoretically the union of
all the points $p_{i,j}$ and $s_{i,j}$, this implies that $C$ is
smooth at its intersection points with $R$. 
\qed


\paragraph{} \label{p:nodal}
{\itshape
We eventually prove that under the Assumption~\ref{P3} the curve
$C$ is nodal, which is Assertion~\ref{t:a} of Theorem~\ref{T}.}

\medskip
Since we already know that the curve $C$ is immersed, it is enough
to show that for all point $p\in C$, $C$ has neither three or more
local branches, nor two or more tangent local branches.

To exclude the former possibility, suppose by contradiction that there
exist $a,b,c \in \bar C$ pairwise distinct such that
$\phi(a)=\phi(b)=\phi(c)$.
The assumption~\ref{P3} implies that the linear series $\bigl|
\omega_{\bar C} \otimes \phi^* \omega_S ^{-1} (-D) \bigr|$ separates
any three points, so there exists a section $\sigma \in H^0 \bigl(\bar
C, \omega_{\bar C} \otimes \phi^* \omega_S ^{-1} (-D) \bigr)$ such
that
\[
% v_a(\sigma), v_b(\sigma) \geq 1
\sigma (a) = \sigma (b) =0
\quad \text{and} \quad %v_c(\sigma)=0;
\sigma (c) \neq 0;
\]
it corresponds to a first-order deformation of $\phi$ leaving both
$\phi(a)$ and $\phi(b)$ fixed while moving $\phi(c)$. By generality of
$[C]$, there is correspondingly an actual deformation of the curve $C$
for which the three local branches under consideration are no longer
intersecting in a common point, a contradiction to the generality of
$[C]$ in $V$ (see, e.g., \cite[Prop.~1.4]{DS15}).

We exclude the second possibility in a similar fashion.
Suppose by contradiction that there
exist $a,b \in \bar C$ distinct such that $\phi(a)=\phi(b)$ and $\Img
d\phi_a = \Img d\phi_b$. Again since $\bigl| \omega_{\bar C} \otimes \phi^*
\omega_S ^{-1} (-D) \bigr|$ separates any three points, there exists
$\sigma \in H^0 \bigl(\bar C, \omega_{\bar C} \otimes \phi^*
\omega_S ^{-1} (-D) \bigr)$ such that
$\sigma (a) = 0$ and $\sigma (b) \not\in \Img d\phi_a$.
It corresponds to a first-order deformation of $\phi$ leaving 
$\phi(a)$ fixed while moving $\phi(b)$ in a direction transverse to
the common tangent to the two local branches of $C$ under
consideration. This contradicts the generality of $[C]$ as before.
\qed

\bigskip\noindent
This ends the proof of Theorem~\ref{T}.


\section{A dimensional characterization of logarithmic
  Severi varieties}
\label{S:dim-charact}

We consider a pair $(S,R)$ consisting of a smooth surface
$S$ and a reduced boundary divisor $R$, as described in
\ref{S:results}.
In this Section we give an upper bound
for the dimension of families $V$ of (not necessarily reduced) curves in
$S$ with prescribed homology class and genus, together with a
dimensional characterization of logarithmic Severi varieties: it turns
out that the irreducible components of logarithmic Severi varieties
are essentially those families for which the upper bound is reached.
The content of this section is basically \cite[Cor.~2.7]{ch}.
The main result, Proposition~\ref{pr:charact}, is a generalization of
Zariski's dimensional characterization of (classical) Severi varieties
\cite{zariski}.

\paragraph{}
\label{p:fam-curves}
Let $V$ be an irreducible locally closed subset of the Hilbert scheme
of curves on $S$,
and suppose that it parametrizes genus $g$ curves in the
following sense: for a general member $X$ of $V$, there exists a
smooth curve $C$ of genus $g$,
and a morphism $\phi: C \to X$, not constant on any
component of $C$, and such that the push-forward in the sense of
cycles $\phi_* [C]$ equals the fundamental cycle of $X$.

\paragraph{}
\label{p:positivity}
Let $\xi \in \NS (S)$ be the homology class of members of $V$.
Letting the general member $X$ of $V$ have irreducible components
$X_1,\ldots,X_n$, with respective classes $\xi_1,\ldots,\xi_n$,
we assume furthermore:
\begin{equation*}
  \forall i=1,\ldots,n:
  \quad
  -(K_S+R) \cdot \xi_i >0,
\end{equation*}
so that we may apply \ref{P0} without any restriction on the contact
conditions with $R$.


\begin{proposition} \label{pr:charact}
% \renewcommand{\theequation}
% {\arabic{section}.\arabic{paragraph}.\alph{equation}}
Consider a finite subset $\Omega \subset R$.
Under the above assumptions in
\ref{p:fam-curves}
and \ref{p:positivity}, 
for all general member $X$ of $V$, one has
\begin{equation} \label{char-dim}
\dim (V) \leq -(K_S+R) \cdot \xi + g -1 + \Card \bigl( (X \cap R)
\setminus \Omega \bigr),
\end{equation}
where the last number is defined set-theoretically
(\ie we do not count with multiplicities).

Moreover, if equality holds in \eqref{char-dim}, then
there exist $\alpha,\beta$ such that
$V$ is a dense subset of a
component of a log-Severi variety $V^\xi _g (\alpha,\beta)(\Omega)$ if
and only if  
\begin{equation} \label{char-unibranch}
\Card \bigl( \phi^{-1}(R) \bigr) = \Card (X \cap R),
\end{equation}
with $\phi: C \to X$ a genus $g$ morphism as above. 
\setcounter{equation}{0}
\end{proposition}

\bigskip
Note that $\alpha$ and $\beta$ are of course uniquely determined by
the contacts of $X$ and $L$.
Before proving this statement we make a few observations, in the hope
that they will clarify some of its subtleties.

\begin{remark}
Proposition~\ref{pr:charact} is really a result about families of
embedded curves in $S$, not families of maps.

Indeed, if a general member $X$ is not reduced, then genus $g$ maps
$\phi:C \to X$ as above involve multiple covers, and there is in general
a positive dimensional family of maps giving the same $X$, so that the
family of maps corresponding to $V$ has in general dimension larger
than $V$.

When equality holds in \eqref{char-dim}, the map $\phi$ is necessarily
a birational isomorphism on each component of $C$.
If moreover $g\geq 1$, then the general member of $V$ is actually
reduced. See \ref{p:char-mult}
for precisions about this.
\end{remark}


\begin{remark}
  % \par \smallskip \noindent (b)
A straightforward corollary of
Proposition~\ref{pr:charact} which may be useful for the applications
is that the inequality~\eqref{char-dim} still holds if we only assume
$C$ to be reduced and replace $g$ by the \emph{arithmetic} genus of
$C$; this alternative inequality is always strict when $C$ is not
smooth.
\end{remark}


% \bigskip
% \subparagraph{Remark} \label{r:unibranch}
\begin{remark}
\label{r:unibranch}
Assumption~\eqref{char-unibranch} ensures that
the normalization of $X$ is unibranch over the points in $X \cap R$.

\subparagraph{Example} Set $(S,R) = (\P^2, L)$ whith $L$ a line, and
$\xi = 3 [H]$ with $[H]$ the hyperplane class. The family $V$ of
plane cubics with one node on $L$ and otherwise smooth has dimension
$7$, which equals
\[
\underbrace{-(K_S+R) \cdot \xi}
_{=2[H] \cdot 3[H] = 6}
 + \underbrace{g} _{=0} -1 + 
\underbrace{\Card \bigl( (X \cap R)
\setminus \Omega \bigr)}
_{=2}
\quad \text{with $\Omega = \emptyset$.}
\]
It is a divisor in the log-Severi variety
$V^{3[H]}_0(0,3)(\emptyset)$, but it is not a component of the family 
$V^{3[H]}_0(0,[1,1])(\emptyset)$ of rational plane cubics with one
variable tangency along $L$, which has dimension $7$ as well.
\end{remark}


% \medskip
% %\subparagraph{Remark} 
\begin{remark}
  % (b)
In the equality case for \eqref{char-dim}, if one replaces
\eqref{char-unibranch} with the weaker condition that
\begin{equation}
\label{char-unibranch-weak}
\Card \bigl( \phi^{-1} (R \setminus \Omega) \bigr) =
\Card \bigl( (X \cap L) \setminus \Omega \bigr),
\end{equation}
the families that we get that are not log-Severi varieties may be
considered as ``log-Severi varieties with $\Omega$ containing repeated
points'',
see Example~\ref{ex:Omega-w-repet} below.
(These are not log-Severi varieties according to
Definition~\ref{d:log-severi}).

Beware that in \cite[Cor.~2.7]{ch}, the weaker
\eqref{char-unibranch-weak} is used instead of
\eqref{char-unibranch},
which is slightly inaccurate. 

\medskip
\subparagraph{Example}
\label{ex:Omega-w-repet}
Set $(S,R) = (\P^2,L)$ as above, and $\xi = 4
[H]$, and fix $p\in L$. The family of plane quartics with one triple
point at $p$ has dimension $\binom 6 2 - 1 -6=8$, which equals 
\[
\underbrace{-(K_S+R) \cdot \xi}
_{=2[H] \cdot 4[H] = 8}
 + \underbrace{g} _{=0} -1 + 
\underbrace{\Card \bigl( (X \cap L)
\setminus \Omega \bigr)}
_{=1}
\quad \text{with $\Omega = \{ p \}$.}
\]
One may wish to consider it as $V^{3[H]}_0(3,1) (p,p,p)$.
\end{remark}



\subsubsection*{Proof of Proposition~\ref{pr:charact}}
%\bigskip % \vparskip
% \subparagraph{Proof of Proposition~\ref{pr:charact}.}
% \renewcommand{\theequation}
% {\arabic{section}.\arabic{paragraph}.\arabic{subparagraph}.\arabic{equation}}
%\begin{proof}[Proof of Proposition~\ref{pr:charact}]
We divide the proof into several steps, which correspond to paragraphs
\ref{p:char-main}--\ref{p:red-induc}.  We first treat the case when
$X$ is irreducible; the general case is taken care of by induction in
\ref{p:red-induc}.
\vspace{-1ex}
\paragraph{} \label{p:char-main}
We first prove the proposition under the assumption that $X$ is
reduced and irreducible; in this case $\phi$ is the normalization of
$X$ and $C \cong \bar X$.
\par If $e:=  \Card \bigl( (X \cap R) \setminus \Omega \bigr) = 0$,
then the statement is a slight variant of part~\ref{P0} of the main
Theorem~\ref{T}: we get the required inequality \eqref{char-dim}
exactly as in paragraph~\ref{p:dim-logsev}, with $D=\phi^* R$ and
$D_0=0$ in \eqref{div-tg-cond} and \eqref{ramif-var} respectively. The
only difference with the setting of \ref{p:dim-logsev} is that here
two distinct points of the support of $\phi^*R \subset \bar X$ may
have the same image by $\phi$ in $X$; this makes absolutely no
difference in the argument.
\par Now if \eqref{char-unibranch} holds, then $\bar X$ is unibranch over
the points of $X \cap R$. This implies that $V$ is contained in a
certain log-Severi variety $V_g^\xi (\alpha,0)(\Omega)$. If moreover
equality holds in \eqref{char-dim}, then $V$ is dense in an
irreducible component of this same log-Severi variety by \ref{P0}.

\smallskip
\par In the case when $e>0$, we consider the map
\[
\rho: V \to \Sym ^e R
\]
sending a curve to its reduced intersection scheme with $R \setminus
\Omega$; this may not be well-defined everywhere since $e$ may drop
along certain closed subschemes of $V$, but it is in a neighbourhood
of $[X]$.
\par Then we can apply the $e=0$ case of the Proposition to the fibres
of $\rho$; for a general $\Sigma \in \Sym^e R$, setting $\Omega' =
\Omega \cup \Supp \Sigma$ one gets that the fibre $\rho ^{-1} (\Sigma)$ has
dimension at most $-(K_S+R)\cdot \xi
+g-1$. Inequality~\eqref{char-dim} follows, and the equality case of
the Proposition as well, again applying the $e=0$ case to the fibres
of $\rho$.
\smallskip
\subparagraph*{Remark} Note that the above reasoning also proves that,
if $V$ is dense in a suitable irreducible component of a log-Severi
variety,
then the map $\rho : V \to \Sym^e R$ is dominant.


\paragraph{} \label{p:char-mult}
Let us now consider the case when $X$ is non-reduced, but still
irreducible; we shall show that inequality~\eqref{char-dim} holds, and
that it is almost always strict; when equality holds in
\eqref{char-dim}, condition \eqref{char-unibranch} does not hold.
This will also prove the second part of the proposition, since $V$ is
not a dense subset of a component of a log-Severi variety 
when $X$ is non-reduced.

\par We have to consider $\phi: C \to X$ where $X$ is non-reduced but
irreducible, and $C$ may be reducible. We let $m>1$ be the degree of
$\phi$, i.e.\ the sum of the degrees of the various $\phi_i: C_i \to
X$. The key is to write the appropriate version of the
Riemann--Hurwitz Formula: we have
\[
2g-2 = \deg (\omega_C) \geq m\, \deg (\omega_{X_{\rm red}}) = m(2q-2),
\]
% which gives $g \geq mh-m+1$.
with $q$ the arithmetic genus of $X_\red$.
Let $h$ be the geometric genus of $X_\red$: we have
$h \leq q$, so that eventually
$g-1 \geq m(h-1)$.

Then we apply Proposition~\ref{pr:charact} in the
reduced case, which we have already proven above, to the reduced curve
$X_\red$ underlying $X$: it has class
$\frac 1 m \xi$, so we get
\begin{align*}
  \dim (V)
  &\leq -(K_S+R) \cdot \frac 1 m \xi + h -1 +
    \Card \bigl( (X \cap R) \setminus \Omega \bigr)\\
  &\leq -(K_S+R) \cdot \frac 1 m \xi + \frac {g-1} m +
    \Card \bigl( (X \cap R) \setminus \Omega \bigr);
\end{align*}
recall that $X\cap R$ is considered as a set, so that
\[
  \Card \bigl( (X \cap R) \setminus \Omega \bigr)
  =
  \Card \bigl( (X_\red \cap R) \setminus \Omega \bigr).
\]
Now the required inequality \eqref{char-dim} follows from the basic
inequality:
\begin{equation}
  \tag{$\star$}
  \label{basic}
  -(K_S+R) \cdot \frac 1 m \xi + \frac {g-1} m 
  % + \Card \bigl( (X \cap R) \setminus \Omega \bigr)
  \leq
  -(K_S+R) \cdot \xi + {g-1}.
  % + \Card \bigl( (X \cap R) \setminus \Omega \bigr)
\end{equation}
If $g\geq 1$,
the latter inequality \eqref{basic} is straightforward, and always
strict, as 
$-(K_S+R) \cdot \xi >0$ and $m>1$.
If $g\leq 0$ however, one has
$-(K_S+R) \cdot \xi \geq m$ on the one hand,
because $\frac 1 m \xi$ is an integral class,
and $g\geq -m+1$, with equality holding if and only if $C$ is the
disjoint union of $m$ smooth rational curves;
thus inequality \eqref{basic} holds also in this case, and it is
an equality if and only if
$-(K_S+R) \cdot \frac 1 m \xi = 1$ and
$C$ is the disjoint union of $m$ smooth rational curves.
When the latter condition is realized, 
condition~\eqref{char-unibranch} does not hold.


\medskip
\subparagraph{Example}
Let $S$ be the projective plane blown-up at eight general points, with
exceptional divisors $E_1,\ldots,E_8$,
and take $R=0$.
We consider the class
\[
  \xi = m(3H-\tsum_{i=1}^8 E_i)
\]
where $H$ as usual denotes the pull-back to $S$ of the line class on
$\P^2$.
Let $X_0$ be an irreducible rational curve in the linear system
$|3H-\tsum_{i=1}^8 E_i|$, and consider the family $V$ consisting
solely of $X=mX_0$ as a $0$-dimensional family of curves of genus
$-m+1$, by means of the morphism $\phi: C \to X$ consisting of $m$
disjoint copies of the normalisation of $X_0$.
Equality holds for $V$ in \eqref{char-dim}.



\paragraph{} \label{p:red-induc}
It remains to consider the case when $X$ is reducible. Proceeding
by induction on the number of irreducible components, we may assume
that $X=X_1 \cup X_2$ where $X_1$ and $X_2$ move in two families $V_1$
and $V_2$ of curves of genera $g_1$ and $g_2$ respectively,
such that $V \subseteq V_1 \times V_2$ and the Proposition holds for
$V_1$ and $V_2$. Adding the two corresponding inequalities 
gives
\begin{equation} \label{sev-comps}
\begin{aligned}
\dim (V) & \leq \dim (V_1) + \dim (V_2) \\
&= -(K_S+R)\cdot \xi + (g_1+g_2-1) -1
+ \Card \bigl( (X_1 \cap R) \setminus \Omega \bigr)
+ \Card \bigl( (X_2 \cap R) \setminus \Omega \bigr).
\end{aligned}
\end{equation}
If $(X_1 \cap X_2 \cap R) \setminus \Omega$ is empty then this
readily gives the
required inequality,
and the second part of the proposition in the equality case also
follows.

So let us consider the case when
$(X_1 \cap X_2 \cap R) \setminus \Omega$ is non-empty,
and let us
assume for simplicity that this set consists of only one point $p$,
the general case being strictly similar.
In this case condition \eqref{char-unibranch} does not hold because
$p$ has at least two preimages.


\par If $p$ is a fixed point of the intersection with $R$ for either
one of the two families, say $V_1$, then it is also a fixed point for
the other family:
indeed, otherwise, by the generality of $X$ we could perturb $X_2$ a
little so that it does not pass through $p$, and then $p$ is no longer
a point in $X_1 \cap X_2 \cap R$.
In this case, applying the proposition to
$V_1$ and $V_2$ with $\Omega':=\Omega \cup \{p \}$, one gets
\[
\dim (V) \leq -(K_S+R)\cdot \xi + (g_1+g_2-1) -1
+ \underbrace {\Card \bigl( (X_1 \cap R) \setminus \Omega' \bigr)
+ \Card \bigl( (X_2 \cap R) \setminus \Omega' \bigr)}
_{=  \Card \bigl( (X \cap R) \setminus \Omega \bigr) -1},
\]
and the result follows;
note that inequality \eqref{char-dim} is strict in this case.


\par Otherwise $p$ is variable for both $V_1$ and $V_2$; in this case $V$
necessarily has codimension at least $1$ in $V_1 \times V_2$ (this may
be proved for instance as in \ref{p:char-main} by applying the
Proposition to the fibres of the projection $V \to V_1$), and
therefore \eqref{sev-comps} gives the required
inequality \eqref{char-dim}.
Equality may hold in \eqref{char-dim}, but $V$ cannot be dense in a
component of a log-Severi variety, since it already has positive
codimension in $V_1 \times V_2$.

\medskip
\subparagraph{Example}
Take $S=\P^2$ and $R$ a line, let
$V_1 = V_2 = V^{[H]}_0(0,1)(\emptyset)$,
and consider $V$ the sub-family of $V_1\times V_2$ parametrizing the
sums of two lines, the intersection point of which lies on $R$. Then
$V$ has dimension $3$, and parametrizes curves of genus $-1$, so that
equality holds in \eqref{char-dim} because $\Card(X\cap R)=1$ for a
general membre $X$ of $V$.
It has codimension $1$ in $V_1\times V_2$, which is an irreducible
component of $V^{[2H]}_{-1}(0,2)(\emptyset)$. Concretely, on $V$ we
are artificially decreasing $\Card(X\cap R)$ by imposing that two
contact points with $R$ coincide, and the latter prescription is not
of Severi type.


\bigskip % \vparskip
\noindent
The proof of Proposition~\ref{pr:charact} is now over.
\qed




\section{Examples}
\label{S:examples}


\subsection{An example with contact points in special position}

In this short subsection I give an example illustrating
(i) the effect of having the points in $\Omega$ in special position
(which is also a theme in Subsection~\ref{s:logK3}
below),
and (ii) the importance of considering the positivity of
$-K_S\cdot C-\deg \phi_*D$
(in the notation of Theorem~\ref{T})
on all irreducible components of $C$ separately.


\begin{example}
\label{ex:Omega-special}
Let $S$ be the projective plane, $R$ be a smooth cubic,
and $\Omega$ be cut out on $R$ by another cubic $R'$.
We consider the Severi variety
$V^4_0(9,3)(\Omega)$ of rational quartics passing through the
$9$ intersection points of $R$ and $R'$ (and thus with $3$ unassigned
additional contact points with $R$);
it has expected dimension
\[
  -(\underbrace{K_S+R}_{=0})\cdot \xi
  + \underbrace{g}_{=0}-1
  + \underbrace {|\beta|}_{=3}
  = 2.
\]

It has a $3$-dimensional irreducible component $V_\nir$
parametrizing reducible quartics $C_1+C_2$ where $C_1$ is a cubic in
the pencil generated by $R$ and $R'$, and $C_2$ is a line.
The component $V_\nir$ thus has dimension larger than expected, and
indeed \ref{P0} does not apply in this case because,
in the notation of Theorem~\ref{T},
\[
  -K_S\cdot C_1-\deg \restr {\phi_*D} {C_1} = 0.
\]

The Severi variety
$V^4_0(9,3)(\Omega)$ has another component $V_\irr$,
which parametrizes irreducible quartics $C$. This time,
\[
  -K_S\cdot C-\deg {\phi_*D} = 3,
\]
so \ref{P0} applies and all irreducible components of $V_\irr$ have
dimension $2$ as expected. 
It is however not obvious that there indeed exist irreducible rational
quartics passing through $\Omega$ (so that $V_\irr$ is non-empty): we
give an argument in the next paragraph.
\end{example}

\paragraph{}
Le me now show that $V_\irr$ introduced above is non-empty,
following a suggestion of Edoardo Sernesi.
% Continuing with the situation of
% Example~\ref{ex:Omega-special},
Consider the family $W$ of
reducible quartics $C_1+C_2$, where $C_1$ and $C_2$ are two conics,
passing respectively through the first five points of $\Omega$, and
through the remaining four points. Since no four points of $\Omega$
are aligned, $C_1$ is fixed and $C_2$ moves in a pencil, hence
$W$ has dimension $1$ as expected.
Besides, 
\[
  -K_S\cdot C_1-\deg \restr {\phi_*D} {C_1} = 1
  \quad \text{and}
  \quad
  -K_S\cdot C_2-\deg \restr {\phi_*D} {C_2} = 2,
\]
so \ref{P0} indeed applies to $W$.

The fact that the dimension of $W$ equals the expected dimension
implies that the nodes of a general member of $W$ may be smoothed
independently, \ie a general member of $W$ may be deformed in such a
way that an arbitrary subset of its nodes are preserved while the
other are smoothed. Indeed the assumption implies that $W$ is smooth
at a general point $[C]$,
and the conditions defining its tangent space as a linear subspace 
of $H^0(C,\O_C(C))$ are independent, hence these conditions may be
relaxed independently.
This is a standard argument going back to Severi himself, of which a
modern account may be found in \cite{tannenbaum}. 

The upshot is that one may smooth one and only one node of a general
member $C_1+C_2$ of $W$, while preserving the condition of passing
through the points in $\Omega$: the result is a necessarily
irreducible quartic curve with three nodes, passing through $\Omega$,
as required.



\subsection{Superabundant log Severi varieties
  coming from double covers}

In this subsection I give examples of superabundant logarithmic
Severi varieties,
\ie such that the dimension exceeds the expected dimension:
the inequality in \ref{P00}
% \eqref{expdim-upbnd}
is strict, and \ref{P0}
does not apply.
These examples live on the projective plane, and come from
linear systems on double covers.
This is taken from \cite{cd-double}.
The examples are given in \ref{ex:superabundant}
below, after a few recaps on double covers.

\paragraph{}
\label{p:double-covers}
We shall use the following elementary facts about double covers.
Let $d$ be a positive integer,
and $B$ be a degree $2d$ curve in $\P^2$.
We consider the double cover $\pi: S \to \P^2$ branched over
$B$. 
Let $H$ be the line class on
$\P^2$, and $L$ be its pull-back to $S$.
For all $k\in \N$ we have
\begin{equation*}
%\label{eq:decomp:kL}
H^0(S,kL) = 
\pi^* H^0(\P^2, kH) \oplus \pi^* H^0(\P^2, kH-{\textstyle\frac 1
  2}B),
\end{equation*}
which is the isotypical decomposition of 
$H^0(S,kL)$ as a representation of $\Z/2\Z$.
The first summand corresponds to divisors that are double covers of
degree $k$ curves in $\P^2$, and the second to divisors that
decompose as $B$ (seen as the ramification divisor in $S$) plus the
double cover of a degree $k-d$ curve in $\P^2$.

\begin{proposition}
For $k\geq d$, the general member $C$ of $|kL|$ is not a double cover
of some hypersurface in $\P^2$, the restriction $\restr \pi C$ is
birational on 
its image, a degree $2k$ hypersurface $C^\flat$ in $\P^2$ everywhere
tangent to $B$, with a node at every point of a
complete intersection $Z$ of type $(k,k-d)$.
\end{proposition}


\begin{proof}
The divisor $C$ belongs to a unique pencil $\vect {A', B+D'}$,
with $A'$ and $D'$ the double covers of curves $A$ and $D$ in
$\P^2$ of respective degrees $k$ and $k-d$.
Thus $C^\flat :=\pi(C)$ belongs to the pencil 
$\vect {2A, B+2D}$, from which it follows that $C^\flat$ is double
along $Z:=A \cap D$, and touches $B$ doubly along $A\cap B$, which
accounts for the whole intersection scheme of $C^\flat$ and $B$. 
The base locus of this pencil is the scheme defined by the
ideal sheaf
$\I_Z^2(\I_A^2+\I_B)$.

The pull-back $\pi^* C^\flat \in |2kL|$ splits as $C+i(C)$, with $i$ the
involution on $V$ associated to $\pi$~; it has a double singularity along
$Z':= \pi^{-1}(Z)$ and $\pi^{-1}(B\cap A)$, with at each point
one local sheet belonging to $C$ and another to $i(C)$. The union 
$Z' \cup \pi^{-1}(B\cap A)$ is the base locus of the pencil 
$\vect {A', B+D'}$.
\end{proof}

\begin{example}
\label{ex:superabundant}
We consider the image 
$V_{B,k}$ in $|2kH|$ of the linear system
$|kL|$ on $S$. It has dimension
\[
h^0(S,kL)-1
% = h^0(\P^2, kH) + h^0(\P^2, (k-d)H) -1,
= h^0(\P^2,kH) + h^0(\P^2,(k-d)H) -1,
\]
and parametrizes curves of geometric genus
\[
g_{k,d} %= p_a(2k)-k(k-d)
=\textstyle \frac 1 2 (2k-1)(2k-2)-k(k-d),
\]
%(with $p_a(l)$ the arithmetic genus of plane curves of degree $l$)
everywhere tangent to $B$; the number of contact points is thus
$2kd$.
% \[
% \frac 1 2 (2kH)\cdot B = 2kd.
% \]

The family of curves $V_{B,k}$ is therefore contained in the
log-Severi variety
$V _{g_{k,d}} ^{2k}(0,[0,2kd])$ of the pair $(\P^2,B)$, 
%in the notation of \ref{sp:notation}.
% By definition, this log-Severi variety parametrizes plane curves of
% degree $2k$ and geometric genus $g_{k,d}$, tangent to $B$ at $2kd$
% unassigned points. 
for which the expected dimension is
\begin{align*}
-(K_{\P^2}+B)\cdot 2kH+g_{k,d}-1+2kd
&= k(k+3-d).
% &= -2k(2d-3)+g_{k,d} -1+2kd
% \\
%&= 2k(3-d)+g_{k,d}-1,
\end{align*}
% \begin{align*}
% \operatorname{expdim}
% \bigl(V _{g_{k,d}} ^{2kH}(0,[0,2kd])\bigr))
% &= 2k(3-d)+g_{k,d}-1
% \\
% &= \textstyle
% 2k(3-d)-1+\frac {(2k-1)(2k-2)} 2 -k(k-d)
% \\
% &= k(k+3-d).
% \end{align*}
By \ref{P0} a component of the Severi variety has
the expected dimension if 
it has an irreducible member and
\[
-K_{\P^2}\cdot 2kH - 2kd \geq 1
\quad \iff
\quad
2k(3-d) \geq 1;
\]
we note that the latter inequality holds if and only if $d \leq 2$.

It turns out that the dimension of our family $V_{B,k}$ exceeds the
expected dimension of the log-Severi variety.
Indeed a direct computation shows that
\begin{align*}
\dim(V_{B,k})
- \expdim
\bigl(V _{g_{k,d}} ^{2kH}(0,[0,2kd])\bigr)
% &= \textstyle
% k^2+3k+1-dk+\frac 1 2 d(d-3)
% \\
% & \textstyle
% \quad - \Bigl[
% k^2+3k-dk
% \Bigr]
% \\
% &= \textstyle
% \frac 1 2 d(d-3)+1
% \\
&=  \textstyle
\frac {(d-1)(d-2)} 2
\\
&= p_g(S)
\end{align*}
(cf.\ \cite[V.22 p.237]{bhpv} for the last equality).
\end{example}




\subsection{Logarithmic \texorpdfstring{$K3$}{} surfaces}
\label{s:logK3}

In this subsection I discuss logarithmic Severi varieties of pairs
$(S,R)$ with $K_S+R=0$, in relation with Severi varieties of $K3$
surfaces. This is a central theme of this volume, and as
such it will be revisited in various other chapters.

\paragraph{$K3$ surfaces}
Let us first consider the case of ``absolute'' $K3$ surfaces: let $S$
be a $K3$ surface, and $R=0$. In this case Theorem~\ref{T} is not
quite accurate, a (well-known) prominent issue being that
the condition in order for \ref{P0} to apply is not verified, and
indeed the expected dimension 
given in \ref{P0} is not the actual dimension. 

Suppose $S$ is equipped
with a polarisation $L$ of genus $p$ (\ie $L^2 = 2p-2$). The expected
dimension of $V_g^L$
as defined in \ref{p:expdim}
is $g-1$, whereas its actual dimension is $g$, if
$0 \leq g \leq p$ and $S$ is very general, say. Technically, the
deformations of $[C] \in V_g^L$ are governed by the invertible sheaf 
$\restr L C \cong \omega_C$, hence the obstruction space is
$H^1(C,\omega_C)$ which is $1$-dimensional;
it turns out however that the equigeneric
deformations of $C$ are unobstructed, even though the obstruction
space is non-trivial.
A conceptual explanation for this is that there exist
non-algebraic $K3$ surfaces, which do not carry any curve at all;
the expected dimension for Severi varieties on $K3$ surfaces thus
becomes accurate if considered in family over all $K3$ surfaces,
including the non-algebraic ones.
I refer to \cite[\S 4.2]{DS15} for a detailed account; in the present
volume, this phenomenon will be considered again in
\cite[subsection~\ref{s:red-th}]{10.th-panoramico},
in the context of Gromov--Witten theory.


\bigskip
We shall now describe some analogous phenomena for $K3$
pairs, by looking at typical examples.

\paragraph{Surfaces with canonical curve sections}
\label{p:can-sect}
Let $S$ be $\P^2$, and $R$ be a smooth cubic; note that in this case
one 
has $K_S+R=0$. Let $C$ be a smooth curve of degree $d \geq 4$ on $S$,
and set 
$\Omega = C \cap R$ (for simplicity we may assume that $C$ and $R$
intersect transversely). The blow-up $S'$ of $\P^2$ at $\Omega$ is a
smooth surface having a unique anticanonical divisor, namely the
proper transform $R'$ of $R$. The linear system $|C'|$ of the proper
transform $C'$ of
$C$ gives a birational model of $S'$ in $\P^p$,
in which the proper transform of $R$ is contracted, and whose hyperplane
sections are the canonical models of the degree $d$ plane curves
passing through $\Omega$ (we have let $p$ equal $\mathrm{p}(d)$, the
genus of smooth plane $d$-ics).

In many aspects the surface $S'$ behaves like a $K3$ surface.
Beware, however, that it may not always be deformed to a $K3$ surface:
this is the case if and only if $d \leq 6$; if
$d>6$ the elliptic singularity on $S'$ gotten from the contraction of
the proper transform of $R$ is not smoothable, see
\cite{abs}.

Surfaces of this kind naturally occur in degenerations of
$K3$ surfaces.
For instance, surfaces $S'$ as above with $d=4$ appear in
degenerations of smooth quartics in $\P^3$
to the union of a smooth cubic and a plane,
see \cite[Section \tref{ssec:another}]{01.ciro};
there we have seen that the logarithmic Severi variety
$V^4_g(12,0)(\Omega)$ of the pair $(\P^2,R)$ appears in the limit of
the Severi varieties of genus $g$ hyperplane sections of smooth
quartics. 

There are of course many variants of this situation.
For instance, Du Val surfaces\footnote
{a genus $p$ Du Val surface is the projective plane blown-up at nine
  points on a smooth cubic $R$, endowed with the linear system of
  the proper transforms of plane curves of degree $3g$ with a
  $g$-tuple ordinary point at the first eight blown-up points, and a
  $(g-1)$-tuple ordinary point at the remaining blown-up point; these
  curves have geometric genus $g$, and the linear system has dimension
  $g$ (note that it has a tenth base point lying on $R$).
}
have been brought in the foreground recently in \cite{abfs}.
In this volume we shall often consider the case when $S$ is a toric
surface, 
and $R$ is a cycle of smooth rational curves, the sum of all toric
divisors of $S$. An emblematic instance of this situation is
that of the pair consisting of $\P^2$ and a triangle, endowed with the
linear system of plane quartics passing through twelve points cut out
as above on the triangle by a quartic; it occurs in the degeneration
of quartic $K3$ surfaces in $\P^3$ to a tetrahedron,
see \cite[\tref{ssec:quartiche}]{01.ciro}
in which it corresponds to the contribution of a face (see ibid.).
Other examples are given in
\cite[Section \tref{s:degenK3}]{11.th-toric-trop}.


\paragraph{Logarithmic $K3$ surfaces}
\label{p:logK3}
Let $S' \subset \P^p$ be as in \ref{p:can-sect}.
For all $g=0,\ldots,p$,
we may view the Severi variety of genus $g$ hyperplane sections of
$S' \subset \P^p$
as the logarithmic Severi variety
$V_p ^{d} (3d,0)(\Omega)$ of the pair $(\P^2,R)$.
Its expected dimension,
as defined in \ref{p:expdim},
% given in \ref{P0}
is $g-1$, whereas its actual dimension is $g$; note that once again
\ref{P0} does not apply, because the required inequality does not
hold. 
In this case the discrepancy between the actual and expected
dimensions
comes from the fact that the points in $\Omega$
are not general points on $R$.
% (and therefore, according to our Definition~\ref{d:log-severi}
% $V_g ^{d} (3d,0)(\Omega)$ is not a Severi variety).
This is illustrated in Examples
\ref{ex:logK3i}
and \ref{ex:logK3ii}
below.

It is pleasant to think of the pair $(\P^2,R)$ endowed with a set
$\Omega$ as a
\emph{logarithmic $K3$ surface}, \emph{algebraic} when $\Omega$ is
cut out on $R$ by a plane curve as above, and
\emph{non-algebraic} otherwise,
when the points in $\Omega$ are in general position.
One may prefer to consider that the logarithmic $K3$ surface is the
equivalent data of the pair $(S',R')$, where $S'$ is the blow-up of
$\P^2$ at $\Omega$, and $R'$ is the proper transform of $R$.
For a more conceptual definition, as well as a classification, I refer
to \cite{iitaka}.

In the logarithmic context, the manoeuver of taking non-algebraic
$K3$'s into account to adjust the expected dimension takes the
following guise:
% To realize $|C'|$ as a Severi variety of the expected dimension, we
% may consider
one chooses an arbitrary point $a \in \Omega$,
and considers
$V_p ^{d} (3d-1,1)(\Omega-a)$
instead of $V_p ^{d} (3d,0)(\Omega)$.
Statement \ref{P0} applies to the former, which thus has both expected
and actual dimension equal to $p$, 
and it turns out 
that the mobile contact point with $R$ remains in fact immobile,
so that all members of
$V_p ^{d} (3d-1,1)(\Omega-a)$
automatically pass through the point $a$ as well.


\medskip
\subparagraph{Example}
\label{ex:logK3i}
Let us illustrate this in the concrete case $d=4$ (then, $p=3$).
The linear system of plane quartics has dimension $14$. 
If we take a set $\Omega$ of $12$ general points on $R$, then the
Severi variety $V_3^4(12,0)(\Omega)$ is empty: $\Omega$ imposes $12$
independent conditions on quartics, the linear system of
quartics through $\Omega$ is $2$-dimensional, and all its members are
made of $R$ plus a line.
On the other hand if we take $\Omega$ the complete intersection of $R$ with
a smooth quartic $C$, then one sees using the restriction exact
sequence 
\begin{equation*}
0 \to 
\O_{\P^2}(1) \to 
\O_{\P^2}(4) \to 
\O_{R}(4) \to 0
\end{equation*}
that the linear system of
quartics through $\Omega$ is $3$-dimensional,
generated by $C$ and the net of reducible quartics containing $R$.
If we take a set $\Omega$ of $11$ general points on $R$, it imposes
$11$ independent conditions on quartics, and 
the linear system of
quartics through $\Omega$ is $3$-dimensional with a $12$-th base point
on $R$. 

\medskip
\subparagraph{Example}
\label{ex:logK3ii}
We may consider the linear system $|2C'|$ in a similar fashion.
% although there is no completely convincing way of realizing it as a
% genuine Severi variety. 
Seen
on $\P^2$, it is the system of plane $(2d)$-ics with a node at each of
the $3d$ points of $\Omega=C \cap R$.

Again we shall work this out in the case $d=4$. 
One has $(2C')^2=4\cdot (C')^2=16=2\cdot 9-2$,
so the adjunction formula on $S'$, which is essentially the same as on a
$K3$ surface, tells us that curves in $|2C'|$ have genus $9$. 
Moreover the Riemann--Roch Formula, which works as on a
$K3$ as well, tells us that $|2C'|$ has dimension $9$.

On the other hand plane octics have
arithmetic genus $21$, so an octic with $12$ nodes has geometric genus
$9$, confirming the above computations carried out on $S'$. 
The linear system of plane octics has dimension $44$.
Since a node at a prescribed point is $3$ conditions, the expected
dimension of a linear system of octics with $12$ nodes at prescribed
points is $44-36=8$.
When the nodes are imposed at a general set of points $\Omega$ on $R$,
this is indeed the correct dimension, and the linear system consists
only of curves made of $R$ plus a quintic curve passing (in general
simply) through $\Omega$.
When $\Omega$ is cut out on $R$ by a quartic curve $C_1$, the linear
system has an extra generator (namely, the curve $2C_1$),
and  thus has one extra dimension.

This may also be verified using a resolution of the ideal sheaf
${\cal I}_\Omega^2$, where ${\cal I}_\Omega$ is the ideal sheaf of
$\Omega \subset \P^2$.
Let $r$ and $f$ be homogeneous equations of the curves $R$ and
$C$ respectively. While for ${\cal I}_\Omega$ there is the Koszul
resolution, for its square we have the exact sequence
\begin{equation*}
\setlength\arraycolsep{4pt}
  0 \to
\O(-10) \oplus
\O(-11)
\xrightarrow 
{\scalebox{.7}
          {$\begin{pmatrix}
          -f & 0\\
          r & -f \\
          0 & r
          \end{pmatrix}$}
}
\O(-6) \oplus
\O(-7) \oplus
\O(-8)
\xrightarrow 
{
(r^2,\, rf,\, f^2)
}
{\cal I}_\Omega ^2 \to 0,
\end{equation*}
which gives $h^0(\O_{\P^2}(8) \otimes {\cal I}_\Omega ^2)=10$ as required.

\medskip
% \paragraph{}
This carries over to all systems $|kC'|$, to the effect that
the condition of having a $k$-uple point at all $3d$ points of
$\Omega=C \cap R$ imposes one less condition on plane $d$-ics
than if the $3d$ points of $\Omega$ were in
general position. We leave this to the reader.



\paragraph{Severi varieties of curves with full contact}
Logarithmic Severi varieties of logarithmic $K3$ surfaces $(S,R)$
parametrizing curves having one point of contact with high order with
$R$ have attracted the attention for several reasons.
A first reason is the possibility, if $(S,R)$ comes from a
degeneration of $K3$ surfaces, to deform such a logarithmic Severi
variety (roughly speaking) to a Severi variety on the nearby $K3$
surfaces, the contact point of high order $m$ deforming to $m-1$
nodes: this is the central theme of the present volume,
in particular see \cite{04b.concettina}.
Besides, this
possibility is not specific to $K3$ surfaces.

Another reason is the search for $\A^1$ curves
(\ie curves isomorphic to the affine line, in other words affine
rational curves) on logarithmic $K3$ surfaces,
which is the analogue of the search for rational curves on $K3$
surfaces. 
Let me use an example to clarify this problem.
Consider the projective plane together with a smooth cubic curve $R$
(and an empty set of points $\Omega$). The problem is to find $\A^1$
curves lying in the open surface $\P^2 \setminus R$.
To this effect it is relevant to consider the logarithmic Severi
varieties
$V_0^d(0,[0,\ldots,0,3d])$
of the pair $(\P^2,R)$.
They have expected dimension $0$, and of course for any such curve the
contact point with $R$ must be one of the $(3d)^2$ order $3d$ torsion
points of $R$.
The problem of the existence of $\A^1$ curves thus corresponds to that
of the non-emptiness of these logarithmic Severi varieties.
The characterization of the log-$K3$ surfaces for which there exists
infinitely many $\A^1$ curves has been carried out in
\cite{chen-zhu}.
The interested reader may also consult \cite{SeveriEnriques}
for other non-emptiness results, in particular
\cite[Prop.~3.12]{SeveriEnriques}.

Logarithmic Severi varieties with one point of full contact have also 
been related in \cite{vertex} with the tropical vertex group.
Elements of this group are formal families of symplectomorphisms of
the 2-dimensional algebraic torus $(\C^*)^2$.
The relevant Severi varieties are the following: let $S$ be a toric
surface, and let $R$ be the sum of all toric divisors
$R_1,\ldots,R_n,R_\out$
($R_\out$ is simply one of the toric divisors, to which we want to
give a special role); one considers logarithmic Severi varieties
of the pair $(S,R)$ of
the form
\[
  V_0^\xi \bigl(
  (\alpha_1,\ldots,\alpha_n,0),
  (0,\ldots,0, [0,\ldots,0,m])
  \bigr)
  (\Omega_1,\ldots,\Omega_n,\emptyset),
\]
which parametrize rational curves having fixed intersection schemes
with $R_1,\ldots,R_n$, and one contact point of maximal order
$m=\xi\cdot R_\out$ with $R_\out$.
These logarithmic Severi varieties have expected and actual dimension
$0$, and the number of points they are made of may be interpreted as
Gromov--Witten invariants. The main result of \cite{vertex} is that
these numbers are structure constants of the tropical vertex group;
they are in fact determined by ordered product
factorizations of commutators in the tropical vertex group, namely
they appear as the coefficients of the logarithms of the factors.


\begin{references}

\begin{thebibliography}[Chapters in this Volume]{XI}

\bibitem[\tref{01.ciro}]{01.ciro}
C.~Ciliberto {\normalfont \smfandname} Th.~Dedieu,
\emph{Limits of nodal curves: generalities and examples}.

\bibitem[\tref{02.edoardo}]{02.edoardo}
E.~Sernesi, \emph{Deformations of curves on surfaces}.

\bibitem[\tref{04.concettina}]{04.concettina}
Th.~Dedieu {\normalfont \smfandname} C.~Galati,
\emph{Degenerations and deformations of generalized Severi varieties}.

\bibitem[\tref{08.th-exem}]{08.th-exem}
Th.~Dedieu,
\emph{The Caporaso--Harris recursion within a degeneration of the
  plane}.

\bibitem[\tref{04b.concettina}]{04b.concettina}
C.~Galati,
\emph{Proving the existence of curves  on smooth surfaces
  by smoothing tacnodes on reducible surfaces}.

\bibitem[\tref{11.th-toric-trop}]{11.th-toric-trop}
  Th.~Dedieu,
  \emph{Enumeration of curves in toric surfaces, tropical geometry,
    and floor diagrams}.
    
\bibitem[\tref{10.th-panoramico}]{10.th-panoramico}
{\Th}.~Dedieu, \emph{Enumerative geometry of {$K3$} surfaces}.

\end{thebibliography}

\begin{thebibliography}[External References]{10}

\bibitem{abfs}
E.~Arbarello, A.~Bruno, G.~Farkas {\normalfont \smfandname} G.~Sacc\`a,
  \emph{Explicit {B}rill-{N}oether-{P}etri general curves}, Comment. Math.
  Helv. \textbf{91} (2016), no.~3, 477--491.

\bibitem{abs}
E.~Arbarello, A.~Bruno {\normalfont \smfandname} E.~Sernesi, \emph{On
  hyperplane sections of {K}3 surfaces}, Algebr. Geom. \textbf{4} (2017),
  no.~5, 562--596.

\bibitem{AC80}
E.~Arbarello {\normalfont \smfandname} M.~Cornalba,
\emph{Su una propriet\`a notevole dei morfismi di una curva a moduli
generali in uno spazio proiettivo},
Rend.\ Sem.\ Mat.\ Univ.\ Politec.\ Torino \textbf{38} (1980), no.~2,
  87--99 (1981).

\bibitem{AC81}
E.~Arbarello {\normalfont \smfandname} M.~Cornalba,
\emph{Su una congettura di
  {P}etri}, Comment. Math. Helv. \textbf{56} (1981), no.~1, 1--38.

\bibitem{bhpv}
W.~P. {Barth}, K.~{Hulek}, C.~A.~M. {Peters} {\normalfont \smfandname} A.~{Van
  de Ven}, \emph{{Compact complex surfaces}}, 2nd enlarged \smfedname, {Ergeb.
  Math. Grenzgeb., 3. Folge}, vol.~4, Berlin: Springer, 2004.

\bibitem{ch}
L.~Caporaso {\normalfont \smfandname} J.~Harris, \emph{Counting plane curves of
  any genus}, Invent. Math. \textbf{131} (1998), no.~2, 345--392.

\bibitem{chen-zhu}
X.~Chen {\normalfont \smfandname} Y.~Zhu, \emph{{$\mathbb{A}^1$} curves on log
  {K}3 surfaces}, Adv. Math. \textbf{313} (2017), 718--745.

\bibitem{cd-double}
C.~Ciliberto {\normalfont \smfandname} {\Th}.~Dedieu, \emph{Double covers and
  extensions}, to appear in Kyoto J. Math.

\bibitem{SeveriEnriques}
C.~Ciliberto, {\Th}.~Dedieu, C.~Galati {\normalfont \smfandname} A.~L. Knutsen,
  \emph{Nonemptiness of {S}everi varieties on {E}nriques surfaces}, Forum Math.
  Sigma \textbf{11} (2023), e52.

\bibitem{DS15}
{\Th}.~Dedieu {\normalfont \smfandname} E.~Sernesi, \emph{Equigeneric and
  equisingular families of curves on surfaces}, Pub. Mat. \textbf{62} (2017),
  175--212.

\bibitem{vertex}
M.~Gross, R.~Pandharipande {\normalfont \smfandname} B.~Siebert, \emph{The
  tropical vertex}, Duke Math. J. \textbf{153} (2010), no.~2, 297--362.

\bibitem{hartshorne-def}
R.~Hartshorne, \emph{Deformation theory}, Graduate Texts in Mathematics,
  vol.~257, Springer, New York, 2010.

\bibitem{iitaka}
S.~Iitaka, \emph{On logarithmic {$K3$} surfaces}, Osaka Math. J. \textbf{16}
  (1979), no.~3, 675--705.

\bibitem{jK96}
J.~Koll{\'a}r, \emph{Rational curves on algebraic varieties}, Ergebnisse der
  Mathematik und ihrer Grenzgebiete. 3. Folge. A Series of Modern Surveys in
  Mathematics, vol.~32, Springer-Verlag, Berlin, 1996.

\bibitem{eS06}
E.~Sernesi, \emph{Deformations of algebraic schemes}, Grundlehren der
  Mathematischen Wissenschaften, vol.~334, Springer-Verlag, Berlin, 2006.

\bibitem{tannenbaum}
A.~Tannenbaum, \emph{Families of algebraic curves with nodes}, Compositio Math.
  \textbf{41} (1980), no.~1, 107--126.

\bibitem{bT80}
B.~Teissier, \emph{{R\'esolution simultan\'ee I, II}}, in \emph{S{\'e}minaire
  sur les singularit{\'e}s des surfaces, Cent. Math. {\'E}c. Polytech.,
  Palaiseau 1976--77}, Lecture Notes in Mathematics, vol.~777, Springer-Verlag,
  Berlin, 1980, 71--146.

\bibitem{zariski}
O.~Zariski,
\emph{Dimension-theoretic characterization of
maximal irreducible algebraic systems of
plane nodal curves of a given order $n$
and with a given number $d$ of nodes},
Am.\ J.\ Math.\ {\bf 104} (1982), no.~1, 209--226.

\end{thebibliography}

\end{references}

\stopcontents[severi]




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End:


==> 04.concettina/lecture3-galati1.tex <==
\chaptitle{Degenerations and deformations of generalized Severi varieties}
\chapauthor{Thomas Dedieu and Concettina Galati}


\startchap
\label{04.concettina}


\newcommand{\Nseq}{\underline{\N}}
\newcommand{\bm}{\mathbf{m}}
\newcommand{\bmm}{{\mathbf{m}-\mathbf{1}}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\irr}{\mathrm{irr}}
\newcommand{\cub}{{3+1}}%{\mathrm{cub}}

\newenvironment{perso}{\color{gray}}{}
\newenvironment{taf}{\color{blue}}{}

% \excludecomment{perso}
% \excludecomment{com}


% \begin{abstract} 
% These two lectures are devoted to the enumerative formula by Caporaso and Harris for the degree of Severi varieties. 
% We focus on part of the proof and in particular on Theorems 1.2 and 1.3 of \cite{caporaso-harris}.
% \end{abstract}



\startcontents[04.concettina]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[04.concettina]{}{1}[2]{}



\bigskip

This text is dedicated to the recursive formula obtained by Caporaso
and Harris \cite{caporaso-harris} as a solution to the problem of
``counting plane curves of any genus'',
see Corollary \ref{c:CHmain}
and Theorem \ref{t:CHirred}.
Fix a degree $d \in \N^*$, and denote by $p_a(d)=\frac 1 2 (d-1)(d-2)$
the genus of smooth plane curves of degree $d$.
For all $g=0,\ldots,p_a(d)$, (reduced) plane curves of degree $d$
and geometric genus
$g$ form a family of pure dimension
$\nu^d_g = 3d+g-1$.
The problem is to find the number of plane curves of degree $d$ and
geometric genus $g$ passing through $\nu^d_g$ general points in the
plane.
It turns out that this number equals the number of $\delta$-nodal plane
curves of degree $d$ which pass through $\nu^d_g$ general points in
the plane, with $\delta = p_a(d)-g$
(a curve is $\delta$-nodal if its singularities are exactly $\delta$
nodes, \ie $\delta$ ordinary double points).

Caporaso and Harris obtain their inductive formula by specializing one
after another the aforementioned $\nu^d_g$ imposed crossing points to
general points on a fixed line $L$.
This may be conveniently formulated in terms of a degeneration of the
projective plane $\P^2$ to the transverse union along a line
of $\P^2$ and a minimal rational ruled surface $\F_1$, using the
formalism presented in \cite{01.ciro}.
We will do it on an example in \cite{08.th-exem}, but here we stick to
the presentation given in \cite{caporaso-harris}.
A similar result for curves on minimal rational ruled surfaces has
been obtained by Vakil \cite{vakil}, following a similar degeneration
procedure, and around the same period of the time. We shall nevertheless
concentrate on the case of plane curves.

The above described degeneration procedure makes it necessary to
generalize the problem. Thus, one is led to count curves of given
degree and genus with, in addition,
a prescribed intersection pattern with the
line $L$, both at assigned and unassigned points. We shall call
\emph{generalized Severi varieties} the families formed by these
curves: they are a particular case of the logarithmic Severi varieties
studied in \cite{03.th-acz}.

We give precise definitions and statements in Section~\ref{S:statements}
below. There, we shall also provide more details about the general
strategy of the proof, which will explain the title of this text.



\section{The counting problem and its solution}
\label{S:statements}

Let us fix once and for all a line $L \subset \P^2$.
We shall use freely the notation and definitions introduced in
\cite[Section \tref{S:results}]{03.th-acz},
in the special case when the pair $(S,R)$ is
$(\P^2,L)$;
every class $\xi \in \NS(\P^2)$ is $d$ times the linear
equivalence class of a line for some integer $d$, and therefore it shall
be denoted simply by $d$.

Let $d\in \N$ and $g\in \Z$,
let $\alpha=(\alpha_i)_{i\geq 1}$ and
$\beta=(\beta_i)_{i\geq 1}$ be two sequences in $\Nseq$ such that
$I\alpha+I\beta =d$, and let
$\Omega = \bigl( \{p _{i,j}\} _{1 \leq j \leq \alpha_i}
\bigr) _{i \geq 1}$ be a set of $\alpha$ points on the line $L$.
The \emph{logarithmic Severi variety}
$V_g^d (\alpha,\beta)(\Omega)$ is the locally closed
subset of $|\O_{\P^2}(d)|$
(the projective space of dimension $\frac 1 2 d(d+3)$ parametrizing all
plane curves of degree $d$)
parametrizing those reduced plane curves of degree $d$ and
geometric genus $g$
that intersect $L$ at the points of $\Omega$ with the multiplicities
prescribed by $\alpha$ and at further unassigned points with the
multiplicities prescribed by $\beta$;
for the rigorous definition,
see \cite[Definition \tref{d:log-severi:curve}]{03.th-acz}.
The points of $\Omega$ shall be referred to as the \emph{fixed}, or
\emph{assigned}, contact points, and the other intersection points with
$L$ as \emph{mobile}, or \emph{unassigned}, contact points
(as it turns out, in the present situation, the unassigned contact
points indeed move as the curves moves in the Severi variety, see
Proposition~\ref{p:zariski} below). 
The relevant notation for these points and their relatives is
explained in Paragraph \ref{p:notat:principles}.
Forgetting about the location of assigned intersection points at
$\Omega$, 
we may also loosely say that the curves in $V_g^d
(\alpha,\beta)(\Omega)$ have intersection pattern with $L$ prescribed
by $\alpha$ and $\beta$.

As it turns out (see Proposition~\ref{p:zariski} below),
the general element of every irreducible component of
$V_g^d (\alpha,\beta)(\Omega)$ has $\delta$ nodes and no further
singularities, with
\[
  \delta = p_a(d)-g =
  \frac 1 2 (d-1)(d-2) -g.
\]
The upshot is that it is indifferent to require either that the
geometric genus be $g$ or that the singularities be exactly $\delta$
nodes. 

\begin{definition}
\label{04:d:log-severi}
For all natural integers $d$ and $\delta$,
and all $\alpha,\beta \in \Nseq$ and $\Omega$ as above,
the \emph{generalized Severi variety}
$V^{d,\delta} (\alpha,\beta)(\Omega)$ is the Zariski closure in
the projective space $|\O_{\P^2}(d)|$ of the logarithmic Severi
variety
$V_{p_a(d)-\delta}^d (\alpha,\beta)(\Omega)$
of the pair $(\P^2,L)$.
\end{definition}

\noindent
In the particular case when
$\alpha=0$, and thus $\Omega = \emptyset$,
and $\beta = (d,0,\ldots)$
(\ie when no conditions are imposed on the intersection with $L$),
the Severi varieties
$V_g^d (\alpha,\beta)(\Omega)$
and $V^{d,\delta} (\alpha,\beta)(\Omega)$ will simply be denoted by
$V^d_g$ and $V^{d,\delta}$, respectively, and called \emph{plain}
Severi varieties.

Although this should not create any problem, beware that
in our notation $V^d_g$ and $V^{d,\delta}$
(with any additional decorations) are respectively 
locally closed and closed in $|\O_{\P^2}(d)|$.

\bigskip
For any point $p\in \P^2$, the degree $d$ plane curves
passing through the point $p$ form a hyperplane
$\orth p$ in the projective space $|\O_{\P^2}(d)|$.
Therefore, the problem of counting curves of degree $d$ and genus $g$
(and no further conditions) mentioned in the introduction
amounts to the problem of computing the degree of the plain Severi
variety $V^{d,\delta} = \smash{\overline V}^d_g$,
with $\delta = p_a(d)-g$.
We shall denote this number by $N^{d,\delta}$.
More generally, for all $\alpha,\beta \in \Nseq$, we shall denote by
$N^{d,\delta}(\alpha,\beta)$ the common degree of all
$V_g^d (\alpha,\beta)(\Omega)$, where $\Omega$ is a general,
cardinality $\alpha$, set of points of $L$.

The recursion procedure of Caporaso and Harris consists in computing
the number $N^{d,\delta}$ by cutting $V^{d,\delta}$ by hyperplanes
$\orth p$ with $p \in L$.
Their main result is Theorem \ref{t:CHmain} below.
We need some additional notation to state it.

\begin{notation}
For all $k\in \N^*$, we let
$e_k = (0,\ldots,0, 1) \in \Nseq$: it is the sequence with only one
non-zero entry, in $k$-th position and equal to $1$
(recall the convention made in \cite{03.th-acz} that we may omit the
infinite sequence of zeros at the end of elements of $\Nseq$).
For all $\beta,\beta'\in\Nseq$, we let
\[
  \textstyle
  I^\beta = \prod_{k\geq 1} k^{\beta_k}
  \qquad \text{and}\qquad
  \binom {\beta'} \beta
  = \prod_{k\geq 1} \binom {\beta'_k} {\beta_k}.
\]
If $\Omega=(\Omega_1,\Omega_2,\ldots)$ is a set of cardinality
$\alpha\in \Nseq$, a subset of $\Omega$ of cardinality $\alpha'\leq
\alpha$ is simply a set
$\Omega'=(\Omega'_1,\Omega'_2,\ldots)$ of cardinality
$\alpha'\in \Nseq$
such that $\Omega'_k \subset \Omega_k$ for all $k\geq 1$.

The following notation is not needed to state the main theorem below,
but we shall use it for the proof and in the more precise
Theorem~\ref{t:CH1.3}.
For all $\beta \in \Nseq$, we let
\[
  \lcm (\beta) = \lcm \{ i: \beta_i \neq 0 \}
  \qquad \text{and}
  \qquad
  \max (\beta) = \max \{ i: \beta_i \neq 0 \}.  
\]
\end{notation}

\begin{convention}
\label{conv:deg-d-1}
In the statement below, generalized Severi varieties
$V^{d-1,\delta'}(\alpha',\beta')(\Omega') \subset |\O_{\P^2}(d-1)|$
are considered as the projective subvarieties of $|\O_{\P^2}(d)|$
parametrizing all curves of the form $C+L$ with
$C\in V^{d-1,\delta'}(\alpha',\beta')(\Omega')$.
We will make this identification freely all along the text, where
needed. 
\end{convention}

\begin{theorem}[Caporaso--Harris]
\label{t:CHmain}
Let $d$ and $\delta$ be natural integers,
and let
$\alpha,\beta \in \Nseq$ be sequences such that $I\alpha+I\beta=d$,
and $\Omega$ be a set of $\alpha$ general points on the line $L$.
Let $p$ be a general point of $L$.
Then one has the following equality of cycles:
\begin{multline}
\label{eq:CH-cycles}
{V}^{d,\delta}(\alpha,\beta)(\Omega)\cap \orth p
  =
  \sum_{k\geq 1:\, \beta_k>0}
  k\cdot
  V^{d,\delta}(\alpha+e_k,\beta-e_k)(\Omega\cup \{p\})
  \\
  +
  \sum_{
    \substack{
      \Omega'\subset \Omega,\, \Card(\Omega')=\alpha' \\
      \beta'\geq \beta:\, I\alpha' +I\beta'=d-1 \\
      \delta' = \delta+|\beta'-\beta|-d+1
    }}
  I^{\beta'-\beta} \binom {\beta'}\beta \cdot
  V^{d-1,\delta'}(\alpha',\beta')(\Omega')
\end{multline}
where, in the first sum,
$\Omega\cup \{p\}$ means that we add the point $p$ to the $k$-th term
of $\Omega=(\Omega_1,\Omega_2,\ldots)$. 
\end{theorem}

Note that, in the above theorem, if we start with a plain Severi
variety for ${V}^{d,\delta}(\alpha,\beta)(\Omega)$
(\ie if $\alpha=0$ and thus $\Omega = \emptyset$, and $\beta = (d)$),
then the
intersection with $\orth p$ decomposes as a sum of genuinely
generalized (\ie non-plain) Severi varieties.
This is why one needs to generalize the problem of counting curves of
fixed degree and genus for the inductive solution proposed by
Caporaso and Harris.

It follows from Proposition~\ref{p:zariski} below that if $p$ is
outside of $\Omega$, then no irreducible component of
${V}^{d,\delta}(\alpha,\beta)(\Omega)$ is contained in the hyperplane
$\orth p$. Therefore, all irreducible varieties appearing on the
right-hand-side of \eqref{eq:CH-cycles} above have codimension one in
${V}^{d,\delta}(\alpha,\beta)(\Omega)$, and indeed we shall verify
this by hand later in the text.
The number $N^{d,\delta}(\alpha,\beta)$ we are looking for is the
degree of ${V}^{d,\delta}(\alpha,\beta)(\Omega)$ as well as that of
the cycle on the
right-hand-side of \eqref{eq:CH-cycles}.
Thus, Theorem~\ref{t:CHmain} has the following direct corollary.

\begin{corollary}
\label{c:CHmain}
Let $d$ and $\delta$ be natural integers,
and let
$\alpha,\beta \in \Nseq$ be sequences such that $I\alpha+I\beta=d$.
Then one has the following equality:
\begin{equation*}
\label{eq:CH-numbers}
  N^{d,\delta}(\alpha,\beta)
  =
  \sum_{k\geq 1:\, \beta_k>0}
  k\cdot N^{d,\delta}(\alpha+e_k,\beta-e_k)
  +
  \sum_{
    \substack{
      \alpha' \leq \alpha \\
      \beta'\geq \beta:\, I\alpha' +I\beta'=d-1 \\
      \delta' = \delta+|\beta'-\beta|-d+1
    }}
  \kern -1em
  I^{\beta'-\beta} \binom {\beta'}\beta
  \binom {\alpha'}\alpha \cdot
  N^{d-1,\delta'}(\alpha',\beta').
\end{equation*}
\end{corollary}

Since the numbers $N^{1,\delta}(\alpha,\beta)$ are readily computed,
the above recursive formula enables one to compute all numbers
$N^{d,\delta}(\alpha,\beta)$, and thus to completely solve our
counting problem.
Note that the recursion indeed terminates, as those terms appearing in
the first sum are all of the form $N^{d,\delta}(\alpha'',\beta'')$ with
$\beta''<\beta$, so that unassigned intersection with $L$ are
exhausted after finitely many applications of the formula,
and then only terms of the form
$N^{d-1,\delta'}(\alpha',\beta')$ appear.
It is of course helpful to watch the inductive process work on a
concrete example. For this we refer to
\cite{08.th-exem}, or
\cite[p.~349]{caporaso-harris}; see also Example~\ref{ex:irred}.

Although, arguably, the relevant enumerative problem is to count
irreducible plane curves of any genus, there is no irreducibility
requirement in our definition of Severi varieties, and therefore the
numbers $N^{d,\delta}(\alpha,\beta)$ count curves regardless of their
being irreducible or not.
It is yet possible to derive a recursion formula counting irreducible
curves using the inductive process of Caporaso and Harris (and so do
they in the original article). We postpone this until
Section~\ref{S:irred}, as the formula is yet more complicated than the
above one, and
having the geometry of the inductive process in mind helps in
understanding it.


\bigskip
The proof of Theorem~\ref{t:CHmain} is in two parts.
The first one consists in using stable reduction in order to limit
the possible irreducible components of the intersection 
of $V^{d,\delta}(\alpha,\beta)(\Omega)$ and $\orth p$.
This is the degeneration part; it is carried out in
Section \ref{s:thm1.2}
and the result is Theorem \ref{t:CH1.2}.
The dimensional characterization of Severi varieties
(Proposition \ref{c:zariski-forte})
is fundamental in identifying the components of
the intersection as generalized Severi varieties.

The second part consists in showing that all the generalized Severi
varieties found in the first part indeed occur as irreducible
components of the intersection
of $V^{d,\delta}(\alpha,\beta)(\Omega)$ and $\orth p$,
and to compute their multiplicites in this intersection.
This is the deformation part; it is carried out in
Section \ref{S:deform}
and the result is Theorem \ref{t:CH1.3}.
A fundamental result for this part is the study of the deformation
space of an $m$-tacnode into $m-1$ nodes, also due to Caporaso and
Harris, and described in \cite{05.margherita}.
The latter result is certainly the central result of this whole volume
of notes.

Theorems \ref{t:CH1.2} and \ref{t:CH1.3} together directly imply
Theorem \ref{t:CHmain}.



\section{Recap on Severi varieties}
\label{S:recap}


\paragraph{}
\label{p:notat:principles}
We shall use consistent notation to denote assigned and unassigned
contact points with the line $L$.
Consider a generalized Severi variety
$V^{d,\delta}(\alpha,\beta)(\Omega)$
as in Definition~\ref{04:d:log-severi}.
The assigned contact points with $L$ are the elements of $\Omega$,
which we write as
$\Omega = \bigl( \{p _{i,j}\} _{1 \leq j \leq \alpha_i}
\bigr) _{i \geq 1}$.
Let $[C]$ be a general member of any irreducible component
of $V^{d,\delta}(\alpha,\beta)(\Omega)$. Denote by
$\bar C \to C$ the normalization of $C$, and by $\phi:\bar C \to \P^2$
its composition with the inclusion $C \subset \P^2$.
By definition of the Severi varieties,
there exist $\alpha$ points $q _{i,j} \in \bar C$,
for all $i\geq 1$ and $1 \leq j \leq \alpha_i$,
and $\beta$ points $r _{i,j} \in \bar C$,
for all $i\geq 1$ and $1 \leq j \leq \beta_i$,
such that
\begin{equation*}
%\label{C1-def}
\forall\, i\geq 1,\
\forall\, j=1,\ldots,\alpha_i: \quad
\phi (q_{i,j}) = p_{i,j} 
\end{equation*}
and
\begin{equation*}
%\label{C2-def}
  \phi^* L =
  \sum _{i\geq 1} \sum _{1 \leq j \leq \alpha_i} i \, q_{i,j}
+ \sum _{i\geq 1} \sum _{1 \leq j \leq \beta_i} i\, r_{i,j}.
\end{equation*}
Moreover, we let $s_{i,j} = \phi(r_{i,j})$
for all $i\geq 1$ and $1 \leq j \leq \beta_i$.

Thus, the assigned and unassigned contact points of $C$ with $L$ are,
respectively, the $p_{i,j}$'s and the $s_{i,j}$'s,
and their respective counterparts on the normalization $\bar C$
are the $q_{i,j}$'s and the $r_{i,j}$'s.\footnote
{The reader may wish to keep in mind that
$\phi(q_{i,j})=p_{i,j}$ whereas
$\phi(r_{i,j})=s_{i,j}$;
thus, beware, $\phi$ goes backwards with the alphabetical order for
the assigned contact points, but forward for the unassigned ones.
}



\bigskip
The two following results are key ingredients in the proof of both
Theorems \ref{t:CH1.2} and \ref{t:CH1.3}.
% They are inspired by Zariski's dimension
% characterization theorem for Severi varieties of plane curves.
They are direct applications of
Theorem \tref{T} and Proposition \tref{pr:charact} in
\cite{03.th-acz}, respectively.
 
\begin{proposition}%[Prop. 2.1 and 2.2 of \cite{caporaso-harris}]
\label{p:zariski}
Let the notation be as in \ref{p:notat:principles}
above.
The generalized Severi variety
$V ^{d,\delta}(\alpha,\beta)(\Omega)$ has pure dimension
$2d+g-1+|\beta|$,
with $g = p_a(d)-\delta$.
Morever:
\begin{compactitem}[---]
\item the curve $C\subset \P^2$ is $\delta$-nodal, and smooth at its
  intersection points with the line $L$;
\item the contact points of $C$ with $L$,
  \ie all the points $p_{i,j}$ and $s_{i,j}$, are altogether pairwise
  distinct; 
\item the counterparts on the normalization $\bar C$ of the contact
  points of $C$ with $L$, 
  \ie all the points $q_{i,j}$ and $r_{i,j}$, are altogether pairwise
  distinct; 
\item for any curve $G$ and finite set $\Gamma$ in $\P^2$,
  if $(G\cup \Gamma) \cap \Omega = \emptyset$
  and $[C]$ is
  general with respect to $G$ and $\Gamma$, then $C$ intersects
  $G$ transversely and does not intersect $\Gamma$.
\end{compactitem}
 \end{proposition} 


   
\begin{proposition}%[Corollary 2.7 of \cite{caporaso-harris}]
\label{c:zariski-forte}
Let $V \subset |\O_{\P^2}(d)|$ be an irreducible variety,
parametrizing genus $g$ curves in the following sense:
for a general member $[X]$ of $V$, there exists a
smooth curve $\tilde X$ of genus $g$,
and a morphism $f: \tilde X \to X$, not constant on any
component of $\tilde X$, and such that the push-forward in the sense of
cycles $f_* \tilde X$ equals the fundamental cycle of $X$.

Let $\Omega \subset L$ be a finite set of points.
For any general member $[X]$ of $V$, one has
\[
  \dim(V)\leq 2d+g-1+
  \Card \bigl( (X \cap L)\setminus \Omega \bigr),
\]
where the last number is defined set-theoretically
(\ie multiplicities do not count).

Moreover, if equality holds, then
there exist $\alpha,\beta \in \Nseq$ such that
$V$ is a dense subset of a
component of the generalized Severi variety
$V^{d,\delta} (\alpha,\beta)(\Omega)$,
$\delta = p_a(d)-g$,
if and only if  
\[
  \Card \bigl( f^{-1}(X \cap L) \bigr) = \Card (X \cap L),
\]
with $f: \tilde X \to X$ a genus $g$ morphism as above. 
\end{proposition}


Lastly, let us mention that, although we pretend not to know it in this
text, all generalized Severi varieties
$V^{d,\delta} (\alpha,\beta)(\Omega)$
have their irreducible components in bijection with the possible
splittings of degree $d$, $\delta$-nodal curves, into several
irreducible components. Thus, for instance, there is at most one
irreducible component of $V^{d,\delta} (\alpha,\beta)(\Omega)$
parametrizing irreducible curves.
This is proved in \cite{harris} for plain Severi varieties, and
in \cite{zahariuc} for generalized Severi varieties.


% \section{Background and notation}\label{sec:background}

% (Qui riprendo della notazione introdotta da Thomas perche' nel mio
% caso e' piu' semplice.)


% We first collect some terminology and notation, in accordance with the one of \cite{caporaso-harris} and of the previous talks. 
% With reference to the {\bf Thomas's Lectures}, in the following two talks we will assume $S=\mathbb P^2$,
% $R=L\subset\mathbb P^2$ a fixed line and $\xi\sim dH$,  where $H\subset \mathbb P^2$ is the linear equivalence 
% class of a line.

% As usually, the \emph{geometric genus} $g(C)$ of a reduced curve $C$ is defined as the genus of its
% normalization $\bar C$.
% %namely 
% %$
% %1 - \chi (\O _{\bar C}) = \sum _{i=1}^n g_i -n +1
% %$
% %where $g_1,\ldots,g_n$ are the respective genera of the connected
% %components $C_1,\ldots,C_n$ of $\bar C$. 
% Moreover, if $C=C_1\cup\cdots\cup C_n$ {\it is a nodal curve with irreducible components} $C_1,...,C_n$, we recall the formula
% for the {\it arithmetic genus}  
% \begin{equation}\label{eq:arith-genus-nodal-curve}
% p_a(C)=1-\chi(\mathcal O_C)=\sum_{i=1}^ng(C_i)+\delta-n+1=\sum_{i=1}^np_a(C_i)+\delta'-n+1,
% \end{equation}
% where $\delta$ is the total number of nodes of $C$ and $\delta'$ is the number of "connection" nodes, i.e. the nodes arising 
% from the intersection of the irreducible components of $C$.
% For every integers $d$ and $g$, we denote by $M _g ^{d, \text{bir}}:=M _g ^{dH, \text{bir}}(\mathbb P^2)$ the space
% parametrizing morphisms
% $
% \phi: C \to S
% $
% from a smooth genus $g$ curve $C$ (projective, but possibly
% disconnected) that are birational to their image, and such that
% $\phi_* [C]$ is a plane curve of degree $d$. Furthermore
% \[
%   V_g ^d \subset\mathbb P^N, \,\textrm{where}\,\,N=\frac{d(d+3)}{2}
% \] 
% denotes the locally closed subscheme of the
% Hilbert scheme of degree $d$ plane curves consisting of those
% points $[C]$ such that $C$ is a reduced plane curve of degree $d$ and has geometric genus $g$.


% %\paragraph{}
% Again, $\Nseq$ denotes the set of sequences $\alpha =
% (\alpha_1,\alpha_2,\ldots)$ of non-negative integers with all but
% finitely many $\alpha_i$ zero. For $\alpha,\alpha' \in \Nseq$, we say that $\alpha
% \geq \alpha'$ if $\alpha_i \geq \alpha'_i$ for all $i \geq 1$, 
% and we recall the definitions
% $
% % \sharp \alpha &= \sharp \{ i : \alpha_i \neq 0\} \,;\\
% |\alpha| = \alpha_1 + \alpha_2 + \cdots $ and
% $
% I\alpha = \alpha_1 + 2\alpha_2 + \cdots + n\alpha_n + \cdots.% \,; \\
% % I ^\alpha &= 1^{\alpha _1} 2^{\alpha _2} \cdots n^{\alpha _n} \cdots
% % \,; \\ % \lcm (\alpha) &= \lcm \{ i: \alpha_i \neq 0 \}
% $
% Moreover,  we let
% \[
%  \sharp \alpha = \sharp \{ i : \alpha_i \neq 0\} \,,
% \,\, I ^\alpha = \Pi_{i\geq 0} i^{\alpha _i} 
%  \, {\rm{and}} \,\,
%  {\rm{lcm}} (\alpha) = {\rm{lcm}} \{ i: \alpha_i \neq 0 \}.
% \]
% Also, we define
% \[
%   \max (\alpha) = \max \{ i: \alpha_i \neq 0 \}.
% \]
% If we set $e_k=(0,...,0,1,0,...)$, where $1$ is the $k^{\rm th}$ term, then, for every  $\alpha\in  \Nseq$,
% we  can write $\alpha=\sum_i\alpha_ie_i.$ If $\alpha, \alpha'\in  \Nseq$, we say that $\alpha\let\alpha'$ if $\alpha_i\leq\alpha_i'$, for every $i$ and
% we set 
% \[
% \left( \begin{array}{c} \alpha \\ \alpha' \end{array} \right)=\Pi_{i\geq 0} \left( \begin{array}{c} \alpha_i \\ \alpha'_i \end{array} \right).
% \] 


% By a set $\Omega$ of cardinality $\alpha \in \Nseq$, we again mean a
% sequence of sets $\Omega = (\Omega_1,\Omega_2,\ldots)$ such that each
% $\Omega_i$ has cardinality $\alpha_i$. 


% \medskip
% Correspondingly, we let 
% \[
%   {V}_g ^d (\alpha,\beta)(\Omega)\subset\mathbb P^N,
% \]
% the Zariski closure be the locally closed subscheme of $V_g^d$ consisting of those
% points $[C]$ such that the normalisation $\nu: \bar C \to C \subset S$
% belongs to $M_g^d(\alpha,\beta)(\Omega)$. 
% % Following \cite{ch}, we call \emph{generalized Severi variety}
% This has been called  \emph{logarithmic Severi variety} of the pair $(\mathbb P^2,R)$
% in the {\bf Thomas's lecture} and \emph{generalized Severi variety} in \cite{caporaso-harris}. We will use the second terminology.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %Teorema 1.2 di Thomas%

% %\medskip \subparagraph{\ Comments and examples.}

% %\begin{theorem}[Extension of Propositions 2.1 and 2.2 of \cite{caporaso-harris}]
% %\label{T}
% %Let $g \in \Z$, $\xi \in \NS (S)$, $\alpha,\beta \in \Nseq$,
% %$\Omega = \{p _{i,j}\} _{1 \leq j \leq \alpha_i} \subset R$ be as in
% %Def.~\ref{04:d:log-severi}, and consider an irreducible component $V$ of
% %${V}_g ^\xi (\alpha,\beta)(\Omega)$.
% %Let $[C]$ be a general member of $V$, $\phi: \bar C \to C
% %\subset S$ its normalization, $q_{i,j}$ ($1 \leq j \leq \alpha_i$),
% %$r_{i,j}$ ($1 \leq j \leq \beta_i$) points on $\bar C$ such that
% %\eqref{C1-def} and \eqref{C2-def} hold.
% %Set
% %\begin{equation*}
% %D= \sum _{1 \leq j \leq \alpha_i} i \, q_{i,j}
% %+ \sum _{1 \leq j \leq \beta_i} (i-1)\, r_{i,j}.
% %\end{equation*}

% %\setcounter{subparagraph}{-1}
% %\smallskip\subparagraph{} \label{P0}
% %If
% %$-K_S \cdot C_i - \deg \left. \phi_* D\right|_{C_i} \geq 1
% %\ \text{for every irreducible component $C_i$ of $C$},$
% %then
% %\begin{equation*}
% %\dim V = -(K_S+R) \cdot \xi +g-1 +|\beta|.
% %\end{equation*}

% %\smallskip\subparagraph{} \label{P1}
% %If
% %$-K_S \cdot C_i - \deg \left. \phi_* D\right|_{C_i} \geq 2
% %\ \text{for every irreducible component $C_i$ of $C$},$
% %then
% %\begin{compactenum}
% %\renewcommand{\theenumi}{\normalfont (\alph{enumi})}
% %{\renewcommand{\theenumi}
%    %   {\normalfont ($\rm\alph{enumi}^{\flat\kern -.3ex \flat}$)}
% %\item 
% %\label{t:a--} 
% %\newcounter{Ta} \setcounter{Ta}{\value{enumi}}
% %the normalization map $\phi$ is an immersion, except
% %possibly at the points $r_{i,j}$;
% %}
% %\item 
% %\label{t:b}
% %the points $q_{i,j}$ and $r_{i,j}$ of $\bar C$ are pairwise
%  % distinct;
% %{\renewcommand{\theenumi}{\normalfont ($\rm\alph{enumi}^\flat$)}
% %\item 
% %\label{t:c-}
% %\newcounter{Tc} \setcounter{Tc}{\value{enumi}}
% %none of the points $s_{i,j} := \phi (r_{i,j})$ belongs to
% %$\Omega$.
% %}
% %\setcounter{memoire}{\value{enumi}}
% %\end{compactenum}

% %\smallskip\subparagraph{} \label{P2}
% %If
% %$-K_S \cdot C_i - \deg \left. \phi_* D\right|_{C_i} \geq 2
% %\ \text{for every irreducible component $C_i$ of $C$},$
% %then
% %\begin{itemize}
% %\item the normalization map $\phi$ is an immersion;
% %\item the points $p_{i,j}$ and $s_{i,j}=\phi(r_{i,j})$ on $C$ are
%   %pairwise distinct.
% %\item the curve $C$ is smooth at its intersection points with $R$;
% %\item for every curve $G \subset S$ and finite set $\Gamma \subset S$
%   %such that $(G\cup \Gamma) \cap \Omega = \emptyset$, if $[C]$ is
%   %general with respect to $G$ and $\Gamma$ then $C$ intersects
%   %$\Gamma$ transversely and does not intersect $\Gamma$.
% %\end{itemize}
% %\begin{compactenum}
% %\renewcommand{\theenumi}{\normalfont (\alph{enumi})}
% %\setcounter{enumi}{\value{Ta}-1}
% %{\renewcommand{\theenumi}{\normalfont ($\rm\alph{enumi}^\flat$)}
% %\item \label{t:a-}
% %the normalization map $\phi$ is an immersion;
% %}
% %\setcounter{enumi}{\value{Tc}-1}
% %\item %\label{t:c}
% %the points $p_{i,j}$ and $s_{i,j}=\phi(r_{i,j})$ on $C$ are
%   %pairwise distinct.
% %\setcounter{enumi}{\value{memoire}}
% %\item 
% %\label{t:d}
% %the curve $C$ is smooth at its intersection points with $R$;
% %\item 
% %\label{t:e}
% %for every curve $G \subset S$ and finite set $\Gamma \subset S$
%   %such that $(G\cup \Gamma) \cap \Omega = \emptyset$, if $[C]$ is
%   %general with respect to $G$ and $\Gamma$ then $C$ intersects
%   %$\Gamma$ transversely and does not intersect $\Gamma$.
% %\end{compactenum}

% %\smallskip\subparagraph{} \label{P3}
% %If
% %$-K_S \cdot C_i - \deg \left. \phi_* D\right|_{C_i} \geq 3
% %\ \text{for every irreducible component $C_i$ of $C$},$
% %then
% %\begin{itemize}
% %\item the curve $C$ is nodal.
% %\end{itemize}
% %\begin{compactenum}
% %\renewcommand{\theenumi}{\normalfont (\alph{enumi})}
% %\setcounter{enumi}{\value{Ta}-1}
% %\item 
% %\label{t:a}
% %the curve $C$ is nodal;
% %\end{compactenum}
% %\end{theorem}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{taf}
  
% \paragraph{Notazioni da introdurre}


% Further notation: in the course of the proof, rather denote sequence
% $\alpha \in \Nseq$
% by $(\alpha_i)_{i\geq 1}$
% rather than $[\alpha_i]_{i\geq 1}$.

% \paragraph{}
% Il faudra \emph{évidemment} donner l'énoncé de la formule de
% récurrence, y compris dans sa version cycles;
% voir alors où énoncer les deux théorèmes principaux. Ce sera sans
% doute bien de donner un exemple également (le même qu'eux sans doute),
% sans marcher sur les plates-bandes du chapitre dédié aux exemples.

% \paragraph{}
% Je pense qu'au point où j'en suis, je peux aussi donner la version
% pour les courbes irréductibles. Avec Remarque~\ref{rk:allred} j'ai
% toute la géométrie, il n'y a plus qu'à faire les comptes et c'est OK.

% \end{taf}


% \section{Lectures 1 and 2 - Concettina}\label{s:concettina1e2}
% The degree of a projective variety $V\subset\mathbb P^N$ is the number of intersection points of $V$ with a general linear subspace $\Lambda$
% of dimension equal to the codimension of $V$. In particular, if $V$ is an irreducible component of the generalized Severi variety 
% ${V}_g ^{d}(\alpha,\beta)(\Omega)$, then $\dim(\Lambda)=\delta=\frac{(d-1)(d-2)}{2}-g.$ Moreover one may consider 
% \[
%   \Lambda=\bigcap_{i=1}^\delta H_{p_i},
% \]
% where $H_p\subset \mathbb P^N$ denotes the hyperplane parametrizing curves 
% passing through a  fixed point $p\in\mathbb P^2$ and $p_1,...,p_\delta$ are general  enough.

% In \cite{caporaso-harris}, the authors provide a complete description, as a scheme, of the hyperplane section ${V}_g ^{d}(\alpha,\beta)(\Omega)\cap H_p$
% when $p$ is a point of $L$. Choosing $p_1,...,p_\delta$ generically on $L$, 
% they obtain an inductive formula for the degree of the generalized Severi variety, which takes their names. The necessity of working with the generalized Severi 
% variety, instead of the traditional one, comes from the fact that when one intersects ${V}_g ^{d}$ with $H_p$, with $p$ in $L$, the result is a union of generalized 
% Severi varieties.

% The description of the hyperplane section ${V}_g ^{d}(\alpha,\beta)(\Omega)\cap H_p$, with $p\in L$, is contained in \cite[Thms 1.2 and 1.3]{caporaso-harris}. To these two
% theorems are devoted the following  two lectures.   In Theorem 1.2, thanks to a very beautiful argument of stable reduction, are enumerated all possibilities for the irreducible components $V$ of  ${V}_g ^{d}(\alpha,\beta)(\Omega)\cap H_p$.
% In Theorem 1.3 is proved that all these possibilities really occur. Moreover, for every irreducible component $V$, studying deformations of tacnodal singularities,
% the authors compute its multiplicity.
 
%  By virtue of Proposition \ref{p:zariski}, if ${V} ^{d, \delta} (\alpha,\beta)(\Omega)\subset\mathbb P^N$ is 
% the Zariski closure be the locally closed subscheme of $V_g^d$ consisting of those
% points $[C]$ such that the normalisation $\nu: \bar C \to C \subset S$
% belongs to $M_g^d(\alpha,\beta)(\Omega)$ and $C$ is a nodal curve, one has that 
% \[
%   {V}^{d,\delta}(\alpha,\beta)(\Omega)={V}_g
%   ^{d}(\alpha,\beta)(\Omega).
% \]
%  We will denote the generalized Severi variety with both symbols.
 
% By the arguments used in the proof of Proposition \ref{p:zariski} one also obtains the following result, that 
% is a dimensional characterization theorem for the generalized Severi varieties. We report the result correcting a misprint in the statement.
% {\bf Thomas, ti prego controlla se ti torna la correzione nello statement.}
 
%  Let $L\subset \mathbb P^2$ be a line and $\Omega\subset L$ a finite subset. Let $V\subset\mathbb P^N$ be a locally closed
%  subset and $[X]\in V$ its general point, corresponding to a possibly non-reduced curve. Let $\pi:W\to X$ be any map from a smooth curve $W$,
%  which is non-constant on any irreducible component of $W$ and whose degree on any irreducible component $X_i$ of $X$ coincides with the multiplicity 
%  of $X_i$ in $X$. In particular $\pi^*{\mathcal O_{\mathbb P^2}(1)}$ has degree $d$. Let $g$ be the geometric genus of $W$
%  and $e$ the cardinality of the intersection $\sharp(X\cap (L\setminus\Omega))$. One then has  
% \\{\color{blue}
%   Aggiustare questo corollario in merito a \cite{03.th-acz}.
%   }

 
%  Our proof of \cite[Thms 1.2 and 1.3]{caporaso-harris} is exactly the one proposed by the authors, reported very shortly. 
 
 
\section{Degenerations of generalized Severi varieties}
% {Theorem 1.2 of \cite{caporaso-harris}}
\label{s:thm1.2}


This section is dedicated to the analysis of how curves in a
generalized Severi variety
${V}^{d,\delta}(\alpha,\beta)(\Omega)$
degenerate when one imposes the passing through a general point of
the line $L$.
The main result of this section is Theorem~\ref{t:CH1.2}
below, but we will also provide in Section \ref{s:localgeom}
a geometric decription of the degeneration
at play, of fundamental importance for the proof of the theorem in the
other direction, \ie Theorem~\ref{t:CH1.3} on deformations of
generalized Severi varieties, which is the object of the next section.

In the following statement,
and as in Convention~\ref{conv:deg-d-1},
for all $\delta',\alpha',\beta',\Omega'$,
the generalized Severi variety
$V^{d-1,\delta'}(\alpha',\beta')(\Omega')$ is identified with a
variety parametrizing degree $d$ curves containing the line $L$,
namely
\[
  \bigl\{
  [C\cup L]:\ 
  [C]\in V^{d-1,\delta'}(\alpha',\beta')(\Omega')
  \bigr\}
  \ \subset
  \
  |\O_{\P^2}(d)|.
\]

\begin{theorem}[{\cite[Theorem 1.2]{caporaso-harris}}]
\label{t:CH1.2}
Let $p\in L$ be a general point,
and let $V$ be an irreducible component of the intersection
\(
  {V}^{d,\delta}(\alpha,\beta)(\Omega)\cap \orth p.
\)
Then $V$ is an irreducible 
component of one of the following varieties:
\begin{compactenum}[a]
\renewcommand{\theenumi}{\alph{enumi})}
\item
\label{case:non-stacca}
for all $k$ such that $\beta_k>0$, the variety
\[
  V^{d,\delta}(\alpha+e_k,\beta-e_k)(\Omega\cup \{p_{k,\alpha_k+1}\})
\]
with $p_{k,\alpha_k+1}=p$;
\item
\label{case:stacca}
for all $\alpha'\leq\alpha$, $\beta'\geq\beta$, and $\delta'\leq
\delta$ such that
\begin{inparaenum}[(i)]
\item $I\alpha' +I\beta'=d-1$, and
\item $\delta-\delta'+|\beta'-\beta|=d-1$,   
\end{inparaenum}
the variety 
\[
  V^{d-1,\delta'}(\alpha',\beta')(\Omega'),
\]
where $\Omega'$ is an arbitrary cardinality $\alpha'$
subset of $\Omega$.
% \ie $\Omega'=\{p_{i,j}'\}_{1\leq j\leq \alpha'_i}$
% and for all $i$, $\{p'_{i,1},\dots,p'_{i,\alpha'_i}\} \subset
% \{p_{i,1},\dots,p_{i,\alpha_i}\}$.
\end{compactenum}
\end{theorem}



\begin{remark}
The condition $\delta-\delta'+|\beta'-\beta|=d-1$ in 
case \ref{case:stacca}, is
equivalent to the condition
$\dim(V^{d-1,\delta'}(\alpha',\beta')(\Omega'))
=\dim({V}^{d,\delta}(\alpha,\beta)(\Omega))-1.$
Indeed,
\begin{align*}
  \dim({V}^{d,\delta}(\alpha,\beta))
  -\dim(V^{d-1,\delta'}(\alpha',\beta'))
  &= (2d+g-1+|\beta|)
    -(2(d-1)+g'-1+|\beta'|)
  \\
  &= g-g'+|\beta-\beta'|-2,
\end{align*}
where we let $g$ and $g'$ be the genera of the members of
${V}^{d,\delta}(\alpha,\beta)$
and $V^{d-1,\delta'}(\alpha',\beta')$
respectively,
and thus
\[
  g-g' =
  \binom {d-1}2 - \delta
  -\binom {d-2}2 + \delta'
  = d-2-\delta+\delta'
\]
by the Pascal Formula.

Later on we will be able to explain geometrically where the
$\delta-\delta'$ nodes degenerate, see Subsection~\ref{s:localgeom}.
\end{remark}

\begin{remark}
Note moreover that, still in case \ref{case:stacca},
the conditions
$\alpha'\leq\alpha$, $\beta'\geq\beta$, and
$I\alpha' +I\beta'=d-1$
altogether imply that $\alpha' < \alpha$,
\ie
there exists an $i_0$ such that
$\alpha'_{i_0} < \alpha_{i_0}$.

It is however possible that $\beta'=\beta$, but in that case
all the irreducible components of
$V^{d,\delta}(\alpha,\beta)$ having
$V$ in their intersection with $\orth p$
parametrize reducible curves, see Remark~\ref{rk:allred}.
\end{remark}



\begin{proof}[Proof of Theorem~\ref{t:CH1.2}]
%\label{p:strategy}
Let $[X_0]$ be a general point of $V$. There are two cases to be
considered. 
The first case is when the curve $X_0$ does not contain $L$.
Then, in order for $[X_0]$ to sit in 
$\orth p$, we must have one of the mobile contact points (which we may
loosely refer to as points of type $\beta$) be at the prescribed point
$p$ (note that by generality, $p$ is off $\Omega$).
Thus one mobile contact point must be turned into an assigned contact
point (\ie a point of type $\beta$ is turned into one of type $\alpha$),
hence $V$ must be contained in a variety
\[
V^{d,\delta}(\alpha+e_k,\beta-e_k)(\Omega\cup \{p_{k,\alpha_k+1}=p\}).
\] 
Since the latter varieties all have pure dimension
$\dim({V}^{d,\delta }(\alpha,\beta)(\Omega))-1=\dim(V)$, this implies
that $V$ is an irreducible component of a generalized Severi variety
as in case \ref{case:non-stacca} of the theorem.

The remaining case is when $X_0$ has $L$ as an irreducible component;
then we shall loosely say that $X_0=L\cup C$.
In this case the content of Theorem~\ref{t:CH1.2} is
Proposition~\ref{pr:degenSeveri} below.
\end{proof}


The proof of Proposition~\ref{pr:degenSeveri} occupies most of this
section. 
The general idea is to apply (a suitable version of) semistable
reduction to a family of general members of
${V}^{d,\delta }(\alpha,\beta)(\Omega)$
degenerating to $X_0$, in order to derive some necessary conditions on
$X_0$ which will limit the number of dimensions in which it can
move. Comparing this with the fact that $X_0$ has to move in dimension 
$\dim({V}^{d,\delta }(\alpha,\beta)(\Omega))-1$, and taking advantage
of the dimensional characterization of generalized Severi varieties
(Corollary~\ref{c:zariski-forte}),
we will then be able to conclude.



\paragraph{Setup}
\label{p:setup}
Let $V$ be an irreducible component of
${V}^{d,\delta}(\alpha,\beta) \cap  \orth p$, the general member of which
has $L$ as an irreducible component.
Let $X_0$ be a general member of $V$, and let $C$ be the sum of the
components of $X_0$ supported on curves different from $L$; we shall
loosely write $X_0 = L\cup C$.



\paragraph{Semistable reduction}
\label{p:semistable}
Let $\Gamma$
%=\{[X_\gamma]\}\subset {V}^{d,\delta}(\alpha,\beta)
be a general analytic curve in
${V}^{d,\delta}(\alpha,\beta)$
passing through the point $[X_0]$,
and let $\cX\to\Gamma$ be the corresponding family of
curves. By the generality of $\Gamma$, its general member $[X_\gamma]$
is general in an irreducible component of ${V}^{d,\delta
}(\alpha,\beta)$, hence it corresponds to a reduced curve $X_\gamma$
with $\delta$ nodes as its only singularities.
% One wants to describe the
% singularities of $X$ and its feature at the intersection points $X\cap
% L$, proving that $[X_0]$ is general in an irreducible component of the
% generalized Severi varieties in $b)$. 

% {\bf Step 1}: {\it Nodal reduction of the family $\mathcal
%   X\to\Gamma$}.
Let $\nu:\Gamma^\nu\to\Gamma$ be the normalization of
$\Gamma$, and let $b_0\in \Gamma^\nu$ be a point with
$\nu(b_0)=[X_0]$.
We let $\cX^\nu$ be the normalization of the total space $\mathcal
X\times_\Gamma \Gamma^\nu$, obtained from $\mathcal{X}$ by the base
change $\Gamma^\nu \to\Gamma$.
The general fibre of
$\mathcal X^\nu\to\Gamma^\nu$ is smooth of genus $g=p_a(d)-\delta$,
by the Teissier Simultaneous Resolution Theorem, see \cite{03.th-acz}.

Applying a suitable version of stable reduction to the family
$\mathcal X^\nu\to\Gamma^\nu$,
we arrive at a family of curves $f:\mathcal Y\to B$, with special fibre
$Y_0=f^{-1}(b_0)$, satisfying the following conditions: 
\begin{compactitem}
 \item $\mathcal Y\to B$ is a nodal reduction of $\mathcal
   X^\nu\to\Gamma^\nu$,
   \ie all fibres of $f$ are reduced, nodal curves,
   and $B$ is a branched cover of $\Gamma ^\nu$;
 \item the total space $\cY$ is smooth;
\item
there are
$|\alpha|$ sections $Q_{i,j}$ ($1\leq j \leq \alpha_i$)
and $|\beta|$ sections $R_{i,j}$ ($1\leq j \leq \beta_i$) of
$\mathcal Y\to B$, altogether pairwise disjoint, such that
$\pi(Q_{i,j})=p_{i,j}$ (the points of $\Omega$), and
for all $b\neq b_0$ one has
\[
  (\restr \pi {Y_b})^*L
  =
  \sum i \restr {Q_{i,j}} {Y_b} +
  \sum i \restr {R_{i,j}} {Y_b};
\]
% if
% $
% \mathcal Y^*=\mathcal Y\setminus f^{-1}(b_0)
% $
% then
% \[
% \pi^{-1}(L)\cap \mathcal Y^*=\sum iQ_{i,j}^* + \sum iR_{i,j}^*,
% \]
% where the determined by the property
% \begin{eqnarray*}
% \pi(Q_{i,j}^*)=p_{i,j} & \mbox{and}\,\,\, R_{i,j}^*\,\,\, \mbox{intersecting the general fibre in a point}\,\, r_{i,j} \\ & \mbox{of multiplicity} \,\, i\,\,  \mbox{in the divisor} 
% \,\,(\pi|_{Y_b})^*L;
% \end{eqnarray*}
% \item the closure $Q_{i,j}$ and $R_{i,j}$ in $\mathcal Y$ of $Q_{i,j}^*$ and $R_{i,j}^*$ are still disjoint and do not pass through any singular point of $Y_0$;
\item the map sending the general fibre $Y_b$ of $\mathcal Y$ to the
  corresponding plane curve $X_{\gamma}$
  extends to a regular map
  $\pi:\mathcal Y\to \mathbb P^2$
    (here $\gamma = \nu(\eta(b))$, see
  diagram \eqref{nodal-reduction} below);
\item the family $\mathcal Y\to B$ is minimal with respect to the
  above properties.
\end{compactitem}
Note that, since $\cY$ is smooth and the $Q_{i,j}$'s and $R_{i,j}$'s
are sections, they do not pass through any singular point of the
central fibre $Y_0$.

The family $\cY \to B$ is obtained from $\cX^\nu \to \Gamma^\nu$ by
applying 
a finite number of base changes and blow-ups. A number of additional
such operations may be required with respect to the usual nodal
reduction in order to first organize the points $q_{i,j}$ and
$p_{i,j}$ on the fibres into sections (a priori they may be permuted
by the monodromy), and then separate these sections.
The situation is summarized in the diagram below.

\begin{equation}\label{nodal-reduction}
\xymatrix{
Q_{i.j},R_{i,j}\ar@{^{(}->}[r]&\mathcal Y\ar@/^/[drrrr]^\pi\ar[rd]\ar[d]^f \\
& B\ar[rd]^\eta \ar@/^/[ul]
& \mathcal X^\nu  \ar[d]\ar[r] & \mathcal X \ar[d]  \ar@{^{(}->}[r]& 
\Gamma\times \mathbb P^2  \ar[r] & \mathbb P^2\\
& &\Gamma^\nu\ar[r] & \Gamma & &
&}
\end{equation}


\subsection{General picture of the degeneration}
\label{s:gnlpict}

\paragraph{Components of the central fibre of $\cY$}
The irreducible components of the central fibre $Y_0$ of $\cY$ come in
three types. Namely, we let:
\begin{compactitem}
\item $\tilde L$ be the union of the components of $Y_0$ on which
  $\pi$ is nonconstant and maps to $L$;
\item $\tilde C$ be the union of the components of $Y_0$
  on which $\pi$ is nonconstant and maps to $C$;
\item $Z$ be the union of the components of $Y_0$ on which $\pi$ is
  constant. 
\end{compactitem}

\paragraph{Degenerations of assigned and mobile contact points}
We shall now relabel the sections $(Q_{i,j})_{1\leq j \leq \alpha_i}$
and $(R_{i,j})_{1\leq j \leq \beta_i}$ according to the type of the
irreducible component of the central fibre they pass through.
We advise the reader to read this paragraph with
Figure~\ref{fig:gnlpict} at hand.

For all $i$, we let $\alpha_i^{ C}$ and
$\alpha_i^{ L}$ be the number of the sections $Q_{i,j}$, $1\leq
j \leq \alpha_i$, passing through $\tilde C$ and $\tilde L$,
respectively. We package all these numbers as sequences
$\alpha^{ C} = (\alpha_i^{ C})_{i\geq 1} \in \Nseq$ and
$\alpha^{ L} = (\alpha_i^{ L})_{i\geq 1} \in \Nseq$,
and label the corresponding sections as
$(Q_{i,j}^{ C})_{1\leq j \leq \alpha_i^{ C}}$
and $(Q_{i,j}^{ L})_{1\leq j \leq \alpha_i^{ L}}$,
their respective intersection points with the central fibre as
$(q_{i,j}^{ C})_{1\leq j \leq \alpha_i^{ C}}$
and $(q_{i,j}^{ L})_{1\leq j \leq \alpha_i^{ L}}$,
and the images by $\pi$ in $L$ of the latter as
$(p_{i,j}^{ C})_{1\leq j \leq \alpha_i^{ C}}$
and $(p_{i,j}^{ L})_{1\leq j \leq \alpha_i^{ L}}$.
(Note that, by definition, also the
$q_{i,j}^{ C} \in \tilde C$ are mapped to $L$ by $\pi$).

% \begin{perso}
% Rigorously, one would prefer notation as \smash{$\alpha^{\tilde C}$} and
% \smash{$\alpha^{\tilde L}$}, but this turns out to be so heavy as to
% have a negative influence on the understandability of the text.
% \end{perso}

Similarly, for all $i$ we let $\beta_i^{ C}$ 
be the number of the sections $R_{i,j}$, $1\leq
j \leq \beta_i$, passing through $\tilde C$.
We also let $\beta^{ C} = (\beta_i^{ C})_{i\geq 1} \in \Nseq$, label the
corresponding sections 
$(R_{i,j}^{ C})_{1\leq j \leq \beta_i^{ C}}$,
and name $(r_{i,j}^{ C})_{1\leq j \leq \beta_i^{ C}}$ their
respective points on the central fibre $Y_0$, and
$(s_{i,j}^{ C})_{1\leq j \leq \beta_i^{ C}}$
their images on $L$ by $\pi$.

The aware reader will have noticed that we have not considered all
possibilities, as there are neither $\alpha^Z$, nor $\beta^Z$ or
$\beta^L$. The reason for this is that these turn out not to exist,
as we will see in
Claims \ref{ass-c} and \ref{csq-1}
below.


\paragraph{New mobile contact points}
\label{p:new-mobile}
We now identify some new points on $\tilde C$ which,
as we shall
see, induce new mobile contact points with $L$ as $C$ moves in
the family $V$.
These are the intersection points of $\tilde C$ with the
vertical part of $\pi^* L$, \ie the part of the divisor
$\pi^*L \subset \mathcal{Y}$ with support 
contained in the central fibre $Y_0$, which is
\[
  (\pi^*L)^{\mathrm{vert}} =
  \pi^*L
  -   \sum i {Q_{i,j}}
  - \sum i {R_{i,j}}.
\]
Thus, for all $i$, we let
$\beta_i^{C\cap L}$ be the number of points in
$\tilde C \cap (\pi^*L)^{\mathrm{vert}}$ appearing with multiplicity
$i$ in the divisor $(\pi^*L)^{\mathrm{vert}}$, and label these points
as $(r_{i,j}^{C \cap L})_{1\leq j \leq \beta_i^{C \cap L}}$. We also
let $(s_{i,j}^{C \cap L})_{1\leq j \leq \beta_i^{C \cap L}}$ be the
images of these points by $\pi$, and
$\beta^{C\cap L} = (\beta_i^{C\cap L})_{i\geq 1} \in \Nseq$.

The reason for the notation is that
it will turn out that the support of
$(\pi^*L)^{\mathrm{vert}}$ is the union of $\tilde L$ and those
connected components of $Z$ which intersect $\tilde L$
(this follows from Claim~\ref{ass-c} below and the argument given in
\ref{p:bound-mob}).
Therefore, on the surface $\cY^\flat$ obtained
from $\cY$ by contracting $Z$, we can see the points
$r_{i,j}^{C\cap L}$ as the intersection points of
(the images in $\cY^\flat$ of) $\tilde C$ and $\tilde L$.


\bigskip
The situation is summarized in Figure~\ref{fig:gnlpict} below.
In fact, we want this figure to picture the situation as it occurs in
reality, 
and therefore we shall make a number of claims
before we draw the picture. The proof of these claims occupies a
substantial part of the remainder of this section.

The final interpretation  in terms of degenerations
of Severi varieties
of the data introduced above
is given in Proposition~\ref{pr:degenSeveri} below.

\begin{claim}
\label{ass-c}
The sections $(Q_{i,j})_{1\leq j \leq \alpha_i}$ and
$(R_{i,j})_{1\leq j \leq \beta_i}$ are disjoint from $Z$.
\end{claim}

\begin{claim}
\label{csq-1}
All sections
$(R_{i,j})_{1\leq j \leq \beta_i}$ pass through $\tilde C$.
\end{claim}

Note that Claims \ref{ass-c} and \ref{csq-1} imply that
\[
  \{Q_{i,j}\}_{1\leq i\leq \alpha_i}=
  \{Q_{i,j}^C\}_{1\leq i\leq\alpha_i'} \cup
  \{Q_{i,j}^L\}_{1\leq i\leq \alpha_i''}
  \quad\text{and}
  \quad
  \{R_{i,j}\}_{1\leq i\leq \alpha_i}=
  \{R_{i,j}^C\}_{1\leq i\leq\alpha_i'}.
\]

\begin{claim}
\label{ass-a}
The curve $\tilde L$ consists of a unique irreducible component, on
which $\pi$ is an isomorphism.
\end{claim}

This claim implies that the line $L$ appears with multiplicity $1$ in
$X_0$, so $X_0 = C \cup L$ with $C$ a degree $d-1$ curve.

\begin{claim}
\label{ass-b}
The curve $Z$ consists of a disjoint union of chains of rational
curves joining $\tilde L$ to $\tilde C$.
\end{claim}

This Claim implies that the surface $\cY^\flat$ obtained from the
smooth surface $\cY$ by contracting $Z$ has only rational double
points as singularities.

\begin{claim}
\label{csq-2}
The map $\pi$ is a birational isomorphism on each irreducible
component of $\tilde C$.
\end{claim}

This Claim implies that the curve $C$ is reduced.

\begin{claim}
\label{csq-3}
The curve $\tilde C$ is smooth (though not connected, in general).
\end{claim}


We may now draw a picture of the situation.
\begin{center}
\includegraphics[]{calY.eps}
\captionof{figure}{General picture of the degeneration}
\label{fig:gnlpict}
\end{center}


We shall prove the following result, which encapsulates
Theorem~\ref{t:CH1.2} in the case of an irreducible component having
general member of the form
$X_0 = C\cup L$.

\begin{proposition}
\label{pr:degenSeveri}
In the situation of \ref{p:setup},
the curve $C$ is a general member of the generalized Severi variety
$V^{d-1,\delta'}(\alpha',\beta')(\Omega')$, where:
\begin{mycpctitem}
\item $\alpha' = \alpha^C$, and
  $\Omega' = (p_{i,j}^C)_{1\leq j \leq \alpha_i^C}$;
\item $\beta' = \beta^C + \beta^{C\cap L}$;
\item $\delta' = \delta - d +1+ |\beta'-\beta|$.
\end{mycpctitem}
\end{proposition}

In other words, we will prove that the assigned contact points for
the curves $X_\gamma$ (recall the notation from \ref{p:semistable})
that
end up on $\tilde C$ transfer to assigned contact points for $C$,
whereas those that end up on $\tilde L$ vanish, being accounted for by
the component $L$ of $X_0=C\cup L$;
moreover, all mobile contact points of $X_\gamma$ end up on $\tilde C$
and thus transfer to mobile contact points on $C$;
the curve $C$ has additional mobile contact points with $L$, which come
out of the intersection points of $\tilde C$ and $\tilde L$ in
$\cY^\flat$.

We will provide an explicit geometric description of the degeneration
of the curves $X_\gamma$ in a neigbourhood of all these points in
Subsection~\ref{s:localgeom} below.
Then, we will be able to track the limits of the
$\delta$ nodes of the curves $X_\gamma$, and thus provide a geometric
explanation for the formula relating $\delta'$ and $\delta$.


\subsection{Simplified proof of Proposition~\ref{pr:degenSeveri}}
\label{s:simplified}

We follow the presentation of \cite{caporaso-harris}, and first give a
proof of Proposition~\ref{pr:degenSeveri}
% (hence also of Theorem~\ref{t:CH1.2})
under some simplifying assumptions, in order to
describe as clearly as possible what is actually going on
in reality.
We shall prove later on that these simplifying assumptions do indeed
hold, in Subsection~\ref{s:complete}.

We have made six claims in Subsection~\ref{s:gnlpict} above, with
numbers \ref{ass-c}--\ref{csq-3}.
Our simplifying assumptions consist in taking the three Claims
\ref{ass-c},
\ref{ass-a}, and
\ref{ass-b} for granted, for the moment.


\paragraph{Proof of Proposition~\ref{pr:degenSeveri}
assuming Claims
\ref{ass-c},
\ref{ass-a}, and
\ref{ass-b}}
\label{p:simplified}
Claim~\ref{ass-b} ensures that the surface $\cY^\flat$ obtained from
$\cY$ by contracting $Z$ has at worst rational double points as
singularities, and is still a nodal reduction of the family
$\cX \to \Gamma$. From now on we work on this new family, and denote any
curve in $\cY^\flat$ image of a curve in $\cY$ by the same symbol
(with the exception of the central fibre of $\cY^\flat$, which we will
denote by $Y_0^\flat$).

Since $Y_0$ and $Y_0^\flat$ are semistable limits of the curves
$X_\gamma$, which are smooth of genus $g$, it holds that
\[
  p_a(Y_0)=p_a(Y_0^\flat) = g.
\]
Claim~\ref{ass-a} ensures that $\tilde L\simeq L$ is rational.
On the other hand,
$Y_0^\flat =\tilde L\cup \tilde C$ is nodal,
and the total number of points in $\tilde C \cap \tilde L$ is
$|\beta^{C\cap L}|$. Thus 
one finds
\begin{equation}
\label{eq:genus-1}
g=p_a(Y_0^\flat)=p_a(\tilde L\cup \tilde C)=p_a(\tilde C)
+|\beta^{C\cap L}|-1.
\end{equation}
% by the formula recalled in \eqref{eq:arith-genus-nodal-curve}.


We shall now apply Corollary~\ref{c:zariski-forte}, which gives a
dimension bound on families of genus $g$ curves
and a dimensional characterization of generalized Severi varieties.
Let $V$ be the irreducible component of
$V^{d,\delta}(\alpha,\beta) \cap \orth p$ of which $X_0=C\cup L$ is a
general member.   
The dimension bound
%Corollary~\ref{c:zariski-forte}
tells us that
\begin{equation}
\label{bnd-dimV}
\dim(V) \leq 2(d-1)+g(\tilde C)-1+|\beta^C+\beta^{C\cap L}|,
\end{equation}
since the number of unassigned contact points of $C$ with $L$ is at
most $|\beta^C+\beta^{C\cap L}|$,
and $C$ has degree at most $d-1$
(indeed, the unassigned contact points of $C$ with $L$
are the points in the support of
$\pi_* \tilde C \cdot L$ off $\Omega$,
one has $\pi_* \tilde C \cdot L = \pi_*(C\cdot \pi^* L)$ by the
projection formula, and the intersection points of $\tilde C$ with the
sections $Q_{ij}$ are mapped to $\Omega$;
besides, Claim~\ref{ass-c} ensures that the number
$|\beta^C+\beta^{C\cap L}|$ does not count
any point in $\tilde C\cap \tilde L \subset Y_0^\flat$ several times).

But
$\orth p$ is a hyperplane which does not contain any irreducible
component of $V^{d,\delta}(\alpha,\beta)(\Omega)$,
by Proposition~\ref{p:zariski}, and since $p \not\in \Omega$.
Hence
\begin{equation}
\label{dimV}
  \dim(V) =
  \dim \bigl( V^{d,\delta}(\alpha,\beta) \bigr) -1
  = 2d+g-2+|\beta|.
\end{equation}
In the upshot, we have the following sequence of equalities and
inequalities: 
\begin{equation}
\label{eq-series}
\begin{aligned}
2d+g+|\beta|-2
&\leq  2(d-1)+g(\tilde C)-1+|\beta^C+\beta^{C\cap L}|
& \hspace{5mm}
& \text{by \eqref{bnd-dimV} and \eqref{dimV}} \\
& \leq  2(d-1)+p_a(\tilde C)-1+|\beta^C+\beta^{C\cap L}|
&& \text{since $g(\tilde C) \leq p_a(\tilde C)$}\\
& =   2(d-1)+g-|\beta^{C\cap L}| +|\beta^C+\beta^{C\cap L}|
&& \text{by \eqref{eq:genus-1}} \\
& =   2(d-1)+g+|\beta^C| \\
& \leq   2(d-1)+g+|\beta|.
\end{aligned}
\end{equation}
We conclude that equality holds throughout. In particular,
\eqref{bnd-dimV} is an equality and therefore, by
Corollary~\ref{c:zariski-forte},
$V$ is an irreducible component of the Severi variety
$V^{d-1,\delta'}(\alpha',\beta')(\Omega')$ where
$\alpha'$, $\Omega'$, and $\beta'$ are as stated in
Proposition~\ref{pr:degenSeveri}, and
$\delta'$ is determined by the geometric genus of $C$
(note in particular that the orders of contacts of $C$ with $L$ are
given by the multiplicities in $\pi^*L \cdot \tilde C$, and therefore
they are indeed $\alpha'$ and $\beta'$).
Yet a couple of words are in order as to why the condition
$\Card(C\cap L)=\Card (\pi^{-1}(C\cap L))$
of Corollary~\ref{c:zariski-forte}
is indeed verified:
on the one hand, it follows from Claim~\ref{ass-c}
that the sections $Q_{i,j}$ are still mutually disjoint in
$\cY^\flat$, so that there is a unique point in $\tilde C$ over each
point of $\Omega'$;
on the other hand, the equality in \eqref{bnd-dimV} implies
(by Corollary~\ref{c:zariski-forte} again) that
$C$ indeed intersects $L$ at $|\beta^C+\beta^{C\cap L}|$ pairwise
distinct points, so that eventually all points in $\pi^{-1}(C\cap L)$
have distinct images in $L$, as required.

To finish, let us explicitly derive the formula for $\delta'$:
it follows from the series of equalities in
\eqref{eq-series} 
that the geometric genus of $C$ is
\[
  g(C) = g(\tilde C) = p_a(\tilde C)
  = g - |\beta^{C\cap L}|+1,
\]
so that
\begin{align*}
  \delta' = \binom {d-2} 2 - g(C)
  &= \binom {d-2} 2 - g + |\beta^{C\cap L}| - 1
  \\
  &= \binom {d-2} 2 - \binom {d-1} 2 + \delta + |\beta^{C\cap L}| - 1
  = \delta -(d-1)+|\beta^{C\cap L}|,
\end{align*}
which is the value asserted in Proposition~\ref{pr:degenSeveri}, as
$\beta^{C\cap L}=\beta'-\beta$,
since $\beta^C = \beta$ by the series of equalities in
\eqref{eq-series}.
\qed


\paragraph{Proof of Claims
  \ref{csq-1},
  \ref{csq-2}, and
  \ref{csq-3}
assuming Claims
\ref{ass-c},
\ref{ass-a}, and
\ref{ass-b}}
As we have already observed, it follows from the series of equalities
in \eqref{eq-series} that $\beta = \beta^C$, which proves
Claim~\ref{csq-1}.

On the other hand, the fact that equality holds in \eqref{bnd-dimV}
implies by Corollary~\ref{c:zariski-forte} that $C$ is reduced. Thus,
Claim~\ref{csq-2} holds.
Eventually, we have already observed that the series of equalities
in \eqref{eq-series} implies the equality
$g(\tilde C) = p_a(\tilde C)$, which proves that $\tilde C$ is smooth,
\ie Claim~\ref{csq-3} holds.
\qed


\subsection{Complete proof of Proposition~\ref{pr:degenSeveri}}
\label{s:complete}


\paragraph{Labelling of the remaining sections}
\label{p:relabel}
In order to prove Claims \ref{ass-c},
\ref{ass-a}, and
\ref{ass-b}, we need to consider the situation
as complicated as it could a priori be,
and therefore to introduce some more notation with respect to that
already given in Subsection~\ref{s:gnlpict}.

Thus, for all $i$ we define (in the surface $\cY$)
% \begin{compactitem}
% \item
  $\beta_i^{C,Z}$ as the number of the sections
  $(R_{i,j})_{1 \leq j \leq \beta_i}$ passing through a connected
  component of $Z$ that intersects $\tilde C$,
and package these numbers in the sequence
$\beta^{C,Z} = (\beta_i^{C,Z})$.

On the other hand we redefine $|\beta^{C\cap L}|$ as
the sum of the number of points of $\tilde C$ meeting $\tilde L$
plus the number of connected components of $Z$ meeting both $\tilde C$
and $\tilde L$. Thus it is the number of intersection points between
$\tilde C$ and $\tilde L$ after we contract $Z$. Note that
$|\beta^{C\cap L}|$ no longer corresponds to an actual sequence
$\beta^{C\cap L} = (\beta^{C\cap L}_i)$; the point is, without
Claim~\ref{ass-b}, there could be a connected component of $Z$ meeting
$\tilde C$ at several distinct points with different multiplicities in
$(\pi^*L)^{\mathrm {vert}}$.

% \item $\beta_i^{Z,L}$ the number of the sections
%   $(R_{i,j})_{1 \leq j \leq \beta_i}$ passing through a connected
%   component of $Z$ that intersects both $\tilde L$ and $\tilde C$.
% \end{compactitem}
% As usual, we package these numbers in the two sequences
% $\beta^{Z,C} = (\beta_i^{Z,C})$ and
% $\beta^{Z,L} = (\beta_i^{Z,L})$.

\paragraph{Bounding the number of mobile contact points of $C$ and
  $L$}
\label{p:bound-mob}
To this end, we note that every connected component of $Z$ mapping to
a point of $L$ by $\pi$ necessarily intersects
either $\tilde L$,
or a section among $Q_{i,j}$ and $R_{i,j}$.
Indeed,
otherwise there would exist a connected component of $\pi^{-1}(L)$
entirely contained in $Z$,
% in particular not containing any
% irreducible component of $\tilde L$.
and thus after contracting $Z$ we would obtain
a surface with an isolated point in the preimage of $L$, which is
impossible.

Therefore the number of mobile contact points of $C$ and $L$
(in $\P^2$) is
bounded from above as follows:
\begin{equation}
\label{bnd-mobile}
  \Card \bigl(C \cap (L - \Omega) \bigr) \leq |\beta^C+\beta^{C,Z}|
  + |\beta^{C\cap L}|.
\end{equation}


\paragraph{Bounding the genus of $C$}
\label{p:gen-bnd2}
As in \ref{p:simplified}, $Y_0$ is a semistable limit of the curves
$X_\gamma$, and therefore $p_a(Y_0)=g$.
Since the number of intersection points between
$\tilde C$ and $\tilde L$ after we contract $Z$ is
$|\beta^{C\cap L}|$, we find that
\begin{equation}
\label{eq:genus-2}
g = p_a(Y_0)
\geq p_a(\tilde L) + p_a(\tilde C) + |\beta^{C\cap L}|-1.
\end{equation}
Note that this inequality is strict if some connected component of $Z$
has positive arithmetic genus, or intersects $\tilde C$ or $\tilde L$
at more than one point.

% Moreover, denoting by $Z_1,...,Z_\gamma$ the connected components of $Z$, again by \eqref{eq:arith-genus-nodal-curve}, one has that
% \begin{eqnarray}
% g=p_a(Y_0) & = & p_a(\tilde L)+p_a(Y)-1+p_a(Z)-1+ \sharp(\tilde L\cap Y)+\sharp((\tilde L\cup Y)\cap Z)\nonumber\\
% & = & p_a(\tilde L)+p_a(Y)-1+\sum_{i=1}^\gamma p_a(Z_i)-\gamma +\sharp(\tilde L\cap Y)+\sharp((\tilde L\cup Y)\cap Z)\label{eq:contradiction-a0}\\
% &\geq &  p_a(\tilde L)+p_a(Y)-1 +\sum_{i=1}^\gamma p_a(Z_i)+ |\beta''|\label{eq:contradiction-a}\\
% &\geq &  p_a(\tilde L)+p_a(Y)-1 + |\beta''|,\label{eq:contradiction-a1}
% \end{eqnarray}
% where we used that the arithmetic genus of a connected nodal curve is non-negative.

\paragraph{Proof of Claim~\ref{ass-a}}
Let $e$ be the multiplicity of $L$ in $X_0=C\cup L$. Then $C$ has
degree $d-e$.
On the other hand, $\tilde L$ is mapped $e:1$ to $L$ by $\pi$, so
by Riemann--Hurwitz we have the inequality
\(
  p_a(\tilde L) \geq -e+1.
\)
Together with \eqref{eq:genus-2}, this gives the
bound:
\begin{equation}
\label{bnd-genus-2}
p_a(\tilde C) \leq g-|\beta^{C\cap L}|+e.
\end{equation}
Now, we argue exactly as in \ref{p:simplified}: by
Corollary~\ref{c:zariski-forte}, we find that the irreducible 
component $V$ of $V^{d,\delta}(\alpha,\beta)\cap \orth p$
that $C$ moves in has dimension at most
\begin{equation}
\label{eq:series2}
\begin{aligned}
2(d-e)+p_a(\tilde C)-1
+|\beta^C+\beta^{C,Z}| + |\beta^{C\cap L}|
& \leq 2(d-e)+g
+ |\beta^C+\beta^{C,Z}| + e-1\\
& =  2d+g
+ |\beta^C+\beta^{C,Z}| -e-1.
\end{aligned}
\end{equation}
But since
\[
  \dim(V) = 
  \dim \bigl(V^{d,\delta}(\alpha,\beta)\bigr)-1
  = 2d+g+|\beta|-2,
\]
and $|\beta| \leq |\beta^C+\beta^{C,Z}|$,
one necessarily has $e=1$.
\qed

\paragraph{Proof of Claim~\ref{ass-b}}
\label{pf:ass-b}
By the fact that \eqref{eq:series2} is in fact an equality, we see
that also \eqref{eq:genus-1} must be an equality.
Thus, as already observed in \ref{p:gen-bnd2}, every connected
component of $Z$ has arithmetic genus $0$,
\ie it is a tree of rational curves, and intersects each of $\tilde L$
and $\tilde C$ at most once.

In order to prove that such a connected component is a chain of
rational curves connecting $\tilde L$ and $\tilde C$,
it is therefore sufficient to prove that any ``end component'' of a
connected component of $Z$ meets either $\tilde C$ or $\tilde L$.
By an end component, we mean an irreducible component $Z_1$ that meets
at most one other irreducible component of $Z$
(one if the corresponding connected component of $Z$ has several
irreducible components, zero if $Z_1$ is itself a connected component
of $Z$).

The key argument is that if an end component $Z_1$
of $Z$ intersects neither
$\tilde C$ nor $\tilde L$, then by the minimality of $\cY$ there must
be at least two of the sections $(Q_{i,j})_{1\leq j \leq \alpha_i}$
and $(R_{i,j})_{1\leq j \leq \beta_i}$ meeting $Z_1$, for otherwise we
could blow down $Z_1$ in $\cY$ and still satisfy all the conditions
imposed on $\cY$. (Note that $Z_1$, being a rational curve
intersecting $Y_0-Z_1$ in exactly one point since $Y_0$ is connected,
is a $(-1)$-curve).

These two sections cannot be both of type $\alpha$,
for otherwise they would be contracted by $\pi$ to the same point of
$L$, which is excluded by the definition of generalized Severi
varieties.
To rule out the other possibilities, we use the fact that since
\eqref{eq:series2} is an equality, 
then also \eqref{bnd-mobile} must be an equality.
But if two sections either both of type $\beta$, or of types $\alpha$
and $\beta$ respectively, meet the same connected component of $Z$,
then the two corresponding points of $C$ in $\P^2$ are the same, hence
\eqref{bnd-mobile} is a strict inequality.
This ends the proof of Claim~\ref{ass-b}.
\qed

% say $Q_{i,j}$ and $Q_{i',j'}$ then one obtains that
% \[\pi(q_{i,j})=p_{i,j}=p_{\alpha,\beta}= \pi(q_{\alpha,\beta}).\]
% But this is a contradiction because, by construction $p_{i,j}\neq p_{\alpha,\beta}$. Assume now that the sections intersecting $W$ are $Q_{i,j}$ and $R_{\alpha,\beta}$.
% Thus $\pi(s_{\alpha,\beta})=r_{\alpha,\beta}=p_{i,j}\in \Omega$ and the inequality in \eqref{eq:bound-punti-liberi} is strict. By Corollary \ref{c:zariski-forte}, one finds that 
% $X$ is general in a family of dimension strictly less that $ 2(d-1)+g(Y)+|\beta'|-1$. On the other hand, again by \eqref{eq:contradiction-a1}, one has that $2(d-1)+g(Y)+|\beta'|-1\leq 2d+g+|\beta|-2$, getting the contradiction. The argument is the same is the two sections are of type $R_{i,j}$ and $R_{\alpha,\beta}$. 


\paragraph{Proof of Claim~\ref{ass-c}}
Now we know that Claim~\ref{ass-b} holds, \ie
the connected components of $Z$ are chains of rational curves
connecting $\tilde C$ and $\tilde L$.
Therefore we can indeed consider the points
$(r_{i,j}^{C \cap L})_{1\leq j \leq \beta_i^{C \cap L}}$
introduced in \ref{p:new-mobile}, and their respective images by $\pi$,
the points $(s_{i,j}^{C \cap L})_{1\leq j \leq \beta_i^{C \cap L}}$
(see also \ref{p:relabel}).

Our main argument here is that \eqref{bnd-mobile} is an equality, 
as we have already observed in \ref{pf:ass-b} above.
If a section of type $\alpha$ intersects a connected component of $Z$,
then the image in $\P^2$ of the point $r_{i,j}^{C\cap L}$
corresponding to this component must lie in $\Omega$, which implies
that \eqref{bnd-mobile} is a strict inequality, a contradiction.

Similarly, if a section of type $\beta$ intersects a connected
component of $Z$,
then the point $r_{i,j}^{C,Z}$ corresponding to this section 
and  the point $r_{i,j}^{C\cap L}$
corresponding to the component of $Z$ have the same image in $\P^2$,
hence \eqref{bnd-mobile} is a strict inequality, a contradiction.
\qed


\bigskip
We have now proved all three Claims \ref{ass-c},
\ref{ass-a}, and
\ref{ass-b}.
In Subsection~\ref{s:simplified}
we had proved Proposition~\ref{pr:degenSeveri} assuming these three
claims.  Thus, we now have a complete proof of
Proposition~\ref{pr:degenSeveri},
and the proof of Theorem~\ref{t:CH1.2} is over.



\subsection{Local picture of the degeneration of curves}
\label{s:localgeom}

We consider the situation set up in \ref{p:setup} and
\ref{p:semistable}, when a general member
$X_\gamma$ of $V^{d,\delta}(\alpha,\beta)$ degenerates
to a curve $X_0 = L \cup C$.
We shall now give a complete description of this degeneration, in its
concrete incarnation as a degeneration of plane curves.
This will be useful in the next section, when we prove the theorem
going the other direction than Theorem~\ref{t:CH1.2} above.

We carry on with the notation introduced above for
Proposition \ref{pr:degenSeveri}.
Something non-trivial happens only at the points where $C$ and $L$
intersect, which come in the following four types:
\ref{p:p_ij''}--\ref{p:s_ij''}.

\paragraph{Vanishing assigned contact points}
\label{p:p_ij''}
These are the points of $\Omega \setminus \Omega'$,
\ie the points $p_{i,j}^L$.
Since $C$ is general in the component $V$ of
$V^{d-1,\delta'}(\alpha',\beta')(\Omega')$,
by Proposition~\ref{p:zariski}
it does not pass through any point $p_{i,j}^L$.
Thus the curve $X_0$ is smooth at those points,
\ie it has only one local branch there, which is an open subset of the
line $L$ itself.

Therefore the degeneration happens like this:
locally at a point $p_{i,j}^L$,
the curves $X_\gamma$, $\gamma \neq 0$,
have one smooth local branch tangent to the order $i$ with $L$, which
degenerates in $X_0$ to an open neighbourhood of $p_{i,j}^L$ in $L$.

\begin{center}
\includegraphics[]{degen-vanish-assign.eps}
\captionof{figure}{Degeneration in a neighbourhood $U$ of a vanishing
  assigned contact point}
\end{center}



\paragraph{Non-vanishing assigned contact points}
\label{p_ij'}
These are the points of $\Omega'$,
\ie the points $p_{i,j}^C$.
Such a point is by definition the image of the point
$q_{i,j}^C \in \tilde C$, and $C$ is smooth at $p_{i,j}^C$ by
Proposition~\ref{p:zariski}. On the other hand
$p_{i,j}^C$ also has a preimage in $\tilde L$, and exactly one as
$\tilde L \to L$ is an isomorphism: let's call it
$(q_{i,j}^C)'$.
It follows that $X_0$ has two smooth local branches at
$p_{i,j}^C$, tangent to $i$-th order, so that $p_{i,j}^C$ is an
$i$-tacnode of $X_0$.

As we have just seen, the map $Y_0 \to X_0$ factors through the
normalization of $p_{i,j}^C$ in $X_0$ (recall that $Y_0$ is the
central fibre of the semistable reduction introduced in
\ref{p:semistable}),
and thus the family $\mathcal{Y}$ is smooth in a neighbourhood of the
two preimages of $p_{i,j}^C$ in $Y_0$.
This implies that the curves $X_\gamma$, as they approach $X_0$,
have two local branches 
analytically locally around $p_{i,j}^C \in \P^2$.

The difference in arithmetic genus between
$Y_b$ and $X_\gamma$ over a neighbourhood of $p_{i,j}^C$ in $\P^2$ is
constant as $b$ moves (with $\gamma = \nu(\eta(b)$, see diagram
\eqref{nodal-reduction}),
because both $\mathcal{Y}$ and $\mathcal{X}$ are flat families.
Moreover, $\mathcal{X}$ is equigeneric over $\Gamma\setminus \{0\}$,
and $\mathcal{Y}$ is a nodal reduction of $\mathcal{X}$, so for $b\neq
0$, the difference in arithmetic genus between
$Y_b$ and $X_\gamma$ is just the sum of the $\delta$-invariants of the
singularities of $X_\gamma$;
since the curves $X_\gamma$ are nodal for $\gamma \neq 0$, this is
therefore the number of nodes of $X_\gamma$ tending to the point
$p_{i,j}^C$ as $\gamma$ tends to $0$.
On the other hand,
over a neighbourhood of $p_{i,j}^C$,
$Y_0 \to X_0$ is the normalization of an $i$-tacnode,
so the difference in arithmetic genus between
$Y_0$ and $X_0$ over a neighbourhood of $p_{i,j}^C$ equals $i$.

The upshot is that locally at $p_{i,j}^C$,
the curves  $X_\gamma$, $\gamma\neq 0$, have two local branches
intersecting transversely in $i$ points tending to the $i$-tacnode of
$X_0$ at  $p_{i,j}^C$;
one of the two branches of $X_\gamma$ is tangent to order $i$ with $L$
at the fixed point $p_{i,j}^C \in \Omega' \subset \Omega$
(this is the branch corresponding to the branch of $Y_b$ intersecting
the section $Q_{i,j}^C$, namely that tending to the branch of $Y_0$
contained in $\tilde C$).


\begin{center}
\includegraphics[]{degen-nonvanish-assign.eps}
\captionof{figure}{Degeneration in a neighbourhood $U$ of a non-vanishing
  assigned contact point}
\end{center}


\paragraph{Limits of unassigned contact points}
\label{s_ij}
These are the points $s_{i,j}^C$.
At those points the situation is almost exactly the same as that at the
points $p_{i,j}^C$ described above, the key point being that the
points $s_{i,j}^C \in L$ have two points in their preimage in $Y_0$,
namely $r_{i,j}^C \in \tilde C$ and an additional point on $\tilde L$,
which we may call $(r_{i,j}^C)'$ so that, as in \ref{p_ij'},
the map $Y_0 \to X_0$ factors through the normalization of the
$i$-tacnode of $X_0$ at $s_{i,j}^C$.
The only difference is that here the branch of $X_\gamma$ which is
tangent to order $i$ with $L$ touches $L$ at a mobile point,
different from $s_{i,j}^C$ by Proposition \ref{p:zariski}
(this is the branch corresponding to the branch of $Y_b$ intersecting
the section $R_{i,j}^C$, which tends to a local branch of
$\tilde C$).


\begin{center}
\includegraphics[]{degen-lim-unassign.eps}
\captionof{figure}{Degeneration in a neighbourhood $U$ of a limit of
  unassigned contact points}
\end{center}


\paragraph{New unassigned contact point}
\label{p:s_ij''}
These are the points $s_{i,j}^{C\cap L}$.
Such a point is the image of a point $r_{i,j}^{C\cap L}$ which,
in the surface $\mathcal Y^\flat$ obtained from $\mathcal Y$ by
contracting $Z$, lies at the intersection of $\tilde C$ and $\tilde
L$; it is thus an ordinary node of the central fibre $Y_0^\flat$
(in fact, seen in $\mathcal Y$ it is a node as well, although
there it may lie on $\tilde C \cap Z$ rather than on
$\tilde C \cap \tilde L$), and the point 
$s_{i,j}^{C\cap L}$ therefore
has only one point in its preimage in $Y_0$.
Since the nearby fibres $Y_b$ are smooth
(because $\mathcal{X}$ is equigeneric over $\Gamma\setminus \{0\}$,
and $\mathcal{Y}$ is a nodal reduction of $\mathcal{X}$), they
have only one branch in an
analytic neighbourhood of the preimage of $s_{i,j}^{C\cap L}$ in
$\mathcal{Y}$, 
and therefore the curves $X_\gamma$, $\gamma \neq 0$, have only one
local branch in a neighbourhood of $s_{i,j}^{C\cap L}$ in $\P^2$.

The points $s_{i,j}^{C\cap L}$ are again $i$-tacnodes of the curve
$X_0$, this time because both $L$ and $C$ are smooth at
$s_{i,j}^{C\cap L}$ by Proposition~\ref{p:zariski}, and intersect
there with multiplicity $i$ because by definition
$s_{i,j}^{C\cap L}$ lies on a component of multiplicity $i$ of
$(\pi^*L)^{\mathrm {vert}}$.
In particular the difference in arithmetic genus between $Y_0$ and
$X_0$ over $s_{i,j}^{C\cap L}$ is $i-1$. Since this difference
for the families $\mathcal Y$ and $\mathcal X$ is
constant over a neighbourhood of $s_{i,j}^{C\cap L}$, and the curves
$X_\gamma$ are nodal for $\gamma \neq 0$, we see that the latter will
have $i-1$ nodes tending to $s_{i,j}^{C\cap L}$.

To sum up, analytically locally around $s_{i,j}^{C\cap L}$,
the curves $X_\gamma$, $\gamma \neq 0$, have one irreducible,
$(i-1)$-nodal local branch, transverse to $L$ and not passing by
$s_{i,j}^{C\cap L}$, degenerating to the $i$-tacnode at
$s_{i,j}^{C\cap L}$ formed by $C$ and $L$.


\begin{center}
\includegraphics[]{degen-new-unassign.eps}
\captionof{figure}{Degeneration in a neighbourhood $U$ of a new
  unassigned contact point}
\end{center}


We emphasize that this phenomenon is arguably the central topic of
this whole volume; its local model has been studied in detail in
the previous chapters \cite{05.margherita}
and \cite{A.swallowtail}.


\bigskip
Whereas the above description of the degeneration will be needed in
the next section, the remainder of this subsection is not necessary
for the proof of the main theorem. I believe it is nevertheless
helpful.

First of all, having the above descriptions at hand, we may now give
the promessed geometric interpretation for the relation between
$\delta$ and $\delta'$ in Theorem~\ref{t:CH1.2} and Proposition
\ref{pr:degenSeveri}.


\paragraph{Book-keeping of the nodes in the degeneration}
As a result of \ref{p:p_ij''}--\ref{p:s_ij''} above, we see that as
$X_\gamma$ degenerates to $X_0=C\cup L$ there are $i$ nodes
of $X_\gamma$ tending to
each point of types $\alpha_i^C$ and $\beta_i^C$
(respectively the preserved tangencies at assigned points, and the
limits of tangencies at unassigned points, which are all preserved),
and $i-1$ nodes of $X_\gamma$ tending to each point of type
$\beta_i^{C\cap L}$ (the new tangency conditions, all at unassigned
points); the degeneration is otherwise equisingular.
Therefore, we have:
\[
  \delta-\delta' = I\alpha^C+I\beta^C
  +\big( I\beta^{C\cap L}-|\beta^{C\cap L}|
  \bigr).
\]
On the other hand we know that,
in the notation of Proposition \ref{pr:degenSeveri},
$\alpha'= \alpha^C$ and $\beta'=\beta^C+\beta^{C\cap L}$, so that
\[
  I\alpha^C+I\beta^C
  +I\beta^{C\cap L} = I\alpha'+I\beta' = C\cdot L = d-1;
\]
since moreover $\beta = \beta^C$, we also have
$|\beta^{C\cap L}|=|\beta'-\beta|$.
Finally, we find 
\[
  \delta-\delta' =
  (d-1)-|\beta'-\beta|
\]
as required.


\bigskip
Lastly, let us analyze the multiplicities of the irreducible
components of $Y_0$ in the divisor $\pi^*L$.
This will be helpful in understanding the multiplicities of the
components of the type $V^{d-1,\delta'}(\alpha',\beta')$
in the intersection of $V^{d,\delta}(\alpha,\beta)$ with the
hyperplane $\orth p$, cf. Theorem \ref{t:CH1.3}.

\paragraph{Multiplicities of the divisor $\pi^*L$ in
  $\mathcal Y$}
Recall that the central fibre $Y_0$ of $\mathcal Y$ is reduced and
consists of
(i) $\tilde L$, an irreducible curve mapped isomorphically
to $L$,
(ii) $\tilde C$, the normalizations of the various irreducible
components of $C$,
and (iii) $Z$, the union of disjoint chains of rational curves joining
$\tilde L$ to $\tilde C$.

Let $m$ be the multiplicity of $\tilde L$ in the divisor $\pi^*L$ on
$\cY$. Let us remind that the integer $m$ records the ramification of
$\pi: \cY \to \P^2$ along $\tilde L$ in the direction normal to
$\tilde L$, hence $m>1$ does not contradict $\restr \pi {\tilde L}$
being an isomorphism onto $L$; instead, if
$\restr \pi {\tilde L}: \tilde L \to L$ had degree $k$, this would
translate into $\pi_* \tilde L = kL$.

The main output of this paragraph will be the divisibility of $m$ by
$\lcm(\beta^{C\cap L}) = \lcm (\beta'-\beta)$.
To see this, consider a point $r_{i,j}^{C\cap L} \in \tilde C$.
By definition, see Paragraph~\ref{p:new-mobile},
$r_{i,j}^{C\cap L}$ sits both on $\tilde C$ and on a multiplicity $i$
component of $(\pi^*L)^{\mathrm{vert}}$,
and we have seen that  $(\pi^*L)^{\mathrm{vert}}$ is supported
on $\tilde L+Z$. Thus, if $i<m$, then $r_{i,j}^{C\cap L}$ sits
on a smooth irreducible rational curve $Z_1 \subset Z$ which has
multiplicity $i$ in $\pi^*L$.
Let $Z_2$ be the next curve in the chain of rational curves joining
$\tilde C$ to $\tilde L$ and containing $Z_1$
(here, 'next' is intended relative to the direction pointing to
$\tilde L$; if $Z_1$ directly joins
$\tilde C$ to $\tilde L$, then we take $Z_2 = \tilde L$), and let
$i_2$ be its multiplicity in $\pi^*L$. Since $\pi$ contracts $Z_1$, we
have $\pi^*L \cdot Z_1 =0$, hence
\[
  (iZ_1+i_2Z_2)\cdot Z_1 = 0.
\]
Since $Z_1$ is a $(-2)$-curve\footnote
{this is well-known and may be seen as follows:
all fibres of $\cY$ are linearly equivalent, and have intersection
number $0$ with $Z_1$; therefore,
$Y_0 \cdot Z_1 = (\tilde C+Z_1+ Z_2)\cdot Z_1=0$,
hence $Z_1^2 = -(\tilde C+\tilde L)\cdot Z_1=-2$.}
and $Z_1\cdot Z_2 = 1$, we find that $i_2=2i$.
We continue by induction to compute the successive multiplicities:
the connected component of $Z$ containing $Z_1$ is a chain of
$(-2)$-curves; let us denote them by $Z_1,\ldots,Z_l$, in
that order, and let $Z_{l+1} = \tilde L$.
Let $i_1,\ldots,i_{l+1}$ be their multiplicities in $\pi^*L$.
Once we know, for some $k\leq l$, that $i_s=si$ for all $s=1,\ldots,k$, we have
\[
  \pi^*L \cdot Z_k =
  (i_{k-1}Z_1+i_kZ_k+i_{k+1}Z_{k+1})\cdot Z_k = 0,
\]
hence
$i_{k+1} = 2i_k-i_{k-1} = (k+1)i$, as required.
Finally, the multiplicity $m$ of $\tilde L=Z_{l+1}$ in $\pi^*L$ equals
$(l+1)i$;
thus, $m$ is divisible by $i$,
and the length of the chain of $(-2)$-curves is $l = {m/i-1}$.
\begin{center}
\begin{minipage}{\textwidth-1mm}
  \centering
\includegraphics{piL.eps}
\captionof{figure}{Multiplicities of the components of
  $(\pi^*L)^{\mathrm {vert}}$}
\end{minipage}
\end{center}

The same argument shows that there are no points $r_{i,j}^{C\cap L}$
with $i>m$, and all points $r_{m,j}^{C\cap L}$ appear directly on
$\tilde L$.

In conclusion, for all $i$ such that
$\beta_i^{C\cap L} = (\beta'-\beta)_i >0$, the multiplicity $m$ is
divisible by $i$;
equivalently, $m$ is divisible by $\lcm (\beta'-\beta)$.




\section{Deformations of generalized Severi varieties}
\label{S:deform}


In this section we prove the result going the other direction than
Theorem~\ref{t:CH1.2}. It
asserts that all the generalized Severi varieties which,
according to
Theorem~\ref{t:CH1.2}, may appear in the hyperplane section
$V^{d,\delta}(\alpha,\beta) \cap \orth p$, do indeed appear.
% Moreover, the result also comprises the multiplicities with which each
% such component appears in the intersection,
% so that the two Theorems \ref{t:CH1.2} and \ref{t:CH1.3} together
% provide a recursive way of computing the degrees of generalized Severi
% varieties, which is the main result of this Chapter.

\begin{theorem}[{\cite[Theorem 1.3]{caporaso-harris}}]
\label{t:CH1.3}
Let $p$ be a general point of $L$.
\begin{asparaenum}[a]
\renewcommand{\theenumi}{\alph{enumi})}
\item
Let
$V'$ be an irreducible component of
$V^{d,\delta}(\alpha+e_k,\beta-e_k)(\Omega \cup \{p\})$
as in part \ref{case:non-stacca} of Theorem~\ref{t:CH1.2}.
Then $V'$ is a component of the intersection
$V^{d,\delta}(\alpha,\beta)(\Omega) \cap \orth p$, and at a general point
of $V'$,
the variety $V^{d,\delta}(\alpha,\beta)$ is smooth and has
intersection multiplicity $k$ with $\orth p$ along $V'$.
\item
\label{t:CH1.3-withL}
Let $V'$ be an irreducible component of
$V^{d-1,\delta'}(\alpha',\beta')(\Omega')$
as in part \ref{case:stacca} of Theorem~\ref{t:CH1.2}.
Then $V'$ is a component of the intersection
$V^{d,\delta}(\alpha,\beta)(\Omega) \cap \orth p$ and, at a general point
of $V'$,
the variety $V^{d,\delta}(\alpha,\beta)$
has $\binom {\beta'} \beta I^{\beta'-\beta}/\lcm(\beta'-\beta)$
local sheets, each of which has
intersection multiplicity $\lcm(\beta'-\beta)$ with $\orth p$ along $V'$. 
Moreover, each of these sheets has
the generic point of $V'$ as a point of multiplicity
\(
{\lcm(\beta'-\beta)}
/{\max(\beta'-\beta)},
\)
\end{asparaenum}
\end{theorem}

In both cases a) and b) the general strategy will be to show that the
general member of $V'$ may be deformed to general members of
$V^{d,\delta}(\alpha,\beta)(\Omega)$.
We treat the two cases separately, in Subsections \ref{s:unassign}
and \ref{s:merge} respectively.

The multiplicity in case a) displays a phenomenon reminiscent of
the fundamental principle of projective duality.
The deformation argument for case b) is much more
demanding, and eventually relies on the local material on deformations
of tacnodes gathered in Chapters \cite{05.margherita}
and \cite{06.francesco}, which is arguably the keystone of the present
volume. 



\subsection{Fixing an unassigned contact point}
\label{s:unassign}

This section is devoted to the proof of part a)
of Theorem~\ref{t:CH1.3}, which is the case when $V'$ parametrizes
curves that do not contain the line $L$, and for which the condition
that they lie on the hyperplane $\orth p$ is accounted for by the fact
that $p$ is one of the assigned contact points.

It is fairly clear that
$V^{d,\delta}(\alpha+e_k,\beta-e_k)(\Omega \cup \{p\})$ is contained
in the hyperplane section of
$V^{d,\delta}(\alpha,\beta)(\Omega)$ by $\orth p$, so the point here is to
establish the assertion on the smoothness and intersection
multiplicity.

The multiplicity is as one would expect it to be from the point of
view of projective duality. Indeed, the latter tells us the
following. Consider a variety
$X \subset \P^N$,
and its dual $\dual X \subset \check \P^N$ in the dual projective
space, which parametrizes hyperplanes in $\P^N$ tangent to $X$.
Then for a general point $p \in X$,
the hyperplane $\orth p \subset \check \P^N$
(consisting of those hyperplanes of $\P^N$ that contain the point $p$)
is tangent to $\dual X$ at the points $\orth T \in \check \P^N$
corresponding to hyperplanes that are tangent to $X$ at $p$.
More generally, one may consider ``osc-dual'' varieties
$X^{\vee_\beta} \subset \check \P^N$ of $X$,
parametrizing hyperplanes of $\P^N$ osculating $X$ to the order
$\beta$,
and then $\orth p$ osculates $X^{\vee_\beta}$ to the order $\beta$
at points $\orth O$ corresponding to osculating
hyperplanes to $X$ at $p$. Some of these are discussed in
Chapter~\cite{th-formulae}.

In the situation under consideration, this has to be applied to
the case when $X$ is
the degree $d-I\alpha$ rational normal curve 
image of $L$ by the linear system cut out by degree $d$ plane curves
with the contact conditions at assigned points determined by $\alpha$
and $\Omega$.
In fact this is exactly what we do in practice, following the approach of
\cite[\S 4.3]{caporaso-harris}, and establishing along the way the
appropriate biduality principle for osculating hyperplanes to rational
normal curves, which is the following.

\begin{proposition}[{\cite[Lemma~4.7]{caporaso-harris}}]
\label{pr:bidualCH}
Consider the line $L \subset \P^2$, and a general point $p$ of $L$.
We assume the data of
$d,\alpha,\beta$, and
$\Omega = (p_{i,j})_{1 \leq j \leq \alpha_i}$
is given as in Theorem~\ref{t:CH1.3};
in particular, $I\alpha+I\beta=d$.
We define the following three loci in $|\O_L(d)|$:
\begin{compactitem}
\item $\orth p = \{ D : p \in D \}$;
\item $\Phi_{\alpha,\beta}(\Omega) =
  \bigl\{
  D = \sum_{1\leq j \leq \alpha_i} i\cdot p_{i,j}
  + \sum_{1\leq j \leq \beta_i} i\cdot s_{i,j}
  \quad \text{for some 
  $s_{i,j}$'s in $L$}
  \bigr\}$;
\item $\Psi_{\alpha,\beta}(\Omega) =
  \bigl\{
  D = k\cdot p+
  \sum_{1\leq j \leq \alpha_i} i\cdot p_{i,j}
  + \sum_{1\leq j \leq (\beta-e_k)_i} i\cdot s_{i,j}
  \quad \text{for some 
  $s_{i,j}$'s in $L$}
  \bigr\}$.
\end{compactitem}
In a neighbourhood of a general point
$[D_0] \in \Psi_{\alpha,\beta}(\Omega)$,
the variety $\Phi_{\alpha,\beta}(\Omega)$ is smooth and has
intersection multiplicity $k$ with the hyperplane $\orth p$ along
$\Psi_{\alpha,\beta}(\Omega)$.
\end{proposition}

\begin{proof}
We will proceed by an explicit local computation.
Let $x$ be an affine coordinate on $L$ centered at the point $p$.
Let the points $p_{i,j}$ have respective coordinates $\lambda_{i,j}$,
and let the points $s_{i,j}^0$ such that
\[
  D_0 = k\cdot p+
  \sum_{1\leq j \leq \alpha_i} i\cdot p_{i,j}
  + \sum_{1\leq j \leq (\beta-e_k)_i} i\cdot s_{i,j}^0
\]
have respective coordinates $\mu_{i,j}$. 
By generality of $D_0$, we may assume
that these coordinates are altogether mutually distinct.

Then we can parametrize a neighbourhood of $[D_0]$ in 
$\Phi_{\alpha,\beta}(\Omega)$ by
\[
  (\epsilon, \epsilon_{i,j})
  \mapsto
  [f(x)] =
  \Bigl[
  (x-\epsilon)^k
  \cdot \prod_{1\leq j \leq \alpha_i} (x-\lambda_{i,j})^i
  \cdot \prod_{1\leq j \leq (\beta-e_k)_i} (x-\mu_{i,j}-\epsilon_{i,j})^i
  \Bigr]
  \in \C_d[x],
\]
from which we see first of all that
$\Phi_{\alpha,\beta}(\Omega)$ is smooth at $[D_0]$.
On the other hand, writing
\[
  f(x) = x^d+b_{d-1}x^{d-1} + \cdots + b_1 x + b_0 \in \C_d[x],
\]
we get a system of affine coordinates on some chart of $|\O_L(d)|$, in
which the hyperplane $\orth p$ is defined by the linear equation
$b_0=0$.
Then, in the local coordinates $(\epsilon, \epsilon_{i,j})$ on
$\Phi_{\alpha,\beta}(\Omega)$ around $[D_0]$, the intersection with
$\orth p$ is defined by the equation
\[
  \prod \lambda_{i,j}^i
  \cdot \epsilon^k
  \cdot \prod (\epsilon_{i,j}+\mu_{i,j})^i
  =0
  \iff
  \epsilon^k
  \cdot \prod (\epsilon_{i,j}+\mu_{i,j})^i
  =0,
\]
hence, locally around $[D_0]$,
it is $k$ times the divisor defined by the equation
$\epsilon = 0$,
and the latter divisor is exactly $\Psi_{\alpha,\beta}(\Omega)$.
\end{proof}


In order to relate the local geometry of generalized Severi varieties
to the model situation of Proposition \ref{pr:bidualCH}, we consider
the restriction map
$\pi: |\O_{\P^2}(d)| \dashrightarrow |\O_L(d)|$.
Note that this is merely the projection from the
codimension $d+1$ linear subspace
$\orth L$
of $|\O_{\P^2}(d)|$ parametrizing curves wich contain $L$.
Finally, observe that the hyperplane 
$\orth p$ of $|\O_{\P^2}(d)|$
is the preimage by $\pi$ of the hyperplane
$\orth p$ of $|\O_L(d)|$.

Let $W$ be the plain Severi variety $V^{d,\delta}$, and denote by
$\pi_W$ the restriction of $\pi$ to $W$.
By definition, using the notation of Proposition \ref{pr:bidualCH}, we
have
\[
  V^{d,\delta}(\alpha,\beta)(\Omega)
  = \pi_W^{-1} \bigl( \Phi_{\alpha,\beta}(\Omega) \bigr)
  \Et
  V^{d,\delta}(\alpha+e_k,\beta-e_k)(\Omega \cup \{p\})
  = \pi_W^{-1} \bigl( \Psi_{\alpha,\beta}(\Omega) \bigr).
\]
Therefore, part a) of Theorem~\ref{t:CH1.3} follows directly from the
following proposition together with
Proposition \ref{pr:bidualCH} above.


\begin{proposition}
\label{pr:unassign:diff}
Let $X_0$ be a general member of (any irreducible component of)
$V^{d,\delta}(\alpha+e_k,\beta-e_k)(\Omega \cup \{p\})$.
The differential of the map
$\pi_W: W \dashrightarrow |\O_L(d)|$ is surjective at the point
$[X_0]$.
\end{proposition}

\begin{proof}
First note that, being general, $X_0$ does not contain $L$ and
therefore $\pi$ is well defined at $[X_0]$.
Since the map $\pi$ is a linear projection, it suffices to show that
the projective tangent space $\T_{[X_0]}W$ to $W=V^{d,\delta}$ at the
point $[X_0]$ intersects the center of the projection transversely,
\ie that the intersection $\T_{[X_0]}W \cap \orth L$ has
codimension $d+1$ in $\T_{[X_0]}W$.

Now, the projective tangent space $\T_{[X_0]}W$ identifies with the
linear series of degree $d$ curves passing through the nodes of $X_0$,
and thus its intersection with $\orth L$ identifies with the
linear series of degree $d-1$ curves passing through the nodes of
$X_0$. By Lemma \ref{l:indep-cond}, these two linear series have
dimensions
$\frac {d(d+3)}2-\delta$ and $\frac {(d-1)(d+2)}2-\delta$
respectively, so the codimension of $\T_{[X_0]}W \cap \orth L$ in
$\T_{[X_0]}W$ equals that of $|\O_{\P^2}(d-1)|$ in $|\O_{\P^2}(d)|$,
which is $d+1$, as we wanted.
\end{proof}


The following lemma is the classical fact that, on a regular surface,
the adjoint series cut out the complete canonical series.
We include the proof for completeness.


\begin{lemma}
\label{l:indep-cond}
Let $C \subset \P^2$ be a $\delta$-nodal curve of degree $d$.
For all $e\geq d-3$, the nodes of $C$ impose independent conditions on
curves of degree $e$.
\end{lemma}

\begin{proof}
It is sufficient to prove that the nodes of $C$ impose independent
conditions on curves of degree $d-3$.
Let $\cI \subset \O_{\P^2}$ be the ideal sheaf of the nodes of $C$ as
a subscheme of $\P^2$, and let $\cA \subset \O_C$ be the conductor
ideal sheaf of $C$ (with respect to its normalization $\bar C$).
The ideal $\cA$ is the restriction of $\cI$ to $C$
(see, \eg \cite[Lemma \tref{L:adj2}]{02.edoardo}), and we have an
exact sequence
\[
  0 \longto \O_{\P^2}(-3)
  \longto \O_{\P^2}(d-3)\otimes \cI
  \longto \O_C(d-3)\otimes \cA
  \longto 0.
\]
It follows that there is an isomorphism
$H^0( \O_{\P^2}(d-3)\otimes \cI)
\cong H^0( \O_C(d-3)\otimes \cA)$.
Now, by \cite[Corollary \tref{C:adj1}]{02.edoardo},
$H^0( \O_C(d-3)\otimes \cA)$ is isomorphic to
$H^0(\bar C, \omega_{\bar C})$, where $\bar C$ still denotes the
normalization of $C$, hence it has dimension $g$, the geometric genus
of $C$, so that finally
\begin{align*}
  h^0\bigl(\O_{\P^2}(d-3)\otimes \cI\bigr)
  &= g = p_a(d)-\delta
  \\
  &= h^0\bigl(\O_{\P^2}(d-3)\bigr) -\delta,
\end{align*}
as we wanted to prove.
\end{proof}



\subsection{Merging a line}
\label{s:merge}


This section is devoted to the proof of part \ref{t:CH1.3-withL}
of Theorem~\ref{t:CH1.3}, which is the case when $V'$ parametrizes
curves containing the line $L$.
The proof will be divided in two parts
(Sections \ref{ss:relaxed}
and \ref{s:merge-zrr})
which we shall describe
shortly, but we first need to introduce some notation.
We advise the reader that he should have Sections
\ref{s:gnlpict}
and \ref{s:localgeom}
clear in mind in order to understand what is going on.

\paragraph{The situation}
\label{p:notation1.3}
We consider a curve $X_0 = C \cup L$, where
$[C]$ is a general member of the component $V'$ of
$V^{d-1,\delta'}(\alpha',\beta')(\Omega')$ we have started with.

We have $\alpha' \leq \alpha$, and correspondingly $\Omega'$ is a
subset of $\Omega$;
by this we mean that
$\Omega' = (p_{i,j}')_{1 \leq j \leq \alpha_i'}$ such that for all $i$,
$(p_{i,j}')_{1 \leq j \leq \alpha_i'}$ is a subsequence of
$(p_{i,j})_{1 \leq j \leq \alpha_i}$.

On the other hand we have $\beta' \geq \beta$,
and we choose a subset $\Lambda = (s_{i,j})_{1 \leq j \leq \beta_i}$
of cardinality $\beta$
of the sequence $(s'_{i,j})_{1 \leq j \leq \beta'_i}$ of unassigned
contact points of $C$ with $L$. 



\paragraph{General strategy}
\label{p:strat1.3}
The first part of the proof will consist in deforming the curve $X_0$
to degree $d$ curves locally equigenerically around the points of
$\Omega'$ and $\Lambda$, while maintaining the contact conditions
encoded in $\alpha,\beta$, and $\Omega$. At a point $p'_{i,j}$ or
$s_{i,j}$, the curve $C\cup L$ has an order $i$ tacnode; the
requirement that the deformation be locally equigeneric around such a
point amounts in pratice to the requirement that the $i$-th order
tacnode deforms into $i$ nodes.

In the second part of the proof we will take care of the
$\beta'-\beta$ remaining mobile contact points, \ie
those points $s'_{i,j}$ that are not in $\Lambda$.
At these points, the curve $C\cup L$ has order $i$ tacnodes as well, but
these ones will be deformed into $i-1$ nodes only.
This will ensure in particular that the line $L$ be merged with $C$
along the 
deformation, so that for instance if $C$ is irreducible, then the
curves deformed from $C\cup L$ will be irreducible as well.

The reader should consult Section~\ref{s:localgeom} to see that
these are indeed the appropriate deformations.
The reason for this two steps deformation process is that we want to
isolate the deformations of $i$-tacnodes to $i-1$ nodes from the rest,
in order to apply the results from the two previous lectures
\cite{05.margherita} and \cite{06.francesco}.
% the deformations in the first step
% on the other hand are perfectly harmless.



\subsubsection{The relaxed Severi variety}
\label{ss:relaxed}

Here we perform the first step of the proof, as described in
\ref{p:strat1.3} above.
The deformation procedure described there will amount to defining a
relaxed Severi variety, seeing $X_0 = C\cup L$ as one of its
members, and showing that our relaxed Severi variety is smooth
at $[X_0]$.

We use the notation introduced in \ref{p:notation1.3} above, and in
particular we fix the choice of a subsequence $\Lambda$.
Moreover we label the points in $\Omega\setminus\Omega'$ as
$(p_{i,j}^L)_{1\leq j \leq \alpha^L_i}$; then, letting
$\alpha^L = (\alpha_i^L)_{i\geq 1}$, we have
$\alpha = \alpha' + \alpha^L$.
Note that around a point $p^L_{i,j}$, the curve $X_0$ has only one
local branch, which is an open subset of the line $L$.

On the other hand, we label the mobile contact points of $C$ with $L$
that have not been included in $\Lambda$ as
$(s_{i,j}^{C\cap L})_{1\leq j \leq \beta^{C\cap L}_i}$;
then, letting
$\beta^{C\cap L} = (\beta_i^{C\cap L})_{i\geq 1}$, we have
$\beta' = \beta + \beta^{C\cap L}$.

\paragraph{The relaxed Severi variety}
In an analytic neighbourhood of the point $[X_0]$ in
$|\O_{\P^2}(d)|$, we define the
\emph{relaxed Severi variety} $W_\Lambda$ to be the closure of the
locus of reduced, degree $d$ curves $X_t$ satisfying the following six
conditions: 
\begin{compactenum}[(i)]
\item\label{relaxed-nodes}
  $X_t$ preserves the $\delta'$ nodes of $C$,
  \ie for every node of $X_0$ off $L$, $X_t$ will have a node
  nearby; 
\item\label{relaxed-alphaL}
 at each point $p^L_{i,j} \in \Omega\setminus\Omega'$,
  $X_t$ has contact of order $i$ with
  $L$; 
\item\label{relaxed:cogenusi}
 in a neighbourhood of each point $p_{i,j}' \in \Omega'$, $X_t$
  has singularities with total cogenus $i$,
  \ie if we let $\bar X_t$ be the normalization of exactly these
  singularities, then $p_a(\bar X_t) = p_a(X_t)-i$;
\item\label{relaxed:cogenusii}
 in a neighbourhood of each point $s_{i,j} \in \Lambda$, $X_t$
  has singularities with total cogenus $i$;
\item in a neighbourhood of each point $p_{i,j}' \in \Omega'$, it
  follows from condition (iii) that $X_t$ has two local branches; we
  require that the one branch that is a deformation of an open subset
  of $C$ has contact of order $i$ with $L$ at $p_{i,j}'$;
\item in a neighbourhood of each point $s_{i,j} \in \Lambda$, the
  curve $X_t$ has two local branches;
  we require that the one branch that is a deformation of an open
  subset of $C$ has contact of order $i$ with $L$ at a point near
  $s_{i,j}$.
\end{compactenum}
Just to be sure, we recall that the curve $X_0=C\cup L$ has an $i$-th
order tacnode at each point $p'_{i,j}\in \Omega'$ or
$s_{i,j}\in \Lambda$, with two local branches that are open subsets of
$C$ and $L$ respectively. Conditions (iii) and (iv) imply that in a
neighbourhood of such a point, the curves $X_t$ have two
local branches as well, which are deformations of open subsets of
$C$ and $L$ respectively.


\bigskip%\paragraph{}
With this definition for the relaxed Severi variety, it is
clear that $[X_0] \in W_\Lambda$.
We could have defined $ W_\Lambda$ alternatively,
by requiring in (iii) and (iv)
that in a neighbourhood of each point $p'_{i,j}$ or $s_{i,j}$,
the curve $X_t$ has $i$ nodes.
The reason why $W_\Lambda$ will be smooth at $[X_0]$ is because the
only special feature of $X_0$ with respect to a general member of
$W_\Lambda$ is that it has several groups of $i$ nodes coming together
as $i$-th order tacnodes (for various $i$'s),
and this is perfectly harmless from the
point of view of the deformation theory of nodal curves:
somehow, this is the classical view that an $i$-th order tacnode is
just $i$ infinitely near ordinary nodes.
This will be made precise when we compute the Zariski tangent space to
$W_\Lambda$ at the point $[X_0]$.

In order to show the smoothness of $W_\Lambda$ at $[X_0]$ we will
compare the dimension of $W_\Lambda$ with that of its tangent space at
$[X_0]$.
We proceed to compute the dimension of $W_\Lambda$ in the next
paragraph.



\paragraph{The relaxed Severi variety as a local sheet of a
 Severi variety}
\label{p:relax-locsheet}
The basic observation in this paragraph
is that the six conditions defining the relaxed
Severi variety $W_\Lambda$ in fact essentially define a generalized
Severi variety in the plain sense. Namely, we are requiring that the
curves $X_t$,
(i) have a certain genus (or, equivalently, cogenus), defined by the
$\delta'$ nodes deformations of those of $C$ and the various groups of
$i$ nodes deformations of the points $p'_{i,j} \in \Omega'$ and
$s_{i,j} \in \Lambda$,
and (ii) satisfy certain contact conditions with $L$.
Specifically, the cogenus,
\ie the difference in arithmetic genus between the curves $X_t$ and
their normalizations, is required to be:
\begin{equation}
\label{eq:relax-nodes}
\begin{aligned}
  \delta'':=
  \delta' +
  I\alpha'+I\beta
  &= \delta' +
  I\alpha'+I\beta'-I(\beta'-\beta)
  \\
  &= \delta' +(d-1)-I(\beta'-\beta)
    = \delta -\bigl(I(\beta'-\beta)-|\beta'-\beta|\bigr)
\end{aligned}
\end{equation}
(for the last equality, recall the relation between $\delta$ and
$\delta'$, given for instance in Theorem~\ref{t:CH1.2}).
On the other hand the contact conditions with $L$ are exactly those
prescribed by $\alpha,\beta$ and $\Omega$. Altogether, these are the
conditions defining the (generalized) Severi variety
$V^{d,\delta''}(\alpha,\beta)(\Omega)$.

The additional requirements in the definition of
$W_\Lambda$ have the effect of selecting an open subset of
some local sheets of
$V^{d,\delta''}(\alpha,\beta)(\Omega)$ at $[X_0]$.
We are first of all requiring
that the $i$ nodes corresponding to a point $p'_{i,j}$ or
$s_{i,j}$ be in a neighbourhood of this same point;
in other words we prescribe among the tacnodes of $X_0$
which deform to $i$ nodes, and which are ignored.
This already selects local sheets of
$V^{d,\delta''}(\alpha,\beta)(\Omega)$ at $[X_0]$,
determined by $\Lambda$:
indeed, if we consider $W_\Lambda$ as a space of maps from curves of
cogenus $\delta''$ to $\P^2$, then the member of $W_\Lambda$
corresponding to
$X_0$ is the partial normalization of $X_0=C\cup L$ at the points of
$\Omega'$ and $\Lambda$;
if one considers another partial normalization of $X_0$ at the points
of $\Omega'$ and some other $\Lambda'$, one gets a curve member of the
space of maps corresponding to $V^{d,\delta''}(\alpha,\beta)(\Omega)$,
which however does not belong to $W_\Lambda$.

We are moreover requiring that,
locally around a point $p'_{i,j}$ or $s_{i,j}$,
the order $i$ contact with $L$ be supported on the one local branch
that is a deformation of the local branch of $C$.
This again, and in the same way as above,
has the effect of operating a selection among the local
sheets of $V^{d,\delta''}(\alpha,\beta)(\Omega)$ at $[X_0]$.

The upshot is that
the relaxed Severi variety $W_\Lambda$ is an open subset in some local 
sheets of the generalized
Severi variety
$V^{d,\delta''}(\alpha,\beta)(\Omega)$.
Since the latter is equidimensional, we have
\[
  \dim(W_\Lambda)
  = \dim \bigl( V^{d,\delta''}(\alpha,\beta) \bigr)
  = 2d+g''+|\beta|-1,
\]
with $g''=p_a(d)-\delta''=\binom {d-1}2 -\delta''$.


\paragraph{The ideal defining the tangent space to the relaxed Severi
  variety}
We shall prove, in Proposition \ref{pr:tg-relaxed} below,
that the tangent space at $[X_0]$ of the relaxed Severi
variety $W_\Lambda$ identifies with the subspace
$H^0(X_0, \cI(d))$ of $H^0(X_0, \O(d))$ defined by an ideal sheal
$\cI$ of $\O_{X_0}$ which we shall now describe,
based on the description of the tangent space of generalized Severi
varieties given in \cite{03.th-acz}.

If $X$ is a $\delta$-nodal curve member of the ordinary Severi variety
$V^{d,\delta}$, then the tangent space $T_{[X]}V^{d,\delta}$ is 
$H^0(X, \cA(d))$, with $\cA$ the ideal sheaf of the points supporting
the nodes of $X$. When 
$i$ of the $\delta$ nodes become infinitely near so as to form an
$i$-th order tacnode, the ideal sheaf $\cA$ has to be modified in the
most straightforward way, \ie it is merely the ideal sheaf of the
possibly infinitely near points supporting the nodes of $X$. In other
words, it is cut out locally at an order $i$ tacnode by 
curves osculating to the order $i$ the two local branches of $X$ at the
tacnode.
%We refer to \cite[\S 3.2]{DS} for more details.

On the other hand we have seen in a previous Lecture,
see \cite[Lemma~\tref{l:log-tg}]{03.th-acz},
that an order
$i$ contact condition with $L$ at an assigned (resp.\ unassigned)
point translates into the vanishing to the order $i$ (resp.\ $i-1$) of
the sections in $H^0(X,N_{X})$ corresponding to vectors tangent
to such deformations.

These considerations motivate the definition of the
ideal sheaf $\cI$.

\medskip
\subparagraph{Definition}
\label{sp:def-ideal}
We consider the curve $X_0=C\cup L$ introduced in \ref{p:notation1.3} 
above.
For all $i,j$ with $1\leq j \leq \alpha_{i}'$, we let
$\lp\cI\alpha_{i,j}$ be the subsheaf of $\O_{X_0}$ of those regular
functions $f$,
such that the restrictions $\restr f C$ and $\restr f L$
vanish at $p_{i,j}'$ to the orders $i$ and $2i$ respectively.

Similarly, for all $i,j$ with $1\leq j \leq \beta_i$, we let
$\lp{\cI}{\beta}_{i,j}$ be the sheaf of regular functions $f$ on $X_0$,
such that
$\restr f C$ and $\restr f L$
vanish at $s_{i,j}$ to the orders $i$ and $2i-1$ respectively.

For all points $x\in X_0$, we denote by $\fm_x$ the ideal sheaf
defining $x$ in $X_0$.
Lastly, we call $u_1,\ldots,u_{\delta'}$ the $\delta'$ nodes of
$C$. Finally, we set:
\begin{equation*}
  \cI =
  \prod _{1 \leq i \leq \delta'} \fm_{u_i}
  \cdot \prod_{1\leq j \leq \alpha_i^L} \fm_{p_{i,j}^L} ^i
  \cdot \prod_{1\leq j \leq \alpha_i '} \lp\cI\alpha_{i,j}
  \cdot \prod_{1\leq j \leq \beta_i} \lp\cI\beta_{i,j}.
\end{equation*}


\begin{proposition}
\label{pr:tg-relaxed}
The relaxed Severi variety $W_\Lambda$ is smooth at $[X_0]$, with
tangent space
\[
  T_{[X_0]} W_\Lambda = H^0(X_0, \cI(d))
  \ \subset
  \
  T_{[X_0]} \bigl( |\O_{\P^2}(d)| \bigr)
  = H^0(X_0, \O_{X_0}(d)),
\]
where $\cI$ is the sheaf of ideals defined in \ref{sp:def-ideal}
above.
\end{proposition}


\begin{proof}
We will compare the deformations of $X_0$ along $W_\Lambda$ with
those of the map given by a certain partial normalization
of $X_0$.
Let
$\mu: \tilde X_0 \to X_0$ be the normalization of $X_0=C\cup L$ at the
nodes $u_i$ of $C$
and at the tacnodes $p_{i,j}' \in \Omega'$ and $s_{i,j}
\in \Lambda$ 
(at which $C$ and $L$ touch), but not at the tacnodes
$s_{i,j}'$, because the latter are off $\Lambda$.
We will consider the deformations of the map $\phi:\tilde X_0 \to
\P^2$ obtained as the composition of $\mu$ with the inclusion $X_0
\subset \P^2$.

The map $\phi$ is unramified, hence its normal sheaf $N_\phi$ is
locally free, equal to 
$\omega_{\tilde X_0} \otimes \phi^* \omega_{\P^2} ^{-1}$, see
\cite[Lemma~\tref{L:Emaps3}]{02.edoardo}.
By Lemma~\ref{l:nonspecial} below,
$H^1(\tilde X_0, N_\phi)$ vanishes, hence the deformation space of
$\phi$ is smooth of dimension
\[
  h^0 (\tilde X_0, N_\phi)
  = h^0 (\tilde X_0,
  \omega_{\tilde X_0} \otimes \phi^* \omega_{\P^2} ^{-1}).
\]
The smoothness of this space ensures in particular the existence of a
map $F$ from a neighbourhood of $[\phi]$ to $|\O_{\P^2}(d)|$,
mapping a deformation of $\phi$ to its image in $\P^2$,
as in \cite[\tref{p:curves-maps}]{03.th-acz}.

The image of $F$ is what we will call
the \emph{superrelaxed Severi variety} $\tilde W_\Lambda$, which 
we define as $W_\Lambda$ but only with the three requirements
\eqref{relaxed-nodes},
\eqref{relaxed:cogenusi},
and \eqref{relaxed:cogenusii}
out of the six defining $W_\Lambda$;
simply put, we just drop the contact conditions with $L$.
Arguing as in \ref{p:relax-locsheet} above, we see that
$\tilde W_\Lambda$ is a local sheet of the plain Severi
variety $V^{d,\delta''}$ at $[X_0]$,
which implies that it has dimension
\[
  \dim(\tilde W_\Lambda) = \dim (V^{d,\delta''})
  = 3d+g''-1.
\]
That $F$ surjects onto a neighbourhood of $[X_0]$ in
$\tilde W_\Lambda$ is a consequence of Teissier's Résolution Simultanée
Theorem, as in \cite[\tref{p:curves-maps}]{03.th-acz}.

In order to analyze the tangent space to $\tilde W_\Lambda$
at $[X_0]$, we let
$\cA = (\O_{X_0}:\mu_*\O_{\tilde X_0})$ be the conductor of
$\tilde X_0$ in $X_0$, see \cite[\S \tref{E:S:cond}]{02.edoardo}.
It is a sheaf of ideals of $\O_{X_0}$, trivial on the open subset onto
which $\mu$ is an isomorphism,
equal to $\fm_{u_i}$ locally at the nodes $u_i$ of $C$,
while locally at the points $p_{i,j}'\in \Omega'$ and $s_{i,j} \in
\Lambda$ it is the sheaf of regular functions vanishing to the order
$i$ on both $C$ and $L$;
this can be seen for instance with \cite[Lemma \tref{L:adj2}]{02.edoardo}.

By \cite[Corollary \tref{C:Emaps1}]{02.edoardo}, one has
$\mu_* N_\phi = \cA\otimes N_{X_0/\P^2}$. Therefore, there is a canonical
isomorphism
\begin{equation*}
\label{isom-de-la-mort}
  H^0(\tilde X_0, N_\phi)
  \cong H^0(X_0,\cA\otimes N_{X_0/\P^2}).
\end{equation*}
This isomorphism identifies with the differential of $F$ at
$[\phi]$, and thus we see that $F$ is an isomorphism onto a
neighbourhood of $[X_0]$ in $\tilde W_\Lambda$;
in particular, the superrelaxed Severi variety $\tilde W_\Lambda$ is
smooth at $[X_0]$, with tangent space
$H^0(X_0,\cA\otimes N_{X_0/\P^2})$.

Now, it follows from \cite[\tref{l:log-tg}]{03.th-acz}
that the Zariski
tangent space at $[\phi]$ to the image by $F^{-1}$ of the relaxed
Severi variety $W_\Lambda \subset \tilde W_\Lambda$ is contained in
\begin{equation*}
  H^0 \biggl( \tilde X_0, N_\phi\Bigl(
  -\sum_{1\leq j \leq \alpha_i^L} i \cdot q_{i,j}^L
  -\sum_{1\leq j \leq \alpha_i '} i\cdot  q_{i,j}'
  -\sum_{1\leq j \leq \beta_i} (i-1)\cdot r_{i,j}
  \Bigr)\biggr),
\end{equation*}
where
(i) $q_{i,j}^L$ is the unique point of $\tilde X_0$ over
$p_{i,j}^L$,
and (ii) $q_{i,j}'$ and $r_{i,j}$ are the points on the proper
transform of $C$ in $\tilde X_0$ lying over $p_{i,j}'$
and $s_{i,j}$ respectively.
Moreover, it follows from the description of $\cA$ given above that
\begin{equation*}
  \cA\otimes \phi_* \O_{\tilde X_0}
  \Bigl(
  -\sum_{1\leq j \leq \alpha_i^L} i \cdot q_{i,j}^L
  -\sum_{1\leq j \leq \alpha_i '} i\cdot  q_{i,j}'
  -\sum_{1\leq j \leq \beta_i} (i-1)\cdot r_{i,j}
  \Bigr)
  = \cI,
\end{equation*}
hence
\begin{equation*}
  \phi_* N_\phi\Bigl(
  -\sum_{1\leq j \leq \alpha_i^L} i \cdot q_{i,j}^L
  -\sum_{1\leq j \leq \alpha_i '} i\cdot  q_{i,j}'
  -\sum_{1\leq j \leq \beta_i} (i-1)\cdot r_{i,j}
  \Bigr)
  = \cI\otimes N_{X_0/\P^2}.
\end{equation*}
Therefore, the Zariski tangent space to the relaxed Severi variety
$W_\Lambda$ at $[X_0]$ is contained in
$H^0(X_0,\cI\otimes N_{X_0/\P^2})$.
Then, the proposition follows from the equality
\[
  h^0(X_0,\cI\otimes N_{X_0/\P^2})
  = \dim (W_\Lambda), 
\]
which is given by \eqref{l:RR2} below.
\end{proof}



\bigskip
The rest of the present Section~\ref{ss:relaxed}
is devoted to some elementary considerations leading to the
non-speciality of the invertible sheaves on
$\tilde X_0$
involved in the above proof,
and the computation of the dimensions of their spaces of
global sections with the Riemann--Roch Formula.


\begin{lemma}
\label{l:nonspecial}
Let $p$ be any point of the
partial normalization $\tilde X_0$, and
\[
  D =
  \sum_{1\leq j \leq \alpha_i^L} i \cdot q_{i,j}^L
  +\sum_{1\leq j \leq \alpha_i '} i\cdot  q_{i,j}'
  +\sum_{1\leq j \leq \beta_i} (i-1)\cdot r_{i,j},
\]
with the notation as in the proof of
Proposition~\ref{pr:tg-relaxed} above.
The two line bundles $N_\phi(-D)$ and $N_\phi(-D-p)$
on $\tilde X_0$ are non-special.
\end{lemma}

\begin{proof}
Let $\tilde C$ and $\tilde L$ be the proper transforms
in $\tilde X_0$ of $C$ and $L$ respectively.
Since $N_\phi = \omega_{\tilde X_0}\otimes \phi^*\omega_{\P^2}^{-1}$
as we have seen above, one has
\begin{equation*}
  \omega_{\tilde X_0}\otimes \bigl(
  N_\phi(-D)
  \bigr) ^{-1}
  = \phi^*\O_{\P^2}(-3) \otimes \O_{\tilde X_0}(D).
\end{equation*}
The degree of the restriction of this line bundle to $\tilde C$
has degree
\begin{align*}
  -3(d-1)+I\alpha'+\bigl( I\beta-|\beta|\bigr)
  &\leq
    -3(d-1)+I\alpha'+I\beta' \\
  &=-2(d-1) <0,
\end{align*}
hence every global section of
$\omega_{\tilde X_0}\otimes N_\phi(-D)^{-1}$ vanishes identically on
$\tilde C$.
One proves similarly that the same holds for
$\omega_{\tilde X_0}\otimes N_\phi(-D-p)^{-1}$, noting that it
restricts on $\tilde C$ to a line bundle of degree
$-2(d-1)+\epsilon$, where $\epsilon$ equals $0$ or $1$ depending on
whether $p$ sits on $\tilde C$ or not.

Thus, 
every global section of
$\omega_{\tilde X_0}\otimes N_\phi(-D)^{-1}$
restricts on $\tilde L$ to a global section of the line bundle
\[
  \phi^*\O_{\P^2}(-3) \otimes \O_{\tilde L}(\restr D {\tilde L})
  \otimes \O_{\tilde L}(-\restr {\tilde C} {\tilde L}),
\]
which has degree
\begin{align*}
  -3 + I\alpha^L -I\beta^{C\cap L}
  &= -3 +I(\alpha-\alpha')-I(\beta'-\beta)
  \\
  &= -3 + (I\alpha+I\beta) -(I\alpha'+I\beta')
  \\
  &= -3 +d-(d-1) = -2.
\end{align*}
Therefore every global section of
$\omega_{\tilde X_0}\otimes N_\phi(-D)^{-1}$
vanishes identically on $\tilde L$ as well, hence
\[
  h^0(\tilde X_0, \omega_{\tilde X_0}\otimes N_\phi(-D)^{-1})
  = h^1(\tilde X_0, N_\phi(-D)) = 0.
\]
One concludes in the same way that every global section of
$\omega_{\tilde X_0}\otimes N_\phi(-D-p)^{-1}$ vanishes identically,
hence $N_\phi(-D-p)$ is non-special.
\end{proof}


\begin{lemma}
\label{l:RR}
\label{l:bpf}
The following equalities hold:
\begin{align}
  \label{l:RR1}
  h^0\bigl(\tilde X_0, N_\phi\bigr)
  &= 3d+g''-1 ;
  \\
  \label{l:RR2}
  h^0\bigl(\tilde X_0, N_\phi(-D)\bigr)
  &= 2d+g''-1+|\beta|.
\end{align}
Moreover, the line bundle $N_\phi(-D)$ has no base point.
\end{lemma}


\begin{proof}
Both equalities follow from the application of the Riemann--Roch
Formula on the curve $\tilde X_0$, which has arithmetic genus $g''$,
see \ref{p:relax-locsheet}.
The line bundle $N_\phi$ equals
$\omega_{\tilde X_0}\otimes \phi^*\omega_{\P^2}^{-1}$ which is
obviously non-special, hence
\begin{align*}
  h^0(N_\phi)
  &= 1-g'' + \deg \bigl(
    \omega_{\tilde X_0}\otimes \phi^*\omega_{\P^2}^{-1}
    \bigr)
  \\
  &= 1-g'' + (2g''-2) +3d
  \\
  &= 3d+g''-1.
\end{align*}
The line bundle $N_\phi(-D)$ is non-special by
Lemma~\ref{l:nonspecial} above, hence
\begin{align*}
  h^0\bigl(N_\phi(-D)\bigr)
  &= 1-g'' + \deg (N_\phi)-\deg(D)
  \\
  &= 3d+g''-1
    -\bigl(I\alpha^L+I\alpha'+I\beta-|\beta|
    \bigr)
  \\
  &= 2d+g''-1+|\beta|,
\end{align*}
because
\[
  I\alpha^L+I\alpha'+I\beta
  = I\alpha+I\beta = d.
\]
Eventually, since for all $p \in \tilde X_0$ the line
bundle $N_\phi(-D-p)$ is non-special as well, we have
\[
  h^0 \bigl(\tilde X_0, N_\phi(-D-p) \bigr)
  = h^0 \bigl(\tilde X_0, N_\phi(-D) \bigr) -1,
\]
hence not all global sections of $N_\phi(-D)$ vanish at $p$.
\end{proof}


\subsubsection{Deformation of order $i$ tacnodes to $i-1$ nodes}
\label{s:merge-zrr}


Here we perform the second step of the proof of
part \ref{t:CH1.3-withL}
of Theorem~\ref{t:CH1.3},
as described in \ref{p:strat1.3} above.
We assume that $\beta'>\beta$, for otherwise there
is nothing left to do in the second step
(see Remark~\ref{rk:allred} below for what happens in this case).

We consider the map
\[
  F_\Lambda: W_\Lambda \to \Delta,
\]
from the relaxed Severi variety $W_\Lambda$, introduced and studied in
the previous Section~\ref{ss:relaxed}, to
the product $\Delta$ of the versal deformation spaces of the tacnodes
$s_{i,j}^{C \cap L}$ of $X_0 = C\cup L$, \ie those tacnodes of $X_0$
not included in $\Lambda$.

We refer to \cite{05.margherita} and \cite{06.francesco} for background and the
necessary material on deformation spaces of tacnodes and their
product. The result we shall need here is \cite[\tref{lemma 4.3}]{06.francesco},
which we now recall in a form adapted to our context.

\paragraph{}
\label{p:restatement-prodtacnodes}
The tacnodes $s_{i,j}^{C \cap L}$ are indexed by $\beta'-\beta$,
and thus
\[
  \Delta = \prod_{i\in\N^*}
  \prod_{1\leq j \leq \beta'_i-\beta_i} \Delta_{i,j},
\]
where each $\Delta_{i,j}$ is the versal deformation space of the
$i$-th order tacnode $s_{i,j} ^{C \cap L}$.
For all $i$ and $j$, we let $\Delta_{i,j;i}$ and $\Delta_{i,j;i-1}$
be the subvarieties of $\Delta_{i,j}$ of those deformations of
$s_{i,j} ^{C \cap L}$ into $i$ and $i-1$ nodes respectively.
We let
\[
  \bm =
  (m_l) _{1\leq l \leq |\beta'-\beta|} =
  \bigl(\,
  \underbrace{1,\ldots,1}_{\beta'_1-\beta_1},
  \quad \ldots,\quad 
  \underbrace{n,\ldots,n}_{\beta'_n-\beta_n}
  \,\bigr)
\]
with $n = \max(\beta'-\beta)$,
and consider
\[
  \Delta_\bm = \prod_{i\in\N^*}
  \prod_{1\leq j \leq \beta'_i-\beta_i} \Delta_{i,j;i},
  \quad\text{and}
  \quad
  \Delta_{\bmm} = \prod_{i\in\N^*}
  \prod_{1\leq j \leq \beta'_i-\beta_i} \Delta_{i,j;i-1}.
\]

Each $\Delta_{i,j}$ is a $(2i-1)$-dimensional affine space, with
coordinates $a_0,\ldots,a_{i-2},b_0,\ldots,b_{i-1}$, such that the
corresponding versal deformation is the hypersurface
\begin{equation}
\label{versal}
  y^2+y(x^i+a_{i-2}x^{i-2}+\cdots +a_0)
  +b_{i-1}x^{i-1}+\cdots +b_0
\end{equation}
in $\A^2_{x,y} \times \A^{2i-1}_{\mathbf a,\mathbf b}$.
In these terms, $\Delta_{i,j;i}$ is the dimension $i-1$ affine
subspace defined by the equations $b_0=\cdots=b_{i-1}=0$.
We consider in addition the hyperplane
$\cH_{i,j} \subset \Delta_{i,j}$ defined by the equation $b_0=0$ in
this system of coordinates. Observe that $\cH_{i,j}$ parametrizes
those deformations of the tacnode defined by $y(y+x^m)=0$ that still
pass through the origin in $\A^2_{x,y}$;
in other words, these are the deformations maintaining one assigned
contact point of order $1$ with the line $y=0$.
The general member of $\cH_{i,j}$ is an irreducible curve.
Eventually we let
\[
  \cH = \bigcup_{i,j} \cH_{i,j}
  \ \subset\ 
  \Delta.
\]

Now, the result is the following.
Let $W \subset \Delta$ be a smooth subvariety of dimension
$\dim(\Delta_{\bmm})+1$, containing $\Delta_{\bmm}$, and such that the
tangent space at the origin $T_0W$ is not contained in $\cH$.
Then, in an étale neighbourhood of the origin $0\in \Delta$,
\[
  W\cap \Delta_\bmm = \Delta_\bm \cup
  \Gamma_1 \cup \cdots \cup \Gamma_\kappa,
\]
where
\[
  \kappa
  = \frac
  {\prod\limits_{1\leq l \leq |\beta'-\beta|} m_l}
  {\underset {1\leq l \leq |\beta'-\beta|} \lcm m_l}
  = \frac
  {I^{\beta'-\beta}}
  {\lcm (\beta'-\beta)},
\]
and $\Gamma_1, \ldots, \Gamma_\kappa$
are distinct reduced unibranched curves, each of which
has the origin as a point of multiplicity
\[
  \frac
  {\underset {1\leq l \leq |\beta'-\beta|} \lcm m_l}
  {\underset {1\leq l \leq |\beta'-\beta|} \max m_l}
  = \frac
  {\lcm(\beta'-\beta)}
  {\max(\beta'-\beta)},
\]
and has intersection multiplicity
$\lcm _{1\leq l \leq |\beta'-\beta|} m_l
= \lcm (\beta'-\beta)$ with $\Delta_\bm$ at the origin.


\bigskip
We now proceed to prove a series of claims in order to see that the
hypotheses of the above statement are verified in our situation,
taking $W = F_\Lambda(W_\Lambda)$.


\begin{claim}
\label{cl:invimage}
The inverse image $W_{\Lambda,\bm} = F_\Lambda^{-1}(\Delta_\bm)$ is the
locus of those members of $W_\Lambda$ that contain $L$.
It is also the intersection of $W_\Lambda$ with the hyperplane
$\orth p \subset |\O_{\P^2}(d)|$, for general $p\in L$.
\end{claim}

\begin{proof}
Let us first prove the first assertion.
The inverse image $F_\Lambda^{-1}(\Delta_\bm)$
is the locus in $W_\Lambda$ along which all the tacnodes
$s_{i,j} ^{C\cap L}$ of $X_0$ deform equigenerically.
Taking in addition into account
the requirements
\eqref{relaxed-nodes},
\eqref{relaxed:cogenusi},
and \eqref{relaxed:cogenusii} in the definition of the relaxed Severi
variety $W_\Lambda$,
we see that the curves in $F_\Lambda^{-1}(\Delta_\bm)$ are equigeneric
deformations of $X_0$.
Therefore they all come from deformations of the map
$\bar\phi: \bar X_0 \to \P^2$ obtained from the total normalization $\nu: \bar
X_0\to X_0$, by the same argument that has been used in the proof of
Proposition~\ref{pr:tg-relaxed}, which is essentially
Teissier's Résolution Simultanée. Now since the normalization $\bar
X_0$ is disconnected, the domain of any deformation of $\bar \phi$ is
disconnected as well by the Principle of Connectedness
(see, \eg \cite[Exercise III.11.4]{hartshorne}).
The upshot is that all curves in $F_\Lambda^{-1}(\Delta_\bm)$ consist
of a deformation of $C$ plus a deformation of $L$.

On the other hand we are assuming here that $\beta' > \beta$, for
otherwise the second step of the proof of 
part \ref{t:CH1.3-withL} of Theorem~\ref{t:CH1.3} is pointless.
Since
\[
  I\alpha+I\beta=d
  \quad \text{and}
  \quad
  I\alpha'+I\beta'=d-1,
\]
it follows that $I(\alpha-\alpha')\geq 2$,
\ie $I\alpha^L \geq 2$.
Now by requirement \eqref{relaxed-alphaL} in the definition of the
relaxed Severi variety, for each member of $F^{-1}(\Delta_\bm)$,
the component that is a deformation of $L$ must satisfy the contact
conditions with $L$ encoded in $\alpha^L$.
Therefore it intersects $L$ in at least two points (possibly
infinitely near), hence it is $L$ itself,
and our first assertion about $F^{-1}(\Delta_\bm)$ is proved.

As for the second assertion, the first assertion gives us of course the
inclusion
$F_\Lambda^{-1}(\Delta_\bm) \subset W_\Lambda \cap \orth p$ for all $p\in L$.
To prove the other inclusion, we note that for all
$p \in L$ neither in $\Omega$ nor in $\Lambda$, any curve in
$W_\Lambda \cap \orth p$ in a neighbourhood of $[X_0]$ has a total of
\[
  I\alpha+I\beta+1 = d+1
\]
imposed points of intersection with $L$ whereas it has degree $d$,
so that it must contain $L$.
\end{proof}


\begin{claim}
\label{cl:allDelta_m}
The image of $F_\Lambda$ contains the locus $\Delta_\bm$.
\end{claim}

\begin{proof}
The projection of $F_\Lambda(W_\Lambda)$ to
the factor $\Delta_{i,j}$ of $\Delta$
contains $\Delta_{i,j;i}$ if and only if
we can find a deformation $X_t$ of $X_0$ along $W_\Lambda$
in which a neighbourhood of the tacnode
$s_{i,j}^{C\cap L} \in X_0$ deforms to a reducible open curve
$X_t^{\circ\prime}+X_t^{\circ\prime\prime}$, such that
$X_t^{\circ\prime}$ and $X_t^{\circ\prime\prime}$ intersect
transversely in $i$ points that can be chosen arbitrarily on
$X_t^{\circ\prime}$.

To see that this holds simultaneously for all tacnodes
$s_{i,j}^{C\cap L} \in X_0$, we note that 
$F_\Lambda^{-1}(\Delta_\bm)$ identifies as in \ref{p:relax-locsheet}
with a local sheet at $[X_0]$
of the Severi variety
\[
  V^{d-1,\delta'} \bigl(
  \alpha', \beta+I(\beta'-\beta) e_1
  \bigr)(\Omega'):
\]
we have seen that $F_\Lambda^{-1}(\Delta_\bm)$ consists of those curve
in $W_\Lambda$ having $L$ as an irreducible component, and these
curves correspond to equigeneric deformations of $C$ maintaining the
contact 
conditions with $L$ in the points $p_{i,j}' \in \Omega'$ and
$s_{i,j} \in \Lambda$, but dropping those in the points encoded in
the points $s_{i,j} \not\in \Lambda$; the latter dropping so to speak
amounts to turn $\beta'-\beta$ into $I(\beta'-\beta) e_1$.

Then the condition we need to verify essentially follows from
Proposition~\ref{p:zariski} applied to
$V^{d-1,\delta'} \bigl(
  \alpha', \beta+I(\beta'-\beta) e_1
  \bigr)(\Omega')$.
More explicitly, the latter Severi variety contains locally around
$[X_0]$ the Severi varieties
\[
  V^{d-1,\delta'} \bigl(
  \alpha' +I(\beta'-\beta) e_1, \beta
  \bigr)(\Omega'\cup \Xi_t),
\]
where $\Xi_t$ is an arbitrary choice of $i$ points on $L$ around each
of the points $s_{i,j}\not\in \Lambda$, which is exactly the condition
we needed to verify.
\end{proof}


\begin{claim}
\label{cl:codim1}
The inverse image 
$W_{\Lambda,\bm} = F_\Lambda^{-1}(\Delta_\bm)$
has codimension one in $W_\Lambda$.
\end{claim}

\begin{proof}
This follows from the identification given above of
$F_\Lambda^{-1}(\Delta_\bm)$
with a local sheet at $[X_0]$
of the Severi variety
\(
  V^{d-1,\delta'} \bigl(
  \alpha', \beta+I(\beta'-\beta) e_1
  \bigr).
\)
Explicitly, this identifications tells us the dimension of
$F_\Lambda^{-1}(\Delta_\bm)$ as in \ref{p:relax-locsheet},
then
\begin{multline*}
  \dim(W_\Lambda)
  -\dim \bigl(F_\Lambda^{-1}(\Delta_\bm) \bigr)
  \\
  \begin{aligned}
    =&
    \Bigl[
    2d +{\textstyle \binom {d-1}2}-\delta'' -1 + |\beta|
    \Bigr]
    % \\
    % &
    -\Bigl[
    2(d-1)
    +{\textstyle \binom {d-2}2}-\delta'
    -1 + |\beta| + I(\beta'-\beta)
    \Bigr]
    \\
    &=2 + (d-2) - (\delta''-\delta')-I(\beta'-\beta),
  \end{aligned}
\end{multline*}
and this equals one by \eqref{eq:relax-nodes}.
\end{proof}


\begin{remark}
It is instructive, although not strictly necessary for
% the current proof of part \ref{t:CH1.3-withL} of Theorem~\ref{t:CH1.3}
our purposes, to
identify the fibre of $F_\Lambda$ over a general point of
$\Delta_\bm$.
We shall obtain such an identification from the considerations in the
proof of 
Claim~\ref{cl:allDelta_m}
above, after we observe that a point of $\Delta_{i,j;i} \subset
\Delta_{i,j}$ corresponds to the choice of $i$ points on one branch of
the tacnode at $s_{i,j}$, but only up to reparametrization. This
amounts to the fact that, in \eqref{versal},
the polynomial
\[
  x^i+a_{i-2}x^{i-2}+\cdots +a_0
\]
defining the unions of these $i$
points has no $x^{i-1}$ term;
any degree $i$ polynomial in $x$ can be put in this form
by a change of variable,
which amounts to translating the roots so that they sum up to zero.

Then the fibre of $F_\Lambda$ over a general point of $\Delta_\bm$
identifies with an open subset of the Severi variety
\begin{equation}
\label{gnl-fibre}
  V^{d-1,\delta'} \bigl(
  \alpha'
  +\bigl[
  I(\beta'-\beta) -|\beta'-\beta|
  \bigr]e_1,\
  \beta + |\beta'-\beta| e_1
  \bigr)(\Omega'\cup \Xi_t^\circ),
\end{equation}
with $\Xi_t^\circ$ an arbitrary choice of $i-1$ points on $L$ around each
of the points $s_{i,j}\not\in \Lambda$.
The fibre of $F_\Lambda$ over the origin of $\Delta$ on the other hand
identifies with an open subset of
\begin{equation}
\label{central-fibre}
V^{d-1,\delta'} (\alpha',\beta')(\Omega'),
\end{equation}
which was indeed our starting point.
It may be useful for the conclusion in \ref{p:conclusion} below to
recall that it has dimension one less than
$V^{d,\delta} (\alpha,\beta)$.

The fibre over the general point of $\Delta_\bm$
and the fibre over the origin have the same dimension: indeed
the Severi varieties
\eqref{gnl-fibre}
and \eqref{central-fibre}
have the same dimension
\begin{equation*}
  2(d-1)+g'-1+|\beta| + |\beta'-\beta|
  \ =
  \
  2(d-1)+g'-1 +|\beta'|,
\end{equation*}
with $g'=p_a(d-1)-\delta' = \binom {d-2}2 - \delta'$.

We leave it to the reader to verify that the latter common dimension
of
the fibre over the general point of $\Delta_\bm$
and the fibre over the origin also equals
\[
  \dim(W_\Lambda)-\dim(\Delta_\bm)-1;
\]
this is yet another straightforward computation after one notes that
\[
  \dim(\Delta_\bm)
  = \sum\nolimits _{1\leq l \leq |\beta'-\beta|} (m_l-1)
  = I(\beta'-\beta) - |\beta'-\beta|.
\]
\end{remark}


\begin{claim}
\label{cl:rk-diff}
Let $dF_\Lambda: T_{[X_0]}W_\Lambda \to T_0\Delta$ be the differential
map of $F_\Lambda$ at the point $[X_0]$.
One has
\[
  \dim\bigl(
  dF_\Lambda ^{-1}(T_0\Delta_\bm)
  \bigr)
  = \dim\bigl(
  F_\Lambda ^{-1}(\Delta_\bm)
  \bigr)
  = \dim (W_\Lambda)-1.
\]
\end{claim}


\begin{proof}
The second equality is Claim~\ref{cl:codim1} above. For the first one,
the key observation is that,
under the isomorphism
\[
  T_{[X_0]}W_\Lambda
  \cong
  H^0 \bigl( X_0, \cI(d) \bigr),
\]
the inverse image of
$T_0\Delta_\bm \subset T_0\Delta$ by the differential $dF_\Lambda$ at
$[X_0]$ is the subspace of sections vanishing identically along $L
\subset X_0$.

The restriction $\restr {\cI(d)} L$ has degree
\[
  d-I\alpha-I\beta = 0,
\]
and is therefore trivial. Now, the restriction map on global sections,
\[
  H^0 \bigl( X_0, \cI(d) \bigr)
  \to H^0 \bigl( L, \restr {\cI(d)} L \bigr) \cong \C,
\]
is non-zero by Lemma~\ref{l:bpf}, hence
\[
  \dim\bigl(
  dF_\Lambda ^{-1}(T_0\Delta_\bm)
  \bigr)
  = h^0 \bigl( X_0, \cI(d) \bigr) -1
  = \dim (W_\Lambda)-1,
\]
where the last equality comes from the smoothness of $W_\Lambda$ at
$[X_0]$.
\end{proof}


\begin{claim}
\label{cl:transverse}
The image of the differential map
$dF_\Lambda: T_{[X_0]}W_\Lambda \to T_0\Delta$
is not contained in $\cH$.%
\end{claim}

\begin{proof}
From the description of $\cH$ in \ref{p:restatement-prodtacnodes},
the inverse image
$(dF_\Lambda)^{-1}(\cH)$
is the union of the subspaces in
$H^0 \bigl( X_0, \cI(d) \bigr)$ of sections vanishing at one point
$s_{i,j}^{C\cap L}$.
By Lemma~\ref{l:bpf} these are all proper subspaces (in fact,
hyperplanes) of $H^0 \bigl( X_0, \cI(d) \bigr)$,
and the claim is proved.
\end{proof}


\paragraph{Conclusion}
\label{p:conclusion}
We may now finish the proof of
part \ref{t:CH1.3-withL} of Theorem~\ref{t:CH1.3}.
It follows from the description given in
Section~\ref{s:localgeom}
that, locally around the point $[X_0]$, the sum of the
local sheets of the
Severi variety $V^{d,\delta}(\alpha,\beta)(\Omega)$ corresponding to
the choice of $\Lambda$
is given as the closure in the relaxed Severi variety $W_\Lambda$ of
the inverse image
\[
  F_\Lambda^{-1} (\Delta_\bmm \setminus \Delta_\bm).
\]

Now, it follows from Claim~\ref{cl:rk-diff} that the differential map
\[
  dF_\Lambda: T_{[X_0]}W_\Lambda \to T_0\Delta
\]
has rank $\dim(\Delta_\bm)+1$,
equal to the dimension of $W = F_\Lambda(W_\Lambda)$.
Thus $W$ is smooth at $[X_0]$, of dimension $\dim(\Delta_\bm)+1$, and
the map $F_\Lambda$ is a submersion over $W$, locally around the origin
in $\Delta$.

The subvariety $W\subset \Delta$ is smooth and, by
Claim~\ref{cl:transverse}, its tangent space is not contained in $\cH$.
We may thus apply the main result of \cite{06.francesco},
to the effect that
\[
  W\cap \Delta_\bmm = \Delta_\bm \cup
  \Gamma_1 \cup \cdots \cup \Gamma_\kappa,
\]
with $\Gamma_1, \ldots, \Gamma_\kappa$ curves as in
\ref{p:restatement-prodtacnodes} above.
The upshot is thus that the local sheets of
$V^{d,\delta}(\alpha,\beta)(\Omega)$ corresponding to
the choice of $\Lambda$ are in the number
\(
\kappa
= {I^{\beta'-\beta}}
/ {\lcm (\beta'-\beta)},
\)
each a fibration over a curve $\Gamma_l$, $l=1,\ldots, \kappa$,
with the fibre
$V^{d-1,\delta'}(\alpha',\beta')(\Omega')$ over the origin.
The local sheet corresponding to the curve $\Gamma_l$ has multiplicity
\(
{\lcm(\beta'-\beta)}
/{\max(\beta'-\beta)}
\)
at the generic point of the fibre over the origin,
\ie the generic point of
$V^{d-1,\delta'}(\alpha',\beta')(\Omega')$,
and intersection multiplicity $\lcm (\beta'-\beta)$ with the inverse
image $F_\Lambda^{-1}(\Delta_\bm)$,
\ie with the hyperplane $\orth p \subset |\O_{\P^2}(d)|$ for general
$p\in L$ by Claim~\ref{cl:invimage},
along the fibre over the origin.

Finally, note that $\binom {\beta'} \beta$ is the number of possible
choices for the subsequence $\Lambda$ of the sequence of unassigned
contact points of $C$ with $L$.
\qed


\bigskip
The proof of Theorem~\ref{t:CH1.3} is now over.
We end this section with a remark about what
happens when $\beta'=\beta$.

As we have already observed, in this case the first step performed in
Subsubsection~\ref{ss:relaxed}
above is sufficient to prove Theorem~\ref{t:CH1.3}.
Indeed, if $\beta=\beta'$, then the relaxed Severi variety $W_\Lambda$
itself is the unique local sheet
of the Severi variety $V^{d,\delta}(\alpha,\beta)(\Omega)$
at $[X_0]$, we already know that it is smooth at $[X_0]$, and there is
nothing else to prove.


\begin{remark}
\label{rk:allred}
If $\beta'=\beta$, then all the irreducible components of
$V^{d,\delta}(\alpha,\beta)$ having
an irreducible component of $V^{d-1,\delta'}(\alpha',\beta')$
in their intersection with the hyperplane
$\orth p \subset |\O_{\P^2}(d)|$
parametrize reducible curves.

Indeed, the members of such a component $W$ in a neighourhood of
$[X_0] = [C\cup L]$
with $[C] \in V^{d-1,\delta'}(\alpha',\beta')$
correspond to deformations of the total
normalization $\bar X_0 \to X_0 \subset \P^2$, and
therefore they are reducible curves because $\bar X_0$ is
disconnected.
This is the same argument we have used in the proof of
Claim~\ref{cl:invimage} above.

Conversely, if $\beta'>\beta$,
and if $V$ is an irreducible component of
$V^{d-1,\delta'}(\alpha',\beta')$
that parametrizes irreducible degree $d-1$ curves,
then all the irreducible components of
$V^{d,\delta}(\alpha,\beta)$ having
$V$ in their intersection with $\orth p$ parametrize irreducible
curves.

Indeed, if $\beta'>\beta$, then there is at least one order $i$ tacnode
of 
$X_0=C\cup L$ that is deformed to $i-1$ nodes only, so that locally
around such a point the two local branches of $X_0$, corresponding
respectively to an irreducible component $C_1$ of $C$ and to $L$,
deform to only one, irreducible, local branch, and thus $C_1$ and $L$
merge into the same irreducible component of the curves $X_t$
neighbouring $X_0$.
\end{remark}



\section{The formula for irreducible curves}
\label{S:irred}

In this section we give and explain the version of Caporaso and
Harris' recursion formula enabling the counting of irreducible curves.
The formula is given in Theorem~\ref{t:CHirred}
below. The key observation to pass from the standard formula to the
formula for irreducible curves is Remark~\ref{rk:allred}
at the end of the previous section.
Let us start with an example.


\begin{example}
\label{ex:irred}
We consider the enumeration of quartics with three nodes and two assigned
simple contact points with the line $L$,
\ie curves parametrized by $V^{4,3}(2,2)(\Omega)$.
By the recursion formula,
we have
\begin{equation}
\label{ex:irred:rec}
  N^{4,3}(2,2)
  = N^{4,3}(3,1)
  + 3N^{3,1}(0,3)
  + 2N^{3,0}(1,2).
\end{equation}
The irreducible components of $V^{4,3}(2,2)(\Omega)$ parametrize
either irreducible quartics, or quartics that are the sum of a cubic
and a line. 
We let $N^{4,3}(2,2)_\irr$ and $N^{4,3}(2,2)_\cub$ be
the respective contributions to $N^{4,3}(2,2)$ of irreducible and
decomposable quartics. 
Thus,
\[
  N^{4,3}(2,2)
  = N^{4,3}(2,2)_\irr
  + N^{4,3}(2,2)_\cub.
\]
Formula \eqref{ex:irred:rec} splits accordingly into
\begin{equation}
\label{ex:irred:recdec}
\begin{aligned}
  N_\irr^{4,3}(2,2)
  &= N_\irr^{4,3}(3,1)
  + 3N_\irr^{3,1}(0,3)
  + 2N_\irr^{3,0}(1,2)
    \qquad \text{and}
  \\
  N_\cub^{4,3}(2,2)
  &= N_\cub^{4,3}(3,1)
  + 3N_\cub^{3,1}(0,3)
  + 2N_\cub^{3,0}(1,2).
\end{aligned}
\end{equation}

Note that all components of $V^{3,1}(0,3)$ and $V^{3,0}(1,2)$
parametrize irreducible cubics, hence
the distribution of $N^{3,1}(0,3)$
into  $N_\irr^{3,1}(0,3)$ and  $N_\cub^{3,1}(0,3)$
(and similarly that of $N^{3,0}(1,2)$)
depends on whether the merging of these irreducible cubics with the
line $L$ produces an irreducible or a decomposable quartic.
The upshot of Remark~\ref{rk:allred} is that
\[
  N^{3,0}(1,2)
  = N^{3,0}(1,2)_\cub
  \Et
  N^{3,1}(0,3)
  = N^{3,1}(0,3)_\irr,
\]
because $\beta'=\beta$ for the former and $\beta'>\beta$ for the
latter, in the notation of Remark~\ref{rk:allred}.
Therefore, \eqref{ex:irred:recdec} reduces to
\begin{equation*}
%\label{ex:irred:recdecred}
\begin{aligned}
  N_\irr^{4,3}(2,2)
  &= N_\irr^{4,3}(3,1)
  + 3N^{3,1}(0,3)
    \qquad \text{and}
  \\
  N_\cub^{4,3}(2,2)
  &= N_\cub^{4,3}(3,1)
  + 2N^{3,0}(1,2).
\end{aligned}
\end{equation*}

Now let us show these formulas in action.
First note that
\begin{equation*}
  N^{3,1}(0,3)=12
  \Et
  N^{3,0}(1,2)=1
\end{equation*}
(the former is the plain number of rational cubics,
while the latter is merely the number of cubics passing through 
one assigned point on $L$,
and passing through eight general crossing points in both cases).

Let us compute the contributions
$N^{4,3}(2,2)_\cub$ and
$N^{4,3}(3,1)_\cub$.
Since $V^{4,3}(2,2)$ has dimension $9$,
$N^{4,3}(2,2)_\cub$ is the number of
quartics decomposed as a cubic plus a line passing through two
assigned points $p_1,p_2$ on $L$, and 
through nine general points $a_1,\ldots,a_9$ in the plane.
There are only the two following possibilities
(recall that in the definition of Severi
varieties it is requested that its members should not contain $L$
itself): 
\begin{compactenum}[(i)]
\item the line passes through one of $p_1$ and $p_2$ and through one
  of the $a_i$'s, and the cubic passes through the remaining nine
  points among $p_1,p_2$, and $a_1,\ldots,a_9$;
\item the line passes through two of the $a_i$'s, and the cubic passes
  through $p_1,p_2$ and the seven points remaining among
  $a_1,\ldots,a_9$.
\end{compactenum}
We thus find
\[
  N^{4,3}(2,2)_\cub
  = 2\times 9 + \textstyle \binom 9 2
  = 54.
\]
Similarly, $N^{4,3}(3,1)_\cub$ counts decomposed quartics passing
through three assigned points $p_1,p_2,p_3$ on $L$
and eight general points $a_1,\ldots,a_8$ on the plane.
We have the same possibilities as
in the previous case, and thus
\[
  N^{4,3}(3,1)_\cub
  = 3\times 8 + \textstyle \binom 8 2
  = 52.
\]

We can now observe that, indeed,
\[
  N^{4,3}(2,2)_\cub = 54
  = N^{4,3}(3,1)_\cub + 2N^{3,0}(1,2) = 52+2\cdot 1.
\]
Besides, one has
$N^{4,3}(2,2)_\irr = N^{4,3}(0,4)_\irr$ because putting two crossing
points on $L$ doesn't put the crossing points in special position,
and therefore $N^{4,3}(2,2)_\irr = 620$, see
\cite[Section \tref{s:ciro-3nodal-4ics}]{01.ciro}, or
\cite[p.~349]{caporaso-harris}.
As a sanity check, note that
\[
  N^{4,3}(2,2) = 674 =
  N^{4,3}(2,2)_\irr + N^{4,3}(2,2)_\cub = 620+54
\]
(see \cite[p.~349]{caporaso-harris} for $N^{4,3}(2,2) = 674$).
On the other hand,
$N^{4,3}(3,1) = 636$ by \cite[p.~349]{caporaso-harris},
hence $N^{4,3}(3,1)_\irr = 636-52 = 584$.
We can now observe that, indeed,
\[
  N_\irr^{4,3}(2,2) = 620 
  = N_\irr^{4,3}(3,1)
  + 3N^{3,1}(0,3)
  = 584 + 3\cdot 12.
\]
\end{example}


The main point in passing from the standard formula to the formula for
irreducible curves is to reconsider Remark~\ref{rk:allred} carefully
in order to make it cover all possible cases. The upshot is the
following.

\paragraph{}
\label{p:cns-irred}
Let the notation be as in Section \ref{s:merge} above.
In particular, we assume that $V^{d-1,\delta'}(\alpha',\beta')$
appears in the intersection of $V^{d,\delta}(\alpha,\beta)$
with the hyperplane $\orth p$, and
let $V'$ be an irreducible component of
$V^{d-1,\delta'}(\alpha',\beta')$.
Let $C$ be a general member of $V'$, and assume that it decomposes
as a union of irreducible curves $C_1,\ldots,C_k$.

Then, a local sheet of
$V^{d,\delta}(\alpha,\beta)$ at the point $[C\cup L]$ parametrizes
irreducible curves if and only if
the corresponding choice of $\Lambda$ as in Paragraph
\ref{p:notation1.3} is such that,
for all $l=1,\ldots,k$, there is at least one unassigned contact
point of $C$ with $L$ on the component $C_l$ that is off $\Lambda$.

Indeed, $\Lambda$ is the subset of cardinality $\beta$ of the set of
unassigned contact points of $C$ with $L$ around which two local
branches are maintained in the deformation of $C\cup L$.
Moreover, two local branches are maintained at all assigned contact
points of $C$ with $L$.
Therefore, the contact points of $C$ with $L$ at which the two local
branches deform to a unique irreducible branch are exactly the points
$s_{i,j}^{C\cap L}$ in the notation introduced at the beginning of
Section \ref{ss:relaxed}, which deform to $i-1$ nodes only; those form
the complement of $\Lambda$ in the set of
unassigned contact points of $C$ with $L$.


\bigskip
The other ingredient of the proof of the recursive formula for
irreducible curves is the following basic enumerative theoretic
computation.


\paragraph{}
\label{p:deg-Segre}
Let $V$ be the sum of irreducible components of
$V^{d,\delta}(\alpha,\beta)$ that parametrizes all the curves that
decompose as unions of irreducible curves $C_1,\ldots,C_k$, such that
for all $l=1,\ldots,k$, the curve $C_l$ is a general member of an
irreducible component of $V^{d_l,\delta_l}(\alpha^l,\beta^l)$.
For all $l$, let
$V_l = V_\irr^{d_l,\delta_l}(\alpha^l,\beta^l)$ be the sum
of irreducible components of $V^{d_l,\delta_l}(\alpha^l,\beta^l)$ that
parametrizes all irreducible members of
$V^{d_l,\delta_l}(\alpha^l,\beta^l)$.
Then, $V$ is the image of the product
$\prod_{l=1}^k V_l$ by the Segre
map
\[
  \Sigma:\,
  \prod\nolimits_{l=1}^k |\O_{\P^2}(d_l)|
  \longrightarrow |\O_{\P^2}(d)|.
\]
The degree of $V$ is the intersection number $V\cdot H^{\dim(V)}$,
where $H$ denotes the
hyperplane class in the Chow ring of $|\O_{\P^2}(d)|$. It may be
computed by pulling-back by $\Sigma$.
One has
$\Sigma^*H = H_1+\cdots + H_k$, where $H_l$ is the hyperplane class of
$|\O_{\P^2}(d_l)|$ for all $l$,
and then
\begin{align*}
  \Bigl(
  \prod\nolimits_{l=1}^k V_l
  \Bigr)
  \cdot (\Sigma^*H)^{\dim(V)}
  &=
  \Bigl(
  \prod\nolimits_{l=1}^k V_l
  \Bigr)
    \cdot (H_1+\cdots + H_k)^{\dim(V)}
  \\
  &=   \Bigl(
  \prod\nolimits_{l=1}^k V_l
  \Bigr)
    \cdot
    \sum_{\nu_1+\cdots+\nu_k = \dim(V)}
    \binom {\dim V}{\nu_1,\ldots,\nu_k}
    H^{\nu_1}_1\cdots H_k^{\nu_k}
  \\
  &=
    \binom {\dim V}{\dim V_1,\ldots,\dim V_k}
    \prod\nolimits_{l=1}^k V_l
    \cdot H_l^{\dim(V_l)},
\end{align*}
by computing in the Chow ring of
$\prod\nolimits_{l=1}^k |\O_{\P^2}(d_l)|$,
as explained in \cite[Section~2.1.4]{3264}.

The above number equals $V\cdot H^{\dim(V)}$ if
the restriction of $\Sigma$ to $\prod_{l=1}^k V_l$
is birational, which happens if and only if the $V_l$'s
are pairwise distinct;
otherwise the restriction of $\Sigma$ has finite degree, equal to the
order of the group of permutations of the factors that leaves the
product unchanged.
The upshot is that, denoting by $\sigma$ the order of this group
(we shall in fact use a refined version of this in the recursion
formula), 
\[
  \deg(V) = \frac 1 \sigma
  \binom {\dim V}{\dim V_1,\ldots,\dim V_k}
  \prod\nolimits_{l=1}^k \deg(V_l).
\]
For the application below, recall that the dimensions of generalized
Severi varieties is given in Proposition~\ref{p:zariski}.
Now, fasten your seatbelts, the formula is the following.


\begin{theorem}
\label{t:CHirred}
For all $d,\delta, \alpha,\beta$ as in Corollary \ref{c:CHmain},
let $N_\irr^{d,\delta}(\alpha,\beta)$ be the number of irreducible
members of the generalized Severi variety
$V^{d,\delta}(\alpha,\beta)(\Omega)$ passing through
$2d+g-1+|\beta|$ general points of the plane
($g=p_a(d)-\delta$), for any general
$\Omega$.
Then,
\begin{multline*}
  N_\irr^{d,\delta}(\alpha,\beta)
  =
  \sum_{k\geq 1:\, \beta_k>0}
  k\cdot N_\irr^{d,\delta}(\alpha+e_k,\beta-e_k)
  \\+
  \sum
  \biggl[
  \frac 1 \sigma
  \binom {2d+g-1+|\beta|}
  {2d_1+g_1-1+|\beta^1|,\,\ldots,\,2d_k+g_k-1+|\beta^k|}
  \cdot \binom {\alpha}{\alpha^1,\ldots,\alpha^k,\alpha-\alpha'}
  \\\cdot
  \prod_{l=1}^k \binom{\beta^l}{\beta^l-\gamma^l}
  \cdot \prod_{l=1}^k I^{\gamma^l}
  \cdot \prod_{l=1}^k N_\irr^{d_l,\delta_l}(\alpha^l,\beta^l)
  \biggr],
\end{multline*}
where the second sum is taken over all integers $k>0$, and
over all collections of integers $d_1,\ldots,d_k$, and
$\delta_1,\ldots,\delta_k$, and all collections of sequences
$\alpha^1,\ldots,\alpha^k$, $\beta^1,\ldots,\beta^k$,
and $\gamma^1,\ldots,\gamma^k$, subject to the relations
\begin{alignat*}{2}
  &&\alpha'= \alpha^1+\cdots+\alpha^k
  &\leq \alpha
  \\
  &&\beta'= \beta^1+\cdots+\beta^k
  &= \beta + \gamma^1 + \cdots + \gamma^k
  \\
  \forall l=1,\ldots,k:&\quad&
  \gamma^l
  &\neq 0
  \\
  &&
  d_1+\cdots+d_k
  &= d-1
  \\
  &&
  \delta_1+\cdots+\delta_k
  &= \delta + |\beta'-\beta|-d+1-\sum_{h<l} d_hd_l,
\end{alignat*}
and $\sigma$ is defined as follows:
define an equivalence relation on $\{1,\ldots,k\}$ by
declaring $h \sim l$ if
\[
  d_h=d_l,\quad
  \delta_h=\delta_l,\quad
  \alpha^h=\alpha^l,\quad
  \beta^h=\beta^l,\quad
  \text{and}\quad \gamma^h=\gamma^l;
\]
then $\sigma$ is the product of the factorials of the cardinalities of the
equivalence classes.
\end{theorem}

In the recursion formula, we have used multinomials for elements of
$\Nseq$; we define them as
\[
  \binom {\alpha}{\alpha^1,\ldots,\alpha^k,\alpha^0}
  = \prod_{i\geq 1}
  \binom {\alpha_i}{\alpha_i^1,\ldots,\alpha_i^k,\alpha_i^0}.
\]
The interpretation of the first sum in the formula should be fairly
clear; let us decipher the second sum.
Each summand corresponds to the contribution of
\[
  \prod_{l=1}^k V_\irr^{d_l,\delta_l}(\alpha^l,\beta^l)
  \ \subset\ 
  V^{d_1+\cdots+d_k,\,
    \delta_1+\cdots + \delta_k + \sum_{h<l} d_hd_l}
  \bigl(\tsum_l \alpha^l, \tsum_l \beta^l\bigr)
\]
to $V_\irr^{d,\delta}(\alpha,\beta) \cap \orth p$
determined by the sequences $\gamma^1,\ldots,\gamma^k \in \Nseq$
in the following way:
for all $l=1,\ldots,k$, $\gamma^l \in \Nseq$ is
the number of unassigned contact points of the general member $C_l$ of 
$V_\irr^{d_l,\delta_l}(\alpha^l,\beta^l)$ at which an open
neighbourhood of $C_l\cup L$ deforms to only one irreducible branch;
the deformation of $C_1\cup \cdots \cup C_k \cup L$ is irreducible if
and only if there is at least one such point for all $l$
(see Paragraph \ref{p:cns-irred} above), which
corresponds to the requirement that $\gamma^l \neq 0$ for all $l$.
Note that the number of nodes of $C_1\cup \cdots \cup C_k$ is indeed
$\delta_1+\cdots + \delta_k + \sum_{h<l} d_hd_l$.

This contribution in fact means the sum of the contributions of all
$\prod_{l=1}^k V_\irr^{d_l,\delta_l}(\alpha^l,\beta^l)(\Omega^l)$,
for all sets $\Omega^1,\ldots,\Omega^k$ of cardinalities
$\alpha^1,\ldots,\alpha^k \in \Nseq$ such that
$\Omega = \bigcup_{l=1}^k\Omega^l$;
the multinomial
$\binom {\alpha}{\alpha^1,\ldots,\alpha^k,\alpha-\alpha'}$
corresponds to the number of possible  $\Omega^1,\ldots,\Omega^k$.
On the other hand, the factor $\frac 1 \sigma$ times the first
multinomial is the degree of
$\prod_{l=1}^k V_\irr^{d_l,\delta_l}(\alpha^l,\beta^l,\gamma^l)$
(see Paragraph \ref{p:deg-Segre}); note
that we have added the decoration $\gamma^l$ (with the meaning
explained above), and the ``stabilizer term'' $\sigma$ has been
changed accordingly in the theorem with respect to
Paragraph \ref{p:deg-Segre}.

We leave to the reader the excellent exercise of filling out the
details of the proof of Theorem \ref{t:CHirred}.



\begin{references}

\begin{thebibliography}[Chapters in this Volume]{XIV}

\bibitem[\tref{01.ciro}]{01.ciro}
C.~Ciliberto {\normalfont \smfandname} Th.~Dedieu,
\emph{Limits of nodal curves: generalities and examples}.

\bibitem[\tref{02.edoardo}]{02.edoardo}
Th.~Dedieu and E.~Sernesi, \emph{Deformations of curves on surfaces}.

\bibitem[\tref{03.th-acz}]{03.th-acz}
Th.~Dedieu,
{\it Geometry of logarithmic Severi varieties at a general point}.

\bibitem[\tref{05.margherita}]{05.margherita}
M. Lelli-Chiesa,
{\itshape Deformations of an $m$-tacnode into $m-1$ nodes}.

\bibitem[\tref{06.francesco}]{06.francesco}
F.~Bastianelli,
{\itshape Products of deformation spaces of tacnodes}.

\bibitem[\tref{A.swallowtail}]{A.swallowtail}
Th.~Dedieu,
{\itshape Geometry of the deformation space of an $m$-tacnode into
  $m-1$ nodes}.

\bibitem[\tref{08.th-exem}]{08.th-exem}
Th.~Dedieu,
\emph{The Caporaso–Harris recursion within a degeneration of the
  plane}.

\bibitem[\tref{13.th-classic}]{th-formulae}
Th.~Dedieu,
{\itshape Some classical formul\ae{} for curves and surfaces}.

\end{thebibliography}

\begin{thebibliography}[External References]{9}

\bibitem{caporaso-harris}
L. Caporaso, J. Harris:
{\it Counting plane curves of any genus},
Invent. Math. {\bf 131} (1998), no.2, 345--392.

\bibitem{caporaso-harris2}
L. Caporaso, J. Harris:
{\it Parameter spaces for curves on surfaces and enumeration of
  rational curves},
Compositio Math. {\bf 113} (1998), no.2, 155--208.

% \bibitem{DS}
% Th.~Dedieu and E.~Sernesi,
% {\itshape Equigeneric and equisingular families of curves on
%   surfaces},
% Publ. Mat. {\bfseries 61} (2017), 175--212.

% \bibitem {Frie} R. Friedman: 
% {\it Global smoothings of varieties with normal
% crossings}, Ann. of Math. {\bf 118} (1983), 75--114.

\bibitem{3264}
D.~Eisenbud {\normalfont \smfandname} J.~Harris, \emph{3264 and all that},
  Cambridge: Cambridge University Press, 2016.

\bibitem{harris}
J.~Harris, 
\emph{On the Severi problem},
Invent. math. {\bf 84}, 445--461 (1986).

\bibitem{hartshorne}
R.~Hartshorne, \emph{Algebraic geometry}, Springer-Verlag, New York-Heidelberg,
  1977, Graduate Texts in Mathematics, No.~52.

% \bibitem{concettina1}
% C. Galati:
% {\it Degenerating curves and surfaces: first results},
% Rend. Circ. Mat. Palermo {\bf 58} (2009), no. 2, 211--243.

% \bibitem{concettina2} C. Galati, A.L. Knutsen: {\it On the existence
%     of curves with $A_k$--singularities on $K3$ surfaces}, math
%   arXiv:1107.4568 (2011).

% \bibitem{harris-morrison}
% J. Harris, I. Morrison:
% {\it Moduli of Curves},
% number 187 in Graduate Texts in Mathematics, 
% Springer-Verlag, 1998.

\bibitem{vakil}
R.~Vakil,
\emph{Counting curves on rational surfaces},
Manuscripta Math.\ {\bf 102}, 53--84 (2000).

\bibitem{zahariuc}
A.~Zahariuc,
\emph{The irreducibility of the generalized Severi varieties},
Proc. London Math. Soc. (3) {\bf 119}, 1431--1463 (2019).

\end{thebibliography}


\end{references}


% \vskip .2cm \noindent
% \textsc{%
% Dipartimento di Matematica e Informatica, 
% Universit\`a degli Studi della Calabria,
% Via Pietro Bucci, cubo 31B,
% 87036 Arcavacata di Rende (CS), Italy} \\
% \texttt{galati@mat.unical.it}



\stopcontents[04.concettina]





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End:


==> 04b.concettina/lecture5-galati.tex <==
\chaptitle[Smoothing tacnodes and other singularities on reducible
surfaces]
{Proving the existence of curves  on smooth surfaces by
  smoothing tacnodes and other singularities on reducible surfaces} 
\chapauthor{Concettina Galati}

\startchap
\label{04b.concettina}


\renewcommand{\p}{\mathrm p}
\let\mathtbb\mathbb
\let\mathbb\mathbf
\newcommand{\ES}{\mathcal{E \kern -.1em S}}
\newcommand{\Singzo}{\mathrm{Sing}^\circ}% fu \mathfrak{Sing}

\begin{abstract} 
Let $\mathcal X\to\mathbb D$ be any flat projective family of complex surfaces parametrized by the disc $\mathbb D$, with smooth total space $\mathcal X$,
smooth general fiber $\mathcal X_t$, and reducible special fiber $\mathcal X_0=\cup X_i$ with normal crossing singularities. Let $C=\cup_i C_i\subset\mathcal X_0$
be a reducible Cartier divisor with only nodes on the smooth locus of $\mathcal X_0$ and tacnodes and nodes on the singular locus $E$ of $\mathcal X_0$. We will 
show how to study deformations of $C$ to nodal curves $C_t\subset\mathcal X_t$ by using Caporaso and Harris' local analysis of the versal deformation space
of an $m$-tacnode in \cite{caporaso-harris} and \cite{caporaso-harris2}. Results of this paper are known. We especially refer to \cite{chen} and \cite{concettina-andreas}. But they are usually proved in literature with some special assumptions on the surfaces $\mathcal X_t$. Here we work in full generality. This paper is in particular a generalization of \cite[Section 3]{concettina-andreas}.
\end{abstract}



\startcontents[04b.concettina]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[04b.concettina]{}{1}[2]{}



\section{Introduction}\label{s:concettina3}

Let $X$ be a smooth complex projective surface and let $D$ be a smooth Cartier divisor of genus $p_a(D)$. Describing the 
 singular elements in the linear system $|D|$ defined by $D$ is not in
 general an easy problem, even if we restrict our interest to the 
 existence of nodal divisors.
There are various deformation arguments which may be helpful case by case. For example, if $X=\mathbb P^2$, we know that,
for any $d\geq 3$, there exist degree $d$ irreducible nodal curves of any genus $0\leq g\leq \frac{(d-1)(d-2)}{2}$, \cf \cite{severi} and \cite{harris}. These 
curves are deformations of a rational nodal plane curve of degree $d$, obtained as a general projection of a rational normal curve 
$C_d\subset\mathbb P^d$ of degree $d$. Notice that $ \frac{(d-1)(d-2)}{2}$ is the number of nodes of a rational nodal plane curve 
and so it  is the maximal number of nodes of an irreducible plane
curve of degree $d$. If $X$ is any smooth complex projective surface
and $D$ is any smooth Cartier divisor, it is not in general obvious how to produce irreducible or even reducible curves $|D|$ with ``the maximum allowed
number of nodes''. One very classical strategy is to degenerate the surface $X\simeq\mathcal X_t$ to a reducible normal crossing surface
$\mathcal X_0$ and to prove the existence of divisors on $X=\mathcal X_t$ with certain singularities as deformations of suitable 
Cartier divisors on $\mathcal X_0$. 
%This kind of degeneration has been applied to the study of Severi variety of nodal curves on a smooth surface
%first in \cite{ran}. 
This method was used in particular by Chen in \cite{chen} to prove the existence of
irreducible rational nodal curves on a very general K3 surface, in the
primitive linear system and in all its multiples. The key idea of
Chen's theorem is to construct, on a suitable reducible K3 surface
$\mathcal X_0=A\cup B$, a curve with tacnodes at points of the
singular locus of $\mathcal X_0$ and to study its deformations on a
very general K3 surface $\mathcal X_t$, by using the analysis of the
locus of $(m-1)$-nodal curves in the versal deformation space of the
$m$-tacnode, carried out in \cite{caporaso-harris} and
\cite{caporaso-harris2},
see \cite{05.margherita}.
The local analysis in \cite{caporaso-harris} and \cite{caporaso-harris2} of versal deformations of tacnodes has later been extended in \cite{concettina-andreas}, where the authors provide a method to construct curves with $A_k$ singularities on smooth surfaces, for every $k\geq 1$. In particular \cite{concettina-andreas} contains a new proof of the aforementioned  Chen's theorem. Results in \cite{concettina-andreas} have later been applied in 
\cite{cdgk} and \cite{cdgk1}. 

In \cite{concettina-andreas} the authors work
in a family of regular surfaces. An output of the present paper is that this
regularity assumption is unnecessary. Here we provide a generalization of
\cite[Section 3]{concettina-andreas} using a simpler notation. We hope it will be clear to the reader how all results of this paper can be generalized
to the study of deformations of reduced curves in a smooth total space with complete intersection singularities, see for example \cite{concettina2}.

This paper is divided in four sections. In Section 2
we describe our degeneration argument and we state our deformation problem (Problem \ref{main-problem}). We moreover collect
several local results  from which, in Section 3, we will deduce our main result, Theorem \ref{independent-smoothing-forte}.
The latter proves in particular
\cite[Proposition \tref{p:zrr}]{01.ciro}; besides, \cite{01.ciro}
contains
many applications of Theorem \ref{independent-smoothing-forte}.

The degeneration argument which we are going to explain in the next section is useful to the study of many problems. For example, in
 \cite{cfgk}, it has been applied to the study of the number of moduli of Severi varieties of nodal curves on K3 surfaces.
Here we will restrict to the existence problem of nodal curves on smooth surfaces. 

\paragraph{Terminology and notation}
We will work over $\mathbb C$. A curve will be a reduced separated scheme of finite type 
and dimension $1$.

\paragraph{Acknowledgments} I would like to thank Thomas Dedieu for reading the preliminar version of this paper.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%It is easy to see that the singularity \eqref{tacnode} at a moving point $p\in E_{i,j}$
 %imposes at most $m-1$ conditions to the linear system $|\mathcal O_{\mathcal X_0}(C)|$, corresponding  to the expected number of conditions
 %imposed by a moving tangency of $C_i$ to $E_{ij}$. One then could expect that a curve $C$ with the  singularity \eqref{tacnode} at a double
 %point $p\in E$ is in the closure of a  universal Severi variety of $(m-1)$-nodal curves. Namely, we expect that a curve $C$ on $\mathcal X_0$
 %with the  singularity \eqref{tacnode} is limit of an $(m-1)$-nodal curve on $\mathcal X_t$ and we also expect to be able to describe all intermediate
 %deformations. 
 



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%



 \section{Our deformation problem}\label{sec: deformation problem}



\paragraph{}
\label{p:setup}
Let $\mathcal X\to\mathbb D$ be a flat projective family of complex surfaces parametrized by the disc $\mathbb D$, with smooth total space $\mathcal X$,
smooth general fiber $\mathcal X_t$, and reducible special fiber
$\mathcal X_0$ with normal crossing singularities, i.e., locally at
every point in the analytic topology, $\mathcal X_0$ is isomorphic to
the closed subset of an open polydisk of $\mathbb C^3$ defined by
$\{(x_1,x_2,x_3)|\Pi_{i=1}^{k}x_{i}=0\}$, where $k$ may be $1,2$, or $3$, \cf \cite{friedman}. Thus every irreducible component $X_i$ of $\mathcal X_0=\cup_{i=1}^r X_i$ is smooth, and the singular locus of $\mathcal X_0$ consists of the intersection locus of its irreducible components, where $\mathcal X_0$ has singularities of multiplicity $2$ or $3$. We denote by $E=\cup_{1\leq i<j\leq r}E_{ij}$ the singular locus of $\mathcal X_0$, where $E_{ij}= X_i\cap X_j$ (possibly empty),  and by $E^o\subseteq E\subset \mathcal X_0$ the set of points of multiplicity exactly $2$.

Let $p\in E^o$ be a double point of $\mathcal X_0$. Working locally at $p$, we may assume that $\mathcal X$ is isomorphic to a closed 
 subset of an open polydisk of $\mathbb C^3\times \mathbb D$, with coordinates $(x,y,z,t)$, in such a way the local analytic equation of $\mathcal X$ at $p$ is given by 
 $$
 xy=t,
 $$ 
 and $xy=t=0$ are the analytic equations of $\mathcal X_0$ at $p.$ 
 
 Now we consider a reduced Cartier divisor 
 $$
 C=\cup_i C_i\subset \mathcal X_0=\cup_{i=1}^r X_i,
 $$
where every $C_i=C\cap X_i\subset X_i$ is a reduced $\delta_i$-nodal curve, that is smooth at every intersection point with $E$ and does not contain any triple point of $\mathcal X_0$. The local equations of $C$ at every intersection point $p\in E_{ij}\cap C=C_i\cap  C_j$  are
\begin{eqnarray}\label{tacnode}
\left\{\begin{array}{l}
y+x-z^m=0\\
xy=t \\
t=0,\\
\end{array}\right.
\end{eqnarray}
for some $m\geq 1$ (depending on $p$).
Thus the singularity of $C$ at $p\in C\cap E_{ij}$ is analytically isomorphic to the planar curve singularity of local equation
\begin{equation}\label{m-tacnode}
f(y,z)=(y-z^{m})y=0,
\end{equation}
which is called a {\it tacnode of order} $m$ or an  $m$-{\it tacnode};
observe that a $1$-tacnode is a node.

Thus the curve 
 $$
 C=\cup_i C_i\subset \mathcal X_0=\cup_{i=1}^r X_i,
 $$
has only planar singularities that are nodes and tacnodes.



\begin{problem}\label{main-problem}
We want to find sufficient conditions for $C\subset\mathcal X_0$ to be deformed to a nodal curve
$C_t\subset\mathcal X_t$. More precisely we want to understand which is the maximal number of nodes of a curve 
$C_t\subset\mathcal X_t$ that is deformation of $C\subset\mathcal X_0$.

\end{problem}


 \begin{remark}\label{rm: naive expectation}
  Every tacnode of $C$ at a moving point $p\in E_{ij}=X_i\cap X_j\subset E$ imposes at most $m-1$ independent conditions to the linear system 
  $|\mathcal O_{\mathcal X_0}(C)|$, being $m-1$ the expected number of conditions imposed to the linear
system $|\mathcal O_{ X_i}(C)|$ by a tangency of order $m$ with $E_{ij}\subset E$ at an unprescribed point.
  Thus the naive expectation is that one may deform $C$ to a curve $C_t\subset\mathcal X_t$ in such a way every $m$-tacnode of $C$ on $E$
 deforms to $m-1$ nodes of $C_t$ and all nodes of $C$ on $\mathcal X_0\setminus E$ are preserved. In this case we will say that {\it an $m$-tacnode
 of $C$ is smoothed to $m-1$ nodes of $C_t$} because $m-1$ nodes
impose one less condition to the arithmetic genus than an $m$-tacnode.
\end{remark}

 \begin{remark}\label{rm: A-k}
Let us recall that an $m$-tacnode is an $A_{2m-1}$ planar curve singularity. An $A_k$ planar curve singularity has analytic equation 
 $y^2-x^{k+1}.$ Every plane curve singularity of multiplicity $2$ is an $A_k$-singularity, for some $k$ and two plane curve singularities of multiplicity 
 two are topologically equivalent if and only if they are analytically equivalent. We refer to \cite{diaz-harris} and  \cite{02.edoardo}
  for the notion of equisingularity from the topological and the analytic point of view for a family of reduced curves on a smooth surface. In particular, for an
 $A_k$-singularity the equisingular ideal coincides with the Jacobian
 ideal, given by $I=J=(y, x^k)$ \cite[Proposition 5.6]{diaz-harris}.
 This implies that an $A_k$-singularity at a moving point of a smooth
 surface imposes as most $k=\dim(\mathbb C[x,y]/J)$ independent
 conditions to a linear system. Now, an $A_k$-singularity locally deforms to an $A_{k'}$-singularity for every  $k'\leq k$.   Thus, in the same vein as in Problem~\ref{main-problem}, one could ask about deformations 
 $C_t\subset\mathcal X_t$ of $C\subset\mathcal X_0$ with $A_k$-singularities. As in Remark \ref{rm: naive expectation}, one expects that the curve singularity \eqref{tacnode} deforms on $\mathcal X_t$ to $d_i$ singularity of type $A_i$, for every multi-index $(d_1,...,d_r)$ such that $\sum_{i}id_i=m-1.$ 
\end{remark}


 Deformations of $C$ in $\mathcal X$ are parametrized by suitable subschemes of the relative Hilbert scheme 
 $\mathcal H^{\mathcal X|\mathbb D}$ of $\mathcal X\to\mathbb D$ \cite{ser}. We denote by $\mathcal H\subset \mathcal H^{\mathcal X|\mathbb D}$ the union of irreducible components
 containing the point $[C]$ corresponding to the curve $C$, and by  $\mathcal H_t$ the fibre of $\mathcal H$ over $t\in \mathbb D$. We say that {\it a Cartier divisor
$C_t\subset\mathcal X_t$ is a deformation of $C\subset\mathcal X_0$ if
the point $[C_t]\in\mathcal H_t$ belongs to a curve
$\gamma\subset\mathcal H$, which is a multi-section of order $r\geq 1$ of $\mathcal H\to\mathbb D$, totally ramified at the point $[C]$, \ie intersecting $\mathcal H_0$ at $r[C]$.}



\subsection{Some local geometry: the versal deformation space of the
  singularities of $C$}
\label{sec: versal geometry}
Every deformations of $C$ in $\mathcal X$ induces a deformation of each singularity of $C$. Isolated singularities, \ie germs of isolated singularities in the analytic topology, have a
moduli space with the property of versality,  \cf \cite[Section 3]{diaz-harris}, \cite[Chapter 2]{ser}, \cite[Chapter 2]{gls} and \cite{02.edoardo}.

For a plane curve singularity $(D,q)$, a versal deformation family is
given by 
\begin{equation}\label{versalfamily}
\xymatrix{
\mathcal C_p=\{g(x,y)+t_1g_1(x,y)+...+t_mg_m(x,y)=0\}  \ar@{^{(}->}[r]  \ar[dr] & \mathbb A^2\times \Delta_{D,q}\ar[d] \\
 &   \Delta_{D,q}={\rm{Spec}}(\mathbb C[t_1,...,t_m])
 }
\end{equation}
where, denoting by  $J_p=(g, \frac{\partial g}{\partial y}, \frac{\partial g}{\partial z})$
the Jacobian ideal of the local equation $g(y,z)$ of $D$ at $p$, the polynomials $g_1(x,y),...,g_m(x,y)$ are such that their images in $\mathbb C(y,z)/J_q$
form a basis of $\mathbb C(y,z)/J_q$, as a $\mathbb C$-vector space. The parameter space
$$
\Delta_{D,q}={\rm{Spec}}(\mathbb C[t_1,...,t_m]),
$$
is a (mini)-versal deformation space of $(D,q)$.  Using the terminology of \cite{diaz-harris}, we will refer to \eqref{versalfamily} as {\it the} \'etale versal deformation family
of the plane curve singularity $(D,q)$, and to $\Delta_{D,q}$ as {\it the} \'etale (mini)-versal deformation space of $(D,q)$.


We now provide an explicit description of the \'etale versal deformation family of every singularity of our curve $C\subset\mathcal X$. At every node $p\in \mathcal X_0\setminus E$, the curve $C$ is analytically equivalent to the plane curve $f(y,z)=yz=0$, thus
 $$
  \mathbb C[y,z]/J_p\simeq  \mathbb C[y,z]/(y,z)\simeq\mathbb C,$$ 
and a versal family for $(C,p)$ is $\mathcal C_p\to
\Delta_{(C,p)}=\rm{Spec}(\mathbb C[t])$, with
$$
\mathcal C_p
= \bigl\{xy+t=0 \bigr\}
\subset \mathbb A^2\times\rm{Spec}(\mathbb C[t]).
$$
The only singular fibre is that over $t=0$, implying that a
deformation of a nodal curve is either a nodal curve or a smooth curve.  
  
At every tacnodal singularity $p\in E_{ij}$, a local equation $f$ of $C$ at $p$ is given by \eqref{m-tacnode}, so that $J_f=(2y-z^m,mz^{m-1}y)$
and
 $$
 \mathbb C[y,z]/J_f\simeq\mathbb C^{2m-1}.
 $$
In particular, at every tacnodal singularity $p\in E_{ij}$ of $C$, choosing 
$$
\{1,\,z,\,z^2,\,\dots,\,z^{m-1},\,y,\,yz,\,yz^2,\,\dots,\,yz^{m-2}\}$$
as a basis for $ \mathbb C[y,z]/J_f$,
a versal deformation family of $(C,p)$ is given by $\mathcal C_p\to \Delta_{(C,p)}$, where 
$$
\Delta_{(C,p)}={\rm{Spec}}(\mathbb C[\alpha_0,...,\alpha_{m-2},\beta_0,...,\beta_{m-1}])
$$
 and $\mathcal C_p\subset \mathbb A^2\times\Delta_{(C,p)}$ has equation
\begin{equation}\label{versal-family-m-tacnode}
\mathcal C_p: F(y,z;\underline\alpha,\underline\beta)=
y^2+\Big(\sum_{i=0}^{m-2}\alpha_iz^i+z^m\Big)y+\sum_{i=0}^{m-1}\beta_iz^i=0,
\end{equation}
where we are using the same notation as in \cite{caporaso-harris} and
\cite{diaz-harris}, see \cite{05.margherita, 06.francesco}.

We now want to introduce the versal property of the versal family  $\mathcal C_p\to\Delta_{(C,p)}$. Keeping in mind \cite[Appendix B]{hartshorne},
 we will do this in the analytic topology instead 
of the \'etale topology as in \cite[Section 3]{diaz-harris}, to simplify notation.


Let us denote by $\mathcal D\to\mathcal H$ the universal family parametrized by the Hilbert scheme $\mathcal H$.
By versality, for every singular point $p$ of $C$, there exist analytic neighborhoods
$U_p$ of $[C]$ in $\mathcal H,$ $U_p^\prime$ of $p$ in $\mathcal D$, and  $V_p$ of $\underline 0$ in $\Delta_{(C,p)}$,
and a map $\phi_p:U_p\to V_p$,
such that the family
$\mathcal D|_{U_p}\cap U_p^\prime$ is isomorphic to the pull-back of
$\mathcal C_p|_{V_p}$ by the map $\phi_p$,
making the following diagram \begin{equation}\label{versal diagram}
\xymatrix{
\mathcal C_p  \ar[d] & \mathcal C_p |_{V_p} \ar[d]  \ar@{_{(}->}[l] & 
U_p\times_{V_p}\mathcal C_p |_{V_p}  \ar[l] \ar[r]^{\hspace{0.5cm}\simeq} \ar[dr] & \mathcal D|_{U_p}\cap U_p^\prime
\ar@{^{(}->}[r]  \ar[d] & \mathcal D  \ar[d] \\
T^1_{C,p} &  V_p \ar@{_{(}->}[l]  & & \ar[ll]_{\phi_p} U_p \ar@{^{(}->}[r]  & \mathcal H}
\end{equation}
commutative. Thus, answering Problem \ref{main-problem} is the same as describing the image of the versal map
\begin{equation}\label{eq: versal map}
  \phi=\prod_{p\in {\rm {Sing}}(C)}\phi_p:
  {\bigcap_{p\in {\rm Sing}(C)} U_p}
  \ \to\  \prod_{p\in {\rm Sing}(C)}\Delta_{(C,p)},
\end{equation}
where ${\rm Sing}(C)$ is the singular locus of $C$. 
 
  
\subsection{Equisingular deformations of $C$}\label{sec: equisingular def}
In order to understand the image of the versal map $\phi$
of \eqref{eq: versal map},
we describe its differential $d\phi_{[C]}$ at the point $[C]\in \bigcap_p U_p\subset\mathcal H,$
which splits in the direct sum $d\phi_{[C]}=\bigoplus_{p\in  {\rm Sing}(C)}d\phi_{p,[C]}$, where $d\phi_{p,[C]}$ is the differential of $\phi_p$ at the point $[C]$.
 
The differential map $d\phi_{[C]}$ can be identified with the map
\begin{equation}\label{eq: differential versal map}
  H^0(\beta)=d\phi_{[C]}=\bigoplus_{p\in {\rm
      Sing}(C)}d\phi_{p,[C]}:H^0(C, \mathcal N_{C|\mathcal X})\ \to\  H^0(C,T^1_C)=\bigoplus_{p\in \textrm{Sing}(C)}T_{C,p}^1 
\end{equation}
induced by the exact sequence
\begin{equation}\label{sequenceone}
  \xymatrix{
0  \ar[r] & \Theta_C\ar[r] & \Theta_{\mathcal X}|_C\ar[r] ^\alpha
& \mathcal N_{C|\mathcal X}\ar[r]^\beta & T^1_C\ar[r] & 0,}
\end{equation}
where  $\Theta_C$ and $ \Theta_{\mathcal X}$ are the tangent sheaves of $C$ and $\mathcal X$, respectively, $\mathcal N_{C|\mathcal X}$ is the normal bundle of $C$ in $\mathcal X$, and $T^1_C$ is the first cotangent sheaf of $C$, \cf \cite[Prop.~1.1.9]{ser}. 
We are in particular using standard identifications of the tangent space $T_{[C]}\mathcal H$ at $[C]$ with $H^0(C, \mathcal N_{C|\mathcal X} )$
and of $T_0\Delta_{(C,p)}$ with $T^1_{C,p}$.
 
The kernel of the sheaf map  $\beta$ in \eqref{sequenceone}
is usually denoted by $\mathcal N^\prime_{C|\mathcal X}$, and is called the {\it equisingular normal sheaf of $C$ in $\mathcal X$}.
This terminology is due to the fact that the origin $\underline 0\in\Delta_{(C,p)}$ is the only point in the mini-versal deformation space  corresponding to 
a singularity analytically equivalent to $(C,p)$. Thus, by the short exact sequence
\begin{equation}\label{sequencetwo}
 \xymatrix{
   0  \ar[r] &\mathcal N'_{C|\mathcal X}\ar[r]
   & \mathcal N_{C|\mathcal X}\ar[r]^\beta & T^1_C\ar[r] & 0,}
\end{equation}
we have that $H^0(C,\mathcal N'_{C|\mathcal X})$ can be identified with the kernel of the differential $d\phi_{[C]}$  in \eqref{eq: differential versal map},
and it parametrizes the tangent space to the analytically equisingular deformation locus of $C$ in $\mathcal X$. One says that 
$H^0(C,\mathcal N'_{C|\mathcal X})$ parametrizes first order infinitesimal deformations of $C$ preserving all singularities of $C$
from the analytic point of view. Similarly, the kernel 
$$\ker(d\phi_{p,[C]})$$
of the differential $d\phi_{p,[C]}:H^0(C,\mathcal N_{C|\mathcal X})\to T^1_{C,p}$ in \eqref{eq: differential versal map}
parametrizes first order infinitesimal deformations of $C$ in $\mathcal X$ which are analytically equisingular at $p$, and 
there is an obvious inclusion $H^0(C,\mathcal N'_{C|\mathcal X})\subset\ker(d\phi_{p,[C]})$.

\begin{definition}\label{def: es}
We denote by
$$\ES(C)=\phi^{-1}(\underline 0,...,\underline 0)$$
the (scheme theoretic) inverse image 
of the origin with respect to the versal map $\phi$ in \eqref {eq:
versal map}. We will call it the \emph{equisingular
deformation locus  of} $C$.
\end{definition}

\begin{remark}
As already observed, the inverse image $\phi^{-1}(\underline 0,...,\underline 0)$ of $(\underline 0,...,\underline 0)$ by the versal map \eqref{eq: versal map}
is, in general, the locus of analytically equisingular deformations of $C$ in $\mathcal X$. Since we assume $C$ with only nodes and tacnodes, analytically equisingular deformations of $C$ in $\mathcal X$ coincide with topologically equisingular deformations of $C$ in $\mathcal X$, cf. Remark \ref{rm: A-k}. For this reason we call
$\ES(C)=\phi^{-1}(\underline 0,...,\underline 0)$ the equisingular deformation locus  of $C$, with no further specification. Similarly, we refer to its tangent space $H^0(C,\mathcal N'_{C|\mathcal X})\simeq T_{[C]}(\ES(C))$ at $[C]$ just as the space of equisingular first order infinitesimal deformations of $C$ in $\mathcal X$.
\end{remark}

\begin{remark}\label{rm: complete intersection}
The versal map $\phi$ in \eqref {eq: versal map}, as well as the description  of its differential $d\phi_{[C]}$
in \eqref{eq: differential versal map},
and the exact sequences \eqref{sequenceone} and \eqref{sequencetwo},
are defined  for {\rm any} reduced Cartier divisor $C$ on $\mathcal X_0$,
whose singularities $(C,p)$ are all reduced complete intersection singularities in $\mathbb C^3$.
Moreover, the 
description of the \'etale versal deformation family of $(C,p)$ provided in \eqref{versalfamily} under the assumption that $(C,p)$ is a planar curve
singularity,
extends to complete intersection curve
singularities in $\mathbb C^n$ (see \cite{gls}, or \cite[Section 3]{concettina2} for an example of explicit computation when $(C,p)$ is a complete
intersection curve singularity in $\mathbb C^3$).
\end{remark}



\begin{lemma}\label{lemma-ker}
Let $\mathcal X\to\mathbb D$ be a flat projective family of complex
surfaces as in \ref{p:setup}. 
\begin{description} 
\item{(a)}
  For {\rm any} reduced Cartier divisor  $C\subset\mathcal X_0$ with
  non-empty intersection with $E$, one has
\begin{equation}\label{kerneldifferenziale1}
H^0(C,\mathcal N^\prime_{C|\mathcal X})=H^0(C,\mathcal N^\prime_{C|\mathcal X_0})\subseteq H^0(C,\mathcal N_{C|\mathcal X_0}).
\end{equation}
More generally, for every intersection point $p\in C\cap E$, the kernel 
of the differential $d\phi_{p,[C]}:H^0(C,\mathcal N_{C|\mathcal X})\to T^1_{C,p}$ in \eqref{eq: differential versal map} is such that
\begin{equation}\label{kerneldifferenziale10}
H^0(C,\mathcal N^\prime_{C|\mathcal X})=H^0(C,\mathcal N^\prime_{C|\mathcal X_0})\subseteq  \ker(d\phi_{p,[C]})\subseteq H^0(C,\mathcal N_{C|\mathcal X_0}).
\end{equation}
\item{(b)} If $C\subset\mathcal X_0$ is a reduced Cartier divisor as above with only $\delta=\sum_i\delta_i$ nodes on $\mathcal X_0\setminus E$ and tacnodes on $E$,
then
$H^0(C,\mathcal N^\prime_{C|\mathcal X})=H^0(C,\mathcal N^\prime_{C|\mathcal X_0})$
is contained  the linear subspace of
sections of $H^0(C,\mathcal N_{C|\mathcal X_0})$ vanishing at every node $p$ of $C$ on $\mathcal X_0\setminus E$ and
vanishing at every $m$-tacnode $p\in E$ of $C$ with multiplicity $m-1$.
\end{description} 
% In particular, if $\delta=\sum_{i}\delta_i$ is the number of nodes of $C$
% on $\mathcal X_0$, then 
%$$
%h^0(C,\mathcal N^\prime_{C|\mathcal X})\geq h^0(C,\mathcal N_{C|\mathcal X})-\delta-\sum_m\sum_{m-{\rm tacnodes\,} p\,\rm{of}\,C\,\rm{on}\, E}(m-1).
%$$
\end{lemma} 

\begin{proof}
We first prove part (a) of the lemma and, in particular, equality \eqref{kerneldifferenziale1} for any reduced Cartier divisor $C$ on $\mathcal X_0$ with non-empty intersection with the singular locus $E$ of $\mathcal X_0$.
Fix any intersection point $p\in E\cap C$. Keeping in mind Remark \ref{rm: complete intersection}, we want to write equisingular infinitesimal first order deformations of $C$ in $\mathcal X$ locally at the point $p$. 
We consider the localized exact sequence
\begin{equation}\label{localizationsequenceone}
\xymatrix{
0\ar[r] & \mathcal N^\prime_{C|\mathcal X,\,p}\ar[r] &
\mathcal N_{C|\mathcal X,\,p}\ar[r] &  T^1_{C,p}\ar[r] & 0.}
\end{equation} 
Fix local analytic coordinates $x,\,y,\,z,\,t$ at $p$ in such a way that $C$ has equations 
$$
t=0,\quad f_1(x,y,z)=0, \quad \text{and}\quad f_2(x,y,z)=xy=0
$$ 
at $p$. Then we may identify:
\begin{itemize}
\item the local ring $\mathcal O_{C,\,p}=\mathcal O_{\mathcal X,p}/\mathcal I_{C|\mathcal X,p}$ of $C$ at $p$ 
with the localization at the origin of $\mathbb C[x,y,z]/(f_1,f_2)$,
\item the $\mathcal O_{C,p}$-module $\mathcal N_{C|\mathcal X,\,p}$ with the free $\mathcal O_{\mathcal X,\,p}$-module 
$\mathfrak{hom}_{\mathcal O_{\mathcal X,\,p}}(\mathcal
I_{C|\mathcal X ,\,p}, \mathcal O_{C,p})$
generated by the
morphisms $f_1^*$ and $f_2^*$,  defined by 
$$f_i^*\bigl(s_1(x,y,z)f_1(x,y,z)+s_2(x,y,z)f_2(x,y,z)\bigr)=s_i(x,y,z),
\quad\mbox{for}\ i=1,\,2,$$
\end{itemize}
and, finally,
\begin{itemize}
\item the $\mathcal O_{C,p}$-module
\begin{eqnarray*}
(\Theta_{\mathcal X}|_C)_{\, p}&\simeq &\Theta_{\mathcal X,p}/(I_{C,p}\otimes\Theta_{\mathcal X,p})\\
& \simeq & \bigl\langle \partial /{\partial x},\,\partial /{\partial y},\,\partial / {\partial z},\,\partial /{\partial t} \bigr\rangle
_{\mathcal O_{C,\,p}} \Big/
\bigl\langle {\partial}/{\partial t}-x\partial /{\partial y}-y\partial /{\partial x}\bigr\rangle
\end{eqnarray*}
with the free $\mathcal O_{\mathcal X,\,p}$-module generated by the derivatives 
$\partial /{\partial x},\partial / {\partial y},\partial /{\partial z}.$ 
\end{itemize}
With these identifications, 
the localization $\alpha_p:(\Theta_{\mathcal X}|_C)_{\, p}\rightarrow \mathcal N_{C|\mathcal X,\,p}$ of the sheaf map $\alpha$ from \eqref{sequenceone} is defined by
\begin{eqnarray*}
\alpha_p(\partial /{\partial x})&=&\,\,\,\,\,\,\Big(s=s_1f_1+s_2f_2\longmapsto
\partial s/\partial x=_{\mathcal O_{C,p}}
s_1\partial f_1 /{\partial x}
+s_2\partial f_2 /{\partial x}\Big)\\
&=&\,\,\,\,\,\, \partial f_1 /{\partial x}f_1^*+yf_2^*,\\
\alpha_p(\partial /{\partial y})&=&\,\,\,\,\,\,\partial f_1 /{\partial y}f^*_1+xf^*_2,\,\,\,\textrm{and}\\
\alpha_p(\partial /{\partial z})&=&\,\,\,\,\,\,\partial f_1 /{\partial z}f^*_1.
\end{eqnarray*}
By definition of $\mathcal N^\prime_{C|\mathcal X}$, a germ $s\in \mathcal N_{C|\mathcal X,\,p}$ 
is equisingular at $p$, \ie $s\in \mathcal N^\prime_{C|\mathcal X,\,p}$, if and only if there exists a germ
$$u=u_x(x,y,z)\partial /{\partial x}+u_y(x,y,z)\partial /{\partial y}+u_z(x,y,z)\partial /{\partial z}\in {(\Theta_{\mathcal X}|_C)}_{p}$$
such that $s=\alpha_p(u)$. Hence, locally at $p$, an  equisingular  first order infinitesimal deformation of $C$ in $\mathcal X$ has equation 
\begin{eqnarray}\label{equisingulardeformationtacnode0}
\left\{\begin{array}{l}
f_1(x,y,z)+\epsilon (u_x\partial f_1 /{\partial x}+u_y\partial f_1 /{\partial z}+u_z\partial f_1 /{\partial z})=0\\
xy+\epsilon (yu_x+xu_y)=0.
\end{array}\right.
\end{eqnarray}
%The first is the local equation of an infinitesimal deformation of  $D$ in $\mathcal X_0$, while the second is the local equation  
% of an infinitesimal 
% deformation of $\mathcal X_0$ in $\mathcal X.$ 
We claim that  the second equation of \eqref{equisingulardeformationtacnode0}
is the local equation at $p$ of an equisingular deformation 
of  $\mathcal X_0$ in $\mathcal X$. Indeed, by the exact sequence

\begin{equation*}\label{eq:standard-sequence-central}
\xymatrix{ 0  \ar[r] &      \Theta_{\mathcal X_0}  \ar[r] &      \Theta_{\mathcal X}|_{\mathcal X_0} \ar[r] & 
\mathcal N_{\mathcal X_0|\mathcal X} \cong\mathcal O_{\mathcal X_0}\ar[r] &   T^1_{\mathcal X_0}\cong\mathcal O_E  \ar[r] &     0, }
\end{equation*} 
one finds that  $\mathcal N'_{\mathcal X_0|\mathcal X}\simeq \mathcal I_{E|\mathcal X_0}.$ 

Now if $s=\alpha_p(u)$ is the localization of a global section
of $\mathcal N'_{C|\mathcal X}$, by the equality 
$H^0(\mathcal X_0, \mathcal N'_{\mathcal X_0|\mathcal X})=H^0(\mathcal X_0, \mathcal I_{E|\mathcal X_0})=0,$ we find that the analytic function
$$yu_x(x,y,z)+xu_y(x,y,z)$$ must be identically zero in the second equation of  
\eqref{equisingulardeformationtacnode0}. This  proves inclusion \eqref{kerneldifferenziale1} and \eqref{kerneldifferenziale10}. 

We now prove part (b) of the lemma. Assume that $C$ is a Cartier
divisor with only $\delta=\sum_i\delta_i$ nodes on $\mathcal
X_0\setminus E$ and tacnodes on $E$, as in \ref{p:setup},
and consider $p\in E\cap C$. In this case we may assume
$$
f_1(x,y,z)=x+y+z^m
$$
so that the equations in \eqref{equisingulardeformationtacnode0} become
\begin{eqnarray}\label{equisingulardeformationtacnode}
\left\{\begin{array}{l}
x+y+z^m+\epsilon (u_x+u_y+mz^mu_z)=0\\
xy+\epsilon (yu_x+xu_y)=0.
\end{array}\right.
\end{eqnarray}
If these equations are the equations of the localization of a global section in $H^0(C,\mathcal N_{C|\mathcal X})$, then, as above,
we find that $yu_x+xu_y$ is identically zero. We deduce in particular that
\begin{itemize} 
\item $u_x(0,0,0)=u_y(0,0,0)=0$, and
\item for every $n\geq 1$, no $z^n$-terms appear in $u_x(x,y,z)$ and $u_y(x,y,z),$ 
no $y^n$-terms and $y^nz^m$-terms appear in $u_x(x,y,z)$ and, 
finally, no $x^n$-terms and $x^nz^m$-terms appear in $u_y(x,y,z).$
\end{itemize}
In particular, if $X_i$, with local equations $x=t=0$, and $X_j$, with local equations $y=t=0$, are the two irreducible components of $\mathcal{X}_0$
containing $p$, then the
local equations at $p$ on $X_i$ of equisingular infinitesimal deformations of $C$ are given by
\begin{eqnarray}\label{equisingulardeformationtacnodeonA}
\left\{\begin{array}{l}
y+z^m+\epsilon (m z^{m-1}u_z(x,y,z)+y q(y,z))=0\\
x=0,
\end{array}\right.
\end{eqnarray}
where $q(y,z)$ is an analytic function in the variables $y$ and $z,$ and similarly on $X_j$. This proves that 
all sections in $H^0(C,\mathcal N'_{C|\mathcal X})$ vanish with multiplicity $m-1$ at every $m$-tacnode of $C$ on $E$.

The fact that all sections of $H^0(C,\mathcal N'_{C|\mathcal X_0})$ vanish at every node $p$ of $C$ on $\mathcal X_0\setminus E$ 
is a very classical result, which can be proved here with the same approach as above, by using that at a node on $\mathcal X_0\setminus E$
the local equations of $C$ are $x-t=t=0=yz$
(see also \cite{02.edoardo}).

Thus the lemma is proved.
\end{proof}

\subsection{Image of the versal map}\label{sec: image versal map}

We now consider: 
\begin{itemize}
\item $\mathcal X\to\mathbb D$ be a flat projective family of complex surfaces with smooth total space $\mathcal X$,
smooth general fibre $\mathcal X_t$ and central fibre $\mathcal X_0$ with normal crossing singularities,
\item $C\subset \mathcal X_0=\cup X_i$ a reduced Cartier divisor with only tacnodes at the intersection points with the singular locus $E=\cup_{ij}E_{ij}$ of $\mathcal X_0$ and
nodes on $\mathcal X_0\setminus E$,
\end{itemize}
as in \ref{p:setup}.


\begin{lemma}\label{lm: diff-point}
In the above setting, let $p\in C\cap E_{ij}\subset\mathcal X_0\subset\mathcal X$ be an $m$-tacnode, with $m\geq 1$.
Then, using the parametrization \eqref{versal-family-m-tacnode} for the mini-versal family of $(C,p)$, 
we have that the image of the differential map
$$
d\phi_{p,[C]}: H^0(C, \mathcal N_{C|\mathcal X})\to T_{C,p}^1=T_{\underline 0}\Delta_{(C,p)} 
$$
is always contained in the linear subspace $H_p:\beta_1=\cdots=\beta_{m-1}=0$,
while the image of the differential map
$$
d\phi_{p,[C]}: H^0(C, \mathcal N_{C|\mathcal X_0})\to T_{C,p}^1=T_{\underline 0}\Delta_{(C,p)} 
$$
is always contained in the  tangent space $\Gamma_p=T_{\underline 0}EG_{(C,p)}:\beta_0=\cdots=\beta_{m-1}=0$ at $\underline 0$
to the equigeneric locus $EG_{(C,p)}$ in $\Delta_{(C,p)}$(\cf \cite{diaz-harris} and \cite{02.edoardo}).
In particular,
the subspace
\begin{equation}\label{equisingular-at-a-point}
\ker(d\phi_{p,[C]})
%=\{\rm infinitesimal \, first \,order\, deformations\, of \,C\,in \, \mathcal X_0\,that\,are\, equisingular\, at\, p\}
\subset H^0(C,\mathcal N'_{C|\mathcal X_0})
\end{equation}
%parametrizing infinitesimal first order deformations of $C$ in $\mathcal X_0$ with are equisingular at $p$,
has dimension
$$ 
\dim(\ker(d\phi_{p,[C]}))\geq h^0(C,\mathcal N_{C|\mathcal X_0})-m+1\geq h^0(C,\mathcal N_{C|\mathcal X})-m.
$$
The differential map $d\phi_{p,[C]}$ is surjective on $H_p$ if and only if the subspace $\ker(d\phi_{p,[C]})$ of infinitesimal  first order deformations of $C$ in $\mathcal X_0$ that are equisingular at $p$ has codimension exactly $m-1$ in $H^0(C,\mathcal N_{C|\mathcal X_0})$.
\end{lemma}

\begin{proof}
We first observe that $H_p$ contains in codimension $1$ the tangent space $$\Gamma_p=T_{\underline 0}EG_{(C,p)}:\beta_0=\cdots=\beta_{m-2}=0$$ at $\underline 0$ to 
the equigeneric locus $EG_{(C,p)}\subset\Delta_{(C,p)}$.  

The image of $U_p\cap \mathcal H_0$
with respect to $\phi_p$
(recall the notation from Diagram \eqref{versal diagram})
is contained in the equigeneric locus 
$EG_{(C,p)}\subset\Delta_{(C,p)}$. Indeed, no matter how we deform $C$ in $\mathcal X_0$, the smooth tangency of the irreducible 
components $C_i$ and $C_j$ with $E_{ij}$ at $p$ deforms to smooth tangencies with $E_{ij}$ at $r\leq m$ points $p_l$, with $1\leq l\leq r$, of multiplicity $m_l$ with 
$\sum_lm_l=m$. This corresponds locally to a deformation of the
$m$-tacnode of $C$ at $p$ into $r$ tacnodes of orders $m_1,\ldots,m_r$,
each decreasing the geometric genus by $m_l$ with respect to the arithmetic genus.
Thus, $d\phi_{p,[C]}(H^0(C, \mathcal N_{C|\mathcal X_0}))\subset
\Gamma_p=T_{\underline 0}EG_{(C,p)}$.
%T_{\underline 0}EG_{(C,p)}:\beta_0=\cdots=\beta_{m-2}=0. $

Now, by the exact sequence 
$$
0\to\mathcal N_{C|\mathcal X_0}\to\mathcal N_{C|\mathcal X}\to\mathcal N_{\mathcal X_0|\mathcal X}=\mathcal O_{\mathcal X_0}\to 0,
$$
we have that $H^0(C,\mathcal N_{C|\mathcal X_0})$ has codimension less or equal to $1$ in $H^0(C,\mathcal N_{C|\mathcal X})$.
If $h^0(C,\mathcal N_{C|\mathcal X_0})=h^0(C,\mathcal N_{C|\mathcal X})$, the lemma is true because $T_{\underline 0}EG_{(C,p)}\subset H_p$.
If $h^0(C,\mathcal N_{C|\mathcal X})=h^0(C,\mathcal N_{C|\mathcal X_0})+1$, it is enough to find a section 
$$\sigma\in H^0(C,\mathcal N_{C|\mathcal X})\setminus H^0(C,\mathcal
N_{C|\mathcal X_0})$$ such that
$d\phi_{p,[C]}(\sigma)\in H_p\setminus T_{\underline 0}EG_{(C,p)}.$ In this case, one has
$$
H^0(C,\mathcal N_{C|\mathcal X})\simeq H^0(C,\mathcal N_{C|\mathcal X_0})\oplus H^0(C,\mathcal O_{\mathcal X_0})\simeq
H^0(C,\mathcal N_{C|\mathcal X_0})\oplus \mathbb C.
$$
The section $\sigma\in H^0(C,\mathcal N_{C|\mathcal X})\setminus
H^0(C,\mathcal N_{C|\mathcal X_0})$ corresponding to the pair
$(\underline 0,1)$ via the above isomorphism has local equations 
\begin{eqnarray}\label{sigma}
\left\{\begin{array}{l}
x+y+z^m=0\\
xy=\epsilon.
\end{array}\right.
\end{eqnarray}  
It follows that the image of $\sigma$ via $d{\phi_{p,[C]}}$ is the point corresponding to the curve $y(y+z^m)=\beta_0$.
This proves the lemma.
\end{proof}



\begin{corollary}\label{cor:diff-point}
In the same setting as above and with the same notation and
hypotheses as in Lemma \ref{lm: diff-point} and Diagram \eqref{versal diagram}, assume that:
\begin{description}
\item{a)} $h^0(C,\mathcal N_{C|\mathcal X_0})=h^0(C,\mathcal N_{C|\mathcal X})-1$;
\item{b)} the relative Hilbert scheme $\mathcal H^{\mathcal X|\mathbb D}$ is smooth at $[C]$ of dimension $h^0(C,\mathcal N_{C|\mathcal X})$;
\item{c)} $\dim(\ker(d\phi_{p,[C]}))=h^0(C,\mathcal N_{C|\mathcal X_0})-m+1.$
\end{description}
Then the image of the versal map 
$$
\phi_p:\mathcal H\cap U_p\to\Delta_{(C,p)}
$$
is a smooth variety of dimension $m$ in $\Delta_{(C,p)}$, with tangent space at $\underline 0$ given by the linear subspace 
$H_p:\beta_1=...=\beta_{m-1}=0$,
while  the image of the versal map 
$$
\phi_p:\mathcal H_0\cap U_p\to\Delta_{(C,p)}
$$
coincides with the equigeneric deformation locus $EG_{(C,p)}\subset\Delta_{(C,p)}$, which is smooth of dimension $m$ at $\underline 0$,
with tangent space given by
$\Gamma_p=T_{\underline 0}EG_{(C,p)}:\beta_0=...=\beta_{m-1}=0$, and whose general element corresponding to an $m$-nodal curve.

Moreover, $\phi_p(\mathcal H\cap U_p)$ intersects the locus of $(m-1)$-nodal curves in $\Delta_{(C,p)}$ along $\Gamma_p\cup\gamma$, where $\gamma$ is a curve that is smooth at $\underline 0$
and intersects $\Gamma_p$ with multiplicity $m$.
In particular the curve $C$ may be deformed in $\mathcal H$ in such a way the tacnode at $p$ is deformed into $m-1$ nodes.
\end{corollary}

\begin{proof}
First observe that, by hypothesis b), there is only one irreducible component $\mathcal H$ of $\mathcal H^{\mathcal X|\mathbb D}$ containing $[C]$,
which is smooth at $[C]$ of dimension $h^0(C,\mathcal N_{C|\mathcal X})$. Moreover, by hypothesis a), the central fibre of $\mathcal H_0$ of $\mathcal H$
is smooth at $[C]$ of dimension $h^0(C,\mathcal N_{C|\mathcal X_0})=h^0(C,\mathcal N_{C|\mathcal X})-1$.

In particular, in Diagram \eqref{versal diagram}, we have that the analytic varieties $\mathcal H\cap U_p$ and $\mathcal H_0\cap U_p$ are irreducible.
It follows that the image of 
$
\phi_p:\mathcal H\cap U_p\to\Delta_{(C,p)}
$ 
is an irreducible variety of dimension $\leq m$, since $\phi_p(\mathcal H_0\cap U_p)$ is contained in the equigeneric locus, which has dimension $m-1$
and  $\phi_p(\mathcal H\cap U_p)$ has dimension $\leq \dim(\phi_p(\mathcal H_0\cap U_p))+1$. In particular, 
$\phi_p$ has general fibre of dimension at least $\dim_{[C]}(\mathcal H)-m$. Under the hypotheses of this corollary, the differential $d\phi_{p,[C]}$ 
has rank $m$. Hence, under hypotheses a), b) and c), 
the fibre $\phi_p^{-1}(\underline 0)$ has dimension exactly $\dim_{[C]}(\mathcal H)-m=h^0(C,\mathcal N_{C|\mathcal X})-m$, and
$\phi_p(\mathcal H\cap U_p)$ is irreducible of dimension $m$ and smooth at $\underline 0$. The fact that
$\phi_p(\mathcal H\cap U_p)$ intersects the locus of $(m-1)$-nodal curves in $\Delta_{(C,p)}$ along $\Gamma_p\cup\gamma$, where $\gamma$ is a curve that is smooth at $\underline 0$
and intersects $\Gamma_p$ with multiplicity $m$ follows from
\cite[Lemma 4.1]{caporaso-harris}, \cf
\cite[Theorem \tref{principale}]{05.margherita}.
\end{proof}

\begin{remark}\label{rm: A-k-smoothing}
Under the hypotheses of Lemma \ref{cor:diff-point}, by \cite[Proposition 3.7 and Corollary 3.12]{concettina-andreas}, one has  more generally that there exist deformations $C_t\subset\mathcal X_t$ of $C\subset \mathcal X_0$ such that the $m$-tacnode of $C$ at $p$ deforms to $d_i$ singularity of type $A_i$, for every multi-index $(d_1,...,d_r)$ such that $\sum_{i}id_i=m-1.$
\end{remark}


The following lemma provides a standard way to verify when the hypothesis c) in Corollary \ref{cor:diff-point} is satisfied.

Let  $W_{p,m-1}^{|C|}\subset |\mathcal O_{\mathcal X_0}(C)|$ be the linear system of Cartier divisors in $|\mathcal O_{\mathcal X_0}(C)|$ intersecting $E$ at $p$ with multiplicity 
$m-1$. We have that
$$
\dim(W_{p,m-1}^{|C|})\geq \dim(|\mathcal O_{\mathcal X_0}(C)|)-m+1.
$$


\begin{lemma}\label{lm:linear-system}
In the same setting as above, and with the same notation and
hypotheses as in Lemma \ref{lm: diff-point}, assume that:
\begin{equation}
\dim(W_{p,m-1}^{|C|})= \dim(|\mathcal O_{\mathcal X_0}(C)|)-m+1.
\end{equation}
Then we have 
$$
\dim(\ker(d\phi_{p,[C]}))=h^0(C,\mathcal N_{C|\mathcal X_0})-m+1.
$$
\end{lemma}
\begin{proof}
By the hypothesis that $\dim(W_{p,m-1}^{|C|})= \dim(|\mathcal O_{\mathcal X_0}(C)|)-m+1$, we have
$$\dim(W_{p,r}^{|C|})= \dim(|\mathcal O_{\mathcal X_0}(C)|)-r+1,$$
for every $r\leq m-1$. Via the natural inclusion 
$$
|\mathcal O_{X_0}(C)|=H^0(\mathcal X_0,\mathcal O_{\mathcal X_0}(C))\big/H^0(\mathcal X_0,\mathcal O_{\mathcal X_0})
\subset H^0(C,\mathcal N_{C|\mathcal X_0})
$$
induced by the standard exact sequence
$$
0\to\mathcal O_{\mathcal X_0}\to\mathcal O_{\mathcal X_0}(C)\to\mathcal O_C(C)\to 0,
$$
we find a chain a codimension $1$ linear subsystems
$$
W_{p,m-1}^{|C|}\subsetneq W_{p,m-2}^{|C|}\subsetneq ...\subsetneq W_{p,1}^{|C|}\subsetneq |\mathcal O_{X_0}(C)|\subset H^0(C,\mathcal N_{C|\mathcal X_0}).
$$
By Lemma \ref{lemma-ker}, we know that $W_{p,r}^{|C|}\cap \ker(d\phi_{p,[C]})\subset W_{p,m-1}^{|C|}$, for every $r\leq m-2$.
Since $H^0(C,\mathcal N_{C|\mathcal X_0})$ is mapped by $d\phi_{p,[C]}$ to the $(m-1)$-dimensional linear subspace $T_{\underline 0}EG\subset T_{\underline 0}\Delta_{(C,p)}$,
we find that $d\phi_{p,[C]}:H^0(C,\mathcal N_{C|\mathcal X_0})\to
T_{\underline 0}EG$ is surjective by standard linear algebra, and thus
$\dim(\ker(d\phi_{p,[C]}))=h^0(C,\mathcal N_{C|\mathcal X_0})-m+1.$ 
\end{proof}

\section{Global deformations of $C$}
Let $\mathcal X\to\mathbb D$ and 
$
C=\cup_{i}C_i\subset\mathcal X_0=\cup_{i}X_i
$
be respectively the flat projective  family of surfaces and the
Cartier divisor $C$ on $\mathcal X_0$ as in \ref{p:setup}. We recall
that $\mathcal X$ has smooth general fibre $\mathcal X_t$ and
reducible central fibre $\mathcal X_0=\cup_{i}X_i$ with normal
crossing singularities. We denoted by $X_i$ the irreducible components
of $\mathcal X_0$, and by $E=\cup_{i,j}E_{ij}$ the singular locus of
$\mathcal X_0$, where $E_{ij}=X_i\cap X_j$. Moreover, we assume that
$C\cap X_i=C_i$ is a reduced $\delta_i$-nodal curve intersecting $E$
at smooth points, in such a way that the only singularities of $C$ are
nodes on $\mathcal X_0\setminus E$ and tacnodes on $E$. For every
tacnode $p$ of $C$, we denote by $m_p$ its order and by
\begin{equation}\label{eq: lmc}
\lambda={\rm lcm}\{m_p|\,p\,\,\textrm{tacnode of}\,\,C\}
\end{equation}
the least common multiple of the $m_p$. We furthermore set
\begin{equation}\label{eq: number of components}
  \mu=\prod_{p\,\,\textrm{tacnode of}\,\,C}m_p
  \quad \text{and} \quad k=\frac{\mu}{\lambda}.
\end{equation}
Finally, we assume that
$C$ has 
$$
\delta=\sum_{i}\delta_i
\quad {\rm{nodes\, on}}\,\, \mathcal X_0\setminus E,
$$
%at points $p_{il}\in X_i$, for every $i$ and $0\leq l\leq\delta_i$ 
and we denote by
$$
\tau_m
\quad {\textrm{the number of }}\,\,m-{\rm{tacnodes}}\,\,{\rm of}\,\, C\,\, {\rm on}\,\, E,
$$
for every $m\geq 1.$

Here we will provide sufficient conditions for $C\subset\mathcal X_0$ to be deformed to a nodal curve $C_t\subset\mathcal X_t$. 

We recall that we denoted by $\mathcal H^{\mathcal X|\mathbb D}$ the
relative Hilbert scheme of the family $\mathcal X\to\mathbb D$, by
$\mathcal H$ the union of the irreducible components of $\mathcal
H^{\mathcal X|\mathbb D}$ containing $[C]$, and by $\mathcal H_t$ the
fibre of $\mathcal H$ over $t\in \mathbb D$. Let now $\mathbb D^o=\mathbb D\setminus \underline 0$, $\mathcal X^o=\mathcal X\setminus\mathcal X_0$, and $\mathcal H^o=\mathcal H\setminus \mathcal H_0$.
For all $\sigma \in \N$, we denote by $\mathcal U_\sigma^{\mathcal
  X^o|\mathbb D^o}\subseteq\mathcal H^o$ the relative Severi variety
of $\sigma$-nodal curves, the fibre of which over $t\in \mathbb D^o$ is 
the locally closed (possibly empty) subscheme $\mathcal
U_\sigma^{\mathcal X_t}\subseteq \mathcal H_t$ (endowed with its
reduced structure)  parametrizing reduced  $\sigma$-nodal Cartier divisors on $\mathcal X_t$.
We moreover denote by $\mathcal V_\sigma^{\mathcal X|\mathbb D}\subseteq\mathcal H$ the Zariski closure in 
$\mathcal H$ of  $\mathcal U_\sigma^{\mathcal X^o|\mathbb D^o}$. 
Observe that, for every $t\neq 0$, the fiber $\mathcal V_\sigma^{\mathcal X_t}$ of $\mathcal V_\sigma^{\mathcal X|\mathbb D}$
over $t$ is the Zariski closure of  $\mathcal U_\sigma^{\mathcal X_t}$, while $\mathcal V_\sigma^{\mathcal X^|\mathbb D}\cap \mathcal H_0$
will have several irreducible components, whose general point corresponds to a curve on $\mathcal X_0$ with singularities possibly different than nodes.

\begin{theorem}\label{independent-smoothing-forte} 
In the above setting, let
$$W^{|C|}_{[C],es}\subset |\mathcal O_{\mathcal X_0}(C)|$$
be the linear system of Cartier divisors in $|\mathcal O_{\mathcal X_0}(C)|$
passing through every node of $C$ on $\mathcal X_0\setminus E$, and  intersecting $E$  with multiplicity $m-1$ at every $m$-tacnode of $C$.
Assume that:
\begin{enumerate}
\item{} $h^0(C,\mathcal N_{C|\mathcal X_0})=h^0(C,\mathcal N_{C|\mathcal X})-1$;\label{eq: independent-smoothing-forte1}
\item{} the relative Hilbert scheme $\mathcal H^{\mathcal X|\mathbb D}$ is smooth at $[C]$ of dimension $h^0(C,\mathcal N_{C|\mathcal X})$.
In particular, there is only one irreducible component $\mathcal H\subset\mathcal H^{\mathcal X|\mathbb D}$ containing $[C]$, which is smooth at $[C]$;\label{eq: independent-smoothing-forte2}
\item{} $\dim(W^{|C|}_{[C],es})=
  \dim \bigl( |\mathcal O_{\mathcal X_0}(C)| \bigr)
  -\delta-\sum_m\tau_m(m-1).$\label{eq: independent-smoothing-forte3}
\end{enumerate}
Then $C\subset\mathcal X_0$   may be deformed to $(\delta+\sum_m\tau_m(m-1))$-nodal curves $C_t\subset\mathcal X_t$, in such a way every node of $C$ on $\mathcal X_0\setminus E$ is preserved, and every $m$-tacnode of $C$ on $E$ is smoothed to $m-1$ nodes. All nodal curves $C_t$ obtained in this way are such that 
\begin{equation}\label{eq: semicontinuity}
h^0(C_t,\mathcal N'_{C_t|\mathcal X_t})=h^0(C_t,\mathcal N_{C_t|\mathcal X_t})-\delta-\sum_m\tau_m(m-1),
\end{equation}
thus,  the corresponding point $[C_t]\in\mathcal H_t$ is a smooth point of the
Severi variety $\mathcal V^{\mathcal X_t}_{\delta+\sum_m\tau_m(m-1)}$. In particular the nodes of $C_t$ may be smoothed independently , i.e. the versal map 
\eqref{eq: versal map} for $C_t$ is surjective. This implies that  
$$
[C]\in\mathcal V_{\sigma}^{\mathcal X|\mathbb D},\,\,\textrm{for\,every}\,\,\sigma\leq\delta+\sum_m\tau_m(m-1).
$$
Moreover, the equisingular deformation locus $\mathcal{ ES}(C)\subset\mathcal X_0$ of $[C]$ in $\mathcal X_0$ (cf. Definition \ref{def: es}) is an analytic open set of the smooth locus of an irreducible component $V_0$ of the central fibre 
$$
\mathcal V_0=\mathcal V_{\delta+\sum_m\tau_m(m-1)}^{\mathcal X|\mathbb D}\cap\mathcal H_0=\mu V_0+\cdots
$$ 
of $\mathcal V_{\delta+\sum_m\tau_m(m-1)}^{\mathcal X|\mathbb D}\subset \mathcal H$, of scheme theoretic multiplicity 
$$\mu=\prod_{p\,\,\textrm{tacnode of}\,\,C}m_p.$$  More precisely, at an analytic neighborhood of $[C]$, the universal Severi variety
$\mathcal V_{\delta+\sum_m\tau_m(m-1)}^{\mathcal X|\mathbb D}$ will be the union of $k$ branches, each intersecting $\mathcal H_0$ at $[C]$ with multiplicity $\lambda$, where $k$ and $\lambda$ are defined by \eqref{eq: number of components}. These $k$ local analytic branches of $\mathcal V_{\delta+\sum_m\tau_m(m-1)}^{\mathcal X|\mathbb D}$ will all be smooth at $[C]$ if $\lambda=m_p$, for some tacnode $p$ of $C$; otherwise they will all be singular at $[C]$, with multiplicity 
$\lambda\over {\rm max}\{m_p|\,p\,\,\textrm{tacnode of}\,\,C\}$.
\end{theorem}


\begin{remark}\label{rm:hypothesis three}
Hypothesis 3 in Theorem \ref{independent-smoothing-forte} can be weakened by asking 
\begin{equation}\label{independent-smoothing-debole} 
h^0(C,\mathcal N'_{C|\mathcal X})=h^0(C,\mathcal N'_{C|\mathcal X_0})=h^0(C,\mathcal N_{C|\mathcal X_0})-\delta-\sum_m\tau_m(m-1).
\end{equation}
As we will observe in the proof of the theorem, under hypotheses 1 and 2, we have that hypothesis 3 is a sufficient condition for the equality \eqref{independent-smoothing-debole}.
The reason we preferred this statement of Theorem \ref{independent-smoothing-forte}  is that hypothesis 3 in the theorem 
is usually easier to be verified than \eqref{independent-smoothing-debole}. 

We finally observe that, if 
\begin{equation}\label{eq: relative linear system}
H^0(C,\mathcal N_{C|\mathcal X_0})=H^0(C,\mathcal O_C(C)),
\end{equation} 
which happens in particular if the family $\mathcal X\to\mathbb D$
is a family of regular surfaces
(\ie $h^1(\mathcal X_t,\mathcal O_{\mathcal X_t})=0$ for all $t$),
then, under hypotheses 1, 2, and 3 of Theorem
\ref{independent-smoothing-forte}, we have that $H^0(C,\mathcal N'_{C|\mathcal X})=W^{|C|}_{[C],es}.$ Indeed, if \eqref {eq: relative linear system}
holds, then
$H^0(C,\mathcal N'_{C|\mathcal X})\subseteq W^{|C|}_{[C],es}$ by Lemma
\ref{lemma-ker}, and this inclusion is in fact an equality for dimensional reason.
\end{remark}


\begin{remark}\label{rm: 1tacnode}
In Theorem \ref{independent-smoothing-forte}, the nodes of $C$ on $E$ cannot be preserved by deforming $C$ to a  
curve in $\mathcal X_t$, with  $t\neq 0$. This is a very general result that holds for any reduced Cartier divisor on $X_0$ with a node on $E$
under our hypotheses on $\mathcal X\to\mathbb D$, \ie just assuming $\mathcal X\to\mathbb D$ a flat projective family of surfaces with smooth
total space, smooth general fibre and central fibre $\mathcal X_0$ with normal crossing singularities (or more generally, with normal crossing singularity at a neighborhood of the node). A proof of this can be found in \cite[Section 2]{concettina1}.
This also follows from the hypotheses \ref{eq: independent-smoothing-forte1}, \ref{eq: independent-smoothing-forte2}  of Theorem \ref{independent-smoothing-forte},
by Lemma \ref{lemma-ker}. In order to see this, we fix a node $p$ of $C$ on $E$, and we consider the diagram \eqref{versal diagram}. What we want to prove is that 
\begin{equation}\label{eq: 1-tacnode}
\phi_p^{-1}(\underline 0)= U_p\cap \mathcal H_0.
\end{equation}
By Lemma  \ref{lemma-ker}, we know that 
$$T_{\underline 0}(\phi_p^{-1}(\underline 0))=\ker(d\phi_{p,[C]})\subseteq H^0(C,\mathcal N_{C|\mathcal X_0}),$$ and, by the hypothesis \ref{eq: independent-smoothing-forte1} of Theorem \ref{independent-smoothing-forte}, we get that $\dim(T_{\underline 0}(\phi_p^{-1}(\underline 0)))=h^0(C,\mathcal N_{C|\mathcal X_0})=h^0(C,\mathcal N_{C|\mathcal X})-1$. Now observe that 
$U_p\cap \mathcal H_0\subset \phi_p^{-1}(\underline 0)$ because every deformation of $C$ in $\mathcal X_0$ preserves the node of $C$ at $p$. Finally, by the hypotheses 
\ref{eq: independent-smoothing-forte1} and \ref{eq:
  independent-smoothing-forte2} in Theorem
\ref{independent-smoothing-forte}, we have that $\mathcal H_0$ is
smooth at $[C]$ of dimension $h^0(C,\mathcal N_{C|\mathcal
  X_0})=h^0(C,\mathcal N_{C|\mathcal X})-1$. This proves \eqref{eq:
  1-tacnode}, which in particular says that Theorem \ref{independent-smoothing-forte} completely answers Problem \ref{main-problem} for a curve $C$ verifying the hypothesis \eqref{independent-smoothing-debole}.
\end{remark}


\begin{proof}[Proof of Theorem \ref{independent-smoothing-forte}]
%We first observe that, by the hypotheses \ref{eq: independent-smoothing-forte1} and \ref{eq: independent-smoothing-forte2}, the
%relative Hilbert scheme $\mathcal H^{\mathcal X|\mathbb D}$ of $\mathcal X\to\mathbb D$ is smooth at $[C]$ and the Hilbert scheme of $\mathcal X_0$ are  of %dimension respctively
%$h^0(C,\mathcal N_{C|\mathcal X})$ and $h^0(C,\mathcal N_{C|\mathcal X_0})$.
Let ${\rm Sing}(C)$ be the singular locus of $C$. For every singular point $p\in {\rm Sing}(C)$, we consider the mini-versal deformation space $\Delta_{(C,p)}$ described in Section \ref{sec: versal geometry}, the versal map \eqref{eq: versal map}
\begin{equation*}
  \phi=\prod_{p\in {\rm {Sing}}(C)}\phi_p:
  \bigcap_{p\in {\rm Sing}(C)} U_p
  \ \to\  \prod_{p\in {\rm Sing}(C)}\Delta_{(C,p)},
\end{equation*}
and its differential
\begin{equation*}%\label{eq: differential versal map}
  d\phi_{[C]}=\bigoplus_{p\in {\rm
      Sing}(C)}d\phi_{p,[C]}:H^0(C, \mathcal N_{C|\mathcal X})\ \to\  H^0(C,T^1_C)=\bigoplus_{p\in \textrm{Sing}(C)}T_{C,p}^1 
\end{equation*}
at $[C]\in \mathcal H$, described in Sections \ref{sec: equisingular def} and \ref{sec: image versal map}.

Arguing exactly as in the proof of Lemma \ref{lm:linear-system}, we see that 
$$
W^{|C|}_{[C],es}\subset |\mathcal O_{\mathcal X_0}(C)|\subset H^0(C,\mathcal N_{C|\mathcal X_0}),
$$
and the hypothesis \ref{eq: independent-smoothing-forte3} of the theorem implies that
the image of the differential
$d\phi_{[C]}$
% $$
% d\phi_{[C]}=\oplus_{p\in \rm {\rm Sing}(C)}d\phi_{p,[C]}:H^0(C, \mathcal N_{C|\mathcal X_0})\to H^0(C,T^1_C)=\oplus_{p\in \textrm{Sing}(C)}T_{C,p}^1 
% $$
has dimension $\delta+\sum_m\tau_m(m-1)$, hence
\begin{equation}\label{eq: independent-smoothing-forte}
  \dim\bigl(\ker(d\phi_{[C]})\bigr)
  =h^0(C,\mathcal N'_{C|\mathcal X})
  =h^0(C,\mathcal N'_{C|\mathcal X_0})=h^0(C,\mathcal N_{C|\mathcal X_0})
-\delta-\sum_m\tau_m(m-1).
\end{equation}
This in turn implies that
$$
\dim\bigl(\ker(d\phi_{p,[C]})\bigr)=h^0(C,\mathcal N_{C|\mathcal
  X_0})-m+1,\quad 
\text{for every $m$-{tacnode} $p\in E\cap C$ of $C$}
$$
and 
$$
\dim\bigl(\ker(d\phi_{p,[C]})\bigr)
=h^0(C,\mathcal N_{C|\mathcal X_0})-1,
\quad \text{for every node of $C$ {in} $\mathcal X_0\setminus E$.}
$$
In particular, Corollary \ref{cor:diff-point} applies at every $m$-tacnode $p$ of $ C$ on $E$.

Now, by Remark \ref{rm: 1tacnode}, we know that every $1$-tacnode
(\ie node) of $C$ on $E$ is necessarily smoothed as we deform $C\subset\mathcal X_0$ outside the central fibre of $\mathcal X\to\mathbb D$. Thus, denoting by 
$$
\Singzo(C)={\rm Sing}(C)\,\setminus\,\{\textrm{nodes on}\,\, E\},
$$
we may restrict our attention to the versal map
\begin{equation}\label{eq: esclusi-nodi-su-E}
  \varphi= \prod_{p\in \Singzo(C)}\phi_p:
  \bigcap_{p\in \Singzo(C)} U_p
  \ \to \ 
  \raisebox{-.3em}{\bigg(}
  \prod_{m\geq 2}
  \prod_{\substack{
      p\in E\cap C\\
      m\textrm{-tacnode}}
  }
  \Delta_{(C,p)})
    \raisebox{-.3em}{\bigg)}
    \times
    \prod_{\substack{
        p\in C\setminus E\\
        \textrm{node}}
    }
    \Delta_{(C,p)}
\end{equation}
and its differential at $[C]$, 
$$
d\varphi_{[C]}:H^0(C, \mathcal N_{C|\mathcal X})
\ \to\
  \raisebox{-.3em}{\bigg(}
\bigoplus_{m\geq 2} 
\bigoplus_{\substack{
      p\in E\cap C\\
      m\textrm{-tacnode}}
  }
  T_{C,p}^1
  \raisebox{-.3em}{\bigg)}
\oplus
\bigoplus_{\substack{
        p\in C\setminus E\\
        \textrm{node}}
    }
T_{C,p}^1,
$$ 
obtained by composing $d\phi_{[C]}$ with the natural projection
map. By Lemma \ref{lm: diff-point} and Corollary \ref{cor:diff-point},
and using the notation therein,
we know that
$$
d\varphi_{[C]}\bigl(H^0(C, \mathcal N_{C|\mathcal X})\bigr)
\subseteq
  \raisebox{-.3em}{\bigg(}
\bigoplus_{m\geq 2} 
\bigoplus_{\substack{
      p\in E\cap C\\
      m\textrm{-tacnode}}
  }
  H_p
  \raisebox{-.3em}{\bigg)}
  \oplus
  \bigoplus_{\substack{
        p\in C\setminus E\\
        \textrm{node}}
    }
    T_{C,p}^1
$$ 
and
$$
d\varphi_{[C]}(H^0(C, \mathcal N_{C|\mathcal X_0}))\subseteq
\raisebox{-.3em}{\bigg(}
\bigoplus_{m\geq 2} 
\bigoplus_{\substack{
      p\in E\cap C\\
      m\textrm{-tacnode}}
  }
\Gamma_p
\raisebox{-.3em}{\bigg)}
\oplus
\bigoplus_{\substack{
        p\in C\setminus E\\
        \textrm{node}}
    }
T_{C,p}^1.
$$ 
More precisely, observing that
$$
\ker(d\varphi_{[C]})=H^0(C, \mathcal N'_{C|\mathcal X_0})\subseteq H^0(C, \mathcal N_{C|\mathcal X_0})
$$
because every node on $E$ is trivially preserved if we deform $C$ in $\mathcal X_0$, by \eqref{eq: independent-smoothing-forte}
we get that $d\varphi_{[C]}(H^0(C, \mathcal N_{C|\mathcal X_0}))$ has dimension 
$$\sum_m\tau_m(m-1)+\delta=
\dim
\raisebox{-.3em}{\Bigg[}
\raisebox{-.3em}{\bigg(}
\bigoplus_{m\geq 2} 
\bigoplus_{\substack{
      p\in E\cap C\\
      m\textrm{-tacnode}}
  }
\Gamma_p
\raisebox{-.3em}{\bigg)}
\oplus
\bigoplus_{\substack{
        p\in C\setminus E\\
        \textrm{node}}
    }
    T_{C,p}^1
    \raisebox{-.3em}{\Bigg]}.
$$
Thus we obtain that
\begin{equation}\label{eq: cond1}
  d\varphi_{[C]}\bigl(H^0(C, \mathcal N_{C|\mathcal X_0})\bigr)=
  \raisebox{-.3em}{\bigg(}
\bigoplus_{m\geq 2} 
\bigoplus_{\substack{
      p\in E\cap C\\
      m\textrm{-tacnode}}
  }
\Gamma_p
\raisebox{-.3em}{\bigg)}
\oplus
\bigoplus_{\substack{
        p\in C\setminus E\\
        \textrm{node}}
    }
T_{C,p}^1,
\end{equation}
and
\begin{equation}\label{eq: cond2}
  d\varphi_{[C]}(H^0(C, \mathcal N_{C|\mathcal X}))= \Omega
  \oplus
\bigoplus_{\substack{
        p\in C\setminus E\\
        \textrm{node}}
    }
T_{C,p}^1,
\end{equation}%\label{eq: omega}%
for some linear subspace
$\Omega\subset
\bigoplus_{m\geq 2} \bigoplus_{p}H_p$ containing 
$\bigoplus_{m\geq 2} \bigoplus_{p}\Gamma_p$ in codimension $1$. Arguing as in the proof of Corollary \ref{cor:diff-point}, 
we get that:
\begin{itemize}
\item  the versal map $\varphi$ defined in \eqref{eq: esclusi-nodi-su-E} maps 
$\mathcal H_0$ surjectively onto the product
$$\Big(\prod_{m\geq 2}
\prod_{\substack{
      p\in E\cap C\\
      m\textrm{-tacnode}}
  }
\Gamma_p\Big)\times \underline 0\times ...\times \underline 0,$$
\item the image of $\varphi$ is an analytic variety, smooth
  of dimension $\sum_m\tau_m(m-1)+\delta+1$ at $\underline 0$, 
  which is a product
$$
\mathcal  W\times\prod_{p\in C\setminus E\,\,\textrm{node}}\Delta_{(C,p)},
$$
where $\mathcal W\subset
\prod_{m\geq 2} \bigl(\prod_{p\in E\cap C\ m\text{-tacnode}}\Delta_{(C,p)}
\bigr)$
may be identified with the image of the versal map
\begin{equation}\label{eq: solo-tacnodi}
  \psi=\prod_{p\in \Singzo(C)\cap E}\phi_p:
  \bigcap_{p\in \Singzo(C)\cap E} U_p
  \ \to \ 
  \prod_{m\geq 2}
  \prod_{\substack{
      p\in E\cap C\\
      m\textrm{-tacnode}}
  }
  \Delta_{(C,p)}.
\end{equation}
\end{itemize}
In particular, $\mathcal W$
is a smooth analytic variety of dimension $\sum_m\tau_m(m-1)+1$,
with tangent space $T_0\mathcal W = \Omega$ at $\underline 0$, where
$\Omega$ is as in \eqref{eq: cond2}. %{eq: omega}.
Keeping in mind the affine equations of the subspaces $\Gamma_p\subset H_p\subset \Delta_{(C,p)}$ in Lemma \ref{lm: diff-point}, the theorem follows by 
\cite[Lemma 4.4]{caporaso-harris} (see
\cite[Lemma \tref{lemma 4.4}]{06.francesco}), as we shall now explain.

To help the reader comparing our notation with that in \cite{caporaso-harris}, we observe that,  for every $m$-tacnode $(C,p)$, our subspace $\Gamma_p\subset\Delta_{(C,p)}$ is denoted in \cite[Lemma 4.4]{caporaso-harris} by $\Delta_{i,m_i}$. Moreover, the product of the  subspaces $\Gamma_p$ is denoted in \cite[Lemma 4.4]{caporaso-harris} by $\Delta_m$. Finally, the curves denoted by $\Gamma_1,...,\Gamma_k$ in the statement of \cite[Lemma 4.4]{caporaso-harris}, will be denoted here by
$\gamma_1,...,\gamma_k$.


By \cite[Lemma 4.4]{caporaso-harris}, we have that the intersection of $\mathcal W$
with the locus of $\sum_m\tau_m(m-1)$-nodal curves in
$\prod_{m\geq 2}
\prod_{p\in E\cap C\ m\text{-tacnode}}\Delta_{(C,p)}$ is given by 
$$
\Big(\prod\nolimits_{m\geq 2}
\prod\nolimits_{p\in E\cap C\ m\text{-tacnode}}
\Gamma_p\Big)
\cup \gamma_1\cup \cdots \cup\gamma_k,
$$
where $\gamma_1,\ldots,\gamma_k\subset\mathcal W$ are distinct, reduced, unibranched curves having intersection multiplicity exactly $\lambda$
with
$\prod_{m\geq 2}
\prod_{p\in E\cap C\ m\text{-tacnode}}\Gamma_p$
at the origin, with $\lambda$ and $k$ as defined in \eqref{eq: lmc} and \eqref{eq: number of components}. The curves
$\gamma_1,...,\gamma_k$ are all smooth at $[C]$ if $\lambda=m_p$, for
some tacnode $p$ of $C$; otherwise they are all singular at $[C]$,
with multiplicity
$\lambda/ {\rm max}\{m_p|\,p\,\,\textrm{tacnode of}\,\,C\}.$


The proof of the theorem is now complete if we observe that
the versal map $\varphi$ defined by \eqref{eq: esclusi-nodi-su-E} has differential of
maximal rank at $[C]$, thus
$$
\varphi^{-1}(\gamma_1\cup...\cup\gamma_k\times\underline 0\times...\times\underline 0)
$$
is locally a fibration over $\gamma_1\cup...\cup\gamma_k\times\underline 0\times...\times\underline 0$ with smooth fibre of dimension
$h^0(C,\mathcal N_{C|\mathcal X})-\delta-\sum_m\tau_m(m-1)$, and it
actually consists of $k$ analytic branches of
$\mathcal V_{\delta+\sum_m\tau_m(m-1)}^{\mathcal X|\mathbb D}$  at $[C]$.
The fact that, if $[C_t]$ is general in one of these analytic branches of $\mathcal V_{\delta+\sum_m\tau_m(m-1)}^{\mathcal X|\mathbb D}$,
then \eqref{eq: semicontinuity} holds, follows by semicontinuity.
\end{proof}


\begin{remark}
Theorem \ref{independent-smoothing-forte} proves in particular
\cite[Proposition \tref{p:zrr}]{01.ciro}; besides, \cite{01.ciro}
contains many 
applications of Theorem \ref{independent-smoothing-forte}. In order to help the reader compare  Theorem \ref{independent-smoothing-forte} 
with \cite[Proposition \tref{p:zrr}]{01.ciro},
we observe that \cite[Proposition \tref{p:zrr}]{01.ciro} is stated under the assumption that
$\Hilb(\mathcal L)$ (notation from loc.\ cit.)
is an irreducible component of the relative Hilbert scheme of curves
in the family of surfaces $S\to\mathbb D$,
see \cite[Section \tref{s:resolving}]{01.ciro}.
\end{remark}

\begin{remark}
The failure of hypothesis 3 in Theorem \ref{independent-smoothing-forte} is not always an obstruction
to study deformations of $C$ outside $\mathcal X_0$. It may happen for example that the singularities of $C$ do not impose 
the expected number of conditions because several nodes of $\mathcal
X_0\setminus E$ are ``disconnecting nodes'', \ie normalizing $C$ at
these nodes produces a reducible curve, and for some geometric reason
it is not possible to deform $C$ on $\mathcal X_t$ to a reducible curve. In this case the disconnecting
nodes cannot be preserved by deforming $C$ outside the central fibre,
and the singularities of $C$ do not impose the expected number of
conditions. This  happens for example for curves constructed in
\cite[Section 4]{concettina-andreas}.

When hypothesis 3 in \ref{independent-smoothing-forte} Theorem fails,
one has to restrict the attention on the subset of singularities
imposing the right number of conditions (namely, $1$ condition for a node on
$\mathcal X_0\setminus E$, and $m-1$ conditions for an $m$-tacnode on $E$) to the linear system $|\mathcal O_{\mathcal X_0}(C)|$, and study the versal map 
only for this subset of singularities.
\end{remark}


\begin{remark}\label{rm: A-k-smoothing-global}
Under the hypotheses of Theorem \ref{independent-smoothing-forte}, by \cite[Proposition 3.7 and Corollary 3.12]{concettina-andreas}, one has  more generally that there exist deformations $C_t\subset\mathcal X_t$ of $C\subset \mathcal X_0$ so that every $m$-tacnode $p$ of $C$ is  deformed to  $d_{i,p}$ singularity of type $A_i$, for every multi-index $(d_{1,p},...,d_{r,p})$ such that $\sum_{i}id_{i,p}=m-1,$ and every node of $C\subset \mathcal X_0$ is preserved. For these curves $C_t$ the equality \eqref{eq: semicontinuity} still holds, thus the corresponding generalized universal Severi variety is smooth at $[C_t]$, but describing its local geometry at $[C_0]$ is much more complicated.
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





\begin{references}

\begin{thebibliography}[Chapters in this Volume]{XIV}

\bibitem[\tref{01.ciro}]{01.ciro}
C.~Ciliberto,
\emph{Limits of nodal curves: generalities and examples}.

\bibitem[\tref{02.edoardo}]{02.edoardo}
Th.~Dedieu {\normalfont \smfandname} E.~Sernesi,
\emph{Deformations of curves on surfaces}.

% \bibitem[\tref{03.th-acz}]{03.th-acz}
% Th.~Dedieu,
% \emph{Geometry of logarithmic Severi varieties at a general point}.

\bibitem[\tref{05.margherita}]{05.margherita}
M.~Lelli-Chiesa,
\emph{Deformations of an $m$-tacnode into $m-1$ nodes}.

\bibitem[\tref{06.francesco}]{06.francesco},
F.~Bastianelli,
\emph{Products of deformation spaces of tacnodes}.

% \bibitem[\tref{04.concettina}]{04.concettina}
% Th.~Dedieu {\normalfont \smfandname} C.~Galati,
% \emph{Degenerations and deformations of generalized Severi varieties}.

% \bibitem[\tref{04b.concettina}]{04b.concettina}
% C.~Galati,
% \emph{Proving the existence of curves  on smooth surfaces
%   by smoothing tacnodes on reducible surfaces}.

% \bibitem[\tref{11.th-toric-trop}]{11.th-toric-trop}
%   Th.~Dedieu,
%   \emph{Enumeration of curves in toric surfaces, tropical geometry,
%     and floor diagrams}.

% \bibitem[\tref{13.th-classic}]{13.th-classic}
% Th.~Dedieu,
% \emph{Some classical formul{\ae} for curves and surfaces}.

% \bibitem[\tref{14.th-vainsencher}]{14.th-vainsencher}
% Th.~Dedieu,
% \emph{Node polynomials for curves on surfaces}.

% \bibitem[\tref{16.th+l-redres}]{16.th+l-redres}
% L.~Busé {\normalfont \smfandname} Th.~Dedieu,
% \emph{Generalized weight properties of resultants and discriminants,
% and applications to projective enumerative geometry}.

\end{thebibliography}

\begin{thebibliography}[External References]{99}

\bibitem{caporaso-harris}
L.~Caporaso, J.~Harris:
{\it Counting plane curves of any genus}, Invent. Math. {\bf 131} (1998), no.2, 345--392.

\bibitem{caporaso-harris2}
L.~Caporaso, J.~Harris:
{\it Parameter spaces for curves on surfaces and enumeration of rational curves},
Compositio Math. {\bf 113} (1998), no.2, 155--208.

\bibitem{chen} X.~Chen: {\it Rational curves on K3 surfaces}, J. Alg. Geom. {\bf 8} (1999), no.2, 245--278.

\bibitem{cdgk} C.~Ciliberto, T.~Dedieu, C.~Galati, A.~L.~Knutsen: {\it Nonemptiness of Severi varieties on Enriques surfaces}, Forum Math. - Sigma, {\bf 11} Paper No. e52, 32 pp. (2023).

\bibitem  {cdgk1} C. Ciliberto, Th. Dedieu, C. Galati, A. Knutsen:  {\it Severi varieties on blow-ups of the symmetric square of an elliptic curve}, Math. Nacthr., {\bf 296} (2), (2023), 574--587.

\bibitem  {cfgk} C. Ciliberto, F. Flamini, C. Galati, A. L. Knutsen: {\it  Moduli of nodal curves on K3 surfaces}, Adv. Math., {\bf 309} (2017), 624--654.

\bibitem{clm} C.~Ciliberto, A.~F.~Lopez, R.~Miranda: {\it Projective degenerations of $K3$ surfaces, 
Gaussian maps and Fano threefolds}, Invent. Math. {\bf 114} (1993), 641--667.

\bibitem {friedman} R.~Friedman: {\it Global smoothings of varieties with normal crossings}, Ann. of Math. {\bf 118} (1983), 75--114.


\bibitem{concettina1}
C.~Galati: {\it Degenerating curves and surfaces: first results},
Rend. Circ. Mat. Palermo {\bf 58} (2009), no. 2, 211--243.

\bibitem{concettina-andreas} C.~Galati, A.~L.~Knutsen: {\it On the existence of curves with $A_k$--singularities on $K3$ surfaces}, .
Math. Res. Lett. {\bf 21} (2014), no.5, 1069--1109.

\bibitem{concettina2} C.~Galati: {\it On the existence of curves with a triple point on a K3
surface},  Rend. Lincei Mat. Appl. {\bf 23} (2012), no. 3, 295--317.


\bibitem{gls} G.~M.~Greuel, C.~Lossen, E.~Shustin: {\em Introduction to Singularities and 
Deformations}, Springer Monographs in Mathematics, Springer (2007).


\bibitem{diaz-harris} S.~Diaz, J.~Harris: {\em Ideals associated to deformations of singular
plane curves}, Trans. Amer. Math. Soc. {\bf{309}} (1988), 433--468.

\bibitem{harris} J.~Harris: {\it On the Severi problem} Inventiones Math. {\bf 84} (1986), 445--461.


\bibitem{harris-morrison}
J.~Harris, I.~Morrison: {\it Moduli of Curves}, number 187 in Graduate Texts in Mathematics, 
Springer-Verlag, 1998.

\bibitem{hartshorne} R.~Hartshorne: {\em Algebraic Geometry},  
Graduate Texts in Mathematic {\bf 52}, Springer (1997).

\bibitem {ran} Z.~Ran: {\it Families of plane curves and their limits: Enriques' conjecture and beyond},  Annals of Math., {\bf 130} (1), (1989), 121--157.

\bibitem{ser} E.~Sernesi: {\em Deformations of Algebraic Schemes},  
A Series of Comprehensive Studies in Mathematics {\bf 334}, Springer--Verlag, Berlin, 2006.

\bibitem{severi} F.~Severi: {\it Vorlesungen $\ddot{u}$ber Algebraische Geometrie}, Teubner, Leipzig (1921).

\end{thebibliography}

\end{references}


\vskip .2cm \noindent
\textsc{%
Dipartimento di Matematica e Informatica, 
Universit\`a degli Studi della Calabria,
Via Pietro Bucci, cubo 31B,
87036 Arcavacata di Rende (CS), Italy} \\
\texttt{galati@mat.unical.it}



\stopcontents[04b.concettina]




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End: 
 	


==> 05.margherita/tacnodi.tex <==
% \input{enumTV}

% \begin{document}

\chaptitle{Deformations of an $m$-tacnode into $m-1$ nodes}
\chapauthor{Margherita Lelli-Chiesa}

\startchap
\label{05.margherita}

           \newcommand\Y{{\mathcal Y}}
          \newcommand\E{{\mathcal E}}
          
          \newcommand\bP{{\mathbb P}}
          
          \newcommand\W{\mathcal W}
          \newcommand\oo{\mathcal O}
          \newcommand\cO{\mathcal O}
          \newcommand\cM{\mathcal M}



\startcontents[05.margherita]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[05.margherita]{}{1}[2]{}

\let\mathbb\mathbf


\bigskip
This text is dedicated to a somewhat technical-looking statement
(Theorem~\ref{principale}) which is the cornerstone of many results
in this volume:
it is the key to understand the phenomenon of, loosely speaking,
$(m-1)$-nodal curves
degenerating to $m$-tacnodal curves within a degeneration of smooth
surfaces to the transverse union of two surfaces.
About this phenomenon see, in particular,
\cite{01.ciro, 04.concettina, 15.tacnodo}.


\section{Statement of results}

Let $C$ be a planar curve. A point $P\in C$ is called an $m$-tacnode if the local equation of $C$ at $P$ has the form $y(y+x^m)=0$, where $(x,y)$ are local coordinates centered at $P$. The Jacobian ideal of $C$ at $P$ is $J=(2y+x^m,yx^{m-1})$ and
$$
\mathcal{O}_{\mathbb{A}^2}/J=\langle y,xy,\ldots,x^{m-2}y,1,x,\ldots,x^{m-1}\rangle.
$$
We denote by $\pi:S\to \Delta$ the versal deformation space of $P\in C$, where $\Delta\simeq \mathbb{A}^{2m-1}_{\alpha_0,\ldots,\alpha_{m-2},\beta_0,\ldots,\beta_{m-1}}$, and $S\subset\Delta\times\mathbb{A}^2_{x,y}$ is defined by the equation 
\begin{equation}\label{equa}
y^2+yx^m+\alpha_{m-2}yx^{m-2}+\ldots+\alpha_1yx+\alpha_0y+\beta_{m-1}x^{m-1}+\ldots+\beta_1x+\beta_0=0,
\end{equation}
see \cite[Section~5]{02.edoardo}.
We set
\begin{eqnarray}
\Delta_m&:=&\{(\underline{\alpha},\underline{\beta})\in\Delta\,|\,\pi^{-1}(\underline{\alpha},\underline{\beta})\textrm{ has }m\textrm{ nodes}\},\\
\Delta_{m-1}&:=&\{(\underline{\alpha},\underline{\beta})\in\Delta\,|\,\pi^{-1}(\underline{\alpha},\underline{\beta})\textrm{ has }m-1\textrm{ nodes}\}.
\end{eqnarray}

\begin{proposition}
\label{prop:localgeom}
\def\fakesubparagraph{%
  \par\noindent%
  \refstepcounter{subparagraph}%
  {\normalfont \thesubparagraph}%
  }
\fakesubparagraph{}\label{uno}
The locus $\Delta_m$ is smooth of dimension $m-1$, and it is defined in $\Delta$ by the equations $\beta_0=\beta_1=\ldots=\beta_{m-1}=0$.
\fakesubparagraph{}\label{due}
The locus $\Delta_{m-1}$ has dimension $m$, and has $m$ local sheets
at a general point of $\Delta_m$.
\end{proposition}%

\begin{proof}
The equation of $\pi^{-1}(\underline{\alpha},\underline{\beta})$ has degree two in $y$ and its discriminant is given by
$$
\delta_{\underline{\alpha},\underline{\beta}}(x)=(x^m+\alpha_{m-2}x^{m-2}+\ldots+\alpha_1x+\alpha_0)^2-4(\beta_{m-1}x^{m-1}+\ldots+\beta_1x+\beta_0).
$$
If $V$ denotes the space of monic polynomials of degree $2m$ in $x$
with no degree $2m-1$  term, the regular map $\delta:\Delta\to V$ mapping a point $(\underline{\alpha},\underline{\beta})$ to its discriminant $\delta_{\underline{\alpha},\underline{\beta}}(x)$ is an isomorphism; indeed, $\underline{\alpha}$ and $\underline{\beta}$ can be easily expressed in terms of the coefficients of $\delta_{\underline{\alpha},\underline{\beta}}(x)$. We remark that, for fixed $(\underline{\alpha},\underline{\beta})$, the locus $\pi^{-1}(\underline{\alpha},\underline{\beta})$ is a double cover of the $x$-axis branched along the vanishing locus of $\delta_{\underline{\alpha},\underline{\beta}}(x)$, which is a divisor of degree $2m$. 

A point $(\underline{\alpha},\underline{\beta})$ lies in $\Delta_m$
whenever $\delta_{\underline{\alpha},\underline{\beta}}(x)$ has $m$
double roots, that is, if and only if
$\delta_{\underline{\alpha},\underline{\beta}}(x)$ is a square,
equivalently if and only if $\beta_0=\beta_1=\ldots=\beta_{m-1}=0$. This proves \ref{uno}.

Analogously, $(\underline{\alpha},\underline{\beta})$ lies in $\Delta_{m-1}$ exactly when $\delta_{\underline{\alpha},\underline{\beta}}(x)$ has $m-1$ double roots, that is, we can rewrite the discriminant as
\begin{equation}\label{radici}
  \delta_{\underline{\alpha},\underline{\beta}}(x)
  =\left( \prod_{i=1}^{m-1}(x-a_i)^2 \right) \cdot (x^2+bx+c),
\end{equation}
where in fact $b=2\sum_{i=1}^{m-1} a_i$ because the degree $2m-1$ term
of $\delta_{\underline{\alpha},\underline{\beta}}(x)$ vanishes. Hence,
$\Delta_{m-1}$ has dimension $m$, and the $m$ local sheets at a general
point of $\Delta_m$ as in \ref{due} reflect the possibilities for
choosing $m-1$ double roots out of $m$.
\end{proof}

Our main goal is to prove the following theorem.
\begin{theorem}[{\cite[Lemma 2.8]{CH0}}]
\label{principale}
Let $\Lambda\subset \Delta$ be a smooth $m$-dimensional variety such that:
\begin{compactenum}[(i)]
\item $\Lambda$ contains $\Delta_m$;
\item the tangent space $T_{\underline{0}}\Lambda$ of $\Lambda$ at $\underline{0}$ is not contained in the hyperplane $H$ defined by the equation $\beta_0=0$.
\end{compactenum}
Then, we have $\Lambda\cap\Delta_{m-1}=\Delta_m\cup\Psi$, where $\Psi$ is a smooth curve intersecting $\Delta_m$ at $\underline{0}$ with multiplicity $m$.
\end{theorem}

Note that $\Delta_{m-1}$ and $\Lambda$ both have codimension $m-1$ in
$\Delta$, which has dimension $2m-1$, so that the expected dimension
for their intersection is $1$. The theorem thus states that if
$\Lambda$ contains $\Delta_m$, under a suitable transversality
assumption, namely (ii), the intersection $\Lambda\cap\Delta_{m-1}$
residual to the obvious superabundant component $\Delta_m$ has the
expected dimension. 

The reader may also consult \cite{A.swallowtail} for complements and
detailed examples.

\section{Proof of the main theorem in
  a model case}

We first prove  Theorem \ref{principale}
in the special case where
$\Lambda=\Lambda_0=\{\beta_1=\ldots=\beta_{m-1}=0\}$. 

 Equation \eqref{equa} of $S$ restricted to $\Lambda$ is:
\begin{equation}\label{zione}
y^2+yx^m+\alpha_{m-2}yx^{m-2}+\ldots+\alpha_1yx+\alpha_0y+\beta_0=0,
\end{equation}
and the discriminant of a point $(\underline{\alpha},\underline{\beta})\in \Lambda$ has the form:
\begin{equation}\label{dis}
 \delta_{\underline{\alpha},\underline{\beta}}(x)=(x^m+\alpha_{m-2}x^{m-2}+\ldots+\alpha_1x+\alpha_0)^2-4\beta_0.
 \end{equation}
If $\beta_0=0$, then $(\underline{\alpha},\underline{\beta})$ lies in
$\Delta_m$. Therefore, $\Lambda\cap\Delta_{m-1}$ contains $\Delta_m$
with multiplicity $m$, since by Proposition~\ref{prop:localgeom}
$\Delta_{m-1}$ has multiplicity $m$ along $\Delta_m$.

From now on, we assume $\beta_0\neq 0$, set $\nu(x):=x^m+\alpha_{m-2}x^{m-2}+\ldots+\alpha_1x+\alpha_0$ and rewrite \eqref{dis} as:
\begin{equation}\label{cri}
\delta_{\underline{\alpha},\underline{\beta}}(x)=(\nu(x)-2\sqrt{\beta_0})(\nu(x)+2\sqrt{\beta_0}).
\end{equation}
Note that the polynomials $\nu(x)-2\sqrt{b}$ and $\nu(x)+2\sqrt{b}$
have no common roots since $\beta_0\neq 0$. We impose that
$\delta_{\underline{\alpha},\underline{\beta}}(x)$ has $m-1$ double
roots, taking advantage of the following lemma.

\begin{lemma}
\label{l:claim}
Let $\gamma:=2\sqrt{\beta_0}$ with $\beta_0\neq 0$. Then, for every integer $m\geq 2$ there exists a polynomial
$$
\nu_\gamma(x):=x^m+c_{m-2}(\gamma)x^{m-2}+\ldots+c_1(\gamma)x+c_0(\gamma)$$
in $x$ with complex coefficients $c_i(\gamma)$ such that $c_{m-2}(\gamma)\neq 0$ and the following are satisfied:
\begin{enumerate}[(a)]
\item if $m=2l+1$ is odd, then both $\nu_\gamma(x)+\gamma$ and $\nu_\gamma(x)-\gamma$ have $l$ double roots;
\item if $m=2l$ is even, then $\nu_\gamma(x)+\gamma$ (respectively, $\nu_\gamma(x)-\gamma$) has $l$ (resp., $l-1$) double roots.
\end{enumerate}
Furthermore, $\nu_\gamma(x)$ is unique up to replacing it with
$\nu_\gamma(\xi x)$ for some $m$-th root $\xi$ of unity, and it is odd
(respectively, even) if $m$ is.
\end{lemma}



Taking the lemma for granted, we set  $m:=2l+\epsilon$ with $\epsilon\in\{0,1\}$ depending on the parity of $m$ and consider the polynomial $$\nu_1(x)=x^m+c_{m-2}(1)x^{m-2}+c_{m-4}(1)x^{m-4}+\ldots+c_\epsilon(1)x^\epsilon$$ obtained for $\gamma=1$. For any other $\gamma\in\mathbb{C}^*$, by setting $\gamma:=u^m$, we get $\nu_\gamma(x)=u^m\nu_1\left(\frac{x}{u}\right)$. The coefficients of $\nu_\gamma(x)$ are thus obtained from those of $\nu_1(x)$ in the following way:
$$c_{2h+\epsilon}(\gamma)=c_{2h+\epsilon}(u)=u^{2l-2h}c_{2h+\epsilon}(1), \textrm{ for }0\leq h\leq l-1.$$
By the change of variable $t:=u^2$, the equations 
$$c_{2h+\epsilon}(t)=t^{l-h}c_{2h+\epsilon}(1), \textrm{ for }0\leq h\leq l-1$$
parametrize a curve $\Psi_0$ in $\Lambda\cap\Delta_{m-1}$. This curve is smooth because $c_{m-2}(1)\neq0$, and its contact order with $\Delta_m$ at $\underline{0}$  is $m$ because $\beta_0=\frac{t^m}{4}$. Therefore, it only remains to prove the lemma.


\begin{proof}[Proof of Lemma~\ref{l:claim}]
We first prove the existence of a degree $m$ covering $f:\mathbb{P}^1\to\mathbb{P}^1$ mapping $\infty$ to $\infty$ and with $\{\infty,\gamma,-\gamma\}$ as branch locus; we also require $f$ to be totally ramified at $\infty$ and the number of ramification points in the fiber $f^{-1}(-\gamma)$ (respectively, in $f^{-1}(\gamma)$) to coincide with the number of double roots  we are requiring for the polynomial $\nu_\gamma(x)+\gamma$ (respectively, $\nu_\gamma(x)-\gamma$). 

Assume that $m=2l+1$ is odd. By Riemann's Existence Theorem, the
existence of $f$ is equivalent to the existence of two permutations
$\tau,\sigma$ in the symmetric group $S_m$, each one the product of $l$ disjoint transpositions, such that $\tau\cdot\sigma$ is cyclic of order $m$ in $S_m$. The permutations $\tau:=(1\,2)(3\,4)\cdots(2l-1\, 2l)$ and $\sigma:=(2\,3)(4\,5)\cdots(2l\,2l+1)$ satisfy these requirements and they are the only elements of $S_m$ doing that, up to conjugation. As a consequence, $f$ exists and is unique up to automorphisms of the domain fixing $\infty$. The even case is analogous.

Since $f(\infty)=\infty$, the covering $f$  defines a polynomial
$\nu_\gamma(x)$ satisfying (a) or (b) respectively. By acting with an
automorphism of $\mathbb{P}^1$ fixing $\infty$ (\ie composing
$\nu_\gamma(x)$ with a polynomial of degree $1$), we can assume
$\nu_\gamma(x)$ to be monic and with no degree $m-1$ term. The
polynomial $\nu_\gamma(x)$ is then unique up to replacing it with
$\nu_\gamma(\xi x)$ for some $m$-th root $\xi$ of unity. By
Proposition \ref{chev} in the Appendix, we can therefore assume that
$\nu_1(x)$ coincides with the Chebyshev polynomial of the first kind
$T_m(x)$; in particular, it is even or odd depending on the parity of
$m$,
and the coefficient $c_{m-2}(1)$ is nonzero, as one can easily check using \eqref{cheby} in the Appendix. The same properties hold for $\nu_\gamma(x)$ for any $\gamma=u^m\in\mathbb{C}^*$ because $\nu_\gamma(x)=u^m\nu_1\left(\frac{x}{u}\right)$.

\end{proof}


\section{Proof of  the main theorem in general}

We now prove Theorem \ref{principale} in full generality.

We consider the blow-up $\tau:\widetilde{\Delta}\to\Delta$ of $\Delta$ along $\Delta_m$ and denote by $Z:=\tau^{-1}(\Delta_m)$ the exceptional divisor and by $\Phi:=\tau^{-1}(\underline{0})$ the inverse image of $\underline{0}$. Then $\Phi\simeq \mathbb{P}^{m-1}_{\beta_0,\ldots,\beta_{m-1}}$ can be identified with the space of polynomials of degree at most $m-1$ in $x$ modulo scalars. The open subset $\Phi\supset\Phi_0:=\{\beta_0\neq 0\}$ parametrizes polynomials that do not vanish in $x=0$ and the point $Q=[1:0:\ldots:0]\in \Phi_0$ corresponds to constants. The proof of Theorem \ref{principale} in general is based on the description of the strict transform $\widetilde{\Delta_{m-1}}$ of $\Delta_{m-1}$ in $\widetilde{\Delta}$ and proceeds by steps.

\begin{step}
\label{stepI}
  The point $Q$ lies in $\widetilde{\Delta_{m-1}}$.
\end{step}


Let $\widetilde{\Lambda_0}$ be the strict transform of the linear
space $\Lambda_0=\{\beta_1=\ldots=\beta_{m-1}=0\}$ under $\tau$. We
have already shown that $\Lambda_0\cap\Delta_{m-1}=\Delta_m\cup\Psi_0$
as in Theorem \ref{principale}. Since
$\widetilde{\Lambda_0}\cap\Phi=\{Q\}$, then $Q$ lies in the strict
transform $\widetilde{\Psi_0}$ of the curve $\Psi_0$ and hence also in
$\widetilde{\Delta_{m-1}}$.


\begin{step}
\label{stepII}
  The locus $\Phi$ is an irreducible component of
  $\widetilde{\Delta_{m-1}}\cap Z$ and is the only component
  containing $Q$.
\end{step}


We identify $\Delta_m$ with the space of monic polynomials of degree
$m$ in $x$ with no degree $m-1$ term. Let $\alpha(t)\subset\Delta_m$
be any arc such that $\alpha(0)=\underline{0}$. As $t$ goes to $0$,
all the roots of the polynomial corresponding to $\alpha(t)$ tend to
$x=0$ and hence the limit of $\tau^{-1}(\alpha(t))\cap
\widetilde{\Delta_{m-1}}$ is not contained in $\Phi_0$. As  a
consequence, any component of $\widetilde{\Delta_{m-1}}\cap Z$
containing $Q$ is contained in $\Phi$, and thus coincides with it by
dimensional reason.


\begin{step}
\label{stepIII}
  The strict transform $\widetilde{\Delta_{m-1}}$ is smooth at $Q$.
\end{step}


The previous step implies that the only irreducible component of
$\widetilde{\Lambda_0}\cap \widetilde{\Delta_{m-1}}$ containing $Q$ is
the curve $\widetilde{\Psi_0}$. In particular, the intersection is
proper in a neighborhood of $Q$ (indeed,
$\dim\widetilde{\Lambda_0}
=\dim \widetilde{\Delta_{m-1}}
=m$,
and $\dim\widetilde{\Delta}=2m-1$); smoothness of $\widetilde{\Psi_0}$
thus yields smoothness of $\widetilde{\Delta_{m-1}}$ at $Q$.


\begin{step}
\label{stepIV}
The strict transform $\widetilde{\Delta_{m-1}}$ is smooth at every point of $\Phi_0$.
\end{step}


 For every $c\in \mathbb{C}^*$, let $\sigma_c$ be the automorphism of $\Delta$ such that $\sigma_c(\alpha_i)=c^{m-i}\alpha_i$ for $0\leq i\leq m-2$ and $\sigma_c(\beta_j)=c^{2m-j}\beta_j$ for $0\leq j\leq m-1$. This defines an action of the multiplicative group $\mathbb{C}^*$ on $\Delta$, under which $\Delta_m$ is clearly invariant. Since $\delta_{\sigma_c(\underline{\alpha}),\sigma_c(\underline{\beta})}(x)=c^{2m}\delta_{\underline{\alpha},\underline{\beta}}\left(\frac{x}{c}\right)$, then $\Delta_{m-1}$ is invariant, too. As a consequence, the action of $\mathbb{C}^*$ on $\Delta$ lifts to an action on $\widetilde{\Delta}$ preserving $\widetilde{\Delta_{m-1}}$. Furthermore, $\underline{0}$ is a fixed point lying in the closure of any orbit and hence the lifted action also preserves $\Phi$. In particular, given $c\in \mathbb{C}^*$, we obtain an automorphism $\widetilde{\sigma_c}$ of $\Phi$ mapping a point $P$ of homogeneous coordinates $[\beta_0:\beta_1:\ldots:\beta_{m-1}]$ to $$\widetilde{\sigma_c}(P)=[c^{2m}\beta_0:c^{2m-1}\beta_1:\ldots:c^{m+1}\beta_{m-1}]= [\beta_0:c^{-1}\beta_1:\ldots:c^{-(m-1)}\beta_{m-1}].$$ Since the limit for $c^{-1}$ going to $0$ of $\widetilde{\sigma_c}(P)$ is $Q$ as soon as $\beta_0\neq 0$, this shows that $Q$ lies in the closure of any orbit of $\widetilde{\Delta_{m-1}}$ intersecting $\Phi_0$. The statement thus follows from Step~\ref{stepIII}.


\begin{step}
\label{stepV}
The intersection multiplicity of $\widetilde{\Delta_{m-1}}$ and $Z$ along $\Phi$ is $m$.
\end{step}


Since the intersection multiplicity of $\Psi_0$ and $\Delta_m$ at $\underline{0}$ is $m$, then the same holds for that of $\widetilde{\Psi_0}$ and $Z$ at $Q$. On the other hand, the intersection $\widetilde{\Psi_0}\cap Z$ is contained in $\widetilde{\Delta_{m-1}}\cap Z\cap\widetilde{\Lambda_0}$, and the intersection multiplicity  at $Q$ of $\Phi$ (which is the only component of $\widetilde{\Delta_{m-1}}\cap Z$ containing $Q$ by Step~\ref{stepII}) with $\widetilde{\Lambda_0}$ is $1$, because $\widetilde{\Lambda_0}\cap Z$ is a section of $\tau\vert_Z:Z\to\Delta_m$. The statement follows.


\begin{step}
Conclusion.
\end{step}


Let $\Delta_m\subset \Lambda\subset \Delta$ be as in the hypotheses. Since $\widetilde{\Lambda}\cap Z$ is a section of $\tau\vert_Z:Z\to\Delta_m$, then the intersection $\widetilde{\Lambda}\cap \Phi$ is a point $R$ with multiplicity one. The assumption $T_{\underline{0}}\Lambda\not\subseteq H=\{\beta_0=0\}$ ensures that $R$ lies in $\Phi_0$ and hence $\widetilde{\Delta_{m-1}}$ is smooth at $R$ by Step~\ref{stepIV}. The $m$-dimensional tangent space $T_R\widetilde{\Delta_{m-1}}$ contains $T_R\Phi$, that has dimension $m-1$. Since $T_R\widetilde{\Lambda}\cap T_R\Phi=\{0\}$ and $\dim T_R\widetilde{\Lambda}=m$, then $T_R\widetilde{\Delta_{m-1}}$ and $T_R\widetilde{\Lambda}$ generate the ($2m-1$)-dimensional tangent space $T_R\widetilde{\Delta}$. Equivalently, $\widetilde{\Delta_{m-1}}$ and $\widetilde{\Lambda}$ intersect transversally along a smooth curve $\widetilde{\Psi}$ in a neighborhood of $R$. Moreover, the curve $\widetilde{\Psi}$ is not tangent at $\Phi$ in $R$ (again because $T_R\widetilde{\Lambda}\cap T_R\Phi=\{0\}$) and its intersection multiplicity with $Z$ at $Q$ is $m$ by Step~\ref{stepV}. Therefore, $\Psi:=\tau(\widetilde{\Psi})$ is a smooth curve having intersection multiplicity $m$ with $\Delta_m$ at $\underline{0}$.



\setcounter{section}{0}
\renewcommand{\thesection}{\Alph{section}}
\section{Appendix: Chebyshev polynomials}
There exist four families of Chebyshev polynomials, $T_m, U_m, V_m, W_m$ --- called of the first, second, third and fourth kind --- each satisfying
\begin{equation}\label{cheby}
  P_0(x) = 1, \quad
  \text{and} \quad
  \forall m\geq 1:
  \quad P_{m+1}(x) = 2xP_m(x) - P_{m-1}(x).
\end{equation}
They may be defined by the following choice of initial conditions:
\begin{eqnarray}
T_1(x) & = & x,\\
U_1(x) & = & 2x,\\
V_1(x) & = & 2x - 1,\\
W_1(x) & = & 2x + 1.
\end{eqnarray}
They are the unique polynomials satisfying
\begin{eqnarray}
T_m(\cos \theta) & = & \cos(m\theta),\\
U_m(\cos \theta) & = & \frac{\sin((m+1)\theta)}{\sin \theta},\\
V_m(\cos \theta) & = & \frac{\cos((m+1/2)\theta)}{\cos(\theta/2)},\\
W_m(\cos \theta) & = & \frac{\sin((m+1/2)\theta)}{\sin(\theta/2)}
\end{eqnarray}
for all $\theta \in \R$.
The Chebyshev polynomials of the first kind can be explicitly written
down as
$$T_m(x) = \frac 1 2 \Bigl[
\bigl(x + \sqrt{x^2 - 1}\bigr)^m +
\bigl(x - \sqrt{x^2 - 1}\bigr)^m \Bigr],
$$ and are even (respectively, odd) whenever $m$ is even (respectively, odd). Polynomials of the third and fourth kind satisfy $W_m(x) = (-1)^m V_m(x)$.

These are the first few values of Chebyshev polynomials:
\begin{eqnarray*}
T_0(x) & = & 1,\\
T_1(x) & = & x,\\
T_2(x) & = & 2x^2 - 1,\\
T_3(x) & = & 4x^3 - 3x,\\
T_4(x) & = & 8x^4 - 8x^2 + 1, \dots\\
\\
U_0(x) & = & 1,\\
U_1(x) & = & 2x,\\
U_2(x) & = & 4x^2 - 1,\\
U_3(x) & = & 8x^3 - 4x,\\
U_4(x) & = & 16 x^4 - 12x^2 +1, \dots\\
\\
V_0(x) & = & 1,\\
V_1(x) & = & 2x - 1,\\
V_2(x) & = & 4x^2 - 2x - 1,\\
V_3(x) & = & 8x^3 - 4x^2 - 4x + 1,\\
V_4(x) & = & 16 x^4 - 8x^3 - 12x^2 + 4x + 1, \dots\\
\\
W_0(x) & = & 1,\\
W_1(x) & = & 2x + 1,\\
W_2(x) & = & 4x^2 + 2x - 1,\\
W_3(x) & = & 8x^3 + 4x^2 - 4x - 1,\\
W_4(x) & = & 16 x^4 + 8x^3 - 12x^2 - 4x + 1\dots
\end{eqnarray*}
The next result summarizes some properties of Chebyshev polynomials.

\begin{proposition}\label{chev}
If $m=2l$ is even, then
\begin{itemize}
\item[(a1)]
$T_{m}(x) + 1 = 2 (T_l(x))^2$,
\item[(a2)]
$T_{m}(x) - 1 = 2(x^2-1)(U_l(x))^2$;
\end{itemize}
in particular, the polynomial $T_{m}(x) + 1$ is a perfect square, while $T_{m}(x) - 1$ is the product of a perfect square by a degree two polynomial.

If instead $m= 2l+1$ is odd, then:
\begin{itemize}
\item[(b1)] $T_{m}(x) + 1 = (x+1)V_l(x)^2$,
\item[(b2)] $T_m(x) - 1 = (x-1)W_l(x)^2$;
\end{itemize}
in particular, both $T_{m}(x) + 1$ and $T_{m}(x) -1$ are the product of a perfect square by a linear polynomial.
\end{proposition}

\begin{proof}
Set $x = \cos \theta$. If $m=2l$ is even, then $T_{m}(x) + 1 = \cos(2l\theta) + 1 = 2\cos^2(l\theta) = 2 (T_l(x))^2$. Similarly,
$$T_{m}(x) - 1 = \cos(2l\theta) - 1 = -2\sin^2(l\theta)
= -2\sin^2 \theta \cdot \frac{\sin^2(l\theta)}{\sin^2 \theta}
= 2(x^2-1)(U_l(x))^2.$$
If instead $m = 2l+1$ is odd, one has
$$T_{m}(x) + 1 = \cos(m\theta) + 1 = 2\cos^2(m\theta/2) = 2\cos^2(\theta/2) \cdot \frac{\cos^2(m\theta/2)}{\cos^2(\theta/2)} =(x+1)(V_l(x))^2,$$
and
$$T_{m}(x) - 1 = \cos(m\theta) - 1 = -2\sin^2(m\theta/2)
= -2\sin^2(\theta/2) \cdot \frac{\sin^2(m\theta/2)}{\sin^2(\theta/2)}
=(x-1)(W_l(x))^2.$$
\end{proof}





\begin{references}

\begin{thebibliography}[Chapters in this Volume]{1}
%\let\ref\tmpref

\bibitem[\tref{01.ciro}]{01.ciro}
C.~Ciliberto,
\emph{Limits of nodal curves: generalities and examples}.

\bibitem[\tref{02.edoardo}]{02.edoardo}
E.~Sernesi,
\emph{Deformations of curves on surfaces}.

\bibitem[\tref{04.concettina}]{04.concettina}
Th.~Dedieu, C.~Galati,
\emph{Degenerations and deformations of generalized Severi varieties}.

\bibitem[\tref{15.tacnodo}]{15.tacnodo}
C.~Ciliberto, Th.~Dedieu, C.~Galati,
\emph{Flag semi-stable reduction of tacnodal curves at the limit
  of nodal curves}.

\bibitem[\tref{A.swallowtail}]{A.swallowtail}
Th.~Dedieu,
\emph{Geometry of the deformation space of an $m$-tacnode
into $m-1$ nodes}.

\end{thebibliography}

\begin{thebibliography}[External References]{1}

\bibitem{CH0}
  L.~Caporaso, J.~Harris,
  \emph{Parameter spaces for curves on surfaces and enumeration of
  rational curves}, Compositio Math. \textbf{113} (1998), no.~2, 155--208.

\end{thebibliography}

\end{references}

\stopcontents[05.margherita]

%\end{document}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End: 
 	


==> 06.francesco/06.francesco.tex <==
\chaptitle{Products of deformation spaces of tacnodes}
\chapauthor{Francesco Bastianelli}

\startchap
\label{06.francesco}

% \begin{abstract}
% This short note retraces \cite[Section 4.2]{ch}, concerning Caporaso and Harris' description of products of deformation spaces of higher-order tacnodes.
% This is a lecture given by the author on the occasion of the seminar
%   \emph{Degenerazioni e enumerazione di curve su una superficie}
%   held at University of Rome Tor Vergata in 2015--2017.
% \end{abstract}


\startcontents[francesco]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[francesco]{}{1}[2]{}

\section{Introduction}

This lecture retraces \cite[Section 4.2]{ch}, and concerns Caporaso and Harris' description of products of deformation spaces of higher-order tacnodes. 
Of course, this description relies on the analysis included in \cite{05.margherita} about deformations of a single tacnode. 
The main result of this lecture shall be involved in the proof of
\cite[\tref{04.concettina.main}]{04.concettina}, which is
\cite[Theorem 1.3]{ch},
% Replace \cite[Theorem 1.3]{ch} with the corresponding result in the Lecture Notes
in order to describe the local geometry of hyperplane sections of generalized Severi varieties $V^{d,\delta}(\alpha,\beta)$, around a point $[X_0]$ parameterizing a reducible curve $X_0=X\cup L$ endowed with some tacnodes of orders $m_j$, each deforming to $m_j-1$ nodes on the curves parameterized nearby.

\medskip
We consider a sequence $\underline{m}:=\left(m_1,m_2,\dots,m_n\right)$ of integers $m_j\geq 2$, and we set
\begin{displaymath}
\displaystyle\lambda:=\lcm\left\{m_j\right\}, \qquad \mu:=\prod_j m_j, \qquad \kappa:=\frac{\mu}{\lambda},
\end{displaymath}
where $\lcm$ denotes the least common multiple.\\
For any $1\leq j\leq n$, let $\left(C_j,p_j\right)$ be a tacnode of order $m_j$, and let $\pi_j\colon \mathcal{S}_j\longrightarrow \Delta_j$ be the corresponding versal deformation family described in \cite{05.margherita}.
Therefore, $\Delta_j\cong \mathbb{A}^{2m_j-1}$ is an affine space with coordinates $\left(\underline{a}_j,\underline{b}_j\right)=\left(a_{j,m_j-2},\dots,a_{j,0},b_{j,m_j-1},\dots,b_{j,0}\right)$, the subscheme $\mathcal{S}_j\subset \mathbb{A}^2\times \Delta_j$ has equation 
\begin{displaymath}
y^2+\left(x^{m_j}+a_{j,m_j-2}x^{m_j-2}\dots +a_{j,0}\right)y+b_{j,m_j-1}x^{m_j-1}+\dots +b_{j,0}=0,
\end{displaymath}
and $\pi_j\colon \mathcal{S}_j\longrightarrow \Delta_j$ is the second projection.
Moreover, we introduce the subloci $\Delta_{j,m_j}$ and $\Delta_{j,m_j-1}$ of $\Delta_j$ as 
\begin{displaymath}
\displaystyle\Delta_{j,m_j}:=\overline{\left\{\left(\underline{a}_j,\underline{b}_j\right)\in \Delta_j\left|\pi_j^{-1}\left(\underline{a}_j,\underline{b}_j\right)\text{ is a curve having }m_j\text{ nodes}\right.\right\}}
\end{displaymath}
and 
\begin{displaymath}
\displaystyle\Delta_{j,m_j-1}:=\overline{\left\{\left(\underline{a}_j,\underline{b}_j\right)\in \Delta_j\left|\pi_j^{-1}\left(\underline{a}_j,\underline{b}_j\right)\text{ is a curve having }m_j-1\text{ nodes}\right.\right\}}.
\end{displaymath}
We recall that $\Delta_{j,m_j}\cong \mathbb{A}^{m_j-1}$ is the linear
$(m_j-1)$-dimensional subspace given by the equations
$b_{j,m_j-1}=\dots=b_{j,0}=0$, and it is the locus over which the
fibers $\pi_j^{-1}\left(\underline{a}_j,\underline{b}_j\right)$ are
reducible plane curves, whereas $\Delta_{j,m_j-1}$ is an
$m_j$-dimensional subvariety containing $\Delta_{m_j}$. 

Then we define
\begin{displaymath}
\displaystyle\Delta:=\Delta_{1}\times\dots\times \Delta_n,
\end{displaymath}  
\begin{displaymath}
\displaystyle\Delta_{\underline{m}}:=\Delta_{1,m_1}\times\dots\times\Delta_{n,m_n},
\end{displaymath}  
and
\begin{displaymath}
\displaystyle\Delta_{\underline{m}-1}:=\Delta_{1,m_1-1}\times\dots\times\Delta_{n,m_n-1},
\end{displaymath}  
so that $\Delta\cong \mathbb{A}^{\Sigma(2m_j-1)}$ is an affine space
endowed with coordinates
$\left(\underline{a}_1,\underline{b}_1,\dots,\underline{a}_n,\underline{b}_n\right)$,
the linear subspace $\Delta_{\underline{m}}\cong
\mathbb{A}^{\Sigma(m_j-1)}$ is given by equations
$\left\{ b_{j,i}=0,\
  1\leq j\leq n,
  \ 0\leq i\leq
  m_{j}-1 \right\}$, and  $\Delta_{\underline{m}-1}$ is a subvariety of
dimension $\sum m_j$ containing $\Delta_{\underline{m}}$. 
Finally, we set 
\begin{displaymath}
H:=\bigcup_j \left\{b_{j,0}=0\right\},
\end{displaymath} 
which is a union of hyperplanes of $\Delta$.

We now state the main result of this lecture (\cf \cite[Lemma 4.3]{ch}).
Along the same lines as \cite[\tref{principale}]{05.margherita}
(\cf \cite[Lemma 4.1]{ch}),
it describes the local intersection at the origin $\underline{0}\in
\Delta$ between $\Delta_{\underline{m}-1}$ and varieties
$W\subset \Delta$ containing $\Delta_{\underline{m}}$ as a subvariety
of codimension 1 and satisfying a suitable transversality assumption.

\begin{lemma}\label{lemma 4.3}
Let $W\subset \Delta$ be a smooth subvariety of dimension $\sum (m_j-1)+1$ containing $\Delta_{\underline{m}}$, and such that the tangent space $T_{\underline{0}}W$ at the origin $\underline{0}\in \Delta$ is not contained in $H$.
Then, in an \'etale neighborhood of the origin,
\begin{displaymath}
W\cap \Delta_{\underline{m}-1}=\Delta_{\underline{m}}\cup\Gamma_1\cup\Gamma_2\cup\dots\cup\Gamma_\kappa,
\end{displaymath}
where $\Gamma_1,\dots,\Gamma_\kappa\subset W$ are distinct reduced unibranched curves such that each $\Gamma_\alpha$ has intersection multiplicity $\left(\Gamma_\alpha\cdot \Delta_{\underline{m}}\right)_{\underline{0}}=\lambda$ with $\Delta_{\underline{m}}$ at the origin, and the origin is a point of multiplicity $\mathrm{mult}_{\underline{0}}\left(\Gamma_\alpha\right)=\frac{\lambda}{\max_j \left\{m_j\right\}}$ of $\Gamma_\alpha$. 
\end{lemma}

Note that $\Delta_{\underline{m}-1}$ has codimension $\sum(m_j-1)$ in
$\Delta$, so the expected dimension of the intersection
$W \cap \Delta_{\underline{m}-1}$ is $1$.

\begin{remark}
\begin{inparaenum}[(i)]
\item 
The intersection multiplicity at $\underline{0}\in\Delta$ between $\Delta_{\underline{m}}$ and the reducible curve $\Gamma:=\Gamma_1\cup\dots\cup\Gamma_\kappa$ is $\left(\Gamma\cdot \Delta_{\underline{m}}\right)_{\underline{0}}=\kappa\lambda=\mu$, in analogy with the case of a single tacnode.

\item
If $\lambda=m_j$ for some $j$, then all the curves $\Gamma_\alpha$ are smooth.
\end{inparaenum}
\end{remark}

\medskip
Before proving Lemma \ref{lemma 4.3}, we state another result which shall turn out to be equivalent to it.
We denote by 
\begin{displaymath}
\widetilde{\Delta}:=\mathrm{Bl}_{\Delta_{\underline{m}}}\Delta\stackrel{\pi}{\longrightarrow} \Delta
\end{displaymath}
the blow-up of $\Delta$ along $\Delta_{\underline{m}}$.
Let $E\subset \widetilde{\Delta}$ be the exceptional divisor, and let $F:=\pi^{-1}\left(\underline{0}\right)\subset E$ be the fibre over the origin $\underline{0}\in \Delta$.
Finally, let $\widetilde{\Delta}_{\underline{m}-1}$ and $\widetilde{H}$ denote the proper transforms of $\Delta_{\underline{m}-1}$ and $H$, respectively.
Then the following holds (\cf \cite[Lemma 4.4]{ch}).
\begin{lemma}\label{lemma 4.4}
The intersection $\widetilde{\Delta}_{\underline{m}-1}\cap E$ contains $F$ as a component of multiplicity $\mu$.
Moreover, in an \'etale neighborhood of any point $p\in F$ not contained in $\widetilde{H}$, the variety $\widetilde{\Delta}_{\underline{m}-1}$ consists of $\kappa$ reduced branches, each having multiplicity $\frac{\lambda}{\max_j \left\{m_j\right\}}$ along $F$, intersection number $\lambda$ with $E$ along $F$, and tangent cone at $p$ supported on a linear space contained in $E$.
\end{lemma}



\section{Proofs}

In analogy with the argument used to deduce \cite[Lemma 4.1]{ch},
the proof of Lemma \ref{lemma 4.3} proceeds in three steps.
The first one consists of proving the assertion when $W$ is assumed to be a linear space.
Then we use it to achieve Lemma \ref{lemma 4.4}. 
Finally, we conclude by deducing Lemma \ref{lemma 4.3} for an arbitrary subvariety $W$ satisfying the hypothesis of the statement. 

\paragraph{Proof of Lemma \ref{lemma 4.3} with linear $W\subset
  \Delta$}

We assume that $W\cong \mathbb{A}^{\Sigma\left(m_j-1\right)+1}$ is a linear subspace of $\Delta$ such that $\Delta_{\underline{m}}\subset W$ and $W=T_{\underline{0}}W\not\subset H$.
Thus $\Delta_{\underline{m}}\subset H$ is a hyperplane in $W$,
and we may choose a point $v\in \Delta\smallsetminus H$ such that
$W=\langle \Delta_{\underline{m}}, v\rangle$, \ie $W$ is the linear span of $\Delta_{\underline{m}}$ and $v$.

For any $1\leq j\leq n$, let $\rho_j\colon \Delta\longrightarrow \Delta_j$ be the $j^{\mathrm{th}}$ projection, and let $t\colon W\longrightarrow \mathbb{C}$ be a non-zero linear function vanishing along the hyperplane $\Delta_{\underline{m}}$.
We note that $\rho_j\left(\Delta_{\underline{m}-1}\right)=\Delta_{m_j-1}$ and $\rho_j\left(\Delta_{\underline{m}}\right)=\Delta_{m_j}$.
Moreover, setting $W_j:=\rho_j(W)$ and $v_j:=\rho_j(v)$, we have that $v_j\in W_j\smallsetminus \Delta_{m_j}$ as $v\not\in H$.
Thus $W_j=\langle \Delta_{m_j}, v_j\rangle\subset \Delta_j$ is an $m_j$-dimensional plane not contained in the hyperplane $\left\{b_{j,0}=0\right\}$.
In particular $W_j$ satisfies the hypothesis of
\cite[\tref{principale}]{05.margherita},
%\cite[Lemma 4.1]{ch}
so the intersection between $\Delta_{m_j-1}$ and $W_j$ in $\Delta_j$ consists of the union of $\Delta_{m_j}$ and a smooth curve $\Gamma_j$ having intersection multiplicity $\left(\Gamma_j\cdot \Delta_{m_j}\right)_{\underline{0}}=m_j$ with $\Delta_{m_j}$ at the origin $\underline{0}\in \Delta_j$. 
Therefore, in some \'etale neighborhood of the origin
$\underline{0}\in W_j$, we may choose local coordinates
$\left(x_{j,0},\dots,x_{j,m_j-2},t_j\right)$ such that
$\rho_j^*\left(t_j\right)=t$,%
\footnote{It suffices to choose $t_j\colon W_j\longrightarrow
  \mathbb{C}$ to be a linear function such that
  $t_j(\Delta_{m_j})=0$ and $t_j(v_j)=t(v)$.}
$\Delta_{m_j}$ is the hyperplane with equation $t_j=0$, and the curve $\Gamma_j$ is defined by 
the equations
\begin{displaymath}
x_{j,1}=\dots=x_{j,m_j-2}=0\quad\text{and}\quad t_j=\left(x_{j,0}\right)^{m_j}.
\end{displaymath}

Then the functions $t=\rho_j^*\left(t_j\right)$ and $y_{j,i}:=\rho_j^*\left(x_{j,i}\right)$, with $1\leq j\leq n$ and $1\leq i\leq m_j-2$, define a system of local coordinates on some \'etale neighborhood of $W$ at the origin.
It follows from their very definition that the intersection $W\cap \Delta_{\underline{m}-1}$ consists of the plane $\Delta_{\underline{m}}=\left\{t=0\right\}$ and of the subvariety $\Gamma$ defined by 
the equations
\begin{equation}\label{equation etale coordinates}
t=\left(y_{j,0}\right)^{m_j}\quad\text{ and }\quad y_{j,i}=0,
\qquad
\text{for $1\leq j\leq n$ and $1\leq i\leq m_j-2$.}
\end{equation}
We point out that $\Gamma$ is a curve, as for any fixed value of $t\in
\mathbb{C}$, there exist finitely many $\bigl((\sum m_j-1)
+1\bigr)$-tuples $\left(y_{1,0},\dots,y_{n,m_n-2},t\right)$ satisfying
\eqref{equation etale coordinates}, which depend only on the choice of
an $m_j^{\text{th}}$ root of $t$ for each coordinate $y_{j,0}$.  

In order to parameterize any branch of $\Gamma$, let us consider a sequence $\underline{\zeta}:=\left(\zeta_1,\zeta_2,\dots,\zeta_n\right)$ such that each $\zeta_j$ is a $m_j^{\text{th}}$ root of unity.
Then we define a local parameterization $\varphi_{\underline{\zeta}}\colon \mathbb{C}\longrightarrow W$ as 
\begin{equation}\label{equation parameterization of Gamma}
\displaystyle z\longmapsto \left\{
\begin{array}{ccll}
t & = & z^{\lambda} & \\
y_{j,0} & = &\displaystyle  \frac{z^{\frac{\lambda}{m_j}}}{\zeta_j} & \text{for }1\leq j\leq n  \\   
y_{j,i} & = & 0 & \text{for }1\leq j\leq n\text{ and }1\leq i\leq m_j-2,     
\end{array}\right.
\end{equation}
and we denote by $\Gamma_{\underline{\zeta}}$ its image.
Notice that the map $\varphi_{\underline{\zeta}}$ is injective.%
\footnote{ Suppose that $\varphi_{\underline{\zeta}}(z)=\varphi_{\underline{\zeta}}(w)$ for some $z,w\in \mathbb{C}$. 
Then $(z/w)^{\frac{\lambda}{m_j}}=1$ for any $j$, hence $z/w$ is a $\nu^{\mathrm{th}}$ root of unity, where $\nu$ divides any $\frac{\lambda}{m_j}$.
Thus $\nu=1$ as $\lambda$ is the least common multiple of the integers $m_j$, hence $z=w$.}
Furthermore, every branch of $\Gamma$ can be parameterized in this way: for any point $\underline{y}\in\Gamma$ with coordinates $\left(y_{1,0},\dots,y_{n,m_n-2},t\right)$, it is enough to choose a $\lambda^{\mathrm{th}}$ root $z$ of $t$ and set $\zeta_{j}=z^{\frac{\lambda}{m_j}}/y_{j,0}$, which is an $m_j^{\text{th}}$ root of unity by \eqref{equation etale coordinates}.
We also point out that the multiplicity of $\Gamma_{\underline{\zeta}}$ at the origin is the least power of $z$ appearing in the parameterization, \ie $\mathrm{mult}_{\underline{0}}(\Gamma_{\underline{\zeta}})=\frac{\lambda}{\max_j \left\{m_j\right\}}$.
On the other hand, the intersection multiplicity at the origin between $\Gamma_{\underline{\zeta}}$ and the hyperplane $\Delta_{\underline{m}}=\left\{t=0\right\}$ is $\bigl(\Gamma_{\underline{\zeta}}\cdot \Delta_{\underline{m}}\bigr)_{\underline{0}}=\lambda$, as $t = z^{\lambda}$ on $\Gamma_{\underline{\zeta}}$.
Therefore the behavior of the branches of $\Gamma$ satisfies the statement, and it remains to enumerate them.

To this aim, we note that two distinct sequences
$\underline{\zeta}:=\left(\zeta_1,\zeta_2,\dots,\zeta_n\right)$ and
$\underline{\eta}:=\left(\eta_1,\eta_2,\dots,\eta_n\right)$
parameterize the same branch if and only if
$\zeta_j=\varepsilon^{\frac{\lambda}{m_j}}\eta_j$ for all $j$,
where $\varepsilon$ is
some $\lambda^{\mathrm{th}}$ root of unity.%
\footnote{
  Indeed,
  $\varphi_{\underline{\zeta}}(z)=\varphi_{\underline{\eta}}(w)$ for
  some $z,w\in \mathbb{C}$ if and only if $(z/w)^{\lambda}=1$ and
  $\eta_j z^{\frac{\lambda}{m_j}}=\zeta_j w^{\frac{\lambda}{m_j}}$,
  that is $z=\varepsilon w$ for some $\lambda^{\mathrm{th}}$ root
  $\varepsilon$ of unity and
  $\zeta_j=\varepsilon^{\frac{\lambda}{m_j}} \eta_j$.}

Moreover, $\zeta_j=\varepsilon^{\frac{\lambda}{m_j}}\zeta_j$ for any $j$ if and only if $\varepsilon=1$ \footnote{ Notice that $\varepsilon^{\frac{\lambda}{m_j}}=1$ for any $j$ if and only if $\varepsilon$ is a $\nu^{\mathrm{th}}$ root of unity, where $\nu$ divides any $\frac{\lambda}{m_j}$. Hence $\nu=1$.}.
We conclude that the number of branches of $\Gamma$ equals the number of sequences  $\underline{\zeta}:=\left(\zeta_1,\zeta_2,\dots,\zeta_n\right)$ divided by the number of $\lambda^{\mathrm{th}}$ roots of unity, that is $\kappa=\frac{\mu}{\lambda}$.
Thus we achieved Lemma \ref{lemma 4.3} when $W$ is assumed to be a linear subspace of $\Delta$.
\qed
%\end{proof}


We now turn to prove Lemma \ref{lemma 4.4}.

\paragraph{Proof of Lemma \ref{lemma 4.4}}
Let $G$ be the Grassmannian of vector subspaces of $\Delta\cong \mathbb{A}^{\Sigma (2m_j-1)}$ of dimension $\sum (m_j-1) +1$, and let $B\cong \mathbb{P}^{\Sigma m_j -1}$ be the subvariety of $G$ parameterizing those subspaces containing $\Delta_{\underline{m}}\cong \mathbb{A}^{\Sigma (m_j-1)}$.
Let $W_{\underline{b}}$ denote the subspace parameterized by $\underline{b}\in B$, and consider the incidence variety $\Lambda:=\left\{\left.(\underline{y},\underline{b})\in \Delta\times B\right| \underline{y}\in W_{\underline{b}}\right\}\subset \Delta\times B$. 
Then $\Lambda$ is the restriction to $B$ of the universal family over $G$, and it fits in the following diagram
\begin{equation}\label{diagram Grassmannian}
\xymatrix{ \Lambda \ar[d]_{\mathrm{pr}_1} \ar[dr]^{\mathrm{pr}_2} & \\ \Delta \ar@{-->}[r]^{\psi}   & B, }
\end{equation}
where $\mathrm{pr}_1$ and $\mathrm{pr}_2$ are the natural projections, while $\psi$ is the map sending any $\underline{y}\in\Delta\smallsetminus\Delta_{\underline{m}}$ to the point parameterizing the linear span $\langle \underline{y},\Delta_{\underline{m}}\rangle\subset \Delta$ \footnote{We note that $B$ is naturally identified with the projectivization $\mathbb{P}\left(\Delta/\Delta_{\underline{m}}\right)\cong \mathbb{P}^{\Sigma m_j -1}$ of the quotient $\Delta/\Delta_{\underline{m}}$. Under this identification, we may view $\psi$ as the map sending a point $\underline{y}=\left(\underline{a}_1,\underline{b}_1,\ldots \underline{a}_n,\underline{b}_n\right)\in \Delta\smallsetminus \Delta_{\underline{m}}$ to the point $\underline{b}\in  \mathbb{P}\left(\Delta/\Delta_{\underline{m}}\right)$ having homogeneous coordinates $\underline{b}=\left[\underline{b}_1,\ldots ,\underline{b}_n\right]$.}.
We point out that $\mathrm{pr}_1\colon \Lambda \longrightarrow \Delta$ is an isomorphism outside $(\mathrm{pr}_1)^{-1}\left(\Delta_{\underline{m}}\right)$, whereas the fibre $(\mathrm{pr}_1)^{-1}(\underline{y})$ over any point $\underline{y}\in \Delta_{\underline{m}}$ is a section of $\mathrm{pr}_2$, that is a projective space of dimension $\sum m_j -1$.
Therefore $\mathrm{pr}_1\colon \Lambda \longrightarrow \Delta$ coincides with the blow-up $\widetilde{\Delta}:=\mathrm{Bl}_{\Delta_{\underline{m}}}\Delta\stackrel{\pi}{\longrightarrow} \Delta$ of $\Delta$ along $\Delta_{\underline{m}}$ (see, \eg \cite[p.604]{gh}).
\footnote{In other terms, the dominant rational map $\psi\colon \Delta\dashrightarrow \mathbb{P}\left(\Delta/\Delta_{\underline{m}}\right)$ can be resolved to a morphism by blowing up $\Delta$ along the indeterminacy locus $\Delta_{\underline{m}}$.}.

 Consider the proper transforms $\widetilde{\Delta}_{\underline{m}-1},\widetilde{H}\subset \widetilde{\Delta}$ of $\Delta_{\underline{m}-1}$ and $H$.
Let $\widetilde{\Delta}_{\underline{m}-1}^0\subset \widetilde{\Delta}_{\underline{m}-1}$ and $\Delta_{\underline{m}-1}^0\subset \Delta_{\underline{m}-1}$ denote the open subsets of points not lying on $\widetilde{H}$ and $H$, respectively, and let $B_0\subset B$ be the open subvariety parameterizing subspaces not contained in $H$.
Then the diagram \eqref{diagram Grassmannian} restricts to
\begin{equation}\label{diagram Blow-up}
\xymatrix{\widetilde{\Delta}_{\underline{m}-1}^0 \ar[d]_{\pi_0} \ar[dr]^{\tau_0} & \\ \Delta_{\underline{m}-1}^0 \ar[r]^{\psi_0}   & B_0. }
\end{equation}  
We note that the closure
$\overline{(\psi_0)^{-1}(\underline{b})}\subset
\Delta_{\underline{m}-1}$ of the fibre over a point $\underline{b}\in
B_0$ is the residual intersection
of $\Delta_{\underline{m}-1}$ and the subspace $W_{\underline{b}}$
when we remove $\Delta_{\underline{m}}$.
By Lemma \ref{lemma 4.3} applied to $W_{\underline{b}}\cong
\mathbb{A}^{\Sigma(m_j-1)+1}$, in some \'etale neighborhood of the
origin $\underline{0}\in \Delta$, the latter intersection consists of $\kappa$ distinct reduced unibranched curves $\Gamma_1,\dots,\Gamma_{\kappa}$, each satisfying $\left(\Gamma_\alpha\cdot \Delta_{\underline{m}}\right)_{\underline{0}}=\lambda$ and $\mathrm{mult}_{\underline{0}}\left(\Gamma_\alpha\right)=\frac{\lambda}{\max_j \left\{m_j\right\}}$.
Notice that the proper transform
$\widetilde{W}_b=(\mathrm{pr}_2)^{-1}(\underline{b})$ of $W_b$ meets
the fibre $F:=\pi^{-1}(\underline{0})$ at a single point $p\in
\widetilde{\Delta}\smallsetminus \widetilde{H}$
(recall that $\pi: \widetilde{\Delta} \to \Delta$ is the blow-up is
the blow-up along $\Delta_{\underline m}$, which identifies with
$\pr_1: \Lambda \to \Delta$).
It follows that in some \'etale neighborhood of $p$, the closure of the fibre $(\tau_0)^{-1}(\underline{b})\subset \widetilde{\Delta}_{\underline{m}-1}$ consists of the proper transforms $\widetilde{\Gamma}_1,\dots,\widetilde{\Gamma}_{\kappa}$ of the curves $\Gamma_\alpha\subset \Delta_{\underline{m}-1}$. 
Moreover, any $\widetilde{\Gamma}_\alpha$ is a reduced unibranched curve such that 
\begin{equation}\label{equation multiplicity 1}
\bigl(\widetilde{\Gamma}_\alpha\cdot E\bigr)_{p}=\bigl(\Gamma_\alpha\cdot \Delta_{\underline{m}}\bigr)_{\underline{0}}=\lambda
\end{equation} 
and 
\begin{equation}\label{equation multiplicity 2}
\bigl(\widetilde{\Gamma}_\alpha\cdot F\bigr)_p=\mathrm{mult}_{\underline{0}}\bigl(\Gamma_\alpha\bigr)=\frac{\lambda}{\max_j \left\{m_j\right\}},
\end{equation}
by the Projection Formula and \cite[Lemma 1.40 p.28]{ko}.

Finally, as we vary $\underline{b}\in B_0$, each $\widetilde{\Gamma}_\alpha$ describes a reduced branch $\widetilde{\Delta}^\alpha$ of $\widetilde{\Delta}_{\underline{m}-1}$ having multiplicity $\frac{\lambda}{\max_j \left\{m_j\right\}}$ along $F$, intersection number $\lambda$ with $E$ along $F$, and since the curves $\widetilde{\Gamma}_\alpha$ are unibranched, the tangent cone to $\widetilde{\Delta}^\alpha$ at $p$ is supported on a linear space contained in $E$.
In particular, the intersection $\widetilde{\Delta}_{\underline{m}-1}\cup E$ contains the whole fibre $F$, with multiplicity given by the sum of the intersection multiplicities along $F$ between $E$ and each branch of $\widetilde{\Delta}_{\underline{m}-1}$, that is $\kappa\lambda=\mu$. 
\qed
%\end{proof}


Finally, we conclude this lecture by proving Lemma \ref{lemma 4.3} for an arbitrary subvariety $W\subset \Delta$ satisfying the hypothesis of the statement.

\paragraph{Proof of Lemma \ref{lemma 4.3}}
Let $W\subset \Delta$ be a smooth $\left(\sum(m_j-1) +1\right)$-dimensional variety containing $\Delta_{\underline{m}}$ and such that $T_{\underline{0}}W\not\subset H$.
By the smoothness of $W$, its proper transform $\widetilde{W}\subset
\widetilde{\Delta}$ intersects the exceptional divisor $E$
transversally, and cuts out on the latter a section over
$\widetilde{\Delta}_{\underline{m}}$. 
Moreover, since $T_{\underline{0}}W\not\subset H$, we have that
$\widetilde{W}$ meets $F:=\pi^{-1}(\underline{0})$ at a single point
$p\in \widetilde{\Delta}$ which lies off $\widetilde{H}$, hence $T_p\widetilde{W}\cap T_pF=\left\{0\right\}$.
By Lemma \ref{lemma 4.4}, in some \'etale neighborhood of $p$, the variety $\widetilde{\Delta}_{\underline{m}-1}$ consists of $\kappa$ reduced sheets $\widetilde{\Delta}^1,\dots,\widetilde{\Delta}^n$, and the tangent cone to a branch $\widetilde{\Delta}^\alpha$ at $p$ is supported on a linear space $L\subset E$.
In particular, $T_pF\subset L\subset E$.
We notice that $\dim L=\dim \widetilde{\Delta}^\alpha=\sum m_j$, and $\dim T_pF=\dim F=\sum m_j -1=\dim \widetilde{\Delta}^\alpha-1$.
Thus $\dim\bigl(T_p\widetilde{W}\cap L\bigr)\leq 1$, so that the linear span of $T_p\widetilde{W}$ and $L$ satisfies 
\begin{eqnarray*}
\dim \langle T_p\widetilde{W},L\rangle & \geq & \dim T_p\widetilde{W} +\dim L -1=\sum (m_j-1)+1+\sum m_j -1\\
& = & \sum (2m_j-1)=\dim \widetilde{\Delta},
\end{eqnarray*}
that is $\langle T_p\widetilde{W},L\rangle=T_p\widetilde{\Delta}$. 
Therefore, the intersection around $p$ between $\widetilde{W}$ and $\widetilde{\Delta}^\alpha$ is transverse, and it consists of a unibranched reduced curve $\widetilde{\Gamma}_\alpha$ such that $\bigl(\widetilde{\Gamma}_\alpha\cdot F\bigr)_p$ equals the multiplicity $\frac{\lambda}{\max_j \left\{m_j\right\}}$ of $\widetilde{\Delta}^\alpha$ along $F$, and $\bigl(\widetilde{\Gamma}_\alpha\cdot E\bigr)_{p}$ is the intersection number $\lambda$ between $\widetilde{\Delta}^\alpha$ and $E$ along $F$.

For any $1\leq \alpha\leq \kappa$, we consider the reduced curve $\Gamma_\alpha:=\pi\bigl(\widetilde{\Gamma}_\alpha\bigr)$, and  in some \'etale neighborhood of the origin, we have 
$$\Delta_{\underline{m}-1}\cap W=\Delta_{\underline{m}}\cup \Gamma_1\cup \dots\cup\Gamma_\kappa.$$ 
Since each $\widetilde{\Gamma}_\alpha$ meets $E$ only at the point $p$, the curve $\Gamma_\alpha$ is unibranched as well.
Furthermore, by arguing as in \eqref{equation multiplicity 1} and \eqref{equation multiplicity 2}, we deduce that each $\Gamma_\alpha$ satisfies $\mathrm{mult}_{\underline{0}}\left(\Gamma_\alpha\right)=\bigl(\widetilde{\Gamma}_\alpha\cdot F\bigr)_p=\frac{\lambda}{\max_j \left\{m_j\right\}}$ and $\left(\Gamma_\alpha\cdot \Delta_{\underline{m}}\right)_{\underline{0}}=\bigl(\widetilde{\Gamma}_\alpha\cdot E\bigr)_{p}=\lambda$.
Thus Lemma \ref{lemma 4.3} follows.
\qed
%\end{proof}



\begin{references}

\begin{thebibliography}[Chapters in this Volume]{1}
%\let\ref\tmpref
  
\bibitem[\tref{04.concettina}]{04.concettina}
  Th.~Dedieu {\normalfont \smfandname} C.~Galati,
  \emph{Degenerations and deformations of generalized Severi varieties}.
  
\bibitem[\tref{05.margherita}]{05.margherita}
  M.~Lelli-Chiesa,
  \emph{Deformations of an $m$-tacnode into $m-1$ nodes}.

\end{thebibliography}

\begin{thebibliography}[External References]{1}

\bibitem{ch}
L.~Caporaso {\normalfont \smfandname} J.~Harris, \emph{Counting plane curves of any genus}, Invent. Math. \textbf{131} (1998), no.~2, 345--392.

\bibitem{gh}
P.~A.~Griffiths {\normalfont \smfandname} J.~Harris, \emph{Principles of Algebraic Geometry}, Pure and Applied Mathematics, Wiley Interscience, New York, 1978.

\bibitem{ko}
J.~Koll\'ar, \emph{Lectures on resolution of singularities}, Annals of Mathematics Studies 166, Princeton University Press, Princeton, NJ, 2007.

\end{thebibliography}

\end{references}

\stopcontents[francesco]






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End:


==> 15.tacnodo/tacnodo.tex <==
\chaptitle{Flag semi-stable reduction of tacnodal curves at the limit
  of nodal curves}
\chapauthor{Ciro Ciliberto, Thomas Dedieu, and Concettina Galati}

\startchap
\label{15.tacnodo}


% macros specifiques tacnodo
\let\oldsharp\sharp
\def\sharp#1{\vphantom{#1}^\oldsharp \kern -.1em #1}

\def\e{\epsilon}

\newenvironment{figbox}
{\noindent\begin{minipage}{\textwidth}
\begin{center}}
{\end{center}
\end{minipage}}


%%%%%%%%
%% smash
% For comparison, the existing overlap macros:
% \def\llap#1{\hbox to 0pt{\hss#1}}
% \def\rlap#1{\hbox to 0pt{#1\hss}}
\def\clap#1{\hbox to 0pt{\hss#1\hss}}
\def\mathllap{\mathpalette\mathllapinternal}
\def\mathrlap{\mathpalette\mathrlapinternal}
\def\mathclap{\mathpalette\mathclapinternal}
\def\mathllapinternal#1#2{%
\llap{$\mathsurround=0pt#1{#2}$}}
\def\mathrlapinternal#1#2{%
\rlap{$\mathsurround=0pt#1{#2}$}}
\def\mathclapinternal#1#2{%
\clap{$\mathsurround=0pt#1{#2}$}}


\renewcommand{\O}{\mathcal{O}}

\setdefaultenum{(i)}{}{}{}
%\setdefaultitem{---}{}{}{}

\renewcommand{\figurename}{Figure}


\startcontents[15.tacnodo]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[15.tacnodo]{}{1}[2]{}


\newcommand{\taf}[1]{{\color{blue}#1}}


\section*{Introduction}

The objective of this note is to provide down-to-earth
explanations of the following phenomenon, which is a
central theme of the present collection of articles.
It is studied in detail in \cite{05.margherita},
following Caporaso and Harris \cite{CH0,CH},
and in \cite{04b.concettina} in the same context that we are
considering here;
it also appears in various guises in many other places.

Let $\cS \to \A^1$ be a family of surfaces such that the general
member $S_t$, $t\neq 0$, is a smooth projective surface, and the
central member $S_0$ is the union of two smooth projective
surfaces intersecting transversely along a smooth curve $B$.
Let $\cL$ be a line bundle on $\cS$, and consider the family of Severi
varieties 
\[
\mathring\cV =
\coprod\nolimits _{t \neq 0} V^1(S_t,L_t)
\longrightarrow \mathring\A^1 = \A^1 -\{0\},
\]
where $V^1(S_t,L_t)$ is the family of $1$-nodal curves in the
linear system $|L_t|$ on the surface $S_t$,
with $L_t=\restr {\mathcal L} {S_t}$.
Let $V_0$ be the family of curves in the linear system $|L_0|$ on
$S_0$ having a \emph{tacnode} along $B$, \ie $V_0$ is the family of curves
$C_0 \in |L_0|$, such that there exists a point $p \in B \cap C_0$, at
which $C_0$ locally consists of two smooth branches $C_0' \subset
S_0'$ and $C_0'' \subset S_0''$, both of which are tangent to $B$ at
$p$.
Then, at least in principle, $V_0$ appears in
the central fibre of the closure $\smash{\overline\cV}$ of
$\mathring{\cV}$, with multiplicity $2$.

We carry out a detailed local study of the nodes degenerating to a
tacnode in the above situation, with stable reduction as a central
concept.
We investigate in particular the following questions,
with various points of view:
\begin{inparaenum}
\item in which way is such a tacnodal curve of the appropriate genus?
\item why does it count with multiplicity $2$?
\item
\label{q:sstable}
how should one modify the family of surfaces in order to see a
tacnodal limit curve in $S_0$ as a nodal curve in an alternative
semi-stable limit of the $S_t$'s?
\end{inparaenum}

The multiplicity $2$ is fairly straightforward to understand, \cf
\ref{p:mult2}.
Seeing the tacnodal curve
as a curve of the appropriate genus may be done in various ways,
according to the chosen point of view, and is not always
straightforward. We do provide a solution to
problem~\eqref{q:sstable}, but the conclusion is that although it is
possible to see one tacnodal limit curve as a nodal curve in some
semi-stable limit of the $S_t$'s, it is impossible to do it
simultaneously for all
curves of the family $V_0$. Therefore, tacnodal curves in the
degeneration cannot be avoided, and have to be considered as
definitely acceptable limits of nodal curves in their own right:
in \cite[Section \tref{s:Severi-1}]{01.ciro}, a degeneration of surfaces
is said to be well-behaved if the limits of Severi varieties can all
be accounted for, up to some reduction, by families of nodal and
tacnodal curves: the upshot of our discussion here is that it is
hopeless to ask that the limits of Severi varieties be accounted for
only by families of nodal curves.

The text is organized as follows.
Section~\ref{S:synth} is meant as an overview of this note, and
hopefully clarifies in what sense we study the questions (i-ii-iii)
mentioned above:
in this section,
% In Section~\ref{S:synth},
we outline various ways of viewing a
tacnodal curve as an 
appropriate limit of $1$-nodal curves,
% by working out a global example
in order to illustrate all the local computations performed in the
subsequent sections.
In Section~\ref{S:equations}, we give the equations of the local
situation we want to study, namely
$1$-nodal curves in smooth surfaces degenerating to a tacnodal curve in the
transverse union of two smooth surfaces.
In Section~\ref{S:abstract-normaliz}, we perform the stable reduction
of a family of $1$-nodal curves degenerating to a tacnodal curve,
forgetting about the ambient degeneration of surfaces.
The stable reduction process in this section is rather simple
(we first normalize the total space, which normalizes the general
fibres, then do some modifications, 
and finally return to $1$-nodal general fibres), but it
is unfortunately not suitable to answer question (iii) above.
Therefore, 
in Section~\ref{S:abstract-nodal}, we compute the same stable reduction
without normalizing the total space.
% as the method of
% Section~\ref{S:abstract-normaliz} is no longer suitable when we take
% the degeneration of surfaces into account.
Finally, we are able to answer question~\eqref{q:sstable} in
Section~\ref{S:flag}, providing what we call a
\emph{flag semi-stable reduction} of the nodes degenerating to a tacnode
inside surface sheets degenerating to two smooth transverse sheets.
The name refers to the fact that we perform semi-stable reduction
simultaneously for the family of curves and for the ambient family of
surfaces.



\section{Synthetic descriptions of nodal curves 
degenerating to tacnode}
\label{S:synth}

In this section we outline various ways to see a tacnodal
curve as the (equigeneric) limit of nodal curves, in the context
described in the introduction above.
We do not enter in too many details for the moment; a fully rigorous
treatment will be given in the next sections.

\paragraph{An example of ambient deformation space}
We will follow throughout this section the guiding example of smooth
quartics degenerating to two quadrics, and their hyperplane sections.

Let  $\cS \to \A^1$ be  a pencil of quartic hypersurfaces in $\P^3$,
generated by a general quartic $S_\infty$, and the sum $S_0$ of two
smooth quadrics $S_0'$ and $S_0''$ intersecting transversely along a
quartic elliptic normal curve $B$.
The total space $\cS$ has ordinary double points at the finitely many
points of $S_\infty \cap B$, which 
one usually prefers to resolve in one way or another;
in our context we can safely ignore this, as our study is local, away
from the incriminated points.
This example is described in more detail in
\cite[\tref{ssec:3nodal:1st}]{01.ciro}.

\paragraph{Degeneration of smooth curves}
A general hyperplane section $C_t$ of $S_t$, $t\neq 0$, is a smooth plane
quartic, and thus has genus $3$. On the other hand, a general hyperplane
section $C_0$ of $S_0$ is the union of two non-degenerate conics meeting
transversely at $4$ points: it has arithmetic genus $3$, and it is a
stable curve of genus $3$.

\begin{figbox}
\includegraphics[width=\textwidth]{synth0.eps}
\captionof{figure}
{Degeneration of smooth curve sections}
\label{fig:synth0}
\end{figbox}

\noindent
On Figure~\ref{fig:synth0} above, the curves $C_0'$ and $C_0''$ are
pictured in $S_0=S_0'\cup S_0''$ following a tropically inspired
design, which is well suited
for our drawings, see \cite{11.th-toric-trop}.


\newlength{\synth}
\settoheight{\synth}{\includegraphics[width=\textwidth]{synth0.eps}}


\paragraph{Degeneration of $1$-nodal curves}
Continuing with our example of a pencil of quartic surfaces,
we now consider for the rest of this section a family of $1$-nodal
hyperplane sections $C_t$ of $S_t$, $t\neq 0$,
degenerating to a tacnodal hyperplane section
$C_0' \cup C_0''$ of $S_0$, \ie $C_0'$ and $C_0''$ are
non-degenerate conics on $S_0'$ and $S_0''$ respectively,
tangent to $B$ at some point $q$, and meeting
transversely at two other points $p_1,p_2 \in B$
(recall that $B$ is the curve $S_0' \cap S_0''$). 

\subparagraph{An abuse of presentation}
In fact, as we shall see in Section \ref{S:equations}, such a family
must be $2$-valued, \ie the curve $C_t$ must consist of two $1$-nodal
hyperplane sections for $t\neq 0$, and the central fibre $C_0$ must be
the double of $C_0'\cup C_0''$ on $S_0$.
This is an important point but we shall ignore it for the moment,
while we are outlining the situation, as it is not the aspect we want
to focus on in this note.
Thus, for the sake of keeping this outline simple,
we shall pretend for the rest of this section that the curves
$C_t$ are irreducible $1$-nodal curves, and $C_0$ is a reduced
tacnodal curve, without any further mention.
In particular, on
Figure~\ref{fig:synth1} and the other figures in this section,
we only picture one $1$-nodal curve tending to
$C_0'\cup C_0''$, whereas in fact there are two.
From Section~\ref{S:equations} on, our treatment will be fully
rigorous without any abuse of presentation. 

\medskip
\begin{figbox}
\includegraphics[height=\synth]{synth1.eps}
\captionof{figure}
{Degeneration of $1$-nodal curves to a tacnodal curve}
\label{fig:synth1}
\end{figbox}

\medskip
The curves $C_t$, $t\neq 0$, have geometric genus $2$. In the next
paragraphs we give various ways of appropriately seeing $C_0$ as a
genus $2$ limit of the $C_t$'s.


\paragraph{Degeneration of the normalizations}
\label{p:synth2}
We may incarnate the $1$-nodal curves $C_t$, $t\neq 0$, as the stable
maps $\bar C_t \to S_t$ given by the normalizations $\bar C_t \to
C_t$; these are maps from smooth, genus $2$, sources.
From this perspective, the relevant incarnation of the curve $C_0$ is
as the image of a stable map as pictured
on Figure~\ref{fig:synth2} below, with source a stable, genus
$2$, curve consisting of two smooth rational components meeting transversely
at three points
(this source is a partial normalization of the tacnode of $C_0$).

\begin{figbox}
\includegraphics[height=\synth]{synth2.eps}
\captionof{figure}
{Degeneration of the normalizations of $1$-nodal curve sections}
\label{fig:synth2}
\end{figbox}

\medskip
To see this, one considers the family $\cC$ of the curves $C_t$, $t\in
\A^1$, and normalize it. It follows from Teissier's simultaneous
resolution theorem \cite{teissier} that the fiber of the normalization
$\bar \cC$ over $t\neq 0$ is the normalization $\bar C_t$. The fibre
over $0$ is computed in \ref{p:abs-normaliz} below; it is singular over the
tacnode, because there is a jump in $\delta$-invariant when the node
of $C_t$ degenerates to the tacnode of $C_0$.
This is compensated for by the
jump in the number of irreducible components, which allows for
the genus to be constant.

\bigskip
The latter point of view is arguably the more transparent. It is yet
also desirable to understand the situation by
seeing the curves $C_t$ as singular curves in the
surfaces $S_t$. 

\paragraph{Degeneration of the stable maps}
\label{p:synth3}
The $1$-nodal curves $C_t$ are stable curves of arithmetic genus $3$. As
such, their limit $C_0$ can be modified into a stable curve of genus
$3$. In other words, the closed immersions $C_t \hookrightarrow S_t$
are stable maps of genus $3$, and have a limit as such. These limits
are pictured on Figure~\ref{fig:synth3} below.

\begin{figbox}
\includegraphics[height=\synth]{synth3.eps}
\captionof{figure}
{Degeneration as stable maps of the immersions of $1$-nodal curve
  sections} 
\label{fig:synth3}
\end{figbox}

\medskip
The component $D$ on Figure~\ref{fig:synth3}
is a $1$-nodal rational curve ($p_a=1$ and $p_g=0$);
it is contracted to the tacnode of $C_0$ by the stable map with target
$S_0$ which is the limit of the maps $C_t \hookrightarrow S_t$.
The computations are carried out in Section~\ref{S:abstract-normaliz}.

One nice feature of this point of view is that we see our limit of
curves of arithmetic genus $3$ with $1$ node as a curve of arithmetic
genus $3$ with $1$ node as well; the node in question is that of the
component $D$
(of course, the source of the limit stable map has other nodes;
what we are saying is that the node of $D$ is the limit of the node of
$C_t$ as $t$ tends to $0$).
The price one pays is that this stable limit of maps has a contracted
component.

\subparagraph{Observation}\medskip
The above model may be used to recover that described in 
\ref{p:synth2}.
To do so, one  simultaneously normalizes the nodes of all the
curves $C_t$: on the central fibre, this normalizes the node of $D$,
which then becomes a destabilizing smooth rational component; the
stable model of the central fibre is obtained by contracting this
component, which gives the central fibre of the family of curves
described in \ref{p:synth2}.

\paragraph{Degeneration of the stable maps, II}
\label{p:synth4}
It frequently happens in practice that one has to modify the family of
surfaces $\cS \to \A^1$ 
% by ``filling some bellows of the accordion
% between $S_0'$ and $S_0''$''
by adding one or more ruled surfaces
over $B$ between $S_0'$ and $S_0$. Typically, one performs a base
change $t \in \A^1 \mapsto t^m \in \A^1$, and then resolves the
singularities of the obtained family.
In particular, the description below is very useful to understand
\cite{07.th-diag-degen}.

Let us assume here that there is one ruled surface $\Sigma_B$ over $B$
between 
our two quadrics $S_0'$ and $S_0''$, and that our family of surfaces
has reduced central fibre. In this model of $\cS$, our tacnodal curve
$C_0$ is modified as indicated on Figure~\ref{fig:synth4},
by the adding of (i) reduced fibres of $\Sigma_B$ to
connect the points on $C_0'$ and $C_0''$ that previously were 
transverse intersection points of $C_0'$ and $C_0''$, and
(ii) one double
fibre to connect the two points that previously were the tacnode.

\medskip
\begin{figbox}
\includegraphics[height=\synth]{synth4.eps}
\captionof{figure}
{Degeneration as stable maps of the immersions of $1$-nodal curve
  sections, II} 
\label{fig:synth4}
\end{figbox}

\medskip
The stable map limit of the immersions $C_t \hookrightarrow S_t$ 
in this context is easily deduced from the limit in
paragraph~\ref{p:synth3}. The two intersection points between $C_0'$
and $C_0''$ are replaced by smooth rational curves $F_1$ and $F_2$,
mapped isomorphically to the corresponding fibres of $\Sigma_B$.
The nodal curve $D$ on the other hand is mapped $2:1$ to the double
fibre ``at the tacnode'', with ramification divisor the sum of the two
points $D\cap C_0'$ and $D \cap C_0''$; the node of $D$ is mapped to
the limit of the nodes of the curves $C_t$ as $t$
approaches $0$, which lies on the double fibre of $\Sigma_D$;
the pre-image of this point in $D$ consists only of the node of $D$.

Alternatively, this limit may be computed using the reduction
which we discuss next, and which is constructed in
Section~\ref{S:flag}.

\paragraph{Flag semi-stable reduction}
Ultimately, one may desire to see the stable limit of the $1$-nodal
curves $C_t$, depicted in Figure~\ref{fig:synth3}, not mapped to $S_0$
with some contracted components, but rather immersed in some
semi-stable limit of the surfaces $S_t$. It is of course asserted by
the general stable reduction theorems that this is possible, provided
one allows the replacement of the stable limit of the $C_t$'s by
another semi-stable model.
We carry this out explicitly in Section~\ref{S:flag}, and the result
is depicted in Figure~\ref{fig:flag-red} there.
We dub this a \emph{flag semi-stable reduction} of the pairs
$(C_t,S_t)$, $t\neq 0$.


\section{The local situation}
\label{S:equations}


In this section, we set up an explicit incarnation of the situation
that we study throughout this text, of a family of $1$-nodal curves
degenerating to a tacnodal curve inside a degeneration of smooth
surfaces to the transverse union of two smooth surfaces.
This is the same setup as in \cite{05.margherita}.

\begin{notation}
\label{notation}
The notation $\A^4_{xyzt}$ denotes the affine $4$-space equipped with
affine coordinates $(x, y, z, t)$; we will also use obvious
variations,
\eg $\A^1_t$ denotes the affine line with affine coordinate $t$.
Similarly, $\P^1_{x:y}$ denotes the projective line with homogeneous
coordinates $(x:y)$, and obvious variations will be used.

The arrow $\A^4_{xyzt}\to \A^1_t$ without further indication denotes
the affine projection map $(x, y, z, t) \in \A^4 \to t\in \A^1$.
\end{notation}

\paragraph{}
We consider the degeneration of surfaces $\cS \to \A^1_t$, where 
the total space $\cS$ is the hypersurface of $\A^4_{xyzt}$
defined by the equation
\begin{equation*}
\cS: xy=t,
\end{equation*}
and the map $\cS \to \A^1_t$ is the restriction of the affine projection
$\A^4_{xyzt}\to \A^1_t$.

For all $t\neq 0$, the fibre $S_t$ of $\cS$ over $t$ is smooth and irreducible, whereas
the central fibre $S_0$ is the union of two planes
$S_0'$ and $S_0''$, defined by the equations 
$t=y=0$ and $t=x=0$ respectively,
which intersect transversely along the line defined by the equations
$x=y=t=0$.

\paragraph{}
\label{p:nod-to-tac}
We want to study degenerations of nodal curves to a tacnodal curve
inside this degeneration of surfaces, \ie families of curves $\cC \to
\A^1$ fitting in a commutative diagram
\begin{equation*}
\xymatrix@=10pt{
\cC \ar@{}|\subset[r] \ar[dr] & \cS \ar[d] \\
& \mathrlap{\A^1} \hphantom{\A}
}
\end{equation*}
such that the fibres $C_t$ with $t \neq 0$ are $1$-nodal curves, and
the central fibre $C_0$ is a curve with a tacnode along the double
curve of $S_0$, by which we mean that $C_0$ consists of two smooth
branches $C_0'$ and $C_0''$ contained in $S_0'$ and $S_0''$
respectively, which intersect in only one point where they are both
tangent to the curve $S_0' \cap S_0''$.

\paragraph{}
As a matter of fact, families of curves as in \ref{p:nod-to-tac}
cannot exist, because if they would, then the singularities of the
curves would form a section of $\cS \to \A^1$ meeting the central
fibre along its double curve, which is impossible since the total
space $\cS$ is smooth.

As we shall now see, there exist instead families of curves with
central fibre the double of the curve $C_0$ as in 
\ref{p:nod-to-tac} above, and fibre over $t\neq 0$ the sum of two
$1$-nodal curves.
We let, indeed, $\sharp\cC \to \A^1_t$ be defined in
$\cS$ by the equation
\begin{equation*}
\sharp\cC: \bigl(x+y-z^2\bigr)^2 = 4t.
\end{equation*}
Its central fibre is indeed the double of a tacnodal curve $C_0$ as
described in 
\ref{p:nod-to-tac}: it is defined by $t=0$, and thus
it is the double of the curve with the following
equations in $\A^3_{xyz}$ (the latter being the central fibre of
$\A^4_{xyzt}\to\A^1_t$):
\begin{equation*}
\left\{
\begin{aligned}
xy &= 0 \\
x+y-z^2 &= 0
\end{aligned}
\right.
\quad \iff\quad 
\left\{
\begin{aligned}
y(y-z)^2 = 0 \\
-x = y-z^2.
\end{aligned}
\right.
\end{equation*}
On the other hand, for all $t_0 \neq 0$, the fibre 
$\sharp C_{t_0}$ consists of two irreducible $1$-nodal curves
$C_{t_0} ^\pm$, with the following equations in
$\A^3_{xyz}$, the fibre of $\A^4_{xyzt}\to\A^1_t$ over $t_0$:
\begin{equation}
\label{eq:Cpm_t_0}
\left\{
\begin{aligned}
-xy +t_0 &= 0 \\
x +y-z^2 \mp 2 \sqrt{t_0} &= 0
\end{aligned}
\right.
\quad \iff\quad 
\left\{
\begin{aligned}
(y \mp \sqrt{t_0})^2-yz^2 =0 \\
-x = y-z^2 \mp 2 \sqrt {t_0}.
\end{aligned}
\right.
\end{equation}


\paragraph{}
\label{p:mult2}
The family $\sharp\cC$ inside $\cS$ over $\A^1$ is the universal local
model for $1$-nodal curves in smooth surfaces degenerating to a
tacnodal curve along the transverse intersection of two smooth surface
sheets. 

The necessity of having two $1$-nodal curves in each fibre $S_t$,
$t\neq 0$, tending to the tacnodal curve $C_0$ explains why a tacnodal
curve in the limit amounts for (at least) two $1$-nodal curves.

\paragraph{}
\label{p:def:Cpm}
Next, we shall perform a degree $2$ base
change in order to separate  $\sharp\cC$ in two
distinct families $\cC^+$ and $\cC^-$ with the same central fibre
$C_0$. 

Thus, let $\tilde\cS \to \A^1_t$ be the family of surfaces with
total space defined by
\begin{equation*}
\tilde\cS: xy=t^2
\end{equation*}
in $\A^4_{xyzt}$, and with the map 
$\tilde\cS \to \A^1_t$ given by the affine projection
$\A^4_{xyzt}\to \A^1_t$.
Note that $\tilde\cS$ is singular along the double
curve of its central fibre $S_0$. There are two families of 
$1$-nodal curves tending to a curve with a tacnode along the double curve
of $S_0$, namely $\cC^\pm$ defined by
\begin{equation*}
\cC^\pm: x+y-z^2 = \pm 2t
\end{equation*}
inside $\tilde\cS$.
We will usually only look at one of these two families,
namely $\cC^-$, which we will
simply denote by $\cC$,
in spite of the conflict of notation with \ref{p:nod-to-tac}.



\section{Abstract reduction of nodes degenerating to a 
tacnode, via normalization of the nodes}
\label{S:abstract-normaliz}


In this section, we compute the stable reduction of
the family $\cC \to \A^1$ of $1$-nodal
curves degenerating to a tacnodal curve described in the previous
section.
We start by normalizing the total space $\cC$, which has the effect of
normalizing the fibres $C_t$ with $t\neq 0$. Then, we make some
modifications in order for the pre-images of the nodes to form two
disjoint sections. The last operation is to glue these two sections,
so that we come back to a family with general member a $1$-nodal curve.

% which is arguably the standard way
% to proceed, and a rather transparent one indeed. 

\paragraph{Setup}
\label{p:setup}
We consider the family $\cC$ defined as $\cC^-$ in \ref{p:def:Cpm}
(recall also Notation~\ref{notation}).
It may be identified with its affine projection in 
$\A^3_{yzt}$, which is defined by the single equation
\begin{equation}
\cC:\quad
y(y-z^2+2t)+t^2=0
\iff (y+t)^2-yz^2=0,
\end{equation}
obtained by eliminating $x$ from the two equations
$xy=t^2$ and $x+y-z^2+2t=0$ defining $\mathcal C^-$.

The total space $\cC$ is a surface with a double curve along
\begin{equation*}
R:\ y+t=z=0,
\end{equation*}
and a pinch point at the origin (which is the intersection point of
$R$ with the central fibre), and is otherwise smooth.
For all $t\neq 0$, $C_t$ is a $1$-nodal curve with its node at $C_t \cap
R$, and $C_0$ is a $1$-tacnodal curve with its tacnode at the pinch point
$C_0 \cap R$.
We let $C_0',C_0''$ be the two irreducible components of $C_0$,
defined respectively by $y=t=0$ and $y-z^2=t=0$.

\paragraph{Normalization of the total space}
\label{p:abs-normaliz}
The first move in the present approach is to normalize the total space
$\cC$. We do this by blowing-up the double curve $R$ in $\cC$.
Let $\e_1: \cC_1 \to \cC$ be the corresponding morphism.

The surface $\cC_1$ lives in the subscheme of the product
$\A^3_{yzt}  \times \P^1_{t_1:z_1}$ defined by the equation
\begin{equation}
\label{p:abs-normaliz:blup}
z_1(y+t)=t_1z,
\end{equation}
in which it is defined by the equation
\begin{equation}
\label{p:abs-normaliz:proper}
t_1^2-yz_1^2=0.
\end{equation}
First note that the surface $\cC_1$ is smooth. 
The exceptional locus of $\e_1$
(i.e.,  the total transform via $\e_1$ of $R$)
is the curve $R_1$ defined by
\begin{equation*}
y+t=z=0
\end{equation*}
in $\cC_1$;
it is a bisection of $\cC_1 \to \A^1_t$
(which is the composed map  $\cC_1 \to \cC\to \A^1_t$),
mapped $2:1$ onto $R$ by
$\e_1$ with ramification over the tacnode.
The central fibre of $\cC_1$ is defined by $t=0$, which gives
$z_1y=t_1z$ by \eqref{p:abs-normaliz:blup},
hence \eqref{p:abs-normaliz:proper} becomes
\begin{equation*}
t_1(t_1-zz_1)=0;
\end{equation*}
thus the central fibre of $\cC_1$
consists of two branches intersecting transversely, which we shall
still denote by $C_0'$ and $C_0''$.
The situation is summed up in Figure~\ref{fig:abstract1}.

\medskip
\begin{figbox}
\includegraphics[height=70pt]{abstract1.eps}
\captionof{figure}
{Normalization of the total space,
$\e_1: \cC_1 \to \cC$}
\label{fig:abstract1}
\end{figbox}

\paragraph{Base change}
The next step is to perform the base change
$t \in \A^1 \mapsto t^2 \in \A^1$ in order to separate the pre-images
of the nodes of the $C_t$'s in two sections.
Let $\tilde \cC_1 \to \cC_1$ be the corresponding double cover. 
In practice, this amounts to replacing $t$ by $t^2$ everywhere in the
equations defining $\cC_1$. The notable fact is that this yields an
ordinary double point on the surface $\tilde \cC_1$ at the point where
$C_0'$ and $C_0''$ intersect.
We call $R_1'$ and $R_1''$ the two irreducible components of the
pre-image of $R_1$.

\paragraph{Resolution}
The next thing we do is to resolve the ordinary double
point of $\tilde \cC_1$.
We call $\bar \cC_1\to \tilde\cC_1$ the corresponding map.  It
is a birational morphism, with exceptional locus a $(-2)$-curve which
we call $E$. The resulting family of curves is depicted on
the right-hand-side of 
Figure~\ref{fig:abstract2}.

\paragraph{Reconstruction of the nodes}
Finally, since what we are looking for is the stable reduction of
the $1$-nodal curves $C_t$, $t\neq 0$, we reconstruct the nodes that
have been normalized in the first step by identifying the two disjoint
sections $R_1'$ and $R_1''$ of the family $\bar\cC_1 \to \A^1$. We
call $\cC_2 \to \A^1$ the obtained family of curves,
see the left-hand-side of Figure~\ref{fig:abstract2}. Its central fibre
is reduced, with a $1$-nodal rational curve $D$ (image of $E$)
connecting $C_0'$ and $C_0''$; the node of $D$ is the limit position
of the nodes of the curves $C_t$, $t\neq 0$.

\medskip
\begin{figbox}
\includegraphics[height=85pt]{abstract2.eps}
\captionof{figure}
{After the base change,
$\cC_2 \leftarrow \bar\cC_1 \to \tilde \cC_1$}
\label{fig:abstract2}
\end{figbox}

\paragraph{Why we're not satisfied with this}
We want to perform the stable reduction of the nodal curves $C_t$ (or
possibly a semi-stable variant of it), while simultaneously performing
the semi-stable reduction of the degeneration of surfaces $\tilde\cS
\to \A^1$, with notation as in Section~\ref{S:equations}.
The main problem with the above described stable reduction process is
that the normalization of the family of curves and later the
reconstruction of the nodes necessitate unwanted modifications of the
surfaces $S_t$, $t\neq 0$.

Indeed, the normalization of $\cC$ inside $\tilde\cS$
requires to blow-up every surface $S_t$, $t\neq 0$ at the point where
the curve $C_t$ has a node, which introduces a $(-1)$-curve.
Finally, once the remaining steps of the reduction of the $C_t$'s
are performed, we have to recontract all these $(-1)$-curves, and this
messes everything up, in particular this destabilizes the central
fibre. We leave it to the reader to check for himself what indeed
happens. 

Our solution is to follow another path to the stable reduction of $\cC$,
which doesn't involve the normalization of the nodal $C_t$'s.
This is what we do in the next section.



\section{Abstract reduction of nodes degenerating to a 
tacnode, maintaining the nodes}
\label{S:abstract-nodal}

\subsection{The construction}

In this section we present our construction of the stable reduction of
the family of $1$-nodal curves $C_t$ without normalizing the nodes.
The setup is the same as that formulated in \ref{p:setup},
and we don't repeat it here. We use Notation~\ref{notation}, as always.

% We follow the following steps to construct a semi-stable reduction of
% the family $\cC$.

\paragraph{Blow-up of the tacnode}
\label{p:blup-tacnode}
Let $\e_1: \cC_1 \to \cC$ be the blow-up of $\cC$ at the origin 
of $\A^3_{yzt}$ (here we use the same
notation as in paragraph \ref {p:abs-normaliz} for a different
blow-up, but we believe this will not cause any confusion). 
We will see that the reduced exceptional locus of $\e_1$ is a smooth
$\P^1$,
which we shall call $E_1$,
and the central fibre of $\cC_1$ consists of the
proper transform of $C_0$, which is the transverse union of two smooth
curves, namely the proper transforms of $C_0'$ and $C_0''$, which we
continue to denote by the same symbols,
plus $E_1$ with multiplicity $2$;
the total space $\cC_1$
has a double curve along the proper transform of $R$, still with a
pinch point at its intersection with the central fibre;
besides this double curve,
$\cC_1$ has an ordinary double point at $C_0' \cap C_0''$, which lies
on $E_1$, and no other singularities.
See Figure~\ref{fig:curves1}.

We realize $\cC_1$ as the proper transform of $\cC$ in the subvariety
of
$\A^3_{yzt} \times \P^2_{y_1:z_1:t_1}$
defined by the equations
\[
\rk \begin{pmatrix}
y & z & t \\
y_1 & z_1 & t_1
\end{pmatrix}
<2.
\]
In the affine chart $t_1=1$, $\cC_1$ has the
equation
\begin{equation}
\cC_1\ \text{in}\ [t_1=1]:\quad
(y_1+1)^2 -y_1z_1^2t=0.
\end{equation}
We thus see that $\cC_1$ has a
double curve along the proper transform $R_1$ of $R$, which has
equations $y_1+1=z_1=0$, with a pinch point at the point 
$(-1:0:1)$ on the exceptional divisor
(the latter is the fibre of $\cC_1$ over the origin
in the projection $\A^3_{yzt} \times \P^2_{y_1:z_1:t_1} \to \A^3_{yzt}$).
In this chart, the proper transform of $C_0$ is at infinity, and the
central fibre $t=0$ is the exceptional divisor, namely the double line
$(y_1+t_1)^2$ in $\P^2$. 

In the affine chart $z_1=1$, we get the equation
\begin{equation}
\label{C1:z}
\cC_1\ \text{in}\ [z_1=1]:\quad
(y_1+t_1)^2 -y_1z=0.
\end{equation}
We thus see that $\cC_1$ has an ordinary double point at the point 
$(0:1:0)$ on the exceptional divisor. 
The central fibre is defined by the equation $t=0$, which gives $t_1z=0$: 
$t_1=0$ is the proper transform of $C_0$, and has equation
$y_1(y_1-z)=0$, while $z=0$ defines the exceptional divisor: it is the
divisor defined by $(y_1+t_1)^2=0$, i.e., $E_1$ with multiplicity $2$.

\medskip
\begin{figbox}
\includegraphics[width=\textwidth]{curves1.eps}
\captionof{figure}
{Blow-up of the tacnode,
$\e_1: \cC_1 \to \cC$}
\label{fig:curves1}
\end{figbox}

\paragraph{Blow-up of the ordinary double point}
\label{p:blup-odp}
Let $\e_2: \cC_2 \to \cC_1$ be the blow-up at the point 
$C_0'\cap C_0'' \cap E_1$. The three curves $C_0', C_0'', E_1$
in $\cC_1$ intersect transversely at this point, hence they are
separated by this blow-up. The reduced exceptional locus is a smooth
$\P^1$, which we shall call $E_2$; it appears with multiplicity $2$ in the
central fibre.
See the right-hand-side of Figure~\ref{fig:norm} for a picture of the
situation.

Note that the central fibre of $\cC_1$ is $C_0'+C_0''+2E_1$, hence it
has multiplicity $4$ at the centre of the blow-up $\e_2$. However,
as we shall now see,
$E_2$ indeed appears only with multiplicity $2$ in the central fibre
of $\cC_1$, 
because the centre of $\e_2$ is a singular point (of multiplicity $2$)
of $\cC_1$.

This is fairly elementary, so we'll only sketch the computations. 
It is enough to consider the part of $\cC_1$ in the affine chart
$z_1=1$, which has equation \eqref{C1:z}. We
add the new set of homogeneous variables $(y_2:z_2:t_2)$ with the new
equations 
\[
\rk \begin{pmatrix}
y_1 & z & y_1+t_1 \\
y_2 & z_2 & t_2
\end{pmatrix}
<2.
\]
Then, $\cC_2$ has equation $t_2^2-y_2z_2=0$. Its central fibre has
equation $t=0$, which, in the affine chart  $y_2=1$, since $t=t_1z$,
$t_1=y_1(t_2-1)$, and $z=y_1z_2$, reads   
\[
(t_2-1)z_2y_1^2=0.
\]
Now,
$t_2-1=0$ defines  one of the two branches $C_0'$ and $C_0''$ (the other is invisible in this affine chart), $z_2=0$
is the equation of the proper transform of $E_1$,
and $y_1^2=0$ that of the exceptional curve
$E_2$ with multiplicity two.


\paragraph{Base change and normalization}
\label{p:2cover}
Let $\tilde\cC_2 \to \cC_2$ be the double covering of $\cC_2$ ramified over
the central fibre, and $\bar\cC_2 \to \tilde\cC_2$ the partial
normalization obtained by leaving only the singularity along the proper
transform of $R$.
As we shall see,
the family $\bar\cC_2 \to \A^1$ is a semi-stable reduction of 
$\cC \to \A^1$. 

Algebraically, $\tilde\cC_2$ is defined by adding a square root of $t$,
i.e., a new variable $s$ with the new equation $s^2=t$, to the
equations of $\cC_2$.
The normalization process may be chopped in several local computation
units, which we gather in Section~\ref{s:loc-modules} below.
The upshot is as follows. 
Denote by abuse of notation $E_1,E_2 \subset \tilde\cC_2$ the
reduced pre-images of $E_1, E_2 \subset \cC_2$. The
normalization may be obtained by successively blowing-up the Weil
divisors $E_1$ and $E_2$.

First, the blow-up of $E_1$ produces two smooth rational curves $E_1'$ and
$E_1''$, disposed as pictured in Figure~\ref{fig:norm},
and both mapped isomorphically onto $E_1$
(to see this, use \ref{p:module-pinch} at the pinch point,
and \ref{sp:module-22i} at $E_1\cap E_2$).
Then, the blow-up of $E_2$ produces a double covering $\bar E_2 \to E_2$,
with $\bar E_2$ a smooth rational curve disposed as 
pictured in Figure~\ref{fig:norm};
this double covering branches at the two points
$C_0'\cap E_2$ and $C_0''\cap \bar E_2$,
and the associated involution exchanges the two points
$E_1'\cap \bar E_2$ and $E_1'' \cap \bar E_2$
(to see this use \ref{sp:module-21} at the two points 
$C_0'\cap E_2$ and $C_0''\cap \bar E_2$,
and \ref{sp:module-22ii} at the point
($E_1'+E_1'')\cap E_2$).

\subparagraph{A useful variant}\medskip
\label{sp:alt-norm}
Although arguably less natural, blowing-up first $E_2$ and then $E_1$
produces the same result.
The blow-up of $E_2$ produces a double cover $\tilde E_2 \to E_2$,
ramified at the two points
$C_0' \cap \tilde E_2$ and $C_0'' \cap \tilde E_2$, and with a
node over the point $E_1 \cap E_2$, as depicted in
Figure~\ref{fig:norm}. 
Then, the blow-up along $E_1$ produces two curves $E_1'$ and $E_1''$
over $E_1$, and resolves the node of $\tilde E_2$.

\begin{figbox}
\includegraphics[width=\textwidth]{curves2.eps}
\captionof{figure}
{Removing the multiplicities,
$\bar\cC_2 \to \tilde\cC_2$}
\label{fig:norm}
\end{figbox}

\paragraph{Conclusion}
It follows from the previous considerations that the family 
$\bar\cC_2 \to \A^1$ is indeed semi-stable.
One may check that the final family has an ordinary double point all
along the proper transform of $R$, i.e., the pinch point has
disappeared. 
To build a stable model out of this semi-stable model,
one has to contract the two
rational curves $E_1'$ and $E_1''$, which turns the curve $\bar E_2$
into a
$1$-nodal rational curve, with its node at the limit of 
the nodes of the curves $C_t$, $t\neq 0$.



\subsection{Ready for use toroidal computations}
\label{s:loc-modules}

In the following paragraphs we gather some local computation,
useful to normalize families of curves gotten by base change
from families with non-reduced but normal crossing central fibre;
the normalization will be expressed as a succession of blow-ups.
We only include the computations needed for \ref{p:2cover} above, but
the reader will undoubtly figure out how to generalize them to similar
situations. \cite[p.~125]{HM} is a useful reference on this subject.

\paragraph{Local situation $x^2y=t^2$}
\label{sp:module-21}
We consider the surface $\cC$ defined by this equation in
$\A^3_{xyt}$, together with the fibration over $\A^1_t$ induced by
the projection $\A^3_{xyt}\to \A^1_t$.
This is the family gotten by a degree two base change totally ramified
at the origin from a central fibre with one double component $2A$ and
one reduced component $B$ meeting transversely, 
defined by the equations $x^2=0$ and $y=0$ respectively.

The normalization of $\cC$ amounts to the blow-up 
$\bar\cC \to \cC$ of the Weil divisor
$A$, defined by the two equations $x=t=0$ (note that $\cC$ has an
ordinary double point at the generic point of $A$, and a pinch point
at the origin). To write down this blow-up, we add the set of
homogeneous coordinates $(x_1:t_1)$ with the new equation
$x_1 t
=t_1 x$.

The surface $\bar\cC$ is defined by the homogeneous equation
\begin{equation}
\label{sp:module-21:proper}
  x_1^2y=t_1^2.
\end{equation}
One thus sees that $\bar\cC$ is smooth.
We claim that its central fibre has the form $\bar A+\bar B$, with two
maps $\bar A \to A$ and $\bar B \to B$ induced by $\bar\cC \to \cC$,
respectively a double covering of $A$ ramified at the point $\bar A
\cap \bar B$, and an isomorphism.

Indeed, the central fibre is defined by $t=0$, which gives $t_1x=0$.
The equations $x=t=0$ define the exceptional divisor in $\bar\cC$;
using \eqref{sp:module-21:proper}, one sees that the exceptional
divisor is a double cover of the line $x=t=0$ in $\A^3_{xyt}$, which
is the divisor $A$. The equation $t_1=0$, on the other hand, implies
$y=0$ by  \eqref{sp:module-21:proper}, and one sees that
it defines a divisor projecting isomorphically to $B$.

\paragraph{Local situation $x^2y^2=t^2$}
We consider the surface $\cC$ defined by this equation in
$\A^3_{xyt}$,
together with the fibration $\cC\to\A^1_t$ defined by affine
projection. 
The central fibre of $\cC$ consists of the two Weil divisors $A$
($y=t=0$) and $B$ ($x=t=0$), each with multiplicity $2$.\smallskip

\subparagraph{Blow-up of the Weil divisor $A$}
\label{sp:module-22i}
We add the homogenous coordinates $(y_1:t_1)$, with the equation 
$y_1t=t_1y$;
the blow-up $\cC_1$ of $\cC$ is defined by the 
equation $x^2y_1^2=t_1^2$.
Let us restrict to the chart $y_1=1$, to fix ideas;
then $\cC_1$ is defined by the equation $x^2=t_1^2$.
The central fibre is defined by $t=0$, which implies $t_1y=0$,
hence it consists of the proper
transform $B_1$ of $B$, still with multiplicity $2$
(defined by $t=t_1=0$, hence $x^2=0$), plus the
exceptional divisor,
defined by $t=y=0$ and $(x-t_1)(x+t_1)=0$,
which is thus a sum $A'+A''$ of two divisors mapping isomorphically to
$A$.


\smallskip
\subparagraph{Successive blow-up of the second Weil divisor $B$}
\label{sp:module-22ii}
Now, we consider the blow-up $\cC_2$ of $\cC_1$ along the Weil divisor
$B_1$, which is the proper transform of $B$ in $\cC_1$.
Thus we blow-up along the subscheme defined by $t_1=x=0$, and take the
proper transform $\cC_2$ of $\cC_1$:
we add the homogenous coordinates $(x_2:t_2)$, with the equation 
$x_2t_1=t_2x$; the blow-up $\cC_2$ of $\cC_1$ is defined by the
equation $x_2^2=t_2^2$ which gives $(x_2:t_2)=(1:\pm 1)$.
The central fibre is defined by $t=0$, which implies $t_1y=0$.
If $t_1=0$, we get $x=0$ and we obtain two reduced curves since
$(x_2:t_2)=(1:\pm 1)$. These are the curves $B'+B''$ because $x=0$. If
$y=0$, we get the equations $x=\pm t_1$, which give the two proper
transforms of $A'$ and $A''$ respectively.


\smallskip
Of course the situation in the present paragraph
is more or less trivial, as the surface $\cC$
has two smooth irreducible components, defined by $xy=t$ and $xy=-t$
respectively, hence its normalization is the disjoint union of these
two components. However, we find it useful to describe the
normalization as an explicit composition of blow-ups.


\paragraph{Local situation $x^2=y^2t^2$}
\label{p:module-pinch}
We consider the surface $\cC$ defined by this equation in
$\A^3_{xyt}$,
together with the fibration over $\A^1_t$ defined by
the projection $\A^3_{xyt} \to \A^1_t$.
The family $\cC \to \A^1$ is gotten by a degree 2 base change from
the family defined by $x^2=y^2t$, which has a double curve dominating
$\A^1$, and a pinch point on the central fibre;
the central fibre is a
smooth curve with multiplicity $2$.

We blow-up the Weil divisor $x=t=0$: this introduces homogeneous
coordinates $(x_1:t_1) \in \P^1$, with the equation $x_1t=t_1x$, and
the blown-up surface is defined by the homogeneous equation 
$x_1^2=y^2 t_1^2$. 
The exceptional divisor is given by the latter equation together with
$x=t=0$, hence it is the union of two lines meeting at the point
$(0,0,0,(0:1))$. The central fibre is defined by 
$t=0$, hence also $t_1x=0$, and one sees that it equals the
exceptional divisor.

The total space is singular along the curve $y=x_1=0$, where it 
uniformly has an ordinary double point. In particular, the pinch
point has been resolved by the blow-up.


\section{The flag reduction}
\label{S:flag}

We now use the construction of Section~\ref{S:abstract-nodal}
in order to perform the semi-stable
reduction of both families $\cC \to \A^1$ and $\tilde\cS \to \A^1$ at
the same time (in the notation of \ref{p:def:Cpm}).

\paragraph{Setup}
We briefly recapitulate the situation.
We consider the threefold $\tilde\cS$ defined by the equation
\begin{equation}
\label{degen-surf}
\tilde\cS: \quad xy=t^2  
\end{equation}
in $\A^4_{xyzt}$, and the map $\tilde\cS \to \A^1$ induced by the
projection $\A^4_{xyzt} \to \A^1_t$.
Thus $\tilde\cS \to \A^1$ is a family of surfaces. 
We call $S_0'$ and $S_0''$ the two components of its central fibre,
defined by $y=t=0$ and $x=t=0$ respectively.
The family of curves $\cC$ studied in
Sections~\ref{S:abstract-normaliz} and \ref{S:abstract-nodal} is a
Cartier divisor of $\tilde \cS$, defined in $\A^4_{xyzt}$ by the equations
\begin{equation}
\label{cC-in-cS}
\cC:\quad
\left\{ 
\begin{aligned}
y+x-z^2+2t &= 0 \\
xy &= t^2.
\end{aligned}
\right.
\end{equation}



% Here, we follow the same steps as in Section~\ref{S:abstract-nodal} to
% construct a semi-stable reduction of $\cC$, with the constraint that
% we want it to live in a semi-stable reduction of $\cS$.

\paragraph{Blow-up of the tacnode}
\label{p:blup-tac-cS}
Let $\e_1: \cS_1 \to \tilde\cS$ be the blow-up of $\tilde\cS$ at the point
$\bz = (0,0,0,0) \in \A^4$, and
let $\cC_1$ be the proper transform of
$\cC$ in $\cS_1$; the restriction $\restr {\e_1} {\cC_1}$ is the same
map $\cC_1 \to \cC$ as in \ref{p:blup-tacnode}.
We call $\Sigma_1$ the exceptional divisor of $\e_1$.

The blow-up amounts to  adding the new homogeneous variables
$(x_1:y_1:z_1:t_1) \in \P^3$,
with the  equations
\begin{equation*}
\rk 
\begin{pmatrix}
x & y & z & t \\
x_1 & y_1 & z_1 & t_1
\end{pmatrix}
<2.
\end{equation*}
The total space $\cS_1$ is defined by these equations plus the
homogeneous equation 
\begin{equation}
\label{eq:cS_1}
x_1y_1 = t_1^2
\end{equation}
in $\A^4_{xyzt} \times \P^3_{x_1:y_1:z_1:t_1}$.
The exceptional divisor $\Sigma_1$ is the corank $1$ quadric defined by
the equation \eqref{eq:cS_1} in $\P^3_{x_1:y_1:z_1:t_1}$
(and it sits over the origin of $\A^4_{xyzt}$).
The central fibre of $\cS_1$ is defined by the equation
$t=0$, which implies $t_1x=t_1y=t_1z=0$,
hence it is the reduced sum of divisors
$S_0'+S_0''+\Sigma_1$, where we denote by abuse of notation
$S_0',S_0'' \subset \cS_1$ the respective
proper transforms of $S_0',S_0'' \subset \tilde\cS$ (the former are the
respective blow-ups of the latter at their smooth point $\bz$).

The surface $\cC_1$
on the other hand is defined inside $\cS_1$ by the same equations as in
\ref{p:blup-tacnode}. We leave it to the reader to check  that the
central fibres of $\cS_1$ and $\cC_1$ are arranged as indicated on 
Figure~\ref{fig:cS_1} (compare also with Figure \ref {fig:curves1}, right-hand-side).

\begin{figbox}
\includegraphics[width=\textwidth]{flag1.eps}
\captionof{figure}
{Blow-up of the tacnode,
$\e_1: \cS_1 \to \cS$}
\label{fig:cS_1}
\end{figbox}

\paragraph{Blow-up of the vertex of $\Sigma_1$}
Let $\e_2: \cS_2 \to \cS_1$ be the blow-up at the point 
$\bz_1=(0,0,0,0,(0:0:1:0)) \in \Sigma_1$,
$\cC_2$ be the proper transform of $\cC_1$, and $\Sigma_2$ be the
exceptional divisor. As usual, we call $\Sigma_1$ its own proper
transform in $\cS_2$.

To fix ideas, we consider the affine chart $z_1=1$ with respect to the homogeneous
coordinates introduced in \ref{p:blup-tac-cS} for the previous
blow-up; there, $\cS_1$ is defined by the affine equation 
$x_1y_1 = t_1^2$ (compare \eqref{eq:cS_1}) in $\A^4$
with coordinates $(x_1,y_1,z,t_1)$.
We add the new homogeneous variables $(x_2:y_2:z_2:t_2) \in \P^3$,
with the new equations
\begin{equation*}
\rk 
\begin{pmatrix}
x_1 & y_1 & z & t_1\\
x_2 & y_2 & z_2 & t_2
\end{pmatrix}
<2.
\end{equation*}
Then $\cS_2$ is defined by the homogeneous equation
\begin{equation}
\label{eq:cS_2}
x_2y_2 = t_2^2.
\end{equation}
Exactly as in \ref{p:blup-tac-cS}, the exceptional divisor $\Sigma_2$
is a corank $1$ quadric surface. 
The central fibre of $\cS_2$ is defined by 
$t=0$, or equivalently (in the affine chart $z_1=1$) by $t_1z=0$. Let
us work in the chart $x_2=1$. Then we have $z=x_1z_2, t_1=x_1t_2$ and
therefore $t _1z=x_1^2z_2t_2$.
Hence the central fibre of $\cS_2$ is the sum of the three divisors
respectively defined in $\cS_2$ by the three equations
$x_1^2=0, z_2=0, t_2=0$.
The first equation gives a double component; the second a
simple component; the third gives $x_2y_2=0$, hence two reduced
components. The double component is necessarily the exceptional
divisor over the vertex of the cone.  The upshot is that the central
fibre is the non-reduced sum
$S_0'+S_0''+\Sigma_1+2\Sigma_2$, with our usual abuse of notation:
$S_0',S_0'' \subset \cS_2$ are the blow-ups of 
$S_0',S_0'' \subset \cS_1$ at their smooth point $\bz_1$,
and $\Sigma_1 \subset \cS_2$ is the blow-up of $\Sigma_1 \subset
\cS_1$ at its vertex (in particular, it is isomorphic to an $\F_2$
minimal rational ruled surface).

Again, the surface $\cC_2$ is defined inside $\cS_2$ by the same
equations as in \ref{p:blup-odp}, and we leave it to the reader to
check  that the central fibres of $\cS_2$ and $\cC_2$ are arranged as
indicated on Figure~\ref{fig:cS_2}, right-hand-side
(compare also with Figure \ref {fig:norm}, right-hand-side).
Note in particular that the curve $E_2$ is contained in $\Sigma_2$ and
tangent to the curve $\Sigma_2 \cap \Sigma_1$.

\begin{figbox}
\includegraphics[width=.8\textwidth]{flag2.eps}
\captionof{figure}
{Blow-up of the vertex of $\Sigma_1$, $\e_2:\cS_2 \to \cS_1$,
and its resolution $\cS_2' \to \cS_2$}
\label{fig:cS_2}
\end{figbox}


\paragraph{Resolution of singularities of $\cS_2$}
\label{p:resol-S_2}
The threefold $\cS_2$ is singular along the curve $S_0' \cap S_0''$,
at the generic point of which it has an $A_1$ singularity.
Let $\cS_2' \to \cS_2$ be the blow-up along this curve, with
exceptional divisor $\Sigma_0$ a $\P^1$-bundle over $S_0' \cap S_0''$.
Then, $\cS_2'$ is non-singular, with central fibre
\begin{equation}
\label{eq:central-S2'}
S_0'+S_0''+\Sigma_1+2\Sigma_2 + \Sigma_0;
\end{equation}
all summands are isomorphic to their counterparts in $\cS_2$ except
$\Sigma_2 \subset \cS_2'$, which is the minimal resolution of the
quadric cone $\Sigma_2 \subset \cS_2$.
On Figure~\ref{fig:cS_2}, left-hand-side,
we picture the central fibre of $\cS_2'$ with
the self-intersections of the
intersection curves of any two of its irreducible components.
One may check that they concord with
the triple-point-formula, which we recall as Lemma~\ref{l:triple-pt} 
below. 

One may prefer to skip step~\ref{p:resol-S_2}; this induces only minor
changes. 

\begin{lemma}[Triple Point Formula, see \cite {CCFM, Frie}]
\label{l:triple-pt}
Let $f: \mathcal{X} \to \A^1$ be a family of surfaces with smooth
total space, 
% such that the general fibre $X_t$ is smooth, and 
such that the central fibre $X_0$ has
simple normal crossing support but may be non-reduced.
Let $Q,Q'$ be irreducible components of $X_0$, with respective
multiplicities $m$ and $m'$ in $X_0$, intersecting along
the \emph{double curve} $B$. Then
\begin{equation*}
m' B_Q^2 %\deg (N_{B\vert Q} )
+m B_{Q'}^2 %\deg(N_{B\vert Q'})
% + \sum ^{\hphantom {Q'' \in \operatorname{Irr}(X_0)}}
% _{\hspace{3em}\mathclap {Q'' \in \operatorname{Irr}(X_0)-\{Q,Q'\}}
% }
+ \sum _{Q'' \neq Q,Q'}
\mult_{X_0}(Q'') \cdot \Card (B \cap Q'')
% +\mathrm{Card}\left\lbrace \begin{array}{c}
% \text{triple points of $S_0$} \\
% \text{along}\ R_s
% \end{array} \right\rbrace
=0,
\end{equation*}
where $Q''$ ranges through all irreducible components of $X_0$ besides
$Q'$ and $Q''$.
\end{lemma}

\medskip
In the above statement, 
$\mult_{X_0}(Q'')$ denotes the multiplicity of $Q''$ in
the central fibre $X_0$, 
and $B_Q^2 = \deg (N_{B/ Q} )$  
(resp.\ $B_{Q'}^2 =\deg(N_{B/ Q'})$)
is the self-intersection of $B$ as a curve in the surface $Q$ (resp.\
$Q'$). 

\paragraph{Base change and resolution}
Let $\tilde\cS_2 \to \cS_2'$ be the double covering ramified over
the central fibre.
% \eqref{eq:central-S2'}.
It is defined by adding a
square root of $t$, i.e., we 
introduce a new variable $s$ with the new equation $s^2=t$, and
consider the family of surfaces $\tilde\cS_2 \to \A^1_s$ defined by
the projection map. 
The proper transform of $\cC_2$ in $\tilde\cS_2$ is isomorphic to the
family $\tilde\cC_2$ of \ref{p:2cover}.

The central fibre of $\tilde\cS_2$ is, of course, the same as that of
$\cS_2'$. We let $\tilde\cS_2' \to \tilde\cS_2$ be the blow-up of the
Weil divisor $\Sigma_2$. This has the effect of replacing $\Sigma_2$
by its double cover $\tilde\Sigma_2$ branched over the anticanonical
divisor 
$(S_0'+S_0''+\Sigma_1+\Sigma_0) \cap \Sigma_2$, and doesn't change
anything else. 

Let $\tilde\cC_2'$ be the proper transform of $\tilde\cC_2$ in
$\tilde\cS_2'$. It is obtained by replacing the curve $E_2$ with its
double cover $\tilde E_2$ branched along the divisor
$(C_0'+C_0''+2E_1) \cap E_2$: this is a rational curve with an ordinary
double point at the intersection with $E_1$ (see \ref{sp:alt-norm}).
The central fibre is depicted on
Figure~\ref{fig:bar-cS_2}, right-hand-side.

One checks with local computations in the style of those in
subsection~\ref{s:loc-modules}\footnote
{for instance, at the generic point of $S_0'\cap \Sigma_2$, 
$\tilde\cS_2$ has an equation equivalent to $a^2b=u^2$, and 
$\tilde\cS_2'\to \tilde\cS_2$ is locally the blow-up of $a=u=0$.
}
that $\tilde\cS_2'$ is singular only
along the four curves at the intersection of one of $S_0',S_0''$ with
one of $\Sigma_0,\Sigma_1$, where it
has lines of $A_1$ double points.
Correspondingly, the surface $\tilde\Sigma_2$ has four ordinary double
points over the double points of the anticanonical divisor of
$\Sigma_2$. 

It follows that the blow-up of $\tilde\cS_2'$ along the four
aforementioned curves is non-singular. We let 
$\bar\cS_2 \to \tilde\cS_2'$ be the corresponding blow-up morphism.
The central fibre of $\bar\cS_2 \to \A^1_s$ is pictured on the
left-hand-side of Figure~\ref{fig:bar-cS_2} below
(see also Figure \ref {fig:norm} central-bottom).
The self-intersections of the double curves of the
central fibre are indicated as well.

\medskip
\begin{figbox}
\includegraphics[width=.9\textwidth]{flag3.eps}
\captionof{figure}
{Base change and resolution}
\label{fig:bar-cS_2}
\end{figbox}

\paragraph{Conclusion}
Eventually, let $\cS_3 \to \bar\cS_2$ be the blow-up along the curve
$E_1$, and $\Sigma_1^1$ its exceptional divisor. 
The curve $E_1$ is contained in $\tilde\cC_2'$, hence the proper
transform of the latter family of curves in $\cS_3$ is isomorphic to
$\bar\cC_2$ in \ref{p:2cover}, see \ref{sp:alt-norm}.
The result is indicated on Figure~\ref{fig:flag-red} below
(see also Figure \ref {fig:norm}, left-hand-side).

\medskip
\begin{figbox}
\includegraphics[height=137pt]{flag4.eps}
\captionof{figure}
{Flag semi-stable reduction, $\cS_3$}
\label{fig:flag-red}
\end{figbox}

\bigskip
This is the flag semi-stable reduction we were looking for:
the family of surfaces $\cS_3$ is semi-stable, and so is the family of
curves $\bar\cC_2$ it contains; thus, we have realized a tacnodal
limit curve of $1$-nodal curves as a curve with one distinguished
node, in a semi-stable limit of the ambient surfaces.

One may in turn modify this flag semi-stable reduction in order to
obtain whatever variant we fancy.
For instance, it is possible to understand in this way 
the model described in \ref{p:synth4}.





\begin{references}

\begin{thebibliography}[Chapters in this Volume]{XIV}

\bibitem[\tref{01.ciro}]{01.ciro}
C.~Ciliberto,
\emph{Limits of nodal curves: generalities and examples}.

\bibitem[\tref{05.margherita}]{05.margherita}
M.~Lelli-Chiesa,
\emph{Deformations of an $m$-tacnode into $m-1$ nodes}.

\bibitem[\tref{04b.concettina}]{04b.concettina}
C.~Galati,
\emph{Proving the existence of curves  on smooth surfaces by
  smoothing tacnodes and other singularities on reducible surfaces}.

\bibitem[\tref{07.th-diag-degen}]{07.th-diag-degen}
Th.~Dedieu,
\emph{Enumeration of curves by floor diagrams, via degenerations of
  the projective plane}.

\bibitem[\tref{11.th-toric-trop}]{11.th-toric-trop}%{chap:tropic}
Th.~Dedieu,
\emph{Enumeration of curves in toric surfaces, tropical geometry, and
floor diagrams}.

\end{thebibliography}

\begin{thebibliography}[External References]{99}

\bibitem {CCFM}
A.~Calabri, C.~Ciliberto, F.~Flamini {\normalfont and} R.~Miranda:
\emph{On the $K^2$ of degenerations of surfaces
and the multiple point formula}, 
Ann. of Math., {\bf 165} (2007), 335--395.

\bibitem{CH0}
  L.~Caporaso, J.~Harris,
  \emph{Parameter spaces for curves on surfaces and enumeration of
  rational curves}, Compositio Math. \textbf{113} (1998), no.~2, 155--208.

\bibitem{CH}
L. Caporaso, J. Harris:
{\it Counting plane curves of any genus}, 
Invent. Math. {\bf 131} (1998), no.2, 345--392.

\bibitem {Frie} R. Friedman: 
{\it Global smoothings of varieties with normal
crossings}, Ann. of Math. {\bf 118} (1983), 75--114.

\bibitem{HM}
J.~Harris {\normalfont and} I.~Morrison, \emph{Moduli of curves},
Graduate Texts in Mathematics, vol.~187, Springer-Verlag, New York, 1998.

\bibitem{teissier} B.~Teissier, 
\emph{{Résolution simultanée I, II}}, in \emph{Séminaire sur
  les singularités des surfaces, Cent. Math. Éc. Polytech., Palaiseau
  1976--77}, Lecture Notes in Mathematics, vol.~777, 
Springer-Verlag, Berlin, 1980, 71--146.
\end{thebibliography}

\end{references}



\stopcontents[15.tacnodo]





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End:


==> A.swallowtail/swallowtail.tex <==
\chaptitle{Geometry of the deformation space of an $m$-tacnode into
  $m-1$ nodes}
\chapauthor{Thomas Dedieu}

\startchap
\label{A.swallowtail}

% \setdefaultenum{(i)}{}{}{}
% \setdefaultitem{---}{}{}{}

\startcontents[swallowtail]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[swallowtail]{}{1}[2]{}

\newcommand{\cusp}{\mathrm{cusp}}

\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother

% \newenvironment{taf}{\color{blue}}{}
\def\taf{\textcolor{blue}}


\section{Introduction}

This appendix complements the previous lecture \cite{05.margherita},
of which we shall keep the notation:
let $\pi: S \to \Delta$ be the versal deformation space of the
$m$-tacnode defined by the equation
$y(y+x^m)=0$ in the affine plane; we have
$\Delta \cong
\A^{2m-1}_{\alpha_0,\ldots,\alpha_{m-2},\beta_0,\ldots,\beta_{m-1}}$,
and $S$ is defined in $\A^2_{x,y}\times \Delta$ by the equation
\[
  y^2 +y(x^m+\alpha_{m-2}x^{m-2}+ \cdots + \alpha_0)
  + \beta_{m-1}x^{m-1}+\cdots + \beta_0.
\]
Inside $\Delta$ we consider the two subvarieties $\Delta_{m-1}$ and
$\Delta_m$, the closures of the two loci of those $t\in \Delta$
such that the curves $\pi^{-1}(t)$ have $m-1$ nodes and $m$ nodes,
respectively.

The goal of \cite{05.margherita} was to establish some properties of
$\Delta_{m-1}$ around the origin in $\Delta$, of fundamental
importance in order to carry out the program of \cite{ch},
see \cite{04.concettina}.
Here we shall provide complementary results, 
and work out detailed examples for $m=2$ and $3$.
The first motivation is that this will hopefully give more insight
into the main result of \cite{05.margherita}, as well as help to
follow the arguments given there.
On the other hand, the variety
$\Delta_{m-1}$ for $m=2$ will show up under another guise in this
volume, see \cite{13.th-classic},
namely as the local model for the dual variety
$\dual X \subset \check \P^3$ of a surface 
$X \subset \P^3$, around a point corresponding to a tacnodal hyperplane
section; this makes $\Delta_{m-1}$ one of the main characters of this
volume. We are therefore interested in more
properties of $\Delta_{m-1}$ than those strictly necessary for the
Caporaso--Harris Program.

Finally, I would like to point out before I start that the
singularity of $\Delta_{m-1}$ at the origin is known for $m=2$ as a
swallowtail singularity,
\emph{queue d'aronde} in french, one of seven elementary situations in
René Thom's \emph{théorie des catastrophes}.


\section{General results}
\label{S:general}

Let $\tau: \tilde \Delta \to \Delta$ be the blow-up along $\Delta_m$;
recall that $\Delta_m \subset \Delta$ is the affine plane with
equations
\[
  \beta_0 = \cdots = \beta_{m-1} = 0,
\]
and it is contained in $\Delta_{m-1}$.
Let $Z \subset \tilde \Delta$ be the exceptional divisor, a
$\P^{m-1}$-bundle over $\Delta_m$, and let $\Phi$ be the fibre of $Z$ over
the origin.
Let $\tilde \Delta_{m-1}$ be the proper transform of $\Delta_{m-1}$.
Let $H$ be the hyperplane $\beta_0=0$ in $\Delta$, and
let $\tilde H$ be its proper transform in $\tilde \Delta$.


The main result of \cite{05.margherita} may be reformulated as
follows, \cf
\cite[Lemma~4.2]{ch}, where the equivalence of the two statements is
proved
(all the ingredients for this proof are present in
\cite{05.margherita}).

\begin{proposition}
\label{pr:bl-up}
Let $Z_{m-1}$ be the intersection
$\tilde \Delta_{m-1} \cap Z$ (this is the exceptional locus of
$\tau: \tilde \Delta_{m-1} \to \Delta_{m-1}$).
Then $Z_{m-1}$ contains $\Phi$ as a component of multiplicity $m$.
Moreover, $\tilde \Delta_{m-1}$ is smooth at all points of $\Phi$ not
in $\tilde H$.
\end{proposition}


We shall now prove the result below, following
\cite[\S 2.4.4]{ch0}.
It is interesting in itself, but also as a pretext to give a local
description of $\Delta_{m-1}$ at an arbitrary point of $\Delta_m$.


\begin{proposition}
\label{pr:lin-sp}
The fibres of $Z_{m-1}$ over $\Delta_m$ are unions of linear spaces.
\end{proposition}

Before we prove this, we introduce a natural stratification of
$\Delta_m$.
Each stratum is the locus in which the $m$-tacnode deforms into $k$
non-infinitely near tacnodes of orders $m_1,\ldots,m_k$ respectively,
with $m_1+\cdots+m_k=m$.

The space $\Delta_m$ identifies with the space of monic
degree $m$ polynomials in $x$ with no $x^{m-1}$-term, and we shall
consider in this space the loci of polynomials having roots with given
multiplicities. For all partition
$m=m_1+\cdots+m_k$, we let
\[
  \Delta\{m_1,\ldots,m_k\} \subset \Delta_m \subset \Delta
\]
be the locus corresponding to monic
degree $m$ polynomials with no $x^{m-1}$-term of the form
$(x-\lambda_1)^{m_1}\cdots (x-\lambda_k)^{m_k}$, with
$\lambda_1,\ldots, \lambda_k$ pairwise distinct.
Note that $\Delta\{m_1,\ldots,m_k\}$ has dimension $k-1$ (because we
impose that there is no $x^{m-1}$-term, equivalently the $\lambda_i$'s
sum up to zero),
so its codimension in $\Delta_m$ is
$m-k = \sum_{i=1} ^k (m_i-1)$.

For $\alpha \in \Delta\{m_1,\ldots,m_k\}$,
the curve $S_\alpha = \pi^{-1}(\alpha) \subset \A^2_{x,y}$
is a reducible curve with two
branches, defined by the two equations
$y=0$ and 
$y=(x-\lambda_1)^{m_1}\cdots (x-\lambda_k)^{m_k}$
respectively; these two branches intersect at the $k$ points
$r_1 = (\lambda_1,0), \ldots, r_k = (\lambda_k,0)$,
with multiplicities $m_1,\ldots,m_k$ respectively.

For all $i=1,\ldots,k$ we consider the versal deformation space
$\Delta(S_\alpha,r_i)$ of the singular point $r_i \in S_\alpha$; note
that this is an $m_i$-tacnode.
There is then a natural map
\[
  \sigma: U \to
  \prod_{i=1}^k \Delta(S_\alpha,r_i),
\]
where $U$ is an open neighbourhood $U$ of $\alpha$ in $\Delta$,
and by the openness of versality it has surjective differential at
$\alpha$;
the fibre of $\sigma$ over the origin parametrizes the equisingular
deformations of $S_\alpha$, for which only the location of the points
$r_i$ varies along the $x$-axis.

For all $i=1,\ldots,k$ we consider the subvarieties
$\Delta_{m_i-1}(r_i)$ and $\Delta_{m_i}(r_i)$ of
$\Delta(S_\alpha,r_i)$, defined as the closures of the loci where
$r_i$ deforms to $m_i-1$ nodes and $m_i$ nodes respectively.
Then, in the neighbourhood $U$ of $\alpha$ in $\Delta$, we have
\[
  \Delta_m = \sigma^{-1} \bigl(
    \Delta_{m_1}(r_1) \times \cdots \Delta_{m_k}(r_k)
  \bigr)
\]
and
\[
  \Delta_{m-1} = \bigcup_{l=1}^k \sigma^{-1} \bigl(
    \Delta_{m_1}(r_1) \times \cdots \times
    \Delta_{m_l-1}(r_l)
    \times \cdots \Delta_{m_k}(r_k)
  \bigr).
\]
From this we see that $\Delta_{m-1}$ has $k$ local sheets in a
neighbourhood of $\alpha$, each containing $\Delta_m$.
The $l$-th sheet looks like the product of
$\Delta_{m_l-1}\subset \Delta_{m_l}$ with some smooth factor,
and along this sheet the fibres of $\pi:S \to \Delta$ have $m_i$ nodes
tending to $r_i$ for $i\neq l$, and $m_l-1$ nodes tending to $r_l$.

We are now ready to prove the statement.

\begin{proof}[Proof of Proposition~\ref{pr:lin-sp}]%
In the above setup,
applying Proposition~\ref{pr:bl-up} to the spaces
$\Delta(S_\alpha,r_i)$, we will be able to describe the fibre of
$Z_{m-1}$ over $\alpha \in \Delta_m$.
Note that $\Phi$, the fibre of $Z$ over the origin, identifies with
the projectivization of the space of degree $m-1$ polynomials in $x$
(with coefficients $\beta_0,\ldots,\beta_{m-1}$),
equivalently with
the projectivization of the space of polynomials modulo
those vanishing to order $m$ at the origin
(\ie $\C[x]/(x^m)$).

Then, for all $l=1,\ldots,k$,
by Proposition~\ref{pr:bl-up} applied to $\Delta_{m_l-1}(r_l)$,
the proper transform of the $l$-th sheet of $\Delta_{m-1}$
intersects the fibre $\Phi_\alpha$ of $Z$ over $\alpha$ in the linear
subspace of $\Phi_\alpha$ corresponding to polynomials in $x$
vanishing to order $m_h$ at $r_h$ for all $h\neq l$;
in other words, if we identify $\Phi_\alpha$ with the projectivization
of
\[
  \C[x]/\bigl(
  (x-\lambda_1)^{m_1}\cdots (x-\lambda_k)^{m_k}
  \bigr)
  \  \cong
  \
  \prod _{h=1} ^k
  \C[x]/\bigl(
  (x-\lambda_h)^{m_h}
  \bigr),
\]
then the proper transform of the $l$-th sheet of $\Delta_{m-1}$
intersects $\Phi_\alpha$ in its linear subspace which is
the projectivization of
$\C[x]/\bigl(  (x-\lambda_l)^{m_l}  \bigr)$
(with multiplicity $m_l$).

In turn, the intersection of $\tilde \Delta_{m-1}$ with the fibre 
$\Phi_\alpha$ of $Z$ over $\alpha$ is the union of these linear spaces
for $l$ ranging from $1$ to $k$.
\end{proof}


\paragraph{A complement}
Consider a small arc $t \in \D \mapsto \alpha(t) \in \Delta_m$ tending
to the origin as $t$ tends to $0$,
where $\D$ stands for the unit disc in $\C$.
If this arc is small enough, then all points $\alpha(t)$
with $t\neq 0$ lie in the same stratum
$\Delta\{m_1,\ldots,m_k\}$.
Moreover, as $t$ goes to $0 \in \D$ the singular points $r_i(t)$ of
the curve $S_{\alpha(t)} \subset \A^2_{x,y}$ tend to the origin.
It follows that the limiting position in $\Phi$ of the intersection
with $\Phi_{\alpha(t)}$ of
the $l$-th sheet of $\Delta_{m-1}$ along $\Delta\{m_1,\ldots,m_k\}$
is the space of polynomials vanishing to order $m-m_l$ at $0$
(in the identification of $\Phi$ with polynomials in $x$ modulo those
vanishing to order $m$ at the origin).

This implies, as in \cite[\tref{stepII}]{05.margherita}, that $\Phi$ is
an irreducible component of $Z_{m-1}$, the general point of which
corresponds to the tangent direction of an arc in $\Delta_{m-1}$ which
intersects $\Delta_m$ only in the origin.



\section{Complete description in the case $m=2$}

When $m=2$ we are considering the versal deformation space
of the ordinary tacnode, defined in $\A^2_{x,y}$ by the equation
$y(y+x^2)=0$; 
this is $S\to \Delta \cong \A^3_{\alpha_0,\beta_0,\beta_1}$, with $S$
defined in $\A^2_{x,y}\times \Delta$ by the equation
\[
  y^2+y(x^2+\alpha_0)+\beta_1 x + \beta_0=0.
\]
We are interested in the surface $\Delta_1 \subset \Delta$ of
deformations of cogenus at least one of the tacnode, especially along
the curve
$\Delta_2 \subset \Delta$ of deformations of cogenus two, which is the
line $\beta_1=\beta_0=0$, along wich the tacnode deforms to two
nodes. The picture looks as follows, as we shall see. 
\begin{center}
\includegraphics{ch-swallowtail.eps}
\captionof{figure}
{Geometry of $\Delta_{1}$ along $\Delta_2$ 
  (beware the singularity along  $\Delta_\cusp$)
\\ (reproduction from \cite[p.181]{ch0})}
\end{center}
The surface $\Delta_1$ has two local sheets along the line $\Delta_2$;
they intersect transversely along the complement of the origin in
$\Delta_1$, but they have the same tangent plane at the origin. Also,
it is important to keep in mind that the surface $\Delta_1$ is
singular along the curve $\Delta_\cusp$, which is the locus along
which the tacnode deforms to an ordinary cusp: the surface $\Delta_1$
has a cuspidal singularity at the generic point of $\Delta_\cusp$,
although this not pictured on the above figure.

The proper transform of $\Delta_1$ under the blow-up of $\Delta$ along
the line $\Delta_2$ looks as follows.
\begin{center}
\includegraphics{ch-blup.eps}
\captionof{figure}
{Intersection of $\tilde\Delta_{1}$ with the exceptional divisor
\\(reproduction from \cite[p.379]{ch})}
\end{center}


\paragraph{Equation of $\Delta_1$}
\label{p:eq-Delta-surf}
The surface $\Delta_1$ is defined in
$\A^3_{\alpha_0,\beta_0,\beta_1}$ by the condition that the
polynomial
\[
  \delta_{\alpha_0,\beta_0,\beta_1} (x)
  = (x^2+\alpha_0)^2 -4(\beta_1 x+\beta_0)
  = x^4+2\alpha_0x^2
  -4\beta_1x
  +\alpha_0^2-4\beta_0
\]
has at least one non-simple root
(see \cite[Section~1]{05.margherita}), equivalently its discriminant
vanishes. Using the formula for the discriminant of monic degree $4$
polynomials with no $x^3$-term, namely
\[
  \Disc(x^4+ax^2+bx+c)
  = -4a^{3}b^{2} +16a^{4}c -27b^{4} +144ab^{2}c -128a^{2}c^{2} +256c^{3},
\]
we find the equation for $\Delta_1$ in
$\A^3_{\alpha_0,\beta_0,\beta_1}$,
\begin{equation}
\label{eq:Delta-surf}
  256\cdot
  (16\alpha_0^3\beta_1^2 +16\alpha_0^2\beta_0^2
  -72\alpha_0\beta_0\beta_1^2 -27\beta_1^4 -64\beta_0^3)
  =0.
\end{equation}
Note that it is quasi-homogeneous of degree $12$ for the weights
$2,4,3$ of $\alpha_0,\beta_0,\beta_1$ respectively.

\paragraph{Equations of the curve $\Delta_\cusp$}
\label{p:D_cusp-elim}
We consider the locus $\Delta_\cusp$ of those $t\in \Delta$ such that
the curve $S_t$ has (at least) a cuspidal singularity.
% \taf{Its equations may (?) be computed as in
% \ref{p:eq-Delta-surf} above by using a
% suitable reduced discriminant, but for now it will be simpler to
% compute them by elimination.}
The locus $\Delta_\cusp$ is defined by the condition that the
polynomial $\delta_{\alpha_0,\beta_0,\beta_1}$ has at least one triple
root, in other words that there exists $u\in \A^1$ such that
\begin{align*}
  \delta_{\alpha_0,\beta_0,\beta_1}(x)
  &= (x-u)^3\cdot (x+3u)
  \\
  &= x^{4} -6u^{2}x^{2} +8u^{3}x -3u^{4}
\end{align*}
(recall that the roots of $\delta_{\alpha_0,\beta_0,\beta_1}$ sum up
to zero as it has no $x^3$-term).
Therefore, $\Delta_\cusp$ is the projection on the second factor of the
complete intersection in
$\A^1_u \times \A^3_{\alpha_0,\beta_0,\beta_1}$ defined by the
equations
\[
  \left\{
    \begin{aligned}
      2\alpha_0 &= -6u^{2}\\
      -4\beta_1 &= 8u^{3}\\
      \alpha_0^2-4\beta_0 &= -3u^{4}.
    \end{aligned}
  \right.
\]
Eliminating $u$ from these equations (note that this can be done
algorithmically), one finds
the following equations defining $\Delta_\cusp$ in
$\A^3_{\alpha_0,\beta_0,\beta_1}$,
\[
  \left\{
    \begin{aligned}
      \alpha_0^2-3\beta_0 &= 0 \\
      4\alpha_0^{3}+27 \beta_1^{2} &=0.
    \end{aligned}
  \right.
\]


\paragraph{Singularities of the surface $\Delta_1$}
To compute the equations of the singularities of $\Delta_1$, we
consider the Jacobian ideal
$(\partial_{\alpha_0} F,
\partial_{\beta_0} F,
\partial_{\beta_1} F)$, where $F$ is the equation of $\Delta_1$
given in \eqref{eq:Delta-surf}.
It readily defines the singular subscheme of $\Delta_1$, since 
$F$ is quasi-homogeneous hence liable to the generalized Euler
formula, \cf \cite[Section 1]{02.edoardo}.
Using a software for symbolic computation with polynomials,
\eg Macaulay2 \cite{M2}
and its command \texttt{primaryDecomposition},
one finds the ideal defining the singular subscheme of $\Delta_1$
is the intersection of the two following primary ideals,
\[
  (\beta_0,\beta_1)
  \quad \text{and}
  \quad
  (9\alpha_0\beta_0^2-4\alpha_0^2\beta_1+24\beta_1^2,\
  8\alpha_0^3-27\beta_0^2-36\alpha_0\beta_1,\
  27\beta_0^4+16\alpha_0^2\beta_1^2-64\beta_1^3)
\]
The former is the defining ideal of $\Delta_2$,
while the latter is not prime,
with radical
the defining ideal of the curve $\Delta_\cusp$.

Also, one sees directly from the equation of $\Delta_1$,
\eqref{eq:Delta-surf},
that it has a triple point at the origin, with tangent cone the triple
plane at the origin $\beta_0^3 = 0$.

\paragraph{Blow-up along the line $\Delta_2$}
The blow-up of $\A^3_{\alpha_0,\beta_0,\beta_1}$ along the line
$\Delta_2$ is the hypersurface in 
$\P^1_{(u_0:u_1)} \times \A^3_{\alpha_0,\beta_0,\beta_1}$ defined by
the equation
$u_0 \beta_1 - u_1\beta_0 =0$.
Pulling back the equation of $\Delta_1$, \eqref{eq:Delta-surf},
we find
\[
  \beta_1^{2}\cdot
  \left(16\alpha_0^{2}u_{0}^{2}-64\beta_1u_{0}^{3}+16\alpha_0^{3}
    -72\alpha_0\beta_1u_{0}-27\beta_1^{2}
  \right) = 0
\]
in the affine chart $u_1 \neq 0$,
and
\[
  \beta_0^{2}\cdot
  \left(16\alpha_0^{2}-64\beta_0 +16\alpha_0^{3}u_{1}^{2}
    -72\alpha_0\beta_0u_{1}^{2}
    -27\beta_0^{2}u_{1}^{4}
  \right) = 0
\]
in the affine chart $u_0 \neq 0$; the factors between parentheses are
thus the defining equations of the proper transform $\tilde \Delta_1$ in
$\A^1_{u_0} \times \A^3_{\alpha_0,\beta_1}$ and
$\A^1_{u_1} \times \A^3_{\alpha_0,\beta_0}$ respectively.
From these equations we see that 
$\tilde \Delta_1$ is smooth in the latter affine chart, and has a
double point at the origin of the former, with tangent cone there
given by $\beta_1^2 = 0$.

To obtain the intersection with the exceptional divisor $Z$, we plug
$\beta_1=0$ and $\beta_0=0$ respectively in these two equations;
we find
\[
  16\alpha_0^{2}(u_{0}^{2}+\alpha_0)=0
  \quad \text{and}
  \quad
  16\alpha_0^{2}(1+\alpha_0u_1^2)=0
\]
for the two equations of $Z_1 = \tilde \Delta_1 \cap Z$ in the two
charts $\A^1_{u_0} \times \A^3_{\alpha_0,\beta_1}$ and
$\A^1_{u_1} \times \A^3_{\alpha_0,\beta_0}$ respectively.
The exceptional divisor $Z_1$ thus has two irreducible component,
the fibre $\Phi_0$, and the hypersurface
$u_0^2+\alpha_0u_1^2)=0$; the latter maps $2:1$ onto the line
$\Delta_2$, and corresponds to the normal directions of the two sheets
of $\Delta_1$ along $\Delta_2$.


\section{The case $m=3$ and beyond}

From this point on it is no longer advisable to do the computations by
hand, and I have used Macaulay2 \cite{M2}.
In fact, even with a computer it is not realistic to go much
further. 
Still we can make some interesting observations, that are summed up in
Subsection~\ref{s:conclusions}. 

\subsection{The case $m=3$}

When $m=3$, we are considering the versal deformation space
of the $3$-tacnode, defined in $\A^2_{x,y}$ by the equation
$y(y+x^3)=0$; 
this is $S\to \Delta \cong
\A^5_{\alpha_0,\alpha_1,\beta_0,\beta_1,\beta_2}$, with $S$ 
defined in $\A^2_{x,y}\times \Delta$ by the equation
\[
  y^2+y(x^3+\alpha_1x+\alpha_0)+\beta_2 x^2 +\beta_1 x + \beta_0=0.
\]
We are interested in the solid $\Delta_2 \subset \Delta$ of
deformations of cogenus at least two of the $3$-tacnode, especially along
the locus
$\Delta_3 \subset \Delta$ of deformations of cogenus three, which is the
plane
$\beta_2=\beta_1=\beta_0=0$ along wich the $3$-tacnode deforms to three
(possibly infinitely near) nodes.

The singularities of $\Delta_2$ are more complicated than those of
$\Delta_1$ in the case $m=2$, and we will content ourselves with the
description of the exceptional divisor of $\tilde \Delta_2$.

\paragraph{Equations of $\Delta_2$}
\label{p:eq-Delta-solid}
We shall proceed by elimination, as in
\ref{p:D_cusp-elim}.
The solid $\Delta_2$ is defined by the condition that the polynomial
\begin{multline}
\label{m3:delta-cart}
  \delta_{\alpha_0,\alpha_1,\beta_0,\beta_1,\beta_2} (x)
  = (x^3+\alpha_1x+\alpha_0)^2 -4(\beta_2 x^2 +\beta_1 x+\beta_0)
  \\
  =
    x^6
    +2 \alpha_1 x^4
    +2\alpha_0 x^3
    +(\alpha_1^2-4\beta_2)x^2
    +(2\alpha_0 \alpha_1-4\beta_1)x
    +(\alpha_0^2-4\beta_0)
\end{multline}
has at least two non-simple roots, equivalently that there exist
$(u,v,w)\in \A^3$ such that
\begin{equation}
\label{m3:delta-param}
  \delta_{\alpha_0,\alpha_1,\beta_0,\beta_1,\beta_2} (x)
  = (x-u)^2(x-v)^2(x-w)(x+2u+2v+w).
\end{equation}
It is thus the projection to the second factor of the complete
intersection in
$\A^3 _{u,v,w} \times
\A^5_{\alpha_0,\alpha_1,\beta_0,\beta_1,\beta_2}$
defined by the four non-trivial equations obtained by identifying the
$x$-terms in \eqref{m3:delta-cart} and \eqref{m3:delta-param}.
Eliminating $u,v,w$ from these equations, for instance by using the
function \texttt{eliminate} from Macaulay2 \cite{M2},
one finds the ideal of $\Delta_2$ in $\Delta$ is the following:
{\footnotesize
  \allowdisplaybreaks
  \begin{multline*}
\begin{multlined}
  \bigl(48\alpha_0\alpha_1^2\beta_2^2 +3\alpha_1^2\beta_0\beta_1
+45\alpha_0\alpha_1\beta_1^2 -72\alpha_0\alpha_1\beta_0\beta_2
+27\alpha_0^2\beta_1\beta_2 \\
-128\alpha_1\beta_1\beta_2^2
+64\alpha_0\beta_2^3 +27\alpha_0\beta_0^2 -125\beta_1^3
+180\beta_0\beta_1\beta_2,
\end{multlined}
\\
\begin{multlined}
9\alpha_1^3\beta_0\beta_1 -9 \alpha_0\alpha_1^2\beta_1^2
+63\alpha_0\alpha_1^2\beta_0\beta_2
-54\alpha_0^2\alpha_1\beta_1\beta_2 -81\alpha_0^3\beta_2^2
+16\alpha_1^2\beta_1\beta_2^2 -128\alpha_0\alpha_1\beta_2^3
-54\alpha_0\alpha_ 1\beta_0^2
\\-81\alpha_0^2\beta_0\beta_1
+25\alpha_1\beta_1^3 -252\alpha_1\beta_0\beta_1\beta_2 +135
\alpha_0\beta_1^2\beta_2 +324\alpha_0\beta_0\beta_2^2
+192\beta_1\beta_2^3 +405\beta_0^2\beta_1,
\end{multlined}
\\
\begin{multlined}
  16 \alpha_1^4\beta_2^2
+16\alpha_1^3\beta_1^2 -16\alpha_1^3\beta_0\beta_2
-216\alpha_0^2\alpha_1\beta_2^ 2 -128\alpha_1^2\beta_2^3
-81\alpha_0\alpha_1\beta_0\beta_1 -135\alpha_0^2\beta_1^2
+135\alpha_0^2 \beta_0\beta_2 \\
-120\alpha_1\beta_1^2\beta_2
+576\alpha_1\beta_0\beta_2^2 +288\alpha_0\beta_1\beta_2^2
+256\beta_2^4 +675\beta_0\beta_1^2 -432\beta_0^2\beta_2,
\end{multlined}
\\
\begin{multlined}
  16\alpha_1^4\beta_0\beta_2 -16\alpha_0\alpha _1^3\beta_1\beta_2
-16\alpha_1^3\beta_0^2 -81\alpha_0\alpha_1^2\beta_0\beta_1
+81\alpha_0^2\alpha_1 \beta_1^2 -216\alpha_0^2\alpha_1\beta_0\beta_2
+135\alpha_0^3\beta_1\beta_2 \\
+16\alpha_1^2\beta_1^2 \beta_2
-128\alpha_1^2\beta_0\beta_2^2 +192\alpha_0\alpha_1\beta_1\beta_2^2
+135\alpha_0^2\beta_0^2 + 240\alpha_1\beta_0\beta_1^2
-225\alpha_0\beta_1^3 +576\alpha_1\beta_0^2\beta_2\\
-252\alpha_0\beta_0\beta_1\beta_2 
-320\beta_1^2\beta_2^2 +256\beta_0\beta_2^3
-432\beta_0^3,
\end{multlined}
\\
\begin{multlined}
81\alpha_0\alpha_1^3\beta_0 \beta_2
-81\alpha_0^2\alpha_1^2\beta_1\beta_2 -1215\alpha_0^3\alpha_1\beta_2^2
+240\alpha_1^3\beta_1 \beta_2^2 -81\alpha_0\alpha_1^2\beta_0^2
-486\alpha_0^2\alpha_1\beta_0\beta_1 -729\alpha_0^3\beta_1^2
\\+240\alpha_1^2\beta_1^3 +729\alpha_0^3\beta_0\beta_2
-420\alpha_1^2\beta_0\beta_1\beta_2 +261\alpha_
0\alpha_1\beta_1^2\beta_2 +1980\alpha_0\alpha_1\beta_0\beta_2^2
+2052\alpha_0^2\beta_1\beta_2^2
\\- 2240\alpha_1\beta_1\beta_2^3
+2560\alpha_0\beta_2^4 +243\alpha_1\beta_0^2\beta_1
+3645\alpha_0\beta_ 0\beta_1^2 -1836\alpha_0\beta_0^2\beta_2
-2300\beta_1^3\beta_2 +3312\beta_0\beta_1\beta_2^2
\bigr).
\end{multlined}
\end{multline*}
}
It has five generators,
quasi-homogeneous of degrees $15,17,16,18,19$ respectively, for the
weights $3,2$ for $\alpha_0,\alpha_1$ and $6,5,4$ for
$\beta_0,\beta_1,\beta_2$.

\paragraph{Tangent cone at the origin}
Using the ideal of $\Delta_2$ in $\Delta$, one finds
(\eg with the function \texttt{tangentCone} of Macaulay2)
its tangent cone at the origin is defined by the primary ideal
\[
  \bigl(
  25\beta_0\beta_1^2-16\beta_0^2\beta_2,\beta_0^2\beta_1,\beta_0^3,27\alpha_0\beta_0^2-125
  \beta_1^3+180\beta_0\beta_1\beta_2\bigr).
\]
It defines a degree $6$ projective scheme, supported over the
$3$-plane
$\beta_1=\beta_2=0$.

\paragraph{Blow-up along the plane $\Delta_3$}
We consider the blow-up of $\Delta$ along $\Delta_3$ as the subvariety
of 
$\P^2_{(u_0:u_1:u_2)}\times
\A^5_{\alpha_0,\alpha_1,\beta_0,\beta_1,\beta_2}$
defined by the equations
$u_j \beta_i - u_i \beta_j =0$ for all distinct $i$ and $j$ in
$\{0,1,2\}$.

Let us consider the affine chart $u_2=1$ to fix ideas;
it may be seen in
$\A^2_{u_0,u_1}\times
\A^3_{\alpha_0,\alpha_1,\beta_2}$
by eliminating $\beta_0$ and $\beta_1$,
since $\beta_0= u_0\beta_2$ and $\beta_1=u_1\beta_2$ in this chart.
The pull-back of the ideal of $\Delta_2$ in $\Delta$
is the intersection of the two primary ideals
$(\beta_2^2)$ and
{\footnotesize
\begin{multline*}
\bigl( 3\alpha_1^2u_0u_1 +45\alpha_0\alpha_1u_1^2 -125\beta_2u_1^3
+48\alpha_0\alpha_1^2 -72 \alpha_0\alpha_1u_0 +27\alpha_0u_0^2
+27\alpha_0^2u_1 -128\alpha_1\beta_2u_1 +180\beta_2u_0u_1 +
64\alpha_0\beta_2,\\
\begin{multlined}
16\alpha_1^3u_1^2 +16\alpha_1^4 -16\alpha_1^3u_0
-81\alpha_0\alpha_1u_0u_1 - 135\alpha_0^2u_1^2
-120\alpha_1\beta_2u_1^2 +675\beta_2u_0u_1^2 -216\alpha_0^2\alpha_1
-128 \alpha_1^2\beta_2
\\+135\alpha_0^2u_0 +576\alpha_1\beta_2u_0
-432\beta_2u_0^2 +288\alpha_0\beta_2u_ 1
+256\beta_2^2,
\end{multlined}
\\
\begin{multlined}
144\alpha_0\alpha_1^2u_1^2 -400\alpha_1\beta_2u_1^3
+144\alpha_0\alpha_1^3 -279 \alpha_0\alpha_1^2u_0
+135\alpha_0\alpha_1u_0^2 +135\alpha_0^2\alpha_1u_1
-400\alpha_1^2\beta_2u _1 +81\alpha_0^2u_0u_1
\\
+792\alpha_1\beta_2u_0u_1 -405\beta_2u_0^2u_1 -135\alpha_0\beta_2u_1^2
+81\alpha_0^3 +320\alpha_0\alpha_1\beta_2 -324\alpha_0\beta_2u_0
-192\beta_2^2u_1,
\end{multlined}
\\
\begin{multlined}
\alpha_1^4u_0 - \alpha_1^3u_0^2
-\alpha_0\alpha_1^3u_1 +81\alpha_0^2\alpha_1u_1^2
+\alpha_1^2\beta_2u_1^2 +15\alpha _1\beta_2u_0u_1^2
-225\alpha_0\beta_2u_1^3 +81\alpha_0^2\alpha_1^2
-135\alpha_0^2\alpha_1u_0 \\
-8\alpha_1^2\beta_2u_0 +54\alpha_0^2u_0^2
+36\alpha_1\beta_2u_0^2 -27\beta_2u_0^3 +54\alpha_0^3u_1
-204\alpha_0\alpha_1\beta_2u_1 \\
+288\alpha_0\beta_2u_0u_1
-20\beta_2^2u_1^2 +108\alpha_0^2\beta_ 2 +16\beta_2^2u_0 \bigr).
\end{multlined}
\end{multline*}      
}%
The latter has four generators, and defines the proper transform
$\tilde \Delta_2$ of $\Delta_2$ in this affine chart.
To obtain the intersection $Z_2$ of $\tilde \Delta_2$ with the
exceptional divisor, we plug in the equation $\beta_2=0$.
We find the ideal of $Z_2$ in 
$\A^2_{u_0,u_1}\times \A^3_{\alpha_0,\alpha_1,\beta_2}$
is the intersection of the three primary ideals
{\footnotesize
  \allowdisplaybreaks
\begin{gather*}
  \bigl(
  \alpha_0\alpha_1,\alpha_0^2,\alpha_1^2u_1 +9\alpha_0u_0,\alpha_1^3
  \bigr),
  \\
  \bigl(
  u_1^2 +\alpha_1 -u_0,u_0u_1 +\alpha_0,\alpha_1u_0 -u_0^2
  -\alpha_0u_1
  \bigr),
\quad  \text{and}
  \\
\begin{multlined}
  \bigl(
  \alpha_1u_0u_1^2 -\alpha_0u_1^3 +\alpha_1^2u_0 -2\alpha_1u_0^2 +u_0^3
  -\alpha_0\alpha_1u_1 +3 \alpha_0u_0u_1 +\alpha_0^2,
  \\16\alpha_1^2u_1^2
+16\alpha_1^3 -31\alpha_1^2u_0 +15\alpha_1u_0^2 +15 \alpha_0\alpha_1u_1
+9\alpha_0u_0u_1 +9\alpha_0^2,\\
\alpha_1^2u_0u_1 +15\alpha_0\alpha_1u_1^2 +16
\alpha_0\alpha_1^2 -24\alpha_0\alpha_1u_0 +9\alpha_0u_0^2
+9\alpha_0^2u_1,\\
\alpha_1^3u_0 -\alpha_1^2 u_0^2 -\alpha_0\alpha_1^2u_1
-6\alpha_0\alpha_1u_0u_1 -9\alpha_0^2u_1^2 -15\alpha_0^2\alpha_1 +9
\alpha_0^2u_0,\\
16\alpha_1^4 -15\alpha_1^2u_0^2 -96\alpha_0\alpha_1^2u_1
-90\alpha_0\alpha_1u_0u_ 1 -135\alpha_0^2u_1^2 -360\alpha_0^2\alpha_1
+216\alpha_0^2u_0
\bigr).
\end{multlined}
\end{gather*}
}%
The first one has radical $(\alpha_0,\alpha_1)$, and defines the fibre
$\Phi_0$ of $Z$ over the origin with multiplicity $3$.
The second one is radical, and defines a locus that dominates
$\Delta_3$
(this can be seen by eliminating the variables $u_0$ and $u_1$, which
gives the zero ideal); moreover, one finds there are three points in
this locus over the generic point of $\Delta_3$.
As for the third one, if we eliminate $u_0$ and $u_1$, we find
the ideal
\[
  \bigl(
  (4\alpha_1^3+27\alpha_0^2)^2
  \bigr),
\]
which is generated by the square of the discriminant of the polynomial
$x^3+\alpha_1x+\alpha_0$;
over the generic point of the locus defined by this discriminant in
$\Delta_3$, we find the the third ideal defines a
line with multiplicity $2$.

Computations in the two other affine charts are similar, although they
take a little more time to the computer.
In conclusion we find that the exceptional divisor $Z_2$
of $\tilde \Delta_2 \to \Delta_2$ has three irreducible components:
(i) the fibre $\Phi_0$ of $Z$ over the origin;
(ii) a surface dominating $\Delta_3$, and corresponding to the normal
directions of the three sheets of $\Delta_2$ along $\Delta_3$;
(iii) a surface fibered in lines over the cuspidal curve
$\Delta\{2,1\} \subset \Delta_3$
(in the notation of Section~\ref{S:general}).


\subsection{General conclusions}
\label{s:conclusions}

\paragraph{Some computations in the case $m=4$}
For $m=4$ it is still possible to compute the defining ideal of
the fourfold $\Delta_3$ in
$\A^7_{\alpha_0,\ldots,\alpha_2, \beta_0,\ldots,\beta_3}$,
although it took about half an hour on my personal computer.

This ideal has $20$ generators, all quasihomogenous if we assign the
weights $4,3,2$ to $\alpha_2,\alpha_1,\alpha_0$
and $8,\ldots,5$ to $\beta_3,\ldots,\beta_0$ respectively.
For what it's worth, the degrees of the generators are
$18, 19, 20, 20, 21, 21, 21, 22, 22, 22, 23, 23, 24, 24, 28, 28, 29,
30, 30, 31$.

The tangent cone to $\Delta_2$ at the origin is supported on the
$4$-plane $\beta_0=\beta_1=\beta_2=0$, and has degree $10$.

I have not been
able to compute a primary decomposition of the intersection of $\tilde
\Delta_3$ with the exceptional divisor $Z$ of the blow-up of $\Delta$
along $\Delta_4$.

\paragraph{General conjectures}
From the above computations one can conjecture that the defining ideal
of $\Delta_{m-1}$ in $\Delta$ will always be quasihomogeneous for the
weights
$m,\ldots,2$
for $\alpha_0,\alpha_{m-2}$
and $2m ,\ldots, m+1$
for $\beta_0,\ldots, \beta_{m-1}$, respectively.

The origin will be a point of multiplicity $\sum_{k=1}^m k$, with
tangent cone there supported on the $m$-plane
$\beta_0=\cdots = \beta_{m-2} =0$.

The exceptional divisor of $\tilde \Delta_{m-1} \to \Delta_{m-1}$ will
have $m-1$ irreducible components, respectively dominating the
following loci in $\Delta_m$~:
$\Delta\{1,\ldots,1\} = \Delta_m,\
\Delta\{2,1,\ldots,1\},\
\ldots,\
\Delta\{m-1,1\}$.

The latter two facts are probably not very hard to prove using the
setup of Section~\ref{S:general}. It is plausible that the first
conjecture may be approached using reduced discriminant theory
(see \cite{16.th-redres}).




% \bibliographystyle{mysmf-alpha}
% \bibliography{swallowtail}
% %\input{swallowtail.bbl}

\begin{references}

\begin{thebibliography}[Chapters in this Volume]{XIV}

\bibitem[\ref{02.edoardo}]{02.edoardo}
E.~Sernesi, \emph{Deformations of curves on surfaces}.

\bibitem[\ref{04.concettina}]{04.concettina}
{\Th}.~Dedieu {\normalfont \smfandname} C.~Galati, \emph{Degenerations and
  deformations of generalized severi varieties}.

\bibitem[\ref{05.margherita}]{05.margherita}
M.~Lelli-Chiesa, \emph{Deformations of an $m$-tacnode into $m-1$ nodes}.

\bibitem[\ref{13.th-classic}]{13.th-classic}
{\Th}.~Dedieu, \emph{Some classical formul{\ae} for curves and surfaces}.

\bibitem[\ref{16.th+l-redres}]{16.th-redres}
L.~Busé {\normalfont \smfandname} {\Th}.~Dedieu, \emph{Generalized weight
  properties of resultants and discriminants, and applications to projective
  enumerative geometry}.

\end{thebibliography}

\begin{thebibliography}[External References]{9}

\bibitem{ch}
L.~Caporaso {\normalfont \smfandname} J.~Harris, \emph{Counting plane curves of
  any genus}, Invent. Math. \textbf{131} (1998), no.~2, 345--392.

\bibitem{ch0}
\bysame , \emph{Parameter spaces for curves on surfaces and enumeration of
  rational curves}, Compositio Math. \textbf{113} (1998), no.~2, 155--208.

\bibitem{M2}
D.~R. Grayson {\normalfont \smfandname} M.~E. Stillman, \emph{Macaulay2, a
  software system for research in algebraic geometry}, Available at
  \url{http://www.math.uiuc.edu/Macaulay2/}.

\end{thebibliography}
  
\end{references}

\stopcontents[swallowtail]





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End: 

